Where Words Begin and End

Forced aligners locate each word of a known transcript in the audio, and many speech pipelines depend on them. In our own data, a widely used CTC aligner inserts a pause at nearly every word boundary, and we found almost no aligner evaluated on telephone audio. We compare nine aligner configurations against human word boundaries on read, conversational and telephone English. The Montreal Forced Aligner (MFA) is the most precise, while CTC aligners consistently start words late, because most frames inside a word go to the blank token. We then fine-tune Whisper with LoRA to predict each word's start and end as timestamp tokens, training only on boundaries placed by people: 47 hours in 87 languages. The resulting aligner is more precise than MFA on every English test condition, and than MFA's own Korean and Dutch models. With FA-Bench's protocol and code on TIMIT, its word-boundary error is 11.6 ms, against 18.2 ms for the best published system. Two choices matter most on telephone conversations: placing the timestamp slots after the word they time, and training on noisy transcripts, which also makes the aligner nearly insensitive to errors in the transcript. The released model reaches 16.0 ms on real landline calls, against 36.5 ms for MFA. The models are available at https://huggingface.co/collections/Scicom-intl/force-alignment

==> numbers.tex <==
% generated by make_tables.py from results/; do not edit
\makeatletter
\newcommand{\val}[1]{\ifcsname v@#1\endcsname\csname v@#1\endcsname\else\textbf{??}\PackageWarning{val}{undefined value #1}\fi}
\expandafter\def\csname v@bb/scicom/codecs/mae\endcsname{11.2}
\expandafter\def\csname v@bb/scicom/dev-mae-hi\endcsname{13.6}
\expandafter\def\csname v@bb/scicom/dev-mae-lo\endcsname{13.2}
\expandafter\def\csname v@bb/scicom/dev-median-hi\endcsname{6.3}
\expandafter\def\csname v@bb/scicom/dev-median-lo\endcsname{6.0}
\expandafter\def\csname v@bb/scicom/mean-mae\endcsname{14.00}
\expandafter\def\csname v@bb/scicom/mean-w20\endcsname{84.91}
\expandafter\def\csname v@bb/scicom/params\endcsname{58}
\expandafter\def\csname v@bb/scicom/rtf\endcsname{0.0090}
\expandafter\def\csname v@bb/scicom/runs\endcsname{5}
\expandafter\def\csname v@bb/scicom/swb/mae\endcsname{23.2}
\expandafter\def\csname v@bb/turbo/codecs/d\endcsname{$-0.1$}
\expandafter\def\csname v@bb/turbo/codecs/mae\endcsname{11.1}
\expandafter\def\csname v@bb/turbo/codecs/se\endcsname{0.08}
\expandafter\def\csname v@bb/turbo/d-mae\endcsname{$+0.01$}
\expandafter\def\csname v@bb/turbo/d-w20\endcsname{$+0.02$}
\expandafter\def\csname v@bb/turbo/dev-mae-hi\endcsname{14.7}
\expandafter\def\csname v@bb/turbo/dev-mae-lo\endcsname{14.3}
\expandafter\def\csname v@bb/turbo/dev-median-hi\endcsname{6.3}
\expandafter\def\csname v@bb/turbo/dev-median-lo\endcsname{6.1}
\expandafter\def\csname v@bb/turbo/faster-pct\endcsname{12}
\expandafter\def\csname v@bb/turbo/mean-mae\endcsname{14.01}
\expandafter\def\csname v@bb/turbo/mean-w20\endcsname{84.94}
\expandafter\def\csname v@bb/turbo/params\endcsname{28}
\expandafter\def\csname v@bb/turbo/rtf\endcsname{0.0079}
\expandafter\def\csname v@bb/turbo/runs\endcsname{3}
\expandafter\def\csname v@bb/turbo/se-mae\endcsname{0.10}
\expandafter\def\csname v@bb/turbo/se-w20\endcsname{0.06}
\expandafter\def\csname v@bb/turbo/swb/d\endcsname{$-0.1$}
\expandafter\def\csname v@bb/turbo/swb/mae\endcsname{23.1}
\expandafter\def\csname v@bb/turbo/swb/se\endcsname{0.35}
\expandafter\def\csname v@bb/v3/codecs/d\endcsname{0.0}
\expandafter\def\csname v@bb/v3/codecs/mae\endcsname{11.1}
\expandafter\def\csname v@bb/v3/codecs/se\endcsname{0.05}
\expandafter\def\csname v@bb/v3/d-mae\endcsname{$+0.16$}
\expandafter\def\csname v@bb/v3/d-w20\endcsname{$+0.02$}
\expandafter\def\csname v@bb/v3/dev-mae-hi\endcsname{13.4}
\expandafter\def\csname v@bb/v3/dev-mae-lo\endcsname{13.1}
\expandafter\def\csname v@bb/v3/dev-median-hi\endcsname{6.3}
\expandafter\def\csname v@bb/v3/dev-median-lo\endcsname{6.1}
\expandafter\def\csname v@bb/v3/mean-mae\endcsname{14.16}
\expandafter\def\csname v@bb/v3/mean-w20\endcsname{84.93}
\expandafter\def\csname v@bb/v3/params\endcsname{58}
\expandafter\def\csname v@bb/v3/rtf\endcsname{0.0094}
\expandafter\def\csname v@bb/v3/runs\endcsname{3}
\expandafter\def\csname v@bb/v3/se-mae\endcsname{0.10}
\expandafter\def\csname v@bb/v3/se-w20\endcsname{0.06}
\expandafter\def\csname v@bb/v3/swb/d\endcsname{$+1.0$}
\expandafter\def\csname v@bb/v3/swb/mae\endcsname{24.2}
\expandafter\def\csname v@bb/v3/swb/se\endcsname{0.43}
\expandafter\def\csname v@buckeye-held/mfa-arpa/amrnb/mae\endcsname{26.3}
\expandafter\def\csname v@buckeye-held/mfa-arpa/amrnb/w20\endcsname{65.2}
\expandafter\def\csname v@buckeye-held/mfa-arpa/ce/mae\endcsname{46.1}
\expandafter\def\csname v@buckeye-held/mfa-arpa/ce/w20\endcsname{55.0}
\expandafter\def\csname v@buckeye-held/mfa-arpa/clean/mae\endcsname{21.5}
\expandafter\def\csname v@buckeye-held/mfa-arpa/clean/w20\endcsname{70.7}
\expandafter\def\csname v@buckeye-held/mfa-arpa/g711u/mae\endcsname{27.0}
\expandafter\def\csname v@buckeye-held/mfa-arpa/g711u/w20\endcsname{64.4}
\expandafter\def\csname v@buckeye-held/mfa-arpa/g723/mae\endcsname{25.6}
\expandafter\def\csname v@buckeye-held/mfa-arpa/g723/w20\endcsname{64.7}
\expandafter\def\csname v@buckeye-held/mfa-arpa/gsm/mae\endcsname{27.1}
\expandafter\def\csname v@buckeye-held/mfa-arpa/gsm/w20\endcsname{64.1}
\expandafter\def\csname v@buckeye-held/mfa-arpa/opus/mae\endcsname{25.6}
\expandafter\def\csname v@buckeye-held/mfa-arpa/opus/w20\endcsname{65.1}
\expandafter\def\csname v@buckeye-held/n-utt\endcsname{199}
\expandafter\def\csname v@buckeye/cfa-edges/clean/ebias\endcsname{14}
\expandafter\def\csname v@buckeye/cfa-edges/clean/ebias-signed\endcsname{$+14$}
\expandafter\def\csname v@buckeye/cfa-edges/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/clean/mae\endcsname{37.0}
\expandafter\def\csname v@buckeye/cfa-edges/clean/median\endcsname{22.0}
\expandafter\def\csname v@buckeye/cfa-edges/clean/over500\endcsname{0.4}
\expandafter\def\csname v@buckeye/cfa-edges/clean/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-edges/clean/sbias\endcsname{16}
\expandafter\def\csname v@buckeye/cfa-edges/clean/sbias-signed\endcsname{$+16$}
\expandafter\def\csname v@buckeye/cfa-edges/clean/w10\endcsname{22.9}
\expandafter\def\csname v@buckeye/cfa-edges/clean/w100\endcsname{93.6}
\expandafter\def\csname v@buckeye/cfa-edges/clean/w20\endcsname{44.5}
\expandafter\def\csname v@buckeye/cfa-edges/clean/w50\endcsname{82.5}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/dmae\endcsname{7.0}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/dw20\endcsname{1.5}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/dw50\endcsname{2.2}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/ebias\endcsname{14}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/ebias-signed\endcsname{$+14$}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/mae\endcsname{44.0}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/median\endcsname{23.1}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/over500\endcsname{0.8}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/sbias\endcsname{16}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/sbias-signed\endcsname{$+16$}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/w10\endcsname{22.3}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/w100\endcsname{91.7}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/w20\endcsname{43.0}
\expandafter\def\csname v@buckeye/cfa-edges/g711u/w50\endcsname{80.3}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/dmae\endcsname{16.0}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/dw20\endcsname{3.7}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/dw50\endcsname{5.8}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/ebias\endcsname{14}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/ebias-signed\endcsname{$+14$}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/mae\endcsname{53.0}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/median\endcsname{25.0}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/over500\endcsname{1.3}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/sbias\endcsname{17}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/sbias-signed\endcsname{$+17$}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/w10\endcsname{21.1}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/w100\endcsname{89.1}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/w20\endcsname{40.8}
\expandafter\def\csname v@buckeye/cfa-edges/gsm/w50\endcsname{76.7}
\expandafter\def\csname v@buckeye/cfa-edges/opus/dmae\endcsname{10.9}
\expandafter\def\csname v@buckeye/cfa-edges/opus/dw20\endcsname{2.8}
\expandafter\def\csname v@buckeye/cfa-edges/opus/dw50\endcsname{3.6}
\expandafter\def\csname v@buckeye/cfa-edges/opus/ebias\endcsname{14}
\expandafter\def\csname v@buckeye/cfa-edges/opus/ebias-signed\endcsname{$+14$}
\expandafter\def\csname v@buckeye/cfa-edges/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-edges/opus/mae\endcsname{47.9}
\expandafter\def\csname v@buckeye/cfa-edges/opus/median\endcsname{24.0}
\expandafter\def\csname v@buckeye/cfa-edges/opus/over500\endcsname{1.0}
\expandafter\def\csname v@buckeye/cfa-edges/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-edges/opus/sbias\endcsname{16}
\expandafter\def\csname v@buckeye/cfa-edges/opus/sbias-signed\endcsname{$+16$}
\expandafter\def\csname v@buckeye/cfa-edges/opus/w10\endcsname{21.7}
\expandafter\def\csname v@buckeye/cfa-edges/opus/w100\endcsname{90.5}
\expandafter\def\csname v@buckeye/cfa-edges/opus/w20\endcsname{41.8}
\expandafter\def\csname v@buckeye/cfa-edges/opus/w50\endcsname{78.9}
\expandafter\def\csname v@buckeye/cfa-segment/clean/ebias\endcsname{14}
\expandafter\def\csname v@buckeye/cfa-segment/clean/ebias-signed\endcsname{$-14$}
\expandafter\def\csname v@buckeye/cfa-segment/clean/fail\endcsname{3}
\expandafter\def\csname v@buckeye/cfa-segment/clean/fail-assert\endcsname{2}
\expandafter\def\csname v@buckeye/cfa-segment/clean/fail-crash\endcsname{1}
\expandafter\def\csname v@buckeye/cfa-segment/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-segment/clean/mae\endcsname{43.3}
\expandafter\def\csname v@buckeye/cfa-segment/clean/median\endcsname{30.4}
\expandafter\def\csname v@buckeye/cfa-segment/clean/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/cfa-segment/clean/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-segment/clean/sbias\endcsname{37}
\expandafter\def\csname v@buckeye/cfa-segment/clean/sbias-signed\endcsname{$+37$}
\expandafter\def\csname v@buckeye/cfa-segment/clean/w10\endcsname{17.2}
\expandafter\def\csname v@buckeye/cfa-segment/clean/w100\endcsname{93.1}
\expandafter\def\csname v@buckeye/cfa-segment/clean/w20\endcsname{33.9}
\expandafter\def\csname v@buckeye/cfa-segment/clean/w50\endcsname{70.5}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/dmae\endcsname{3.9}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/dw50\endcsname{2.1}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/ebias\endcsname{13}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/ebias-signed\endcsname{$-13$}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/fail\endcsname{3}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/fail-assert\endcsname{2}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/fail-crash\endcsname{1}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/mae\endcsname{47.1}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/median\endcsname{32.2}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/over500\endcsname{0.3}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/sbias\endcsname{39}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/sbias-signed\endcsname{$+39$}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/w10\endcsname{16.9}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/w100\endcsname{91.7}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/w20\endcsname{32.7}
\expandafter\def\csname v@buckeye/cfa-segment/g711u/w50\endcsname{68.4}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/dmae\endcsname{10.2}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/dw20\endcsname{2.5}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/dw50\endcsname{4.5}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/ebias\endcsname{13}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/ebias-signed\endcsname{$-13$}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/fail\endcsname{5}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/fail-assert\endcsname{4}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/fail-crash\endcsname{1}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/mae\endcsname{53.5}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/median\endcsname{33.8}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/over500\endcsname{0.5}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/sbias\endcsname{39}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/sbias-signed\endcsname{$+39$}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/w10\endcsname{16.1}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/w100\endcsname{89.1}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/w20\endcsname{31.4}
\expandafter\def\csname v@buckeye/cfa-segment/gsm/w50\endcsname{66.0}
\expandafter\def\csname v@buckeye/cfa-segment/opus/dmae\endcsname{5.9}
\expandafter\def\csname v@buckeye/cfa-segment/opus/dw20\endcsname{2.0}
\expandafter\def\csname v@buckeye/cfa-segment/opus/dw50\endcsname{3.1}
\expandafter\def\csname v@buckeye/cfa-segment/opus/ebias\endcsname{13}
\expandafter\def\csname v@buckeye/cfa-segment/opus/ebias-signed\endcsname{$-13$}
\expandafter\def\csname v@buckeye/cfa-segment/opus/fail\endcsname{5}
\expandafter\def\csname v@buckeye/cfa-segment/opus/fail-assert\endcsname{4}
\expandafter\def\csname v@buckeye/cfa-segment/opus/fail-crash\endcsname{1}
\expandafter\def\csname v@buckeye/cfa-segment/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/cfa-segment/opus/mae\endcsname{49.2}
\expandafter\def\csname v@buckeye/cfa-segment/opus/median\endcsname{32.9}
\expandafter\def\csname v@buckeye/cfa-segment/opus/over500\endcsname{0.3}
\expandafter\def\csname v@buckeye/cfa-segment/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/cfa-segment/opus/sbias\endcsname{39}
\expandafter\def\csname v@buckeye/cfa-segment/opus/sbias-signed\endcsname{$+39$}
\expandafter\def\csname v@buckeye/cfa-segment/opus/w10\endcsname{16.4}
\expandafter\def\csname v@buckeye/cfa-segment/opus/w100\endcsname{90.6}
\expandafter\def\csname v@buckeye/cfa-segment/opus/w20\endcsname{32.0}
\expandafter\def\csname v@buckeye/cfa-segment/opus/w50\endcsname{67.4}
\expandafter\def\csname v@buckeye/hours\endcsname{0.85}
\expandafter\def\csname v@buckeye/lag/amrnb\endcsname{5.000}
\expandafter\def\csname v@buckeye/lag/g711u\endcsname{0.000}
\expandafter\def\csname v@buckeye/lag/g723\endcsname{7.500}
\expandafter\def\csname v@buckeye/lag/gsm\endcsname{0.000}
\expandafter\def\csname v@buckeye/lag/opus\endcsname{0.125}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/ebias\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/fail\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/fail-other\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/mae\endcsname{21.0}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/median\endcsname{10.1}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/rtf\endcsname{0.027}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/sbias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/w10\endcsname{48.0}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/w100\endcsname{97.4}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/w20\endcsname{71.3}
\expandafter\def\csname v@buckeye/mfa-arpa/clean/w50\endcsname{92.3}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/dmae\endcsname{5.6}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/dw20\endcsname{5.8}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/dw50\endcsname{4.8}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/ebias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/fail\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/fail-other\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/mae\endcsname{26.6}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/median\endcsname{11.6}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/rtf\endcsname{0.029}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/sbias\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/w10\endcsname{44.2}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/w100\endcsname{94.9}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/w20\endcsname{65.5}
\expandafter\def\csname v@buckeye/mfa-arpa/g711u/w50\endcsname{87.5}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/dmae\endcsname{5.3}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/dw20\endcsname{6.6}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/dw50\endcsname{5.1}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/ebias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/fail\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/fail-other\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/mae\endcsname{26.3}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/median\endcsname{12.0}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/rtf\endcsname{0.027}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/sbias\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/w10\endcsname{43.3}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/w100\endcsname{95.1}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/w20\endcsname{64.6}
\expandafter\def\csname v@buckeye/mfa-arpa/gsm/w50\endcsname{87.2}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/dmae\endcsname{4.3}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/dw20\endcsname{5.4}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/dw50\endcsname{4.2}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/ebias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/fail\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/fail-other\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/mae\endcsname{25.3}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/median\endcsname{11.5}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/rtf\endcsname{0.027}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/sbias\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/w10\endcsname{44.2}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/w100\endcsname{95.5}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/w20\endcsname{65.9}
\expandafter\def\csname v@buckeye/mfa-arpa/opus/w50\endcsname{88.1}
\expandafter\def\csname v@buckeye/mfa-english/clean/ebias\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-english/clean/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@buckeye/mfa-english/clean/fail\endcsname{4}
\expandafter\def\csname v@buckeye/mfa-english/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/clean/fail-other\endcsname{4}
\expandafter\def\csname v@buckeye/mfa-english/clean/mae\endcsname{24.4}
\expandafter\def\csname v@buckeye/mfa-english/clean/median\endcsname{10.1}
\expandafter\def\csname v@buckeye/mfa-english/clean/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/mfa-english/clean/rtf\endcsname{0.015}
\expandafter\def\csname v@buckeye/mfa-english/clean/sbias\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@buckeye/mfa-english/clean/w10\endcsname{48.3}
\expandafter\def\csname v@buckeye/mfa-english/clean/w100\endcsname{95.8}
\expandafter\def\csname v@buckeye/mfa-english/clean/w20\endcsname{69.1}
\expandafter\def\csname v@buckeye/mfa-english/clean/w50\endcsname{88.9}
\expandafter\def\csname v@buckeye/mfa-english/g711u/dmae\endcsname{5.0}
\expandafter\def\csname v@buckeye/mfa-english/g711u/dw20\endcsname{5.9}
\expandafter\def\csname v@buckeye/mfa-english/g711u/dw50\endcsname{4.1}
\expandafter\def\csname v@buckeye/mfa-english/g711u/ebias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-english/g711u/fail\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/g711u/fail-other\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/g711u/mae\endcsname{29.4}
\expandafter\def\csname v@buckeye/mfa-english/g711u/median\endcsname{12.0}
\expandafter\def\csname v@buckeye/mfa-english/g711u/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/mfa-english/g711u/rtf\endcsname{0.015}
\expandafter\def\csname v@buckeye/mfa-english/g711u/sbias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/g711u/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-english/g711u/w10\endcsname{43.5}
\expandafter\def\csname v@buckeye/mfa-english/g711u/w100\endcsname{93.9}
\expandafter\def\csname v@buckeye/mfa-english/g711u/w20\endcsname{63.1}
\expandafter\def\csname v@buckeye/mfa-english/g711u/w50\endcsname{84.8}
\expandafter\def\csname v@buckeye/mfa-english/gsm/dmae\endcsname{6.7}
\expandafter\def\csname v@buckeye/mfa-english/gsm/dw20\endcsname{7.0}
\expandafter\def\csname v@buckeye/mfa-english/gsm/dw50\endcsname{5.0}
\expandafter\def\csname v@buckeye/mfa-english/gsm/ebias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-english/gsm/fail\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-english/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/gsm/fail-other\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-english/gsm/mae\endcsname{31.1}
\expandafter\def\csname v@buckeye/mfa-english/gsm/median\endcsname{12.8}
\expandafter\def\csname v@buckeye/mfa-english/gsm/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/mfa-english/gsm/rtf\endcsname{0.015}
\expandafter\def\csname v@buckeye/mfa-english/gsm/sbias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/gsm/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-english/gsm/w10\endcsname{41.9}
\expandafter\def\csname v@buckeye/mfa-english/gsm/w100\endcsname{93.3}
\expandafter\def\csname v@buckeye/mfa-english/gsm/w20\endcsname{62.1}
\expandafter\def\csname v@buckeye/mfa-english/gsm/w50\endcsname{83.9}
\expandafter\def\csname v@buckeye/mfa-english/opus/dmae\endcsname{3.4}
\expandafter\def\csname v@buckeye/mfa-english/opus/dw20\endcsname{5.1}
\expandafter\def\csname v@buckeye/mfa-english/opus/dw50\endcsname{3.3}
\expandafter\def\csname v@buckeye/mfa-english/opus/ebias\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@buckeye/mfa-english/opus/fail\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mfa-english/opus/fail-other\endcsname{1}
\expandafter\def\csname v@buckeye/mfa-english/opus/mae\endcsname{27.8}
\expandafter\def\csname v@buckeye/mfa-english/opus/median\endcsname{12.0}
\expandafter\def\csname v@buckeye/mfa-english/opus/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/mfa-english/opus/rtf\endcsname{0.014}
\expandafter\def\csname v@buckeye/mfa-english/opus/sbias\endcsname{2}
\expandafter\def\csname v@buckeye/mfa-english/opus/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@buckeye/mfa-english/opus/w10\endcsname{43.7}
\expandafter\def\csname v@buckeye/mfa-english/opus/w100\endcsname{94.4}
\expandafter\def\csname v@buckeye/mfa-english/opus/w20\endcsname{63.9}
\expandafter\def\csname v@buckeye/mfa-english/opus/w50\endcsname{85.6}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/ebias\endcsname{9}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/ebias-signed\endcsname{$-9$}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/mae\endcsname{41.4}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/median\endcsname{30.4}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/sbias\endcsname{41}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/sbias-signed\endcsname{$+41$}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/w10\endcsname{17.4}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/w100\endcsname{92.8}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/w20\endcsname{33.9}
\expandafter\def\csname v@buckeye/mms-torchaudio/clean/w50\endcsname{71.8}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/dmae\endcsname{2.5}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/dw50\endcsname{1.2}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/ebias\endcsname{8}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/ebias-signed\endcsname{$-8$}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/mae\endcsname{43.9}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/median\endcsname{31.5}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/sbias\endcsname{41}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/sbias-signed\endcsname{$+41$}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/w10\endcsname{17.0}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/w100\endcsname{92.0}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/w20\endcsname{33.2}
\expandafter\def\csname v@buckeye/mms-torchaudio/g711u/w50\endcsname{70.6}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/dmae\endcsname{5.4}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/dw50\endcsname{3.0}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/ebias\endcsname{7}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/ebias-signed\endcsname{$-7$}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/mae\endcsname{46.9}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/median\endcsname{32.8}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/over500\endcsname{0.3}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/sbias\endcsname{41}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/sbias-signed\endcsname{$+41$}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/w10\endcsname{16.5}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/w100\endcsname{90.8}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/w20\endcsname{31.9}
\expandafter\def\csname v@buckeye/mms-torchaudio/gsm/w50\endcsname{68.8}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/dmae\endcsname{3.3}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/dw20\endcsname{1.5}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/dw50\endcsname{2.0}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/ebias\endcsname{8}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/ebias-signed\endcsname{$-8$}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/mae\endcsname{44.8}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/median\endcsname{32.2}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/sbias\endcsname{41}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/sbias-signed\endcsname{$+41$}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/w10\endcsname{16.6}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/w100\endcsname{91.5}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/w20\endcsname{32.4}
\expandafter\def\csname v@buckeye/mms-torchaudio/opus/w50\endcsname{69.8}
\expandafter\def\csname v@buckeye/n-utt\endcsname{1{,}000}
\expandafter\def\csname v@buckeye/n-words\endcsname{11{,}374}
\expandafter\def\csname v@buckeye/qwen3fa/clean/ebias\endcsname{7}
\expandafter\def\csname v@buckeye/qwen3fa/clean/ebias-signed\endcsname{$-7$}
\expandafter\def\csname v@buckeye/qwen3fa/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/clean/mae\endcsname{30.9}
\expandafter\def\csname v@buckeye/qwen3fa/clean/median\endcsname{23.2}
\expandafter\def\csname v@buckeye/qwen3fa/clean/over500\endcsname{0.0}
\expandafter\def\csname v@buckeye/qwen3fa/clean/rtf\endcsname{0.020}
\expandafter\def\csname v@buckeye/qwen3fa/clean/sbias\endcsname{1}
\expandafter\def\csname v@buckeye/qwen3fa/clean/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@buckeye/qwen3fa/clean/w10\endcsname{21.3}
\expandafter\def\csname v@buckeye/qwen3fa/clean/w100\endcsname{97.2}
\expandafter\def\csname v@buckeye/qwen3fa/clean/w20\endcsname{42.5}
\expandafter\def\csname v@buckeye/qwen3fa/clean/w50\endcsname{84.5}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/dmae\endcsname{11.4}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/dw20\endcsname{6.4}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/dw50\endcsname{10.4}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/ebias\endcsname{16}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/ebias-signed\endcsname{$-16$}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/mae\endcsname{42.2}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/median\endcsname{28.4}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/rtf\endcsname{0.020}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/sbias\endcsname{13}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/sbias-signed\endcsname{$+13$}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/w10\endcsname{18.2}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/w100\endcsname{92.1}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/w20\endcsname{36.1}
\expandafter\def\csname v@buckeye/qwen3fa/g711u/w50\endcsname{74.1}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/dmae\endcsname{13.8}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/dw20\endcsname{7.8}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/dw50\endcsname{12.7}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/ebias\endcsname{17}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/ebias-signed\endcsname{$-17$}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/mae\endcsname{44.7}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/median\endcsname{30.0}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/rtf\endcsname{0.020}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/sbias\endcsname{16}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/sbias-signed\endcsname{$+16$}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/w10\endcsname{17.4}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/w100\endcsname{91.1}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/w20\endcsname{34.7}
\expandafter\def\csname v@buckeye/qwen3fa/gsm/w50\endcsname{71.8}
\expandafter\def\csname v@buckeye/qwen3fa/opus/dmae\endcsname{11.9}
\expandafter\def\csname v@buckeye/qwen3fa/opus/dw20\endcsname{6.7}
\expandafter\def\csname v@buckeye/qwen3fa/opus/dw50\endcsname{10.6}
\expandafter\def\csname v@buckeye/qwen3fa/opus/ebias\endcsname{16}
\expandafter\def\csname v@buckeye/qwen3fa/opus/ebias-signed\endcsname{$-16$}
\expandafter\def\csname v@buckeye/qwen3fa/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/qwen3fa/opus/mae\endcsname{42.8}
\expandafter\def\csname v@buckeye/qwen3fa/opus/median\endcsname{28.5}
\expandafter\def\csname v@buckeye/qwen3fa/opus/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/qwen3fa/opus/rtf\endcsname{0.020}
\expandafter\def\csname v@buckeye/qwen3fa/opus/sbias\endcsname{14}
\expandafter\def\csname v@buckeye/qwen3fa/opus/sbias-signed\endcsname{$+14$}
\expandafter\def\csname v@buckeye/qwen3fa/opus/w10\endcsname{18.0}
\expandafter\def\csname v@buckeye/qwen3fa/opus/w100\endcsname{92.0}
\expandafter\def\csname v@buckeye/qwen3fa/opus/w20\endcsname{35.8}
\expandafter\def\csname v@buckeye/qwen3fa/opus/w50\endcsname{73.9}
\expandafter\def\csname v@buckeye/stablets/clean/ebias\endcsname{32}
\expandafter\def\csname v@buckeye/stablets/clean/ebias-signed\endcsname{$-32$}
\expandafter\def\csname v@buckeye/stablets/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/clean/mae\endcsname{61.3}
\expandafter\def\csname v@buckeye/stablets/clean/median\endcsname{39.0}
\expandafter\def\csname v@buckeye/stablets/clean/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/stablets/clean/rtf\endcsname{0.041}
\expandafter\def\csname v@buckeye/stablets/clean/sbias\endcsname{20}
\expandafter\def\csname v@buckeye/stablets/clean/sbias-signed\endcsname{$-20$}
\expandafter\def\csname v@buckeye/stablets/clean/w10\endcsname{15.2}
\expandafter\def\csname v@buckeye/stablets/clean/w100\endcsname{82.7}
\expandafter\def\csname v@buckeye/stablets/clean/w20\endcsname{29.5}
\expandafter\def\csname v@buckeye/stablets/clean/w50\endcsname{59.4}
\expandafter\def\csname v@buckeye/stablets/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@buckeye/stablets/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@buckeye/stablets/g711u/dw50\endcsname{-0.4}
\expandafter\def\csname v@buckeye/stablets/g711u/ebias\endcsname{27}
\expandafter\def\csname v@buckeye/stablets/g711u/ebias-signed\endcsname{$-27$}
\expandafter\def\csname v@buckeye/stablets/g711u/fail\endcsname{1}
\expandafter\def\csname v@buckeye/stablets/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/g711u/fail-other\endcsname{1}
\expandafter\def\csname v@buckeye/stablets/g711u/mae\endcsname{61.9}
\expandafter\def\csname v@buckeye/stablets/g711u/median\endcsname{38.7}
\expandafter\def\csname v@buckeye/stablets/g711u/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/stablets/g711u/rtf\endcsname{0.040}
\expandafter\def\csname v@buckeye/stablets/g711u/sbias\endcsname{11}
\expandafter\def\csname v@buckeye/stablets/g711u/sbias-signed\endcsname{$-11$}
\expandafter\def\csname v@buckeye/stablets/g711u/w10\endcsname{14.8}
\expandafter\def\csname v@buckeye/stablets/g711u/w100\endcsname{82.4}
\expandafter\def\csname v@buckeye/stablets/g711u/w20\endcsname{28.8}
\expandafter\def\csname v@buckeye/stablets/g711u/w50\endcsname{59.9}
\expandafter\def\csname v@buckeye/stablets/gsm/dmae\endcsname{1.5}
\expandafter\def\csname v@buckeye/stablets/gsm/dw20\endcsname{1.0}
\expandafter\def\csname v@buckeye/stablets/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@buckeye/stablets/gsm/ebias\endcsname{28}
\expandafter\def\csname v@buckeye/stablets/gsm/ebias-signed\endcsname{$-28$}
\expandafter\def\csname v@buckeye/stablets/gsm/fail\endcsname{1}
\expandafter\def\csname v@buckeye/stablets/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/gsm/fail-other\endcsname{1}
\expandafter\def\csname v@buckeye/stablets/gsm/mae\endcsname{62.8}
\expandafter\def\csname v@buckeye/stablets/gsm/median\endcsname{39.3}
\expandafter\def\csname v@buckeye/stablets/gsm/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/stablets/gsm/rtf\endcsname{0.040}
\expandafter\def\csname v@buckeye/stablets/gsm/sbias\endcsname{11}
\expandafter\def\csname v@buckeye/stablets/gsm/sbias-signed\endcsname{$-11$}
\expandafter\def\csname v@buckeye/stablets/gsm/w10\endcsname{14.7}
\expandafter\def\csname v@buckeye/stablets/gsm/w100\endcsname{82.0}
\expandafter\def\csname v@buckeye/stablets/gsm/w20\endcsname{28.5}
\expandafter\def\csname v@buckeye/stablets/gsm/w50\endcsname{59.1}
\expandafter\def\csname v@buckeye/stablets/opus/dmae\endcsname{1.0}
\expandafter\def\csname v@buckeye/stablets/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@buckeye/stablets/opus/dw50\endcsname{-0.1}
\expandafter\def\csname v@buckeye/stablets/opus/ebias\endcsname{26}
\expandafter\def\csname v@buckeye/stablets/opus/ebias-signed\endcsname{$-26$}
\expandafter\def\csname v@buckeye/stablets/opus/fail\endcsname{1}
\expandafter\def\csname v@buckeye/stablets/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/stablets/opus/fail-other\endcsname{1}
\expandafter\def\csname v@buckeye/stablets/opus/mae\endcsname{62.3}
\expandafter\def\csname v@buckeye/stablets/opus/median\endcsname{39.0}
\expandafter\def\csname v@buckeye/stablets/opus/over500\endcsname{0.3}
\expandafter\def\csname v@buckeye/stablets/opus/rtf\endcsname{0.040}
\expandafter\def\csname v@buckeye/stablets/opus/sbias\endcsname{9}
\expandafter\def\csname v@buckeye/stablets/opus/sbias-signed\endcsname{$-9$}
\expandafter\def\csname v@buckeye/stablets/opus/w10\endcsname{14.8}
\expandafter\def\csname v@buckeye/stablets/opus/w100\endcsname{82.2}
\expandafter\def\csname v@buckeye/stablets/opus/w20\endcsname{28.6}
\expandafter\def\csname v@buckeye/stablets/opus/w50\endcsname{59.6}
\expandafter\def\csname v@buckeye/sttapi/clean/ebias\endcsname{9}
\expandafter\def\csname v@buckeye/sttapi/clean/ebias-signed\endcsname{$-9$}
\expandafter\def\csname v@buckeye/sttapi/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/clean/mae\endcsname{40.3}
\expandafter\def\csname v@buckeye/sttapi/clean/median\endcsname{27.7}
\expandafter\def\csname v@buckeye/sttapi/clean/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/sttapi/clean/rtf\endcsname{0.038}
\expandafter\def\csname v@buckeye/sttapi/clean/sbias\endcsname{31}
\expandafter\def\csname v@buckeye/sttapi/clean/sbias-signed\endcsname{$+31$}
\expandafter\def\csname v@buckeye/sttapi/clean/w10\endcsname{19.1}
\expandafter\def\csname v@buckeye/sttapi/clean/w100\endcsname{93.0}
\expandafter\def\csname v@buckeye/sttapi/clean/w20\endcsname{37.7}
\expandafter\def\csname v@buckeye/sttapi/clean/w50\endcsname{75.1}
\expandafter\def\csname v@buckeye/sttapi/g711u/dmae\endcsname{2.2}
\expandafter\def\csname v@buckeye/sttapi/g711u/dw20\endcsname{0.2}
\expandafter\def\csname v@buckeye/sttapi/g711u/dw50\endcsname{0.7}
\expandafter\def\csname v@buckeye/sttapi/g711u/ebias\endcsname{9}
\expandafter\def\csname v@buckeye/sttapi/g711u/ebias-signed\endcsname{$-9$}
\expandafter\def\csname v@buckeye/sttapi/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/g711u/mae\endcsname{42.4}
\expandafter\def\csname v@buckeye/sttapi/g711u/median\endcsname{28.0}
\expandafter\def\csname v@buckeye/sttapi/g711u/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/sttapi/g711u/rtf\endcsname{0.038}
\expandafter\def\csname v@buckeye/sttapi/g711u/sbias\endcsname{30}
\expandafter\def\csname v@buckeye/sttapi/g711u/sbias-signed\endcsname{$+30$}
\expandafter\def\csname v@buckeye/sttapi/g711u/w10\endcsname{19.1}
\expandafter\def\csname v@buckeye/sttapi/g711u/w100\endcsname{91.9}
\expandafter\def\csname v@buckeye/sttapi/g711u/w20\endcsname{37.5}
\expandafter\def\csname v@buckeye/sttapi/g711u/w50\endcsname{74.5}
\expandafter\def\csname v@buckeye/sttapi/gsm/dmae\endcsname{4.6}
\expandafter\def\csname v@buckeye/sttapi/gsm/dw20\endcsname{1.2}
\expandafter\def\csname v@buckeye/sttapi/gsm/dw50\endcsname{2.3}
\expandafter\def\csname v@buckeye/sttapi/gsm/ebias\endcsname{9}
\expandafter\def\csname v@buckeye/sttapi/gsm/ebias-signed\endcsname{$-9$}
\expandafter\def\csname v@buckeye/sttapi/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/gsm/mae\endcsname{44.8}
\expandafter\def\csname v@buckeye/sttapi/gsm/median\endcsname{29.0}
\expandafter\def\csname v@buckeye/sttapi/gsm/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/sttapi/gsm/rtf\endcsname{0.038}
\expandafter\def\csname v@buckeye/sttapi/gsm/sbias\endcsname{31}
\expandafter\def\csname v@buckeye/sttapi/gsm/sbias-signed\endcsname{$+31$}
\expandafter\def\csname v@buckeye/sttapi/gsm/w10\endcsname{18.7}
\expandafter\def\csname v@buckeye/sttapi/gsm/w100\endcsname{90.7}
\expandafter\def\csname v@buckeye/sttapi/gsm/w20\endcsname{36.5}
\expandafter\def\csname v@buckeye/sttapi/gsm/w50\endcsname{72.8}
\expandafter\def\csname v@buckeye/sttapi/opus/dmae\endcsname{3.5}
\expandafter\def\csname v@buckeye/sttapi/opus/dw20\endcsname{0.7}
\expandafter\def\csname v@buckeye/sttapi/opus/dw50\endcsname{1.7}
\expandafter\def\csname v@buckeye/sttapi/opus/ebias\endcsname{9}
\expandafter\def\csname v@buckeye/sttapi/opus/ebias-signed\endcsname{$-9$}
\expandafter\def\csname v@buckeye/sttapi/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/sttapi/opus/mae\endcsname{43.7}
\expandafter\def\csname v@buckeye/sttapi/opus/median\endcsname{28.5}
\expandafter\def\csname v@buckeye/sttapi/opus/over500\endcsname{0.2}
\expandafter\def\csname v@buckeye/sttapi/opus/rtf\endcsname{0.038}
\expandafter\def\csname v@buckeye/sttapi/opus/sbias\endcsname{31}
\expandafter\def\csname v@buckeye/sttapi/opus/sbias-signed\endcsname{$+31$}
\expandafter\def\csname v@buckeye/sttapi/opus/w10\endcsname{18.5}
\expandafter\def\csname v@buckeye/sttapi/opus/w100\endcsname{91.3}
\expandafter\def\csname v@buckeye/sttapi/opus/w20\endcsname{37.0}
\expandafter\def\csname v@buckeye/sttapi/opus/w50\endcsname{73.4}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/ebias\endcsname{10}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/mae\endcsname{36.3}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/median\endcsname{24.2}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/over500\endcsname{0.0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/rtf\endcsname{0.022}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/sbias\endcsname{6}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/sbias-signed\endcsname{$+6$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/w10\endcsname{21.5}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/w100\endcsname{94.8}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/w20\endcsname{42.1}
\expandafter\def\csname v@buckeye/whisper-tm-cal/clean/w50\endcsname{79.0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/dw50\endcsname{0.6}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/ebias\endcsname{11}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/ebias-signed\endcsname{$+11$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/mae\endcsname{37.0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/median\endcsname{24.7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/rtf\endcsname{0.022}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/sbias\endcsname{7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/w10\endcsname{20.4}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/w100\endcsname{94.6}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/w20\endcsname{41.2}
\expandafter\def\csname v@buckeye/whisper-tm-cal/g711u/w50\endcsname{78.5}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/dmae\endcsname{1.7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/dw20\endcsname{2.4}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/dw50\endcsname{1.8}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/ebias\endcsname{12}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/ebias-signed\endcsname{$+12$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/mae\endcsname{38.0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/median\endcsname{25.7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/rtf\endcsname{0.021}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/sbias\endcsname{8}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/sbias-signed\endcsname{$+8$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/w10\endcsname{20.1}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/w100\endcsname{94.4}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/w20\endcsname{39.7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/gsm/w50\endcsname{77.3}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/dmae\endcsname{1.1}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/dw20\endcsname{1.5}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/dw50\endcsname{1.2}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/ebias\endcsname{11}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/ebias-signed\endcsname{$+11$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/mae\endcsname{37.4}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/median\endcsname{25.2}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/over500\endcsname{0.0}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/rtf\endcsname{0.022}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/sbias\endcsname{7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/w10\endcsname{20.4}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/w100\endcsname{94.4}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/w20\endcsname{40.7}
\expandafter\def\csname v@buckeye/whisper-tm-cal/opus/w50\endcsname{77.9}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/ebias\endcsname{882}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/ebias-signed\endcsname{$+882$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/mae\endcsname{1491.6}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/median\endcsname{1109.9}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/over500\endcsname{75.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/rtf\endcsname{0.031}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/sbias\endcsname{867}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/sbias-signed\endcsname{$+867$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/w10\endcsname{0.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/w100\endcsname{8.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/w20\endcsname{0.4}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/clean/w50\endcsname{1.8}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/dmae\endcsname{36.1}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/dw20\endcsname{-0.0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/ebias\endcsname{991}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/ebias-signed\endcsname{$+991$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/mae\endcsname{1527.7}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/median\endcsname{1142.0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/over500\endcsname{75.8}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/rtf\endcsname{0.034}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/sbias\endcsname{981}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/sbias-signed\endcsname{$+981$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/w10\endcsname{0.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/w100\endcsname{8.4}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/w20\endcsname{0.4}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/g711u/w50\endcsname{1.9}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/dmae\endcsname{-37.5}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/dw20\endcsname{-0.1}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/dw50\endcsname{-0.1}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/ebias\endcsname{791}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/ebias-signed\endcsname{$+791$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/mae\endcsname{1454.1}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/median\endcsname{1074.8}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/over500\endcsname{73.8}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/rtf\endcsname{0.034}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/sbias\endcsname{780}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/sbias-signed\endcsname{$+780$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/w10\endcsname{0.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/w100\endcsname{8.5}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/w20\endcsname{0.4}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/gsm/w50\endcsname{2.0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/dmae\endcsname{10.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/dw20\endcsname{-0.1}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/dw50\endcsname{-0.1}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/ebias\endcsname{902}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/ebias-signed\endcsname{$+902$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/mae\endcsname{1501.8}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/median\endcsname{1109.1}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/over500\endcsname{75.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/rtf\endcsname{0.034}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/sbias\endcsname{891}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/sbias-signed\endcsname{$+891$}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/w10\endcsname{0.2}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/w100\endcsname{8.5}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/w20\endcsname{0.5}
\expandafter\def\csname v@buckeye/whisper-tm-cfg/opus/w50\endcsname{2.0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/ebias\endcsname{105}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/ebias-signed\endcsname{$-105$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/mae\endcsname{127.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/median\endcsname{100.0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/over500\endcsname{0.8}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/rtf\endcsname{0.031}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/sbias\endcsname{100}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/sbias-signed\endcsname{$-100$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/w10\endcsname{1.9}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/w100\endcsname{48.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/w20\endcsname{4.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/clean/w50\endcsname{16.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/dw20\endcsname{-0.0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/dw50\endcsname{-0.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/ebias\endcsname{106}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/ebias-signed\endcsname{$-106$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/mae\endcsname{127.9}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/median\endcsname{100.6}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/over500\endcsname{0.8}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/rtf\endcsname{0.030}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/sbias\endcsname{100}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/sbias-signed\endcsname{$-100$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/w10\endcsname{1.8}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/w100\endcsname{47.7}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/w20\endcsname{4.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/g711u/w50\endcsname{16.4}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/dmae\endcsname{-0.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/dw20\endcsname{-0.4}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/dw50\endcsname{-1.0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/ebias\endcsname{106}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/ebias-signed\endcsname{$-106$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/mae\endcsname{127.0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/median\endcsname{100.0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/over500\endcsname{0.8}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/rtf\endcsname{0.031}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/sbias\endcsname{100}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/sbias-signed\endcsname{$-100$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/w10\endcsname{2.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/w100\endcsname{48.1}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/w20\endcsname{4.6}
\expandafter\def\csname v@buckeye/whisper-tm-oai/gsm/w50\endcsname{17.2}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/dmae\endcsname{-0.3}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/dw20\endcsname{-0.1}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/dw50\endcsname{-0.8}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/ebias\endcsname{105}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/ebias-signed\endcsname{$-105$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/mae\endcsname{126.9}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/median\endcsname{100.0}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/over500\endcsname{0.8}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/rtf\endcsname{0.032}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/sbias\endcsname{100}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/sbias-signed\endcsname{$-100$}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/w10\endcsname{1.9}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/w100\endcsname{48.4}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/w20\endcsname{4.3}
\expandafter\def\csname v@buckeye/whisper-tm-oai/opus/w50\endcsname{17.0}
\expandafter\def\csname v@buckeye/whisperx/clean/ebias\endcsname{6}
\expandafter\def\csname v@buckeye/whisperx/clean/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@buckeye/whisperx/clean/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/clean/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/clean/mae\endcsname{50.2}
\expandafter\def\csname v@buckeye/whisperx/clean/median\endcsname{40.0}
\expandafter\def\csname v@buckeye/whisperx/clean/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/whisperx/clean/rtf\endcsname{0.018}
\expandafter\def\csname v@buckeye/whisperx/clean/sbias\endcsname{56}
\expandafter\def\csname v@buckeye/whisperx/clean/sbias-signed\endcsname{$+56$}
\expandafter\def\csname v@buckeye/whisperx/clean/w10\endcsname{14.0}
\expandafter\def\csname v@buckeye/whisperx/clean/w100\endcsname{89.9}
\expandafter\def\csname v@buckeye/whisperx/clean/w20\endcsname{27.1}
\expandafter\def\csname v@buckeye/whisperx/clean/w50\endcsname{61.2}
\expandafter\def\csname v@buckeye/whisperx/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@buckeye/whisperx/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@buckeye/whisperx/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@buckeye/whisperx/g711u/ebias\endcsname{6}
\expandafter\def\csname v@buckeye/whisperx/g711u/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@buckeye/whisperx/g711u/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/g711u/mae\endcsname{50.6}
\expandafter\def\csname v@buckeye/whisperx/g711u/median\endcsname{40.0}
\expandafter\def\csname v@buckeye/whisperx/g711u/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/whisperx/g711u/rtf\endcsname{0.014}
\expandafter\def\csname v@buckeye/whisperx/g711u/sbias\endcsname{55}
\expandafter\def\csname v@buckeye/whisperx/g711u/sbias-signed\endcsname{$+55$}
\expandafter\def\csname v@buckeye/whisperx/g711u/w10\endcsname{13.7}
\expandafter\def\csname v@buckeye/whisperx/g711u/w100\endcsname{89.9}
\expandafter\def\csname v@buckeye/whisperx/g711u/w20\endcsname{26.4}
\expandafter\def\csname v@buckeye/whisperx/g711u/w50\endcsname{60.9}
\expandafter\def\csname v@buckeye/whisperx/gsm/dmae\endcsname{1.4}
\expandafter\def\csname v@buckeye/whisperx/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@buckeye/whisperx/gsm/dw50\endcsname{1.1}
\expandafter\def\csname v@buckeye/whisperx/gsm/ebias\endcsname{7}
\expandafter\def\csname v@buckeye/whisperx/gsm/ebias-signed\endcsname{$+7$}
\expandafter\def\csname v@buckeye/whisperx/gsm/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/gsm/mae\endcsname{51.6}
\expandafter\def\csname v@buckeye/whisperx/gsm/median\endcsname{40.6}
\expandafter\def\csname v@buckeye/whisperx/gsm/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/whisperx/gsm/rtf\endcsname{0.014}
\expandafter\def\csname v@buckeye/whisperx/gsm/sbias\endcsname{56}
\expandafter\def\csname v@buckeye/whisperx/gsm/sbias-signed\endcsname{$+56$}
\expandafter\def\csname v@buckeye/whisperx/gsm/w10\endcsname{13.2}
\expandafter\def\csname v@buckeye/whisperx/gsm/w100\endcsname{89.6}
\expandafter\def\csname v@buckeye/whisperx/gsm/w20\endcsname{25.4}
\expandafter\def\csname v@buckeye/whisperx/gsm/w50\endcsname{60.1}
\expandafter\def\csname v@buckeye/whisperx/opus/dmae\endcsname{1.2}
\expandafter\def\csname v@buckeye/whisperx/opus/dw20\endcsname{1.4}
\expandafter\def\csname v@buckeye/whisperx/opus/dw50\endcsname{0.9}
\expandafter\def\csname v@buckeye/whisperx/opus/ebias\endcsname{7}
\expandafter\def\csname v@buckeye/whisperx/opus/ebias-signed\endcsname{$+7$}
\expandafter\def\csname v@buckeye/whisperx/opus/fail\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/opus/fail-other\endcsname{0}
\expandafter\def\csname v@buckeye/whisperx/opus/mae\endcsname{51.4}
\expandafter\def\csname v@buckeye/whisperx/opus/median\endcsname{40.6}
\expandafter\def\csname v@buckeye/whisperx/opus/over500\endcsname{0.1}
\expandafter\def\csname v@buckeye/whisperx/opus/rtf\endcsname{0.014}
\expandafter\def\csname v@buckeye/whisperx/opus/sbias\endcsname{56}
\expandafter\def\csname v@buckeye/whisperx/opus/sbias-signed\endcsname{$+56$}
\expandafter\def\csname v@buckeye/whisperx/opus/w10\endcsname{13.4}
\expandafter\def\csname v@buckeye/whisperx/opus/w100\endcsname{89.6}
\expandafter\def\csname v@buckeye/whisperx/opus/w20\endcsname{25.7}
\expandafter\def\csname v@buckeye/whisperx/opus/w50\endcsname{60.2}
\expandafter\def\csname v@ce/aug0/buckeye/ce/mae\endcsname{18.6}
\expandafter\def\csname v@ce/aug0/buckeye/ce/w20\endcsname{76}
\expandafter\def\csname v@ce/aug0/buckeye/clean/mae\endcsname{12.3}
\expandafter\def\csname v@ce/aug0/buckeye/clean/w20\endcsname{86}
\expandafter\def\csname v@ce/aug0/buckeye/codecs/mae\endcsname{15.4}
\expandafter\def\csname v@ce/aug0/buckeye/codecs/w20\endcsname{81}
\expandafter\def\csname v@ce/aug0/timit/ce/mae\endcsname{20.9}
\expandafter\def\csname v@ce/aug0/timit/ce/w20\endcsname{70}
\expandafter\def\csname v@ce/aug0/timit/clean/mae\endcsname{10.4}
\expandafter\def\csname v@ce/aug0/timit/clean/w20\endcsname{89}
\expandafter\def\csname v@ce/aug0/timit/codecs/mae\endcsname{17.1}
\expandafter\def\csname v@ce/aug0/timit/codecs/w20\endcsname{75}
\expandafter\def\csname v@ce/ctcw/buckeye/ce/mae\endcsname{17.4}
\expandafter\def\csname v@ce/ctcw/buckeye/ce/w20\endcsname{75}
\expandafter\def\csname v@ce/ctcw/buckeye/clean/mae\endcsname{14.0}
\expandafter\def\csname v@ce/ctcw/buckeye/clean/w20\endcsname{81}
\expandafter\def\csname v@ce/ctcw/buckeye/codecs/mae\endcsname{14.7}
\expandafter\def\csname v@ce/ctcw/buckeye/codecs/w20\endcsname{79}
\expandafter\def\csname v@ce/ctcw/timit/ce/mae\endcsname{19.9}
\expandafter\def\csname v@ce/ctcw/timit/ce/w20\endcsname{70}
\expandafter\def\csname v@ce/ctcw/timit/clean/mae\endcsname{16.4}
\expandafter\def\csname v@ce/ctcw/timit/clean/w20\endcsname{76}
\expandafter\def\csname v@ce/ctcw/timit/codecs/mae\endcsname{16.4}
\expandafter\def\csname v@ce/ctcw/timit/codecs/w20\endcsname{76}
\expandafter\def\csname v@ce/default/buckeye/ce/mae\endcsname{17.0}
\expandafter\def\csname v@ce/default/buckeye/ce/w20\endcsname{79}
\expandafter\def\csname v@ce/default/buckeye/clean/mae\endcsname{12.0}
\expandafter\def\csname v@ce/default/buckeye/clean/w20\endcsname{86}
\expandafter\def\csname v@ce/default/buckeye/codecs/mae\endcsname{12.9}
\expandafter\def\csname v@ce/default/buckeye/codecs/w20\endcsname{85}
\expandafter\def\csname v@ce/default/timit/ce/mae\endcsname{16.6}
\expandafter\def\csname v@ce/default/timit/ce/w20\endcsname{79}
\expandafter\def\csname v@ce/default/timit/clean/mae\endcsname{10.5}
\expandafter\def\csname v@ce/default/timit/clean/w20\endcsname{89}
\expandafter\def\csname v@ce/default/timit/codecs/mae\endcsname{11.2}
\expandafter\def\csname v@ce/default/timit/codecs/w20\endcsname{88}
\expandafter\def\csname v@ce/mfa/buckeye/ce/mae\endcsname{46.1}
\expandafter\def\csname v@ce/mfa/buckeye/ce/w20\endcsname{55}
\expandafter\def\csname v@ce/mfa/buckeye/clean/mae\endcsname{21.5}
\expandafter\def\csname v@ce/mfa/buckeye/clean/w20\endcsname{71}
\expandafter\def\csname v@ce/mfa/buckeye/codecs/mae\endcsname{26.6}
\expandafter\def\csname v@ce/mfa/buckeye/codecs/w20\endcsname{65}
\expandafter\def\csname v@ce/mfa/timit/ce/failed\endcsname{37}
\expandafter\def\csname v@ce/mfa/timit/ce/mae\endcsname{43.1}
\expandafter\def\csname v@ce/mfa/timit/ce/w20\endcsname{53}
\expandafter\def\csname v@ce/mfa/timit/clean/mae\endcsname{19.1}
\expandafter\def\csname v@ce/mfa/timit/clean/w20\endcsname{68}
\expandafter\def\csname v@ce/mfa/timit/codecs/mae\endcsname{25.7}
\expandafter\def\csname v@ce/mfa/timit/codecs/w20\endcsname{63}
\expandafter\def\csname v@ce/post/buckeye/ce/mae\endcsname{15.9}
\expandafter\def\csname v@ce/post/buckeye/ce/w20\endcsname{80}
\expandafter\def\csname v@ce/post/buckeye/clean/mae\endcsname{11.3}
\expandafter\def\csname v@ce/post/buckeye/clean/w20\endcsname{86}
\expandafter\def\csname v@ce/post/buckeye/codecs/mae\endcsname{12.0}
\expandafter\def\csname v@ce/post/buckeye/codecs/w20\endcsname{86}
\expandafter\def\csname v@ce/post/timit/ce/mae\endcsname{16.3}
\expandafter\def\csname v@ce/post/timit/ce/w20\endcsname{78}
\expandafter\def\csname v@ce/post/timit/clean/mae\endcsname{10.5}
\expandafter\def\csname v@ce/post/timit/clean/w20\endcsname{89}
\expandafter\def\csname v@ce/post/timit/codecs/mae\endcsname{11.2}
\expandafter\def\csname v@ce/post/timit/codecs/w20\endcsname{88}
\expandafter\def\csname v@ce/posttn/buckeye/ce/mae\endcsname{15.9}
\expandafter\def\csname v@ce/posttn/buckeye/ce/w20\endcsname{80}
\expandafter\def\csname v@ce/posttn/buckeye/clean/mae\endcsname{11.1}
\expandafter\def\csname v@ce/posttn/buckeye/clean/w20\endcsname{86}
\expandafter\def\csname v@ce/posttn/buckeye/codecs/mae\endcsname{11.7}
\expandafter\def\csname v@ce/posttn/buckeye/codecs/w20\endcsname{86}
\expandafter\def\csname v@ce/posttn/timit/ce/mae\endcsname{16.4}
\expandafter\def\csname v@ce/posttn/timit/ce/w20\endcsname{78}
\expandafter\def\csname v@ce/posttn/timit/clean/mae\endcsname{10.7}
\expandafter\def\csname v@ce/posttn/timit/clean/w20\endcsname{89}
\expandafter\def\csname v@ce/posttn/timit/codecs/mae\endcsname{11.3}
\expandafter\def\csname v@ce/posttn/timit/codecs/w20\endcsname{87}
\expandafter\def\csname v@ce/rel-turbo/buckeye/ce/mae\endcsname{14.5}
\expandafter\def\csname v@ce/rel-turbo/buckeye/ce/w20\endcsname{81}
\expandafter\def\csname v@ce/rel-turbo/buckeye/clean/mae\endcsname{11.3}
\expandafter\def\csname v@ce/rel-turbo/buckeye/clean/w20\endcsname{86}
\expandafter\def\csname v@ce/rel-turbo/buckeye/codecs/mae\endcsname{12.7}
\expandafter\def\csname v@ce/rel-turbo/buckeye/codecs/w20\endcsname{84}
\expandafter\def\csname v@ce/rel-turbo/timit/ce/mae\endcsname{14.1}
\expandafter\def\csname v@ce/rel-turbo/timit/ce/w20\endcsname{82}
\expandafter\def\csname v@ce/rel-turbo/timit/clean/mae\endcsname{10.9}
\expandafter\def\csname v@ce/rel-turbo/timit/clean/w20\endcsname{88}
\expandafter\def\csname v@ce/rel-turbo/timit/codecs/mae\endcsname{11.8}
\expandafter\def\csname v@ce/rel-turbo/timit/codecs/w20\endcsname{86}
\expandafter\def\csname v@ce/rel-v3/buckeye/ce/mae\endcsname{13.5}
\expandafter\def\csname v@ce/rel-v3/buckeye/ce/w20\endcsname{82}
\expandafter\def\csname v@ce/rel-v3/buckeye/clean/mae\endcsname{11.2}
\expandafter\def\csname v@ce/rel-v3/buckeye/clean/w20\endcsname{86}
\expandafter\def\csname v@ce/rel-v3/buckeye/codecs/mae\endcsname{12.5}
\expandafter\def\csname v@ce/rel-v3/buckeye/codecs/w20\endcsname{85}
\expandafter\def\csname v@ce/rel-v3/timit/ce/mae\endcsname{13.4}
\expandafter\def\csname v@ce/rel-v3/timit/ce/w20\endcsname{83}
\expandafter\def\csname v@ce/rel-v3/timit/clean/mae\endcsname{10.6}
\expandafter\def\csname v@ce/rel-v3/timit/clean/w20\endcsname{89}
\expandafter\def\csname v@ce/rel-v3/timit/codecs/mae\endcsname{11.8}
\expandafter\def\csname v@ce/rel-v3/timit/codecs/w20\endcsname{86}
\expandafter\def\csname v@ce/timit/n-common\endcsname{1{,}307}
\expandafter\def\csname v@class/cfa-edges/offset/burst\endcsname{1}
\expandafter\def\csname v@class/cfa-edges/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/cfa-edges/offset/closure\endcsname{17}
\expandafter\def\csname v@class/cfa-edges/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/cfa-edges/offset/fricative\endcsname{2}
\expandafter\def\csname v@class/cfa-edges/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/cfa-edges/offset/liquid\endcsname{22}
\expandafter\def\csname v@class/cfa-edges/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/cfa-edges/offset/nasal\endcsname{12}
\expandafter\def\csname v@class/cfa-edges/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/cfa-edges/offset/vowel\endcsname{18}
\expandafter\def\csname v@class/cfa-edges/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/cfa-edges/onset/burst\endcsname{12}
\expandafter\def\csname v@class/cfa-edges/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/cfa-edges/onset/closure\endcsname{22}
\expandafter\def\csname v@class/cfa-edges/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/cfa-edges/onset/fricative\endcsname{13}
\expandafter\def\csname v@class/cfa-edges/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/cfa-edges/onset/liquid\endcsname{8}
\expandafter\def\csname v@class/cfa-edges/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/cfa-edges/onset/nasal\endcsname{9}
\expandafter\def\csname v@class/cfa-edges/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/cfa-edges/onset/vowel\endcsname{4}
\expandafter\def\csname v@class/cfa-edges/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/cfa-segment/offset/burst\endcsname{24}
\expandafter\def\csname v@class/cfa-segment/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/cfa-segment/offset/closure\endcsname{39}
\expandafter\def\csname v@class/cfa-segment/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/cfa-segment/offset/fricative\endcsname{26}
\expandafter\def\csname v@class/cfa-segment/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/cfa-segment/offset/liquid\endcsname{5}
\expandafter\def\csname v@class/cfa-segment/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/cfa-segment/offset/nasal\endcsname{20}
\expandafter\def\csname v@class/cfa-segment/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/cfa-segment/offset/vowel\endcsname{18}
\expandafter\def\csname v@class/cfa-segment/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/cfa-segment/onset/burst\endcsname{2}
\expandafter\def\csname v@class/cfa-segment/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/cfa-segment/onset/closure\endcsname{47}
\expandafter\def\csname v@class/cfa-segment/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/cfa-segment/onset/fricative\endcsname{38}
\expandafter\def\csname v@class/cfa-segment/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/cfa-segment/onset/liquid\endcsname{32}
\expandafter\def\csname v@class/cfa-segment/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/cfa-segment/onset/nasal\endcsname{35}
\expandafter\def\csname v@class/cfa-segment/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/cfa-segment/onset/vowel\endcsname{27}
\expandafter\def\csname v@class/cfa-segment/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/mfa-arpa/offset/burst\endcsname{2}
\expandafter\def\csname v@class/mfa-arpa/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/mfa-arpa/offset/closure\endcsname{18}
\expandafter\def\csname v@class/mfa-arpa/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/mfa-arpa/offset/fricative\endcsname{2}
\expandafter\def\csname v@class/mfa-arpa/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/mfa-arpa/offset/liquid\endcsname{6}
\expandafter\def\csname v@class/mfa-arpa/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/mfa-arpa/offset/nasal\endcsname{6}
\expandafter\def\csname v@class/mfa-arpa/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/mfa-arpa/offset/vowel\endcsname{3}
\expandafter\def\csname v@class/mfa-arpa/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/mfa-arpa/onset/burst\endcsname{18}
\expandafter\def\csname v@class/mfa-arpa/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/mfa-arpa/onset/closure\endcsname{4}
\expandafter\def\csname v@class/mfa-arpa/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/mfa-arpa/onset/fricative\endcsname{7}
\expandafter\def\csname v@class/mfa-arpa/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/mfa-arpa/onset/liquid\endcsname{6}
\expandafter\def\csname v@class/mfa-arpa/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/mfa-arpa/onset/nasal\endcsname{2}
\expandafter\def\csname v@class/mfa-arpa/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/mfa-arpa/onset/vowel\endcsname{1}
\expandafter\def\csname v@class/mfa-arpa/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/mfa-english/offset/burst\endcsname{5}
\expandafter\def\csname v@class/mfa-english/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/mfa-english/offset/closure\endcsname{26}
\expandafter\def\csname v@class/mfa-english/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/mfa-english/offset/fricative\endcsname{4}
\expandafter\def\csname v@class/mfa-english/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/mfa-english/offset/liquid\endcsname{4}
\expandafter\def\csname v@class/mfa-english/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/mfa-english/offset/nasal\endcsname{5}
\expandafter\def\csname v@class/mfa-english/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/mfa-english/offset/vowel\endcsname{3}
\expandafter\def\csname v@class/mfa-english/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/mfa-english/onset/burst\endcsname{22}
\expandafter\def\csname v@class/mfa-english/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/mfa-english/onset/closure\endcsname{6}
\expandafter\def\csname v@class/mfa-english/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/mfa-english/onset/fricative\endcsname{7}
\expandafter\def\csname v@class/mfa-english/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/mfa-english/onset/liquid\endcsname{10}
\expandafter\def\csname v@class/mfa-english/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/mfa-english/onset/nasal\endcsname{2}
\expandafter\def\csname v@class/mfa-english/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/mfa-english/onset/vowel\endcsname{0}
\expandafter\def\csname v@class/mfa-english/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/mms-torchaudio/offset/burst\endcsname{25}
\expandafter\def\csname v@class/mms-torchaudio/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/mms-torchaudio/offset/closure\endcsname{36}
\expandafter\def\csname v@class/mms-torchaudio/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/mms-torchaudio/offset/fricative\endcsname{28}
\expandafter\def\csname v@class/mms-torchaudio/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/mms-torchaudio/offset/liquid\endcsname{0}
\expandafter\def\csname v@class/mms-torchaudio/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/mms-torchaudio/offset/nasal\endcsname{12}
\expandafter\def\csname v@class/mms-torchaudio/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/mms-torchaudio/offset/vowel\endcsname{13}
\expandafter\def\csname v@class/mms-torchaudio/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/mms-torchaudio/onset/burst\endcsname{6}
\expandafter\def\csname v@class/mms-torchaudio/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/mms-torchaudio/onset/closure\endcsname{54}
\expandafter\def\csname v@class/mms-torchaudio/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/mms-torchaudio/onset/fricative\endcsname{41}
\expandafter\def\csname v@class/mms-torchaudio/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/mms-torchaudio/onset/liquid\endcsname{36}
\expandafter\def\csname v@class/mms-torchaudio/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/mms-torchaudio/onset/nasal\endcsname{39}
\expandafter\def\csname v@class/mms-torchaudio/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/mms-torchaudio/onset/vowel\endcsname{33}
\expandafter\def\csname v@class/mms-torchaudio/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/qwen3fa/offset/burst\endcsname{7}
\expandafter\def\csname v@class/qwen3fa/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/qwen3fa/offset/closure\endcsname{27}
\expandafter\def\csname v@class/qwen3fa/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/qwen3fa/offset/fricative\endcsname{0}
\expandafter\def\csname v@class/qwen3fa/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/qwen3fa/offset/liquid\endcsname{2}
\expandafter\def\csname v@class/qwen3fa/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/qwen3fa/offset/nasal\endcsname{5}
\expandafter\def\csname v@class/qwen3fa/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/qwen3fa/offset/vowel\endcsname{1}
\expandafter\def\csname v@class/qwen3fa/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/qwen3fa/onset/burst\endcsname{6}
\expandafter\def\csname v@class/qwen3fa/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/qwen3fa/onset/closure\endcsname{8}
\expandafter\def\csname v@class/qwen3fa/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/qwen3fa/onset/fricative\endcsname{2}
\expandafter\def\csname v@class/qwen3fa/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/qwen3fa/onset/liquid\endcsname{13}
\expandafter\def\csname v@class/qwen3fa/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/qwen3fa/onset/nasal\endcsname{10}
\expandafter\def\csname v@class/qwen3fa/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/qwen3fa/onset/vowel\endcsname{8}
\expandafter\def\csname v@class/qwen3fa/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/stablets/offset/burst\endcsname{77}
\expandafter\def\csname v@class/stablets/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/stablets/offset/closure\endcsname{84}
\expandafter\def\csname v@class/stablets/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/stablets/offset/fricative\endcsname{68}
\expandafter\def\csname v@class/stablets/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/stablets/offset/liquid\endcsname{45}
\expandafter\def\csname v@class/stablets/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/stablets/offset/nasal\endcsname{58}
\expandafter\def\csname v@class/stablets/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/stablets/offset/vowel\endcsname{23}
\expandafter\def\csname v@class/stablets/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/stablets/onset/burst\endcsname{18}
\expandafter\def\csname v@class/stablets/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/stablets/onset/closure\endcsname{3}
\expandafter\def\csname v@class/stablets/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/stablets/onset/fricative\endcsname{15}
\expandafter\def\csname v@class/stablets/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/stablets/onset/liquid\endcsname{20}
\expandafter\def\csname v@class/stablets/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/stablets/onset/nasal\endcsname{15}
\expandafter\def\csname v@class/stablets/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/stablets/onset/vowel\endcsname{42}
\expandafter\def\csname v@class/stablets/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/sttapi/offset/burst\endcsname{24}
\expandafter\def\csname v@class/sttapi/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/sttapi/offset/closure\endcsname{34}
\expandafter\def\csname v@class/sttapi/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/sttapi/offset/fricative\endcsname{29}
\expandafter\def\csname v@class/sttapi/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/sttapi/offset/liquid\endcsname{7}
\expandafter\def\csname v@class/sttapi/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/sttapi/offset/nasal\endcsname{17}
\expandafter\def\csname v@class/sttapi/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/sttapi/offset/vowel\endcsname{10}
\expandafter\def\csname v@class/sttapi/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/sttapi/onset/burst\endcsname{5}
\expandafter\def\csname v@class/sttapi/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/sttapi/onset/closure\endcsname{42}
\expandafter\def\csname v@class/sttapi/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/sttapi/onset/fricative\endcsname{30}
\expandafter\def\csname v@class/sttapi/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/sttapi/onset/liquid\endcsname{26}
\expandafter\def\csname v@class/sttapi/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/sttapi/onset/nasal\endcsname{27}
\expandafter\def\csname v@class/sttapi/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/sttapi/onset/vowel\endcsname{24}
\expandafter\def\csname v@class/sttapi/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@class/whisperx/offset/burst\endcsname{16}
\expandafter\def\csname v@class/whisperx/offset/burst/n\endcsname{906}
\expandafter\def\csname v@class/whisperx/offset/closure\endcsname{26}
\expandafter\def\csname v@class/whisperx/offset/closure/n\endcsname{1{,}088}
\expandafter\def\csname v@class/whisperx/offset/fricative\endcsname{18}
\expandafter\def\csname v@class/whisperx/offset/fricative/n\endcsname{2{,}611}
\expandafter\def\csname v@class/whisperx/offset/liquid\endcsname{16}
\expandafter\def\csname v@class/whisperx/offset/liquid/n\endcsname{986}
\expandafter\def\csname v@class/whisperx/offset/nasal\endcsname{4}
\expandafter\def\csname v@class/whisperx/offset/nasal/n\endcsname{1{,}728}
\expandafter\def\csname v@class/whisperx/offset/vowel\endcsname{19}
\expandafter\def\csname v@class/whisperx/offset/vowel/n\endcsname{3{,}705}
\expandafter\def\csname v@class/whisperx/onset/burst\endcsname{24}
\expandafter\def\csname v@class/whisperx/onset/burst/n\endcsname{1{,}270}
\expandafter\def\csname v@class/whisperx/onset/closure\endcsname{73}
\expandafter\def\csname v@class/whisperx/onset/closure/n\endcsname{2{,}029}
\expandafter\def\csname v@class/whisperx/onset/fricative\endcsname{58}
\expandafter\def\csname v@class/whisperx/onset/fricative/n\endcsname{2{,}919}
\expandafter\def\csname v@class/whisperx/onset/liquid\endcsname{46}
\expandafter\def\csname v@class/whisperx/onset/liquid/n\endcsname{1{,}463}
\expandafter\def\csname v@class/whisperx/onset/nasal\endcsname{60}
\expandafter\def\csname v@class/whisperx/onset/nasal/n\endcsname{774}
\expandafter\def\csname v@class/whisperx/onset/vowel\endcsname{60}
\expandafter\def\csname v@class/whisperx/onset/vowel/n\endcsname{2{,}569}
\expandafter\def\csname v@edges/buckeye/cfa-edges/first-start/mean\endcsname{75}
\expandafter\def\csname v@edges/buckeye/cfa-edges/first-start/median\endcsname{47}
\expandafter\def\csname v@edges/buckeye/cfa-edges/interior/mean\endcsname{32}
\expandafter\def\csname v@edges/buckeye/cfa-edges/interior/median\endcsname{21}
\expandafter\def\csname v@edges/buckeye/cfa-edges/last-end/mean\endcsname{103}
\expandafter\def\csname v@edges/buckeye/cfa-edges/last-end/median\endcsname{69}
\expandafter\def\csname v@edges/buckeye/cfa-segment/first-start/mean\endcsname{63}
\expandafter\def\csname v@edges/buckeye/cfa-segment/first-start/median\endcsname{47}
\expandafter\def\csname v@edges/buckeye/cfa-segment/interior/mean\endcsname{41}
\expandafter\def\csname v@edges/buckeye/cfa-segment/interior/median\endcsname{29}
\expandafter\def\csname v@edges/buckeye/cfa-segment/last-end/mean\endcsname{78}
\expandafter\def\csname v@edges/buckeye/cfa-segment/last-end/median\endcsname{84}
\expandafter\def\csname v@edges/buckeye/mfa-arpa/first-start/mean\endcsname{26}
\expandafter\def\csname v@edges/buckeye/mfa-arpa/first-start/median\endcsname{20}
\expandafter\def\csname v@edges/buckeye/mfa-arpa/interior/mean\endcsname{20}
\expandafter\def\csname v@edges/buckeye/mfa-arpa/interior/median\endcsname{10}
\expandafter\def\csname v@edges/buckeye/mfa-arpa/last-end/mean\endcsname{29}
\expandafter\def\csname v@edges/buckeye/mfa-arpa/last-end/median\endcsname{19}
\expandafter\def\csname v@edges/buckeye/mfa-english/first-start/mean\endcsname{46}
\expandafter\def\csname v@edges/buckeye/mfa-english/first-start/median\endcsname{30}
\expandafter\def\csname v@edges/buckeye/mfa-english/interior/mean\endcsname{22}
\expandafter\def\csname v@edges/buckeye/mfa-english/interior/median\endcsname{10}
\expandafter\def\csname v@edges/buckeye/mfa-english/last-end/mean\endcsname{53}
\expandafter\def\csname v@edges/buckeye/mfa-english/last-end/median\endcsname{33}
\expandafter\def\csname v@edges/buckeye/mms-torchaudio/first-start/mean\endcsname{58}
\expandafter\def\csname v@edges/buckeye/mms-torchaudio/first-start/median\endcsname{41}
\expandafter\def\csname v@edges/buckeye/mms-torchaudio/interior/mean\endcsname{40}
\expandafter\def\csname v@edges/buckeye/mms-torchaudio/interior/median\endcsname{29}
\expandafter\def\csname v@edges/buckeye/mms-torchaudio/last-end/mean\endcsname{63}
\expandafter\def\csname v@edges/buckeye/mms-torchaudio/last-end/median\endcsname{41}
\expandafter\def\csname v@edges/buckeye/qwen3fa/first-start/mean\endcsname{41}
\expandafter\def\csname v@edges/buckeye/qwen3fa/first-start/median\endcsname{20}
\expandafter\def\csname v@edges/buckeye/qwen3fa/interior/mean\endcsname{30}
\expandafter\def\csname v@edges/buckeye/qwen3fa/interior/median\endcsname{23}
\expandafter\def\csname v@edges/buckeye/qwen3fa/last-end/mean\endcsname{38}
\expandafter\def\csname v@edges/buckeye/qwen3fa/last-end/median\endcsname{27}
\expandafter\def\csname v@edges/buckeye/stablets/first-start/mean\endcsname{45}
\expandafter\def\csname v@edges/buckeye/stablets/first-start/median\endcsname{27}
\expandafter\def\csname v@edges/buckeye/stablets/interior/mean\endcsname{57}
\expandafter\def\csname v@edges/buckeye/stablets/interior/median\endcsname{37}
\expandafter\def\csname v@edges/buckeye/stablets/last-end/mean\endcsname{169}
\expandafter\def\csname v@edges/buckeye/stablets/last-end/median\endcsname{138}
\expandafter\def\csname v@edges/buckeye/sttapi/first-start/mean\endcsname{56}
\expandafter\def\csname v@edges/buckeye/sttapi/first-start/median\endcsname{40}
\expandafter\def\csname v@edges/buckeye/sttapi/interior/mean\endcsname{38}
\expandafter\def\csname v@edges/buckeye/sttapi/interior/median\endcsname{26}
\expandafter\def\csname v@edges/buckeye/sttapi/last-end/mean\endcsname{74}
\expandafter\def\csname v@edges/buckeye/sttapi/last-end/median\endcsname{60}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cal/first-start/mean\endcsname{79}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cal/first-start/median\endcsname{88}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cal/interior/mean\endcsname{32}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cal/interior/median\endcsname{22}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cal/last-end/mean\endcsname{78}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cal/last-end/median\endcsname{55}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cfg/first-start/mean\endcsname{91}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cfg/first-start/median\endcsname{100}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cfg/interior/mean\endcsname{1626}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cfg/interior/median\endcsname{1244}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cfg/last-end/mean\endcsname{112}
\expandafter\def\csname v@edges/buckeye/whisper-tm-cfg/last-end/median\endcsname{70}
\expandafter\def\csname v@edges/buckeye/whisper-tm-oai/first-start/mean\endcsname{91}
\expandafter\def\csname v@edges/buckeye/whisper-tm-oai/first-start/median\endcsname{100}
\expandafter\def\csname v@edges/buckeye/whisper-tm-oai/interior/mean\endcsname{122}
\expandafter\def\csname v@edges/buckeye/whisper-tm-oai/interior/median\endcsname{100}
\expandafter\def\csname v@edges/buckeye/whisper-tm-oai/last-end/mean\endcsname{280}
\expandafter\def\csname v@edges/buckeye/whisper-tm-oai/last-end/median\endcsname{264}
\expandafter\def\csname v@edges/buckeye/whisperx/first-start/mean\endcsname{63}
\expandafter\def\csname v@edges/buckeye/whisperx/first-start/median\endcsname{42}
\expandafter\def\csname v@edges/buckeye/whisperx/interior/mean\endcsname{47}
\expandafter\def\csname v@edges/buckeye/whisperx/interior/median\endcsname{38}
\expandafter\def\csname v@edges/buckeye/whisperx/last-end/mean\endcsname{99}
\expandafter\def\csname v@edges/buckeye/whisperx/last-end/median\endcsname{81}
\expandafter\def\csname v@edges/swb/cfa-edges/first-start/mean\endcsname{94}
\expandafter\def\csname v@edges/swb/cfa-edges/first-start/median\endcsname{49}
\expandafter\def\csname v@edges/swb/cfa-edges/interior/mean\endcsname{48}
\expandafter\def\csname v@edges/swb/cfa-edges/interior/median\endcsname{22}
\expandafter\def\csname v@edges/swb/cfa-edges/last-end/mean\endcsname{129}
\expandafter\def\csname v@edges/swb/cfa-edges/last-end/median\endcsname{78}
\expandafter\def\csname v@edges/swb/cfa-segment/first-start/mean\endcsname{70}
\expandafter\def\csname v@edges/swb/cfa-segment/first-start/median\endcsname{44}
\expandafter\def\csname v@edges/swb/cfa-segment/interior/mean\endcsname{61}
\expandafter\def\csname v@edges/swb/cfa-segment/interior/median\endcsname{30}
\expandafter\def\csname v@edges/swb/cfa-segment/last-end/mean\endcsname{208}
\expandafter\def\csname v@edges/swb/cfa-segment/last-end/median\endcsname{140}
\expandafter\def\csname v@edges/swb/mfa-arpa/first-start/mean\endcsname{46}
\expandafter\def\csname v@edges/swb/mfa-arpa/first-start/median\endcsname{16}
\expandafter\def\csname v@edges/swb/mfa-arpa/interior/mean\endcsname{34}
\expandafter\def\csname v@edges/swb/mfa-arpa/interior/median\endcsname{11}
\expandafter\def\csname v@edges/swb/mfa-arpa/last-end/mean\endcsname{57}
\expandafter\def\csname v@edges/swb/mfa-arpa/last-end/median\endcsname{24}
\expandafter\def\csname v@edges/swb/mfa-english/first-start/mean\endcsname{68}
\expandafter\def\csname v@edges/swb/mfa-english/first-start/median\endcsname{24}
\expandafter\def\csname v@edges/swb/mfa-english/interior/mean\endcsname{35}
\expandafter\def\csname v@edges/swb/mfa-english/interior/median\endcsname{11}
\expandafter\def\csname v@edges/swb/mfa-english/last-end/mean\endcsname{81}
\expandafter\def\csname v@edges/swb/mfa-english/last-end/median\endcsname{36}
\expandafter\def\csname v@edges/swb/mms-torchaudio/first-start/mean\endcsname{64}
\expandafter\def\csname v@edges/swb/mms-torchaudio/first-start/median\endcsname{41}
\expandafter\def\csname v@edges/swb/mms-torchaudio/interior/mean\endcsname{44}
\expandafter\def\csname v@edges/swb/mms-torchaudio/interior/median\endcsname{29}
\expandafter\def\csname v@edges/swb/mms-torchaudio/last-end/mean\endcsname{74}
\expandafter\def\csname v@edges/swb/mms-torchaudio/last-end/median\endcsname{48}
\expandafter\def\csname v@edges/swb/qwen3fa/first-start/mean\endcsname{51}
\expandafter\def\csname v@edges/swb/qwen3fa/first-start/median\endcsname{27}
\expandafter\def\csname v@edges/swb/qwen3fa/interior/mean\endcsname{40}
\expandafter\def\csname v@edges/swb/qwen3fa/interior/median\endcsname{27}
\expandafter\def\csname v@edges/swb/qwen3fa/last-end/mean\endcsname{60}
\expandafter\def\csname v@edges/swb/qwen3fa/last-end/median\endcsname{34}
\expandafter\def\csname v@edges/swb/stablets/first-start/mean\endcsname{86}
\expandafter\def\csname v@edges/swb/stablets/first-start/median\endcsname{36}
\expandafter\def\csname v@edges/swb/stablets/interior/mean\endcsname{58}
\expandafter\def\csname v@edges/swb/stablets/interior/median\endcsname{37}
\expandafter\def\csname v@edges/swb/stablets/last-end/mean\endcsname{169}
\expandafter\def\csname v@edges/swb/stablets/last-end/median\endcsname{130}
\expandafter\def\csname v@edges/swb/sttapi/first-start/mean\endcsname{58}
\expandafter\def\csname v@edges/swb/sttapi/first-start/median\endcsname{40}
\expandafter\def\csname v@edges/swb/sttapi/interior/mean\endcsname{43}
\expandafter\def\csname v@edges/swb/sttapi/interior/median\endcsname{27}
\expandafter\def\csname v@edges/swb/sttapi/last-end/mean\endcsname{79}
\expandafter\def\csname v@edges/swb/sttapi/last-end/median\endcsname{58}
\expandafter\def\csname v@edges/swb/whisper-tm-cal/first-start/mean\endcsname{224}
\expandafter\def\csname v@edges/swb/whisper-tm-cal/first-start/median\endcsname{149}
\expandafter\def\csname v@edges/swb/whisper-tm-cal/interior/mean\endcsname{39}
\expandafter\def\csname v@edges/swb/whisper-tm-cal/interior/median\endcsname{22}
\expandafter\def\csname v@edges/swb/whisper-tm-cal/last-end/mean\endcsname{79}
\expandafter\def\csname v@edges/swb/whisper-tm-cal/last-end/median\endcsname{53}
\expandafter\def\csname v@edges/swb/whisper-tm-cfg/first-start/mean\endcsname{236}
\expandafter\def\csname v@edges/swb/whisper-tm-cfg/first-start/median\endcsname{161}
\expandafter\def\csname v@edges/swb/whisper-tm-cfg/interior/mean\endcsname{1518}
\expandafter\def\csname v@edges/swb/whisper-tm-cfg/interior/median\endcsname{1121}
\expandafter\def\csname v@edges/swb/whisper-tm-cfg/last-end/mean\endcsname{232}
\expandafter\def\csname v@edges/swb/whisper-tm-cfg/last-end/median\endcsname{136}
\expandafter\def\csname v@edges/swb/whisper-tm-oai/first-start/mean\endcsname{236}
\expandafter\def\csname v@edges/swb/whisper-tm-oai/first-start/median\endcsname{161}
\expandafter\def\csname v@edges/swb/whisper-tm-oai/interior/mean\endcsname{131}
\expandafter\def\csname v@edges/swb/whisper-tm-oai/interior/median\endcsname{102}
\expandafter\def\csname v@edges/swb/whisper-tm-oai/last-end/mean\endcsname{265}
\expandafter\def\csname v@edges/swb/whisper-tm-oai/last-end/median\endcsname{240}
\expandafter\def\csname v@edges/swb/whisperx/first-start/mean\endcsname{67}
\expandafter\def\csname v@edges/swb/whisperx/first-start/median\endcsname{42}
\expandafter\def\csname v@edges/swb/whisperx/interior/mean\endcsname{49}
\expandafter\def\csname v@edges/swb/whisperx/interior/median\endcsname{35}
\expandafter\def\csname v@edges/swb/whisperx/last-end/mean\endcsname{103}
\expandafter\def\csname v@edges/swb/whisperx/last-end/median\endcsname{78}
\expandafter\def\csname v@edges/timit/cfa-edges/first-start/mean\endcsname{25}
\expandafter\def\csname v@edges/timit/cfa-edges/first-start/median\endcsname{18}
\expandafter\def\csname v@edges/timit/cfa-edges/interior/mean\endcsname{27}
\expandafter\def\csname v@edges/timit/cfa-edges/interior/median\endcsname{22}
\expandafter\def\csname v@edges/timit/cfa-edges/last-end/mean\endcsname{60}
\expandafter\def\csname v@edges/timit/cfa-edges/last-end/median\endcsname{55}
\expandafter\def\csname v@edges/timit/cfa-segment/first-start/mean\endcsname{25}
\expandafter\def\csname v@edges/timit/cfa-segment/first-start/median\endcsname{17}
\expandafter\def\csname v@edges/timit/cfa-segment/interior/mean\endcsname{38}
\expandafter\def\csname v@edges/timit/cfa-segment/interior/median\endcsname{32}
\expandafter\def\csname v@edges/timit/cfa-segment/last-end/mean\endcsname{196}
\expandafter\def\csname v@edges/timit/cfa-segment/last-end/median\endcsname{135}
\expandafter\def\csname v@edges/timit/mfa-arpa/first-start/mean\endcsname{26}
\expandafter\def\csname v@edges/timit/mfa-arpa/first-start/median\endcsname{24}
\expandafter\def\csname v@edges/timit/mfa-arpa/interior/mean\endcsname{17}
\expandafter\def\csname v@edges/timit/mfa-arpa/interior/median\endcsname{10}
\expandafter\def\csname v@edges/timit/mfa-arpa/last-end/mean\endcsname{39}
\expandafter\def\csname v@edges/timit/mfa-arpa/last-end/median\endcsname{29}
\expandafter\def\csname v@edges/timit/mfa-english/first-start/mean\endcsname{29}
\expandafter\def\csname v@edges/timit/mfa-english/first-start/median\endcsname{27}
\expandafter\def\csname v@edges/timit/mfa-english/interior/mean\endcsname{19}
\expandafter\def\csname v@edges/timit/mfa-english/interior/median\endcsname{10}
\expandafter\def\csname v@edges/timit/mfa-english/last-end/mean\endcsname{46}
\expandafter\def\csname v@edges/timit/mfa-english/last-end/median\endcsname{36}
\expandafter\def\csname v@edges/timit/mms-torchaudio/first-start/mean\endcsname{24}
\expandafter\def\csname v@edges/timit/mms-torchaudio/first-start/median\endcsname{16}
\expandafter\def\csname v@edges/timit/mms-torchaudio/interior/mean\endcsname{38}
\expandafter\def\csname v@edges/timit/mms-torchaudio/interior/median\endcsname{32}
\expandafter\def\csname v@edges/timit/mms-torchaudio/last-end/mean\endcsname{48}
\expandafter\def\csname v@edges/timit/mms-torchaudio/last-end/median\endcsname{42}
\expandafter\def\csname v@edges/timit/qwen3fa/first-start/mean\endcsname{35}
\expandafter\def\csname v@edges/timit/qwen3fa/first-start/median\endcsname{27}
\expandafter\def\csname v@edges/timit/qwen3fa/interior/mean\endcsname{29}
\expandafter\def\csname v@edges/timit/qwen3fa/interior/median\endcsname{23}
\expandafter\def\csname v@edges/timit/qwen3fa/last-end/mean\endcsname{45}
\expandafter\def\csname v@edges/timit/qwen3fa/last-end/median\endcsname{38}
\expandafter\def\csname v@edges/timit/stablets/first-start/mean\endcsname{64}
\expandafter\def\csname v@edges/timit/stablets/first-start/median\endcsname{34}
\expandafter\def\csname v@edges/timit/stablets/interior/mean\endcsname{68}
\expandafter\def\csname v@edges/timit/stablets/interior/median\endcsname{51}
\expandafter\def\csname v@edges/timit/stablets/last-end/mean\endcsname{222}
\expandafter\def\csname v@edges/timit/stablets/last-end/median\endcsname{192}
\expandafter\def\csname v@edges/timit/sttapi/first-start/mean\endcsname{25}
\expandafter\def\csname v@edges/timit/sttapi/first-start/median\endcsname{18}
\expandafter\def\csname v@edges/timit/sttapi/interior/mean\endcsname{35}
\expandafter\def\csname v@edges/timit/sttapi/interior/median\endcsname{29}
\expandafter\def\csname v@edges/timit/sttapi/last-end/mean\endcsname{58}
\expandafter\def\csname v@edges/timit/sttapi/last-end/median\endcsname{52}
\expandafter\def\csname v@edges/timit/whisper-tm-cal/first-start/mean\endcsname{161}
\expandafter\def\csname v@edges/timit/whisper-tm-cal/first-start/median\endcsname{126}
\expandafter\def\csname v@edges/timit/whisper-tm-cal/interior/mean\endcsname{31}
\expandafter\def\csname v@edges/timit/whisper-tm-cal/interior/median\endcsname{23}
\expandafter\def\csname v@edges/timit/whisper-tm-cal/last-end/mean\endcsname{68}
\expandafter\def\csname v@edges/timit/whisper-tm-cal/last-end/median\endcsname{50}
\expandafter\def\csname v@edges/timit/whisper-tm-cfg/first-start/mean\endcsname{173}
\expandafter\def\csname v@edges/timit/whisper-tm-cfg/first-start/median\endcsname{138}
\expandafter\def\csname v@edges/timit/whisper-tm-cfg/interior/mean\endcsname{1340}
\expandafter\def\csname v@edges/timit/whisper-tm-cfg/interior/median\endcsname{1165}
\expandafter\def\csname v@edges/timit/whisper-tm-cfg/last-end/mean\endcsname{286}
\expandafter\def\csname v@edges/timit/whisper-tm-cfg/last-end/median\endcsname{125}
\expandafter\def\csname v@edges/timit/whisper-tm-oai/first-start/mean\endcsname{173}
\expandafter\def\csname v@edges/timit/whisper-tm-oai/first-start/median\endcsname{138}
\expandafter\def\csname v@edges/timit/whisper-tm-oai/interior/mean\endcsname{144}
\expandafter\def\csname v@edges/timit/whisper-tm-oai/interior/median\endcsname{124}
\expandafter\def\csname v@edges/timit/whisper-tm-oai/last-end/mean\endcsname{312}
\expandafter\def\csname v@edges/timit/whisper-tm-oai/last-end/median\endcsname{290}
\expandafter\def\csname v@edges/timit/whisperx/first-start/mean\endcsname{31}
\expandafter\def\csname v@edges/timit/whisperx/first-start/median\endcsname{19}
\expandafter\def\csname v@edges/timit/whisperx/interior/mean\endcsname{45}
\expandafter\def\csname v@edges/timit/whisperx/interior/median\endcsname{38}
\expandafter\def\csname v@edges/timit/whisperx/last-end/mean\endcsname{86}
\expandafter\def\csname v@edges/timit/whisperx/last-end/median\endcsname{81}
\expandafter\def\csname v@fa/en-rows\endcsname{25{,}696}
\expandafter\def\csname v@fa/grid/buckeye\endcsname{6}
\expandafter\def\csname v@fa/grid/ifa\endcsname{0}
\expandafter\def\csname v@fa/grid/l2arctic\endcsname{89}
\expandafter\def\csname v@fa/grid/seoul\endcsname{0}
\expandafter\def\csname v@fa/grid/swb-icsi\endcsname{18}
\expandafter\def\csname v@fa/grid/timit\endcsname{4}
\expandafter\def\csname v@fa/grid/voxangeles\endcsname{24}
\expandafter\def\csname v@fa/joined-hours\endcsname{33}
\expandafter\def\csname v@fa/swb-train-hours\endcsname{2.1}
\expandafter\def\csname v@fa/train-hours\endcsname{47}
\expandafter\def\csname v@fa/train-hours-exact\endcsname{46.7}
\expandafter\def\csname v@fa/train-languages\endcsname{87}
\expandafter\def\csname v@fa/train-languages-other\endcsname{86}
\expandafter\def\csname v@fa/train-rows\endcsname{49{,}170}
\expandafter\def\csname v@fa/train-words\endcsname{420{,}433}
\expandafter\def\csname v@fa/unseen-languages\endcsname{10}
\expandafter\def\csname v@fb/ctcm/dev/f1\endcsname{0.74}
\expandafter\def\csname v@fb/ctcm/dev/mae\endcsname{19.1}
\expandafter\def\csname v@fb/ctcm/dev/mae-hi\endcsname{19.1}
\expandafter\def\csname v@fb/ctcm/dev/mae-lo\endcsname{19.1}
\expandafter\def\csname v@fb/ctcm/dev/n\endcsname{1}
\expandafter\def\csname v@fb/ctcm/f1\endcsname{0.76}
\expandafter\def\csname v@fb/ctcm/mae\endcsname{19.2}
\expandafter\def\csname v@fb/ctcm/mae-hi\endcsname{19.2}
\expandafter\def\csname v@fb/ctcm/mae-lo\endcsname{19.2}
\expandafter\def\csname v@fb/ctcm/n\endcsname{1}
\expandafter\def\csname v@fb/ctcw/dev/f1\endcsname{0.77}
\expandafter\def\csname v@fb/ctcw/dev/mae\endcsname{18.2}
\expandafter\def\csname v@fb/ctcw/dev/mae-hi\endcsname{18.2}
\expandafter\def\csname v@fb/ctcw/dev/mae-lo\endcsname{18.2}
\expandafter\def\csname v@fb/ctcw/dev/n\endcsname{1}
\expandafter\def\csname v@fb/ctcw/f1\endcsname{0.79}
\expandafter\def\csname v@fb/ctcw/mae\endcsname{18.2}
\expandafter\def\csname v@fb/ctcw/mae-hi\endcsname{18.2}
\expandafter\def\csname v@fb/ctcw/mae-lo\endcsname{18.2}
\expandafter\def\csname v@fb/ctcw/n\endcsname{1}
\expandafter\def\csname v@fb/post/dev/f1\endcsname{0.89}
\expandafter\def\csname v@fb/post/dev/mae\endcsname{10.9}
\expandafter\def\csname v@fb/post/dev/mae-hi\endcsname{11.0}
\expandafter\def\csname v@fb/post/dev/mae-lo\endcsname{10.8}
\expandafter\def\csname v@fb/post/dev/n\endcsname{5}
\expandafter\def\csname v@fb/post/f1\endcsname{0.90}
\expandafter\def\csname v@fb/post/mae\endcsname{11.6}
\expandafter\def\csname v@fb/post/mae-hi\endcsname{11.7}
\expandafter\def\csname v@fb/post/mae-lo\endcsname{11.5}
\expandafter\def\csname v@fb/post/n\endcsname{5}
\expandafter\def\csname v@fb/rel-s6/f1\endcsname{0.88}
\expandafter\def\csname v@fb/rel-s6/mae\endcsname{12.5}
\expandafter\def\csname v@fb/rel-turbo/f1\endcsname{0.88}
\expandafter\def\csname v@fb/rel-turbo/mae\endcsname{12.0}
\expandafter\def\csname v@fb/rel-v3/f1\endcsname{0.89}
\expandafter\def\csname v@fb/rel-v3/mae\endcsname{11.7}
\expandafter\def\csname v@fb/ts/cut-pct\endcsname{36}
\expandafter\def\csname v@fb/ts/dev/f1\endcsname{0.89}
\expandafter\def\csname v@fb/ts/dev/mae\endcsname{11.0}
\expandafter\def\csname v@fb/ts/dev/mae-hi\endcsname{11.2}
\expandafter\def\csname v@fb/ts/dev/mae-lo\endcsname{10.8}
\expandafter\def\csname v@fb/ts/dev/n\endcsname{5}
\expandafter\def\csname v@fb/ts/f1\endcsname{0.89}
\expandafter\def\csname v@fb/ts/mae\endcsname{11.6}
\expandafter\def\csname v@fb/ts/mae-hi\endcsname{11.8}
\expandafter\def\csname v@fb/ts/mae-lo\endcsname{11.4}
\expandafter\def\csname v@fb/ts/n\endcsname{5}
\expandafter\def\csname v@fb/turbopost/dev/f1\endcsname{0.89}
\expandafter\def\csname v@fb/turbopost/dev/mae\endcsname{10.7}
\expandafter\def\csname v@fb/turbopost/dev/mae-hi\endcsname{10.8}
\expandafter\def\csname v@fb/turbopost/dev/mae-lo\endcsname{10.7}
\expandafter\def\csname v@fb/turbopost/dev/n\endcsname{2}
\expandafter\def\csname v@fb/turbopost/f1\endcsname{0.90}
\expandafter\def\csname v@fb/turbopost/mae\endcsname{11.5}
\expandafter\def\csname v@fb/turbopost/mae-hi\endcsname{11.6}
\expandafter\def\csname v@fb/turbopost/mae-lo\endcsname{11.3}
\expandafter\def\csname v@fb/turbopost/n\endcsname{2}
\expandafter\def\csname v@fin/c/10ms/buckeye-codecs/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/buckeye-unseen/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/buckeye-unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/buckeye/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/10ms/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/codecs/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/codecs/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/d\endcsname{$-0.04$}
\expandafter\def\csname v@fin/c/10ms/d-abs\endcsname{0.04}
\expandafter\def\csname v@fin/c/10ms/ifa/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/ifa/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/long/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/10ms/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/se\endcsname{0.07}
\expandafter\def\csname v@fin/c/10ms/seoul/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/10ms/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/swb/d\endcsname{$-0.4$}
\expandafter\def\csname v@fin/c/10ms/swb/se\endcsname{0.4}
\expandafter\def\csname v@fin/c/10ms/timit/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/timit/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/unseen/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/unseen/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/10ms/vox/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/10ms/vox/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/buckeye-codecs/d\endcsname{0.6}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/buckeye-unseen/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/buckeye-unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/buckeye/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/codecs/d\endcsname{0.6}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/d\endcsname{$-0.10$}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/d-abs\endcsname{0.10}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/ifa/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/ifa/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/long/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/long/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/se\endcsname{0.17}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/seoul/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/swb/d\endcsname{$-0.6$}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/swb/se\endcsname{1.0}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/timit/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/timit/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/unseen/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/vox/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/ce-vs-codecs-s5/vox/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/ce-vs-codecs/buckeye-codecs/d\endcsname{0.6}
\expandafter\def\csname v@fin/c/ce-vs-codecs/buckeye-codecs/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/ce-vs-codecs/buckeye-unseen/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/ce-vs-codecs/buckeye-unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs/buckeye/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/ce-vs-codecs/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs/codecs/d\endcsname{0.7}
\expandafter\def\csname v@fin/c/ce-vs-codecs/codecs/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/ce-vs-codecs/d\endcsname{$-0.03$}
\expandafter\def\csname v@fin/c/ce-vs-codecs/d-abs\endcsname{0.03}
\expandafter\def\csname v@fin/c/ce-vs-codecs/ifa/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/ce-vs-codecs/ifa/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs/long/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/ce-vs-codecs/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/ce-vs-codecs/se\endcsname{0.23}
\expandafter\def\csname v@fin/c/ce-vs-codecs/seoul/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/ce-vs-codecs/seoul/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/ce-vs-codecs/swb/d\endcsname{$-0.9$}
\expandafter\def\csname v@fin/c/ce-vs-codecs/swb/se\endcsname{1.6}
\expandafter\def\csname v@fin/c/ce-vs-codecs/timit/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/ce-vs-codecs/timit/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/ce-vs-codecs/unseen/d\endcsname{0.6}
\expandafter\def\csname v@fin/c/ce-vs-codecs/unseen/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/ce-vs-codecs/vox/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/ce-vs-codecs/vox/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/buckeye-codecs/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/buckeye-unseen/d\endcsname{0.3}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/buckeye-unseen/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/buckeye/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/codecs/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/d\endcsname{0.14}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/d-abs\endcsname{0.14}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/ifa/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/ifa/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/long/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/se\endcsname{0.08}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/seoul/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/swb/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/swb/se\endcsname{0.5}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/timit/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/timit/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/unseen/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/vox/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-turbo-vs-s6/vox/se\endcsname{0.4}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/buckeye-codecs/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/buckeye-unseen/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/buckeye-unseen/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/buckeye/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/codecs/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/codecs/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/d\endcsname{$-0.13$}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/d-abs\endcsname{0.13}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/ifa/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/ifa/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/long/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/se\endcsname{0.09}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/seoul/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/swb/d\endcsname{$-0.3$}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/swb/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/timit/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/timit/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/unseen/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/unseen/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/vox/d\endcsname{$-0.3$}
\expandafter\def\csname v@fin/c/final-v3-vs-s6/vox/se\endcsname{0.4}
\expandafter\def\csname v@fin/c/s6-vs-s5/buckeye-codecs/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/s6-vs-s5/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/buckeye-unseen/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/s6-vs-s5/buckeye-unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/buckeye/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/codecs/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/s6-vs-s5/codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/d\endcsname{0.02}
\expandafter\def\csname v@fin/c/s6-vs-s5/d-abs\endcsname{0.02}
\expandafter\def\csname v@fin/c/s6-vs-s5/ifa/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/s6-vs-s5/ifa/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/long/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/s6-vs-s5/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/s6-vs-s5/se\endcsname{0.10}
\expandafter\def\csname v@fin/c/s6-vs-s5/seoul/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/s6-vs-s5/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/swb/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/s6-vs-s5/swb/se\endcsname{0.5}
\expandafter\def\csname v@fin/c/s6-vs-s5/timit/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/s6-vs-s5/timit/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/unseen/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/s6-vs-s5/unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/s6-vs-s5/vox/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/s6-vs-s5/vox/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/buckeye-codecs/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/tn-s5/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/buckeye-unseen/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/tn-s5/buckeye-unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/buckeye/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/tn-s5/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/codecs/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn-s5/codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/d\endcsname{$-0.34$}
\expandafter\def\csname v@fin/c/tn-s5/d-abs\endcsname{0.34}
\expandafter\def\csname v@fin/c/tn-s5/ifa/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/tn-s5/ifa/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn-s5/long/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/long/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/se\endcsname{0.07}
\expandafter\def\csname v@fin/c/tn-s5/seoul/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/tn-s5/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/swb/d\endcsname{$-2.0$}
\expandafter\def\csname v@fin/c/tn-s5/swb/se\endcsname{0.3}
\expandafter\def\csname v@fin/c/tn-s5/timit/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/timit/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/tn-s5/unseen/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/tn-s5/unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn-s5/vox/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/tn-s5/vox/se\endcsname{0.3}
\expandafter\def\csname v@fin/c/tn/buckeye-codecs/d\endcsname{$-0.4$}
\expandafter\def\csname v@fin/c/tn/buckeye-codecs/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn/buckeye-unseen/d\endcsname{$-0.6$}
\expandafter\def\csname v@fin/c/tn/buckeye-unseen/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn/buckeye/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/tn/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn/codecs/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn/codecs/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn/d\endcsname{$-0.14$}
\expandafter\def\csname v@fin/c/tn/d-abs\endcsname{0.14}
\expandafter\def\csname v@fin/c/tn/ifa/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/tn/ifa/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/tn/long/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/tn/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/tn/se\endcsname{0.23}
\expandafter\def\csname v@fin/c/tn/seoul/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn/swb/d\endcsname{$-1.5$}
\expandafter\def\csname v@fin/c/tn/swb/se\endcsname{1.6}
\expandafter\def\csname v@fin/c/tn/timit/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/tn/timit/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/tn/unseen/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn/unseen/se\endcsname{0.2}
\expandafter\def\csname v@fin/c/tn/vox/d\endcsname{0.7}
\expandafter\def\csname v@fin/c/tn/vox/se\endcsname{0.4}
\expandafter\def\csname v@fin/c/turbo-vs-s5/buckeye-codecs/d\endcsname{0.3}
\expandafter\def\csname v@fin/c/turbo-vs-s5/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/turbo-vs-s5/buckeye-unseen/d\endcsname{0.4}
\expandafter\def\csname v@fin/c/turbo-vs-s5/buckeye-unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/turbo-vs-s5/buckeye/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/turbo-vs-s5/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/turbo-vs-s5/codecs/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/turbo-vs-s5/codecs/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/turbo-vs-s5/d\endcsname{$-0.04$}
\expandafter\def\csname v@fin/c/turbo-vs-s5/d-abs\endcsname{0.04}
\expandafter\def\csname v@fin/c/turbo-vs-s5/ifa/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/turbo-vs-s5/ifa/se\endcsname{0.3}
\expandafter\def\csname v@fin/c/turbo-vs-s5/long/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/turbo-vs-s5/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/turbo-vs-s5/se\endcsname{0.08}
\expandafter\def\csname v@fin/c/turbo-vs-s5/seoul/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/turbo-vs-s5/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/turbo-vs-s5/swb/d\endcsname{$-0.7$}
\expandafter\def\csname v@fin/c/turbo-vs-s5/swb/se\endcsname{0.5}
\expandafter\def\csname v@fin/c/turbo-vs-s5/timit/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/turbo-vs-s5/timit/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/turbo-vs-s5/unseen/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/turbo-vs-s5/unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/turbo-vs-s5/vox/d\endcsname{0.2}
\expandafter\def\csname v@fin/c/turbo-vs-s5/vox/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/buckeye-codecs/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/buckeye-codecs/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/buckeye-unseen/d\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/buckeye-unseen/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/buckeye/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/v3-vs-s5/buckeye/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/codecs/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/v3-vs-s5/codecs/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/v3-vs-s5/d\endcsname{$-0.15$}
\expandafter\def\csname v@fin/c/v3-vs-s5/d-abs\endcsname{0.15}
\expandafter\def\csname v@fin/c/v3-vs-s5/ifa/d\endcsname{$-0.3$}
\expandafter\def\csname v@fin/c/v3-vs-s5/ifa/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/long/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/v3-vs-s5/long/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/v3-vs-s5/se\endcsname{0.18}
\expandafter\def\csname v@fin/c/v3-vs-s5/seoul/d\endcsname{0.0}
\expandafter\def\csname v@fin/c/v3-vs-s5/seoul/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/swb/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/v3-vs-s5/swb/se\endcsname{1.4}
\expandafter\def\csname v@fin/c/v3-vs-s5/timit/d\endcsname{$-0.1$}
\expandafter\def\csname v@fin/c/v3-vs-s5/timit/se\endcsname{0.1}
\expandafter\def\csname v@fin/c/v3-vs-s5/unseen/d\endcsname{$-0.2$}
\expandafter\def\csname v@fin/c/v3-vs-s5/unseen/se\endcsname{0.0}
\expandafter\def\csname v@fin/c/v3-vs-s5/vox/d\endcsname{$-0.4$}
\expandafter\def\csname v@fin/c/v3-vs-s5/vox/se\endcsname{0.2}
\expandafter\def\csname v@fin/ce-s5/buckeye-codecs/end\endcsname{12.4}
\expandafter\def\csname v@fin/ce-s5/buckeye-codecs/mae\endcsname{12.6}
\expandafter\def\csname v@fin/ce-s5/buckeye-codecs/start\endcsname{12.8}
\expandafter\def\csname v@fin/ce-s5/buckeye-unseen/end\endcsname{12.4}
\expandafter\def\csname v@fin/ce-s5/buckeye-unseen/mae\endcsname{12.6}
\expandafter\def\csname v@fin/ce-s5/buckeye-unseen/start\endcsname{12.8}
\expandafter\def\csname v@fin/ce-s5/buckeye/end\endcsname{11.0}
\expandafter\def\csname v@fin/ce-s5/buckeye/mae\endcsname{11.3}
\expandafter\def\csname v@fin/ce-s5/buckeye/start\endcsname{11.6}
\expandafter\def\csname v@fin/ce-s5/codecs/end\endcsname{11.6}
\expandafter\def\csname v@fin/ce-s5/codecs/mae\endcsname{11.7}
\expandafter\def\csname v@fin/ce-s5/codecs/start\endcsname{11.9}
\expandafter\def\csname v@fin/ce-s5/ifa/end\endcsname{16.0}
\expandafter\def\csname v@fin/ce-s5/ifa/mae\endcsname{14.7}
\expandafter\def\csname v@fin/ce-s5/ifa/start\endcsname{13.5}
\expandafter\def\csname v@fin/ce-s5/long/end\endcsname{10.2}
\expandafter\def\csname v@fin/ce-s5/long/mae\endcsname{10.5}
\expandafter\def\csname v@fin/ce-s5/long/start\endcsname{10.8}
\expandafter\def\csname v@fin/ce-s5/mean-mae\endcsname{12.93}
\expandafter\def\csname v@fin/ce-s5/mean-w20\endcsname{84.9}
\expandafter\def\csname v@fin/ce-s5/runs\endcsname{2}
\expandafter\def\csname v@fin/ce-s5/seoul/end\endcsname{10.0}
\expandafter\def\csname v@fin/ce-s5/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fin/ce-s5/seoul/start\endcsname{10.8}
\expandafter\def\csname v@fin/ce-s5/swb/end\endcsname{16.6}
\expandafter\def\csname v@fin/ce-s5/swb/mae\endcsname{17.8}
\expandafter\def\csname v@fin/ce-s5/swb/start\endcsname{18.9}
\expandafter\def\csname v@fin/ce-s5/timit/end\endcsname{10.3}
\expandafter\def\csname v@fin/ce-s5/timit/mae\endcsname{10.6}
\expandafter\def\csname v@fin/ce-s5/timit/start\endcsname{10.9}
\expandafter\def\csname v@fin/ce-s5/unseen/end\endcsname{12.3}
\expandafter\def\csname v@fin/ce-s5/unseen/mae\endcsname{12.6}
\expandafter\def\csname v@fin/ce-s5/unseen/start\endcsname{12.9}
\expandafter\def\csname v@fin/ce-s5/vox/end\endcsname{21.3}
\expandafter\def\csname v@fin/ce-s5/vox/mae\endcsname{15.2}
\expandafter\def\csname v@fin/ce-s5/vox/start\endcsname{9.2}
\expandafter\def\csname v@fin/ce-s6/buckeye-codecs/end\endcsname{12.7}
\expandafter\def\csname v@fin/ce-s6/buckeye-codecs/mae\endcsname{12.8}
\expandafter\def\csname v@fin/ce-s6/buckeye-codecs/start\endcsname{12.9}
\expandafter\def\csname v@fin/ce-s6/buckeye-unseen/end\endcsname{13.1}
\expandafter\def\csname v@fin/ce-s6/buckeye-unseen/mae\endcsname{13.1}
\expandafter\def\csname v@fin/ce-s6/buckeye-unseen/start\endcsname{13.1}
\expandafter\def\csname v@fin/ce-s6/buckeye/end\endcsname{11.1}
\expandafter\def\csname v@fin/ce-s6/buckeye/mae\endcsname{11.3}
\expandafter\def\csname v@fin/ce-s6/buckeye/start\endcsname{11.6}
\expandafter\def\csname v@fin/ce-s6/codecs/end\endcsname{11.5}
\expandafter\def\csname v@fin/ce-s6/codecs/mae\endcsname{11.8}
\expandafter\def\csname v@fin/ce-s6/codecs/start\endcsname{12.1}
\expandafter\def\csname v@fin/ce-s6/ifa/end\endcsname{15.8}
\expandafter\def\csname v@fin/ce-s6/ifa/mae\endcsname{14.6}
\expandafter\def\csname v@fin/ce-s6/ifa/start\endcsname{13.4}
\expandafter\def\csname v@fin/ce-s6/long/end\endcsname{10.3}
\expandafter\def\csname v@fin/ce-s6/long/mae\endcsname{10.7}
\expandafter\def\csname v@fin/ce-s6/long/start\endcsname{11.0}
\expandafter\def\csname v@fin/ce-s6/mean-mae\endcsname{13.02}
\expandafter\def\csname v@fin/ce-s6/mean-w20\endcsname{84.8}
\expandafter\def\csname v@fin/ce-s6/runs\endcsname{2}
\expandafter\def\csname v@fin/ce-s6/seoul/end\endcsname{10.0}
\expandafter\def\csname v@fin/ce-s6/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fin/ce-s6/seoul/start\endcsname{10.7}
\expandafter\def\csname v@fin/ce-s6/swb/end\endcsname{16.2}
\expandafter\def\csname v@fin/ce-s6/swb/mae\endcsname{17.7}
\expandafter\def\csname v@fin/ce-s6/swb/start\endcsname{19.2}
\expandafter\def\csname v@fin/ce-s6/timit/end\endcsname{10.5}
\expandafter\def\csname v@fin/ce-s6/timit/mae\endcsname{10.8}
\expandafter\def\csname v@fin/ce-s6/timit/start\endcsname{11.2}
\expandafter\def\csname v@fin/ce-s6/unseen/end\endcsname{12.4}
\expandafter\def\csname v@fin/ce-s6/unseen/mae\endcsname{12.8}
\expandafter\def\csname v@fin/ce-s6/unseen/start\endcsname{13.1}
\expandafter\def\csname v@fin/ce-s6/vox/end\endcsname{21.8}
\expandafter\def\csname v@fin/ce-s6/vox/mae\endcsname{15.6}
\expandafter\def\csname v@fin/ce-s6/vox/start\endcsname{9.5}
\expandafter\def\csname v@fin/final-s6/buckeye-codecs/end\endcsname{12.3}
\expandafter\def\csname v@fin/final-s6/buckeye-codecs/mae\endcsname{12.4}
\expandafter\def\csname v@fin/final-s6/buckeye-codecs/start\endcsname{12.5}
\expandafter\def\csname v@fin/final-s6/buckeye-unseen/end\endcsname{12.5}
\expandafter\def\csname v@fin/final-s6/buckeye-unseen/mae\endcsname{12.5}
\expandafter\def\csname v@fin/final-s6/buckeye-unseen/start\endcsname{12.5}
\expandafter\def\csname v@fin/final-s6/buckeye/end\endcsname{11.2}
\expandafter\def\csname v@fin/final-s6/buckeye/mae\endcsname{11.2}
\expandafter\def\csname v@fin/final-s6/buckeye/start\endcsname{11.2}
\expandafter\def\csname v@fin/final-s6/codecs/end\endcsname{11.8}
\expandafter\def\csname v@fin/final-s6/codecs/mae\endcsname{12.0}
\expandafter\def\csname v@fin/final-s6/codecs/start\endcsname{12.2}
\expandafter\def\csname v@fin/final-s6/ifa/end\endcsname{15.6}
\expandafter\def\csname v@fin/final-s6/ifa/mae\endcsname{14.5}
\expandafter\def\csname v@fin/final-s6/ifa/start\endcsname{13.3}
\expandafter\def\csname v@fin/final-s6/long/end\endcsname{10.4}
\expandafter\def\csname v@fin/final-s6/long/mae\endcsname{10.7}
\expandafter\def\csname v@fin/final-s6/long/start\endcsname{11.0}
\expandafter\def\csname v@fin/final-s6/mean-mae\endcsname{12.88}
\expandafter\def\csname v@fin/final-s6/mean-w20\endcsname{85.0}
\expandafter\def\csname v@fin/final-s6/runs\endcsname{2}
\expandafter\def\csname v@fin/final-s6/seoul/end\endcsname{10.1}
\expandafter\def\csname v@fin/final-s6/seoul/mae\endcsname{10.5}
\expandafter\def\csname v@fin/final-s6/seoul/start\endcsname{10.9}
\expandafter\def\csname v@fin/final-s6/swb/end\endcsname{16.3}
\expandafter\def\csname v@fin/final-s6/swb/mae\endcsname{16.2}
\expandafter\def\csname v@fin/final-s6/swb/start\endcsname{16.0}
\expandafter\def\csname v@fin/final-s6/timit/end\endcsname{10.6}
\expandafter\def\csname v@fin/final-s6/timit/mae\endcsname{10.8}
\expandafter\def\csname v@fin/final-s6/timit/start\endcsname{11.0}
\expandafter\def\csname v@fin/final-s6/unseen/end\endcsname{12.7}
\expandafter\def\csname v@fin/final-s6/unseen/mae\endcsname{13.0}
\expandafter\def\csname v@fin/final-s6/unseen/start\endcsname{13.3}
\expandafter\def\csname v@fin/final-s6/vox/end\endcsname{23.2}
\expandafter\def\csname v@fin/final-s6/vox/mae\endcsname{16.4}
\expandafter\def\csname v@fin/final-s6/vox/start\endcsname{9.6}
\expandafter\def\csname v@fin/final-turbo/buckeye-codecs/end\endcsname{12.6}
\expandafter\def\csname v@fin/final-turbo/buckeye-codecs/mae\endcsname{12.7}
\expandafter\def\csname v@fin/final-turbo/buckeye-codecs/start\endcsname{12.9}
\expandafter\def\csname v@fin/final-turbo/buckeye-unseen/end\endcsname{12.6}
\expandafter\def\csname v@fin/final-turbo/buckeye-unseen/mae\endcsname{12.8}
\expandafter\def\csname v@fin/final-turbo/buckeye-unseen/start\endcsname{13.0}
\expandafter\def\csname v@fin/final-turbo/buckeye/end\endcsname{11.2}
\expandafter\def\csname v@fin/final-turbo/buckeye/mae\endcsname{11.3}
\expandafter\def\csname v@fin/final-turbo/buckeye/start\endcsname{11.4}
\expandafter\def\csname v@fin/final-turbo/codecs/end\endcsname{11.7}
\expandafter\def\csname v@fin/final-turbo/codecs/mae\endcsname{11.8}
\expandafter\def\csname v@fin/final-turbo/codecs/start\endcsname{12.0}
\expandafter\def\csname v@fin/final-turbo/ifa/end\endcsname{15.8}
\expandafter\def\csname v@fin/final-turbo/ifa/mae\endcsname{14.6}
\expandafter\def\csname v@fin/final-turbo/ifa/start\endcsname{13.4}
\expandafter\def\csname v@fin/final-turbo/long/end\endcsname{10.7}
\expandafter\def\csname v@fin/final-turbo/long/mae\endcsname{10.9}
\expandafter\def\csname v@fin/final-turbo/long/start\endcsname{11.1}
\expandafter\def\csname v@fin/final-turbo/mean-mae\endcsname{13.02}
\expandafter\def\csname v@fin/final-turbo/mean-w20\endcsname{84.6}
\expandafter\def\csname v@fin/final-turbo/runs\endcsname{2}
\expandafter\def\csname v@fin/final-turbo/seoul/end\endcsname{10.3}
\expandafter\def\csname v@fin/final-turbo/seoul/mae\endcsname{10.7}
\expandafter\def\csname v@fin/final-turbo/seoul/start\endcsname{11.2}
\expandafter\def\csname v@fin/final-turbo/swb/end\endcsname{16.3}
\expandafter\def\csname v@fin/final-turbo/swb/mae\endcsname{16.3}
\expandafter\def\csname v@fin/final-turbo/swb/start\endcsname{16.2}
\expandafter\def\csname v@fin/final-turbo/timit/end\endcsname{10.6}
\expandafter\def\csname v@fin/final-turbo/timit/mae\endcsname{10.9}
\expandafter\def\csname v@fin/final-turbo/timit/start\endcsname{11.2}
\expandafter\def\csname v@fin/final-turbo/unseen/end\endcsname{12.6}
\expandafter\def\csname v@fin/final-turbo/unseen/mae\endcsname{12.8}
\expandafter\def\csname v@fin/final-turbo/unseen/start\endcsname{13.0}
\expandafter\def\csname v@fin/final-turbo/vox/end\endcsname{23.1}
\expandafter\def\csname v@fin/final-turbo/vox/mae\endcsname{16.5}
\expandafter\def\csname v@fin/final-turbo/vox/start\endcsname{9.8}
\expandafter\def\csname v@fin/final-v3/buckeye-codecs/end\endcsname{12.5}
\expandafter\def\csname v@fin/final-v3/buckeye-codecs/mae\endcsname{12.5}
\expandafter\def\csname v@fin/final-v3/buckeye-codecs/start\endcsname{12.6}
\expandafter\def\csname v@fin/final-v3/buckeye-unseen/end\endcsname{12.5}
\expandafter\def\csname v@fin/final-v3/buckeye-unseen/mae\endcsname{12.6}
\expandafter\def\csname v@fin/final-v3/buckeye-unseen/start\endcsname{12.6}
\expandafter\def\csname v@fin/final-v3/buckeye/end\endcsname{11.0}
\expandafter\def\csname v@fin/final-v3/buckeye/mae\endcsname{11.2}
\expandafter\def\csname v@fin/final-v3/buckeye/start\endcsname{11.4}
\expandafter\def\csname v@fin/final-v3/codecs/end\endcsname{11.7}
\expandafter\def\csname v@fin/final-v3/codecs/mae\endcsname{11.8}
\expandafter\def\csname v@fin/final-v3/codecs/start\endcsname{12.0}
\expandafter\def\csname v@fin/final-v3/ifa/end\endcsname{15.7}
\expandafter\def\csname v@fin/final-v3/ifa/mae\endcsname{14.5}
\expandafter\def\csname v@fin/final-v3/ifa/start\endcsname{13.3}
\expandafter\def\csname v@fin/final-v3/long/end\endcsname{10.2}
\expandafter\def\csname v@fin/final-v3/long/mae\endcsname{10.5}
\expandafter\def\csname v@fin/final-v3/long/start\endcsname{10.8}
\expandafter\def\csname v@fin/final-v3/mean-mae\endcsname{12.75}
\expandafter\def\csname v@fin/final-v3/mean-w20\endcsname{85.2}
\expandafter\def\csname v@fin/final-v3/runs\endcsname{2}
\expandafter\def\csname v@fin/final-v3/seoul/end\endcsname{10.1}
\expandafter\def\csname v@fin/final-v3/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fin/final-v3/seoul/start\endcsname{10.8}
\expandafter\def\csname v@fin/final-v3/swb/end\endcsname{15.8}
\expandafter\def\csname v@fin/final-v3/swb/mae\endcsname{15.9}
\expandafter\def\csname v@fin/final-v3/swb/start\endcsname{16.0}
\expandafter\def\csname v@fin/final-v3/timit/end\endcsname{10.4}
\expandafter\def\csname v@fin/final-v3/timit/mae\endcsname{10.6}
\expandafter\def\csname v@fin/final-v3/timit/start\endcsname{10.9}
\expandafter\def\csname v@fin/final-v3/unseen/end\endcsname{12.5}
\expandafter\def\csname v@fin/final-v3/unseen/mae\endcsname{12.8}
\expandafter\def\csname v@fin/final-v3/unseen/start\endcsname{13.0}
\expandafter\def\csname v@fin/final-v3/vox/end\endcsname{22.8}
\expandafter\def\csname v@fin/final-v3/vox/mae\endcsname{16.1}
\expandafter\def\csname v@fin/final-v3/vox/start\endcsname{9.3}
\expandafter\def\csname v@fin/post-s5/buckeye-codecs/end\endcsname{11.8}
\expandafter\def\csname v@fin/post-s5/buckeye-codecs/mae\endcsname{12.0}
\expandafter\def\csname v@fin/post-s5/buckeye-codecs/start\endcsname{12.1}
\expandafter\def\csname v@fin/post-s5/buckeye-unseen/end\endcsname{12.2}
\expandafter\def\csname v@fin/post-s5/buckeye-unseen/mae\endcsname{12.3}
\expandafter\def\csname v@fin/post-s5/buckeye-unseen/start\endcsname{12.3}
\expandafter\def\csname v@fin/post-s5/buckeye/end\endcsname{11.1}
\expandafter\def\csname v@fin/post-s5/buckeye/mae\endcsname{11.3}
\expandafter\def\csname v@fin/post-s5/buckeye/start\endcsname{11.5}
\expandafter\def\csname v@fin/post-s5/codecs/end\endcsname{10.9}
\expandafter\def\csname v@fin/post-s5/codecs/mae\endcsname{11.2}
\expandafter\def\csname v@fin/post-s5/codecs/start\endcsname{11.4}
\expandafter\def\csname v@fin/post-s5/ifa/end\endcsname{16.0}
\expandafter\def\csname v@fin/post-s5/ifa/mae\endcsname{14.8}
\expandafter\def\csname v@fin/post-s5/ifa/start\endcsname{13.7}
\expandafter\def\csname v@fin/post-s5/long/end\endcsname{10.1}
\expandafter\def\csname v@fin/post-s5/long/mae\endcsname{10.4}
\expandafter\def\csname v@fin/post-s5/long/start\endcsname{10.7}
\expandafter\def\csname v@fin/post-s5/mean-mae\endcsname{13.02}
\expandafter\def\csname v@fin/post-s5/mean-w20\endcsname{85.0}
\expandafter\def\csname v@fin/post-s5/runs\endcsname{5}
\expandafter\def\csname v@fin/post-s5/seoul/end\endcsname{10.0}
\expandafter\def\csname v@fin/post-s5/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fin/post-s5/seoul/start\endcsname{10.8}
\expandafter\def\csname v@fin/post-s5/swb/end\endcsname{16.5}
\expandafter\def\csname v@fin/post-s5/swb/mae\endcsname{18.4}
\expandafter\def\csname v@fin/post-s5/swb/start\endcsname{20.3}
\expandafter\def\csname v@fin/post-s5/timit/end\endcsname{10.3}
\expandafter\def\csname v@fin/post-s5/timit/mae\endcsname{10.5}
\expandafter\def\csname v@fin/post-s5/timit/start\endcsname{10.8}
\expandafter\def\csname v@fin/post-s5/unseen/end\endcsname{11.8}
\expandafter\def\csname v@fin/post-s5/unseen/mae\endcsname{12.2}
\expandafter\def\csname v@fin/post-s5/unseen/start\endcsname{12.6}
\expandafter\def\csname v@fin/post-s5/vox/end\endcsname{21.3}
\expandafter\def\csname v@fin/post-s5/vox/mae\endcsname{15.3}
\expandafter\def\csname v@fin/post-s5/vox/start\endcsname{9.4}
\expandafter\def\csname v@fin/post-s6/buckeye-codecs/end\endcsname{12.0}
\expandafter\def\csname v@fin/post-s6/buckeye-codecs/mae\endcsname{12.2}
\expandafter\def\csname v@fin/post-s6/buckeye-codecs/start\endcsname{12.4}
\expandafter\def\csname v@fin/post-s6/buckeye-unseen/end\endcsname{12.6}
\expandafter\def\csname v@fin/post-s6/buckeye-unseen/mae\endcsname{12.7}
\expandafter\def\csname v@fin/post-s6/buckeye-unseen/start\endcsname{12.8}
\expandafter\def\csname v@fin/post-s6/buckeye/end\endcsname{11.1}
\expandafter\def\csname v@fin/post-s6/buckeye/mae\endcsname{11.4}
\expandafter\def\csname v@fin/post-s6/buckeye/start\endcsname{11.7}
\expandafter\def\csname v@fin/post-s6/codecs/end\endcsname{10.9}
\expandafter\def\csname v@fin/post-s6/codecs/mae\endcsname{11.2}
\expandafter\def\csname v@fin/post-s6/codecs/start\endcsname{11.5}
\expandafter\def\csname v@fin/post-s6/ifa/end\endcsname{15.8}
\expandafter\def\csname v@fin/post-s6/ifa/mae\endcsname{14.6}
\expandafter\def\csname v@fin/post-s6/ifa/start\endcsname{13.5}
\expandafter\def\csname v@fin/post-s6/long/end\endcsname{10.2}
\expandafter\def\csname v@fin/post-s6/long/mae\endcsname{10.5}
\expandafter\def\csname v@fin/post-s6/long/start\endcsname{10.8}
\expandafter\def\csname v@fin/post-s6/mean-mae\endcsname{13.05}
\expandafter\def\csname v@fin/post-s6/mean-w20\endcsname{85.0}
\expandafter\def\csname v@fin/post-s6/runs\endcsname{2}
\expandafter\def\csname v@fin/post-s6/seoul/end\endcsname{10.0}
\expandafter\def\csname v@fin/post-s6/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fin/post-s6/seoul/start\endcsname{10.9}
\expandafter\def\csname v@fin/post-s6/swb/end\endcsname{17.3}
\expandafter\def\csname v@fin/post-s6/swb/mae\endcsname{18.6}
\expandafter\def\csname v@fin/post-s6/swb/start\endcsname{19.9}
\expandafter\def\csname v@fin/post-s6/timit/end\endcsname{10.2}
\expandafter\def\csname v@fin/post-s6/timit/mae\endcsname{10.6}
\expandafter\def\csname v@fin/post-s6/timit/start\endcsname{10.9}
\expandafter\def\csname v@fin/post-s6/unseen/end\endcsname{11.8}
\expandafter\def\csname v@fin/post-s6/unseen/mae\endcsname{12.2}
\expandafter\def\csname v@fin/post-s6/unseen/start\endcsname{12.6}
\expandafter\def\csname v@fin/post-s6/vox/end\endcsname{21.4}
\expandafter\def\csname v@fin/post-s6/vox/mae\endcsname{15.3}
\expandafter\def\csname v@fin/post-s6/vox/start\endcsname{9.2}
\expandafter\def\csname v@fin/post-turbo/buckeye-codecs/end\endcsname{12.2}
\expandafter\def\csname v@fin/post-turbo/buckeye-codecs/mae\endcsname{12.3}
\expandafter\def\csname v@fin/post-turbo/buckeye-codecs/start\endcsname{12.4}
\expandafter\def\csname v@fin/post-turbo/buckeye-unseen/end\endcsname{12.5}
\expandafter\def\csname v@fin/post-turbo/buckeye-unseen/mae\endcsname{12.7}
\expandafter\def\csname v@fin/post-turbo/buckeye-unseen/start\endcsname{12.8}
\expandafter\def\csname v@fin/post-turbo/buckeye/end\endcsname{11.3}
\expandafter\def\csname v@fin/post-turbo/buckeye/mae\endcsname{11.5}
\expandafter\def\csname v@fin/post-turbo/buckeye/start\endcsname{11.6}
\expandafter\def\csname v@fin/post-turbo/codecs/end\endcsname{10.9}
\expandafter\def\csname v@fin/post-turbo/codecs/mae\endcsname{11.0}
\expandafter\def\csname v@fin/post-turbo/codecs/start\endcsname{11.2}
\expandafter\def\csname v@fin/post-turbo/ifa/end\endcsname{16.0}
\expandafter\def\csname v@fin/post-turbo/ifa/mae\endcsname{14.8}
\expandafter\def\csname v@fin/post-turbo/ifa/start\endcsname{13.6}
\expandafter\def\csname v@fin/post-turbo/long/end\endcsname{10.2}
\expandafter\def\csname v@fin/post-turbo/long/mae\endcsname{10.4}
\expandafter\def\csname v@fin/post-turbo/long/start\endcsname{10.6}
\expandafter\def\csname v@fin/post-turbo/mean-mae\endcsname{12.99}
\expandafter\def\csname v@fin/post-turbo/mean-w20\endcsname{84.9}
\expandafter\def\csname v@fin/post-turbo/runs\endcsname{2}
\expandafter\def\csname v@fin/post-turbo/seoul/end\endcsname{10.1}
\expandafter\def\csname v@fin/post-turbo/seoul/mae\endcsname{10.5}
\expandafter\def\csname v@fin/post-turbo/seoul/start\endcsname{11.0}
\expandafter\def\csname v@fin/post-turbo/swb/end\endcsname{16.3}
\expandafter\def\csname v@fin/post-turbo/swb/mae\endcsname{17.7}
\expandafter\def\csname v@fin/post-turbo/swb/start\endcsname{19.2}
\expandafter\def\csname v@fin/post-turbo/timit/end\endcsname{10.3}
\expandafter\def\csname v@fin/post-turbo/timit/mae\endcsname{10.4}
\expandafter\def\csname v@fin/post-turbo/timit/start\endcsname{10.6}
\expandafter\def\csname v@fin/post-turbo/unseen/end\endcsname{11.7}
\expandafter\def\csname v@fin/post-turbo/unseen/mae\endcsname{12.0}
\expandafter\def\csname v@fin/post-turbo/unseen/start\endcsname{12.3}
\expandafter\def\csname v@fin/post-turbo/vox/end\endcsname{21.9}
\expandafter\def\csname v@fin/post-turbo/vox/mae\endcsname{15.5}
\expandafter\def\csname v@fin/post-turbo/vox/start\endcsname{9.2}
\expandafter\def\csname v@fin/post-v3/buckeye-codecs/end\endcsname{12.1}
\expandafter\def\csname v@fin/post-v3/buckeye-codecs/mae\endcsname{12.1}
\expandafter\def\csname v@fin/post-v3/buckeye-codecs/start\endcsname{12.2}
\expandafter\def\csname v@fin/post-v3/buckeye-unseen/end\endcsname{12.3}
\expandafter\def\csname v@fin/post-v3/buckeye-unseen/mae\endcsname{12.4}
\expandafter\def\csname v@fin/post-v3/buckeye-unseen/start\endcsname{12.5}
\expandafter\def\csname v@fin/post-v3/buckeye/end\endcsname{11.0}
\expandafter\def\csname v@fin/post-v3/buckeye/mae\endcsname{11.3}
\expandafter\def\csname v@fin/post-v3/buckeye/start\endcsname{11.5}
\expandafter\def\csname v@fin/post-v3/codecs/end\endcsname{10.9}
\expandafter\def\csname v@fin/post-v3/codecs/mae\endcsname{11.0}
\expandafter\def\csname v@fin/post-v3/codecs/start\endcsname{11.1}
\expandafter\def\csname v@fin/post-v3/ifa/end\endcsname{15.7}
\expandafter\def\csname v@fin/post-v3/ifa/mae\endcsname{14.6}
\expandafter\def\csname v@fin/post-v3/ifa/start\endcsname{13.4}
\expandafter\def\csname v@fin/post-v3/long/end\endcsname{10.0}
\expandafter\def\csname v@fin/post-v3/long/mae\endcsname{10.3}
\expandafter\def\csname v@fin/post-v3/long/start\endcsname{10.5}
\expandafter\def\csname v@fin/post-v3/mean-mae\endcsname{12.88}
\expandafter\def\csname v@fin/post-v3/mean-w20\endcsname{85.2}
\expandafter\def\csname v@fin/post-v3/runs\endcsname{2}
\expandafter\def\csname v@fin/post-v3/seoul/end\endcsname{10.0}
\expandafter\def\csname v@fin/post-v3/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fin/post-v3/seoul/start\endcsname{10.8}
\expandafter\def\csname v@fin/post-v3/swb/end\endcsname{16.8}
\expandafter\def\csname v@fin/post-v3/swb/mae\endcsname{18.3}
\expandafter\def\csname v@fin/post-v3/swb/start\endcsname{19.9}
\expandafter\def\csname v@fin/post-v3/timit/end\endcsname{10.3}
\expandafter\def\csname v@fin/post-v3/timit/mae\endcsname{10.4}
\expandafter\def\csname v@fin/post-v3/timit/start\endcsname{10.6}
\expandafter\def\csname v@fin/post-v3/unseen/end\endcsname{11.8}
\expandafter\def\csname v@fin/post-v3/unseen/mae\endcsname{12.1}
\expandafter\def\csname v@fin/post-v3/unseen/start\endcsname{12.3}
\expandafter\def\csname v@fin/post-v3/vox/end\endcsname{20.9}
\expandafter\def\csname v@fin/post-v3/vox/mae\endcsname{15.0}
\expandafter\def\csname v@fin/post-v3/vox/start\endcsname{9.1}
\expandafter\def\csname v@fin/post10/buckeye-codecs/end\endcsname{11.9}
\expandafter\def\csname v@fin/post10/buckeye-codecs/mae\endcsname{12.0}
\expandafter\def\csname v@fin/post10/buckeye-codecs/start\endcsname{12.2}
\expandafter\def\csname v@fin/post10/buckeye-unseen/end\endcsname{12.3}
\expandafter\def\csname v@fin/post10/buckeye-unseen/mae\endcsname{12.4}
\expandafter\def\csname v@fin/post10/buckeye-unseen/start\endcsname{12.4}
\expandafter\def\csname v@fin/post10/buckeye/end\endcsname{10.9}
\expandafter\def\csname v@fin/post10/buckeye/mae\endcsname{11.2}
\expandafter\def\csname v@fin/post10/buckeye/start\endcsname{11.5}
\expandafter\def\csname v@fin/post10/codecs/end\endcsname{11.0}
\expandafter\def\csname v@fin/post10/codecs/mae\endcsname{11.2}
\expandafter\def\csname v@fin/post10/codecs/start\endcsname{11.4}
\expandafter\def\csname v@fin/post10/ifa/end\endcsname{15.9}
\expandafter\def\csname v@fin/post10/ifa/mae\endcsname{14.8}
\expandafter\def\csname v@fin/post10/ifa/start\endcsname{13.6}
\expandafter\def\csname v@fin/post10/long/end\endcsname{10.3}
\expandafter\def\csname v@fin/post10/long/mae\endcsname{10.6}
\expandafter\def\csname v@fin/post10/long/start\endcsname{10.9}
\expandafter\def\csname v@fin/post10/mean-mae\endcsname{12.99}
\expandafter\def\csname v@fin/post10/mean-w20\endcsname{84.8}
\expandafter\def\csname v@fin/post10/runs\endcsname{5}
\expandafter\def\csname v@fin/post10/seoul/end\endcsname{9.9}
\expandafter\def\csname v@fin/post10/seoul/mae\endcsname{10.3}
\expandafter\def\csname v@fin/post10/seoul/start\endcsname{10.7}
\expandafter\def\csname v@fin/post10/swb/end\endcsname{16.4}
\expandafter\def\csname v@fin/post10/swb/mae\endcsname{18.0}
\expandafter\def\csname v@fin/post10/swb/start\endcsname{19.5}
\expandafter\def\csname v@fin/post10/timit/end\endcsname{10.4}
\expandafter\def\csname v@fin/post10/timit/mae\endcsname{10.6}
\expandafter\def\csname v@fin/post10/timit/start\endcsname{10.8}
\expandafter\def\csname v@fin/post10/unseen/end\endcsname{11.9}
\expandafter\def\csname v@fin/post10/unseen/mae\endcsname{12.2}
\expandafter\def\csname v@fin/post10/unseen/start\endcsname{12.5}
\expandafter\def\csname v@fin/post10/vox/end\endcsname{21.6}
\expandafter\def\csname v@fin/post10/vox/mae\endcsname{15.5}
\expandafter\def\csname v@fin/post10/vox/start\endcsname{9.4}
\expandafter\def\csname v@fin/tn-s5/buckeye-codecs/end\endcsname{11.6}
\expandafter\def\csname v@fin/tn-s5/buckeye-codecs/mae\endcsname{11.7}
\expandafter\def\csname v@fin/tn-s5/buckeye-codecs/start\endcsname{11.8}
\expandafter\def\csname v@fin/tn-s5/buckeye-unseen/end\endcsname{12.2}
\expandafter\def\csname v@fin/tn-s5/buckeye-unseen/mae\endcsname{12.2}
\expandafter\def\csname v@fin/tn-s5/buckeye-unseen/start\endcsname{12.1}
\expandafter\def\csname v@fin/tn-s5/buckeye/end\endcsname{10.8}
\expandafter\def\csname v@fin/tn-s5/buckeye/mae\endcsname{11.1}
\expandafter\def\csname v@fin/tn-s5/buckeye/start\endcsname{11.3}
\expandafter\def\csname v@fin/tn-s5/codecs/end\endcsname{11.2}
\expandafter\def\csname v@fin/tn-s5/codecs/mae\endcsname{11.3}
\expandafter\def\csname v@fin/tn-s5/codecs/start\endcsname{11.5}
\expandafter\def\csname v@fin/tn-s5/ifa/end\endcsname{15.9}
\expandafter\def\csname v@fin/tn-s5/ifa/mae\endcsname{14.6}
\expandafter\def\csname v@fin/tn-s5/ifa/start\endcsname{13.3}
\expandafter\def\csname v@fin/tn-s5/long/end\endcsname{10.2}
\expandafter\def\csname v@fin/tn-s5/long/mae\endcsname{10.5}
\expandafter\def\csname v@fin/tn-s5/long/start\endcsname{10.8}
\expandafter\def\csname v@fin/tn-s5/mean-mae\endcsname{12.68}
\expandafter\def\csname v@fin/tn-s5/mean-w20\endcsname{85.2}
\expandafter\def\csname v@fin/tn-s5/runs\endcsname{2}
\expandafter\def\csname v@fin/tn-s5/seoul/end\endcsname{10.0}
\expandafter\def\csname v@fin/tn-s5/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fin/tn-s5/seoul/start\endcsname{10.7}
\expandafter\def\csname v@fin/tn-s5/swb/end\endcsname{16.3}
\expandafter\def\csname v@fin/tn-s5/swb/mae\endcsname{16.4}
\expandafter\def\csname v@fin/tn-s5/swb/start\endcsname{16.5}
\expandafter\def\csname v@fin/tn-s5/timit/end\endcsname{10.4}
\expandafter\def\csname v@fin/tn-s5/timit/mae\endcsname{10.7}
\expandafter\def\csname v@fin/tn-s5/timit/start\endcsname{10.9}
\expandafter\def\csname v@fin/tn-s5/unseen/end\endcsname{12.3}
\expandafter\def\csname v@fin/tn-s5/unseen/mae\endcsname{12.6}
\expandafter\def\csname v@fin/tn-s5/unseen/start\endcsname{12.9}
\expandafter\def\csname v@fin/tn-s5/vox/end\endcsname{21.1}
\expandafter\def\csname v@fin/tn-s5/vox/mae\endcsname{15.2}
\expandafter\def\csname v@fin/tn-s5/vox/start\endcsname{9.3}
\expandafter\def\csname v@fmt/post/buckeye/end\endcsname{11.1}
\expandafter\def\csname v@fmt/post/buckeye/mae\endcsname{11.3}
\expandafter\def\csname v@fmt/post/buckeye/start\endcsname{11.5}
\expandafter\def\csname v@fmt/post/d-mae\endcsname{$-0.97$}
\expandafter\def\csname v@fmt/post/d-mae-abs\endcsname{0.97}
\expandafter\def\csname v@fmt/post/d-w20\endcsname{$+0.1$}
\expandafter\def\csname v@fmt/post/ifa/end\endcsname{16.0}
\expandafter\def\csname v@fmt/post/ifa/mae\endcsname{14.8}
\expandafter\def\csname v@fmt/post/ifa/start\endcsname{13.7}
\expandafter\def\csname v@fmt/post/long/end\endcsname{10.1}
\expandafter\def\csname v@fmt/post/long/mae\endcsname{10.4}
\expandafter\def\csname v@fmt/post/long/start\endcsname{10.7}
\expandafter\def\csname v@fmt/post/mean-mae\endcsname{13.02}
\expandafter\def\csname v@fmt/post/mean-w20\endcsname{85.0}
\expandafter\def\csname v@fmt/post/runs\endcsname{5}
\expandafter\def\csname v@fmt/post/se-mae\endcsname{0.08}
\expandafter\def\csname v@fmt/post/seoul/end\endcsname{10.0}
\expandafter\def\csname v@fmt/post/seoul/mae\endcsname{10.4}
\expandafter\def\csname v@fmt/post/seoul/start\endcsname{10.8}
\expandafter\def\csname v@fmt/post/swb/end\endcsname{16.5}
\expandafter\def\csname v@fmt/post/swb/gain-pct\endcsname{21}
\expandafter\def\csname v@fmt/post/swb/mae\endcsname{18.4}
\expandafter\def\csname v@fmt/post/swb/start\endcsname{20.3}
\expandafter\def\csname v@fmt/post/swb/start-gain-pct\endcsname{31}
\expandafter\def\csname v@fmt/post/timit/end\endcsname{10.3}
\expandafter\def\csname v@fmt/post/timit/mae\endcsname{10.5}
\expandafter\def\csname v@fmt/post/timit/start\endcsname{10.8}
\expandafter\def\csname v@fmt/post/vox/end\endcsname{21.3}
\expandafter\def\csname v@fmt/post/vox/mae\endcsname{15.3}
\expandafter\def\csname v@fmt/post/vox/start\endcsname{9.4}
\expandafter\def\csname v@fmt/post/z-mae\endcsname{8.1}
\expandafter\def\csname v@fmt/pre/buckeye/end\endcsname{11.0}
\expandafter\def\csname v@fmt/pre/buckeye/mae\endcsname{12.0}
\expandafter\def\csname v@fmt/pre/buckeye/start\endcsname{13.1}
\expandafter\def\csname v@fmt/pre/ifa/end\endcsname{16.3}
\expandafter\def\csname v@fmt/pre/ifa/mae\endcsname{15.2}
\expandafter\def\csname v@fmt/pre/ifa/start\endcsname{14.1}
\expandafter\def\csname v@fmt/pre/long/end\endcsname{10.1}
\expandafter\def\csname v@fmt/pre/long/mae\endcsname{10.3}
\expandafter\def\csname v@fmt/pre/long/start\endcsname{10.4}
\expandafter\def\csname v@fmt/pre/mean-mae\endcsname{14.00}
\expandafter\def\csname v@fmt/pre/mean-w20\endcsname{84.9}
\expandafter\def\csname v@fmt/pre/runs\endcsname{5}
\expandafter\def\csname v@fmt/pre/seoul/end\endcsname{10.3}
\expandafter\def\csname v@fmt/pre/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@fmt/pre/seoul/start\endcsname{12.6}
\expandafter\def\csname v@fmt/pre/swb/end\endcsname{16.9}
\expandafter\def\csname v@fmt/pre/swb/mae\endcsname{23.2}
\expandafter\def\csname v@fmt/pre/swb/start\endcsname{29.5}
\expandafter\def\csname v@fmt/pre/timit/end\endcsname{10.3}
\expandafter\def\csname v@fmt/pre/timit/mae\endcsname{10.5}
\expandafter\def\csname v@fmt/pre/timit/start\endcsname{10.7}
\expandafter\def\csname v@fmt/pre/vox/end\endcsname{21.4}
\expandafter\def\csname v@fmt/pre/vox/mae\endcsname{15.4}
\expandafter\def\csname v@fmt/pre/vox/start\endcsname{9.3}
\expandafter\def\csname v@fmt/round/buckeye/end\endcsname{11.2}
\expandafter\def\csname v@fmt/round/buckeye/mae\endcsname{12.1}
\expandafter\def\csname v@fmt/round/buckeye/start\endcsname{13.1}
\expandafter\def\csname v@fmt/round/d-mae\endcsname{$+0.26$}
\expandafter\def\csname v@fmt/round/d-mae-abs\endcsname{0.26}
\expandafter\def\csname v@fmt/round/d-w20\endcsname{$-0.4$}
\expandafter\def\csname v@fmt/round/ifa/end\endcsname{16.3}
\expandafter\def\csname v@fmt/round/ifa/mae\endcsname{15.3}
\expandafter\def\csname v@fmt/round/ifa/start\endcsname{14.4}
\expandafter\def\csname v@fmt/round/long/end\endcsname{10.5}
\expandafter\def\csname v@fmt/round/long/mae\endcsname{10.7}
\expandafter\def\csname v@fmt/round/long/start\endcsname{11.0}
\expandafter\def\csname v@fmt/round/mean-mae\endcsname{14.26}
\expandafter\def\csname v@fmt/round/mean-w20\endcsname{84.5}
\expandafter\def\csname v@fmt/round/runs\endcsname{2}
\expandafter\def\csname v@fmt/round/se-mae\endcsname{0.20}
\expandafter\def\csname v@fmt/round/seoul/end\endcsname{10.6}
\expandafter\def\csname v@fmt/round/seoul/mae\endcsname{11.7}
\expandafter\def\csname v@fmt/round/seoul/start\endcsname{12.8}
\expandafter\def\csname v@fmt/round/swb/end\endcsname{17.4}
\expandafter\def\csname v@fmt/round/swb/mae\endcsname{23.6}
\expandafter\def\csname v@fmt/round/swb/start\endcsname{29.7}
\expandafter\def\csname v@fmt/round/timit/end\endcsname{10.6}
\expandafter\def\csname v@fmt/round/timit/mae\endcsname{10.9}
\expandafter\def\csname v@fmt/round/timit/start\endcsname{11.2}
\expandafter\def\csname v@fmt/round/vox/end\endcsname{21.5}
\expandafter\def\csname v@fmt/round/vox/mae\endcsname{15.4}
\expandafter\def\csname v@fmt/round/vox/start\endcsname{9.4}
\expandafter\def\csname v@fmt/round/z-mae\endcsname{2.2}
\expandafter\def\csname v@fmt/whisper/buckeye/end\endcsname{24.0}
\expandafter\def\csname v@fmt/whisper/buckeye/mae\endcsname{25.7}
\expandafter\def\csname v@fmt/whisper/buckeye/start\endcsname{27.4}
\expandafter\def\csname v@fmt/whisper/d-mae\endcsname{$+5.12$}
\expandafter\def\csname v@fmt/whisper/d-mae-abs\endcsname{5.12}
\expandafter\def\csname v@fmt/whisper/d-w20\endcsname{$-1.7$}
\expandafter\def\csname v@fmt/whisper/ifa/end\endcsname{16.7}
\expandafter\def\csname v@fmt/whisper/ifa/mae\endcsname{15.7}
\expandafter\def\csname v@fmt/whisper/ifa/start\endcsname{14.6}
\expandafter\def\csname v@fmt/whisper/long/end\endcsname{10.5}
\expandafter\def\csname v@fmt/whisper/long/mae\endcsname{11.5}
\expandafter\def\csname v@fmt/whisper/long/start\endcsname{12.4}
\expandafter\def\csname v@fmt/whisper/mean-mae\endcsname{19.12}
\expandafter\def\csname v@fmt/whisper/mean-w20\endcsname{83.2}
\expandafter\def\csname v@fmt/whisper/runs\endcsname{2}
\expandafter\def\csname v@fmt/whisper/se-mae\endcsname{1.39}
\expandafter\def\csname v@fmt/whisper/seoul/end\endcsname{21.2}
\expandafter\def\csname v@fmt/whisper/seoul/mae\endcsname{22.8}
\expandafter\def\csname v@fmt/whisper/seoul/start\endcsname{24.3}
\expandafter\def\csname v@fmt/whisper/swb/end\endcsname{26.0}
\expandafter\def\csname v@fmt/whisper/swb/mae\endcsname{31.4}
\expandafter\def\csname v@fmt/whisper/swb/start\endcsname{36.8}
\expandafter\def\csname v@fmt/whisper/timit/end\endcsname{10.7}
\expandafter\def\csname v@fmt/whisper/timit/mae\endcsname{11.8}
\expandafter\def\csname v@fmt/whisper/timit/start\endcsname{12.9}
\expandafter\def\csname v@fmt/whisper/vox/end\endcsname{20.7}
\expandafter\def\csname v@fmt/whisper/vox/mae\endcsname{15.1}
\expandafter\def\csname v@fmt/whisper/vox/start\endcsname{9.5}
\expandafter\def\csname v@fmt/whisper/z-mae\endcsname{42.7}
\expandafter\def\csname v@ifa/ft-ctcm-full/clean/mae\endcsname{17.8}
\expandafter\def\csname v@ifa/ft-ctcm-full/clean/median\endcsname{10.0}
\expandafter\def\csname v@ifa/ft-ctcm-full/clean/over500\endcsname{0.16}
\expandafter\def\csname v@ifa/ft-ctcm-full/clean/w100\endcsname{98.8}
\expandafter\def\csname v@ifa/ft-ctcm-full/clean/w20\endcsname{73.5}
\expandafter\def\csname v@ifa/ft-ctcm-full/clean/w50\endcsname{94.8}
\expandafter\def\csname v@ifa/ft-ctcm-lora/clean/mae\endcsname{18.6}
\expandafter\def\csname v@ifa/ft-ctcm-lora/clean/median\endcsname{10.4}
\expandafter\def\csname v@ifa/ft-ctcm-lora/clean/over500\endcsname{0.20}
\expandafter\def\csname v@ifa/ft-ctcm-lora/clean/w100\endcsname{98.8}
\expandafter\def\csname v@ifa/ft-ctcm-lora/clean/w20\endcsname{73.1}
\expandafter\def\csname v@ifa/ft-ctcm-lora/clean/w50\endcsname{94.6}
\expandafter\def\csname v@ifa/ft-ctcw-full/clean/mae\endcsname{17.4}
\expandafter\def\csname v@ifa/ft-ctcw-full/clean/median\endcsname{9.9}
\expandafter\def\csname v@ifa/ft-ctcw-full/clean/over500\endcsname{0.20}
\expandafter\def\csname v@ifa/ft-ctcw-full/clean/w100\endcsname{99.0}
\expandafter\def\csname v@ifa/ft-ctcw-full/clean/w20\endcsname{75.5}
\expandafter\def\csname v@ifa/ft-ctcw-full/clean/w50\endcsname{95.5}
\expandafter\def\csname v@ifa/ft-ctcw-lora/clean/mae\endcsname{18.1}
\expandafter\def\csname v@ifa/ft-ctcw-lora/clean/median\endcsname{9.9}
\expandafter\def\csname v@ifa/ft-ctcw-lora/clean/over500\endcsname{0.26}
\expandafter\def\csname v@ifa/ft-ctcw-lora/clean/w100\endcsname{99.0}
\expandafter\def\csname v@ifa/ft-ctcw-lora/clean/w20\endcsname{74.9}
\expandafter\def\csname v@ifa/ft-ctcw-lora/clean/w50\endcsname{95.4}
\expandafter\def\csname v@ifa/ft-ts-1k-s1/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-1k-s1/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-1k-s1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-1k-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-1k-s1/clean/w20\endcsname{79.5}
\expandafter\def\csname v@ifa/ft-ts-1k-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-1k/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-1k/clean/median\endcsname{8.3}
\expandafter\def\csname v@ifa/ft-ts-1k/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-1k/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-1k/clean/w20\endcsname{79.2}
\expandafter\def\csname v@ifa/ft-ts-1k/clean/w50\endcsname{96.7}
\expandafter\def\csname v@ifa/ft-ts-4k/clean/mae\endcsname{15.1}
\expandafter\def\csname v@ifa/ft-ts-4k/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-4k/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-4k/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-4k/clean/w20\endcsname{78.0}
\expandafter\def\csname v@ifa/ft-ts-4k/clean/w50\endcsname{96.7}
\expandafter\def\csname v@ifa/ft-ts-6k/clean/mae\endcsname{15.7}
\expandafter\def\csname v@ifa/ft-ts-6k/clean/median\endcsname{9.1}
\expandafter\def\csname v@ifa/ft-ts-6k/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-6k/clean/w100\endcsname{99.0}
\expandafter\def\csname v@ifa/ft-ts-6k/clean/w20\endcsname{77.0}
\expandafter\def\csname v@ifa/ft-ts-6k/clean/w50\endcsname{96.2}
\expandafter\def\csname v@ifa/ft-ts-a02/clean/mae\endcsname{15.3}
\expandafter\def\csname v@ifa/ft-ts-a02/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-a02/clean/over500\endcsname{0.12}
\expandafter\def\csname v@ifa/ft-ts-a02/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-a02/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-a02/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-attn/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-attn/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-attn/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-attn/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-attn/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-attn/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-aug0-s1/clean/mae\endcsname{15.8}
\expandafter\def\csname v@ifa/ft-ts-aug0-s1/clean/median\endcsname{8.9}
\expandafter\def\csname v@ifa/ft-ts-aug0-s1/clean/over500\endcsname{0.16}
\expandafter\def\csname v@ifa/ft-ts-aug0-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-aug0-s1/clean/w20\endcsname{77.9}
\expandafter\def\csname v@ifa/ft-ts-aug0-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-aug0-s2/clean/mae\endcsname{15.1}
\expandafter\def\csname v@ifa/ft-ts-aug0-s2/clean/median\endcsname{8.9}
\expandafter\def\csname v@ifa/ft-ts-aug0-s2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-aug0-s2/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-aug0-s2/clean/w20\endcsname{78.1}
\expandafter\def\csname v@ifa/ft-ts-aug0-s2/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-aug0/clean/mae\endcsname{15.5}
\expandafter\def\csname v@ifa/ft-ts-aug0/clean/median\endcsname{8.8}
\expandafter\def\csname v@ifa/ft-ts-aug0/clean/over500\endcsname{0.12}
\expandafter\def\csname v@ifa/ft-ts-aug0/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-aug0/clean/w20\endcsname{77.7}
\expandafter\def\csname v@ifa/ft-ts-aug0/clean/w50\endcsname{96.1}
\expandafter\def\csname v@ifa/ft-ts-aug100/clean/mae\endcsname{15.2}
\expandafter\def\csname v@ifa/ft-ts-aug100/clean/median\endcsname{9.3}
\expandafter\def\csname v@ifa/ft-ts-aug100/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-aug100/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-aug100/clean/w20\endcsname{78.1}
\expandafter\def\csname v@ifa/ft-ts-aug100/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-aug25-s1/clean/mae\endcsname{15.1}
\expandafter\def\csname v@ifa/ft-ts-aug25-s1/clean/median\endcsname{8.8}
\expandafter\def\csname v@ifa/ft-ts-aug25-s1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-aug25-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-aug25-s1/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-aug25-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-aug25-s2/clean/mae\endcsname{15.0}
\expandafter\def\csname v@ifa/ft-ts-aug25-s2/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-aug25-s2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-aug25-s2/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-aug25-s2/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-aug25-s2/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-aug25/clean/mae\endcsname{15.1}
\expandafter\def\csname v@ifa/ft-ts-aug25/clean/median\endcsname{8.8}
\expandafter\def\csname v@ifa/ft-ts-aug25/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-aug25/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-aug25/clean/w20\endcsname{77.9}
\expandafter\def\csname v@ifa/ft-ts-aug25/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-aug75/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-aug75/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-aug75/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-aug75/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-aug75/clean/w20\endcsname{78.6}
\expandafter\def\csname v@ifa/ft-ts-aug75/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-augamr-s1/clean/mae\endcsname{15.2}
\expandafter\def\csname v@ifa/ft-ts-augamr-s1/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-augamr-s1/clean/over500\endcsname{0.12}
\expandafter\def\csname v@ifa/ft-ts-augamr-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-augamr-s1/clean/w20\endcsname{78.6}
\expandafter\def\csname v@ifa/ft-ts-augamr-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-augamr/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-augamr/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-augamr/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-augamr/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-augamr/clean/w20\endcsname{78.5}
\expandafter\def\csname v@ifa/ft-ts-augamr/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-auxw-s1/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-auxw-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-auxw-s1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-auxw-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-auxw-s1/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-auxw-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-auxw/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-auxw/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-auxw/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-auxw/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-auxw/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-auxw/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-auxwp-s1/clean/mae\endcsname{15.3}
\expandafter\def\csname v@ifa/ft-ts-auxwp-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-auxwp-s1/clean/over500\endcsname{0.14}
\expandafter\def\csname v@ifa/ft-ts-auxwp-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-auxwp-s1/clean/w20\endcsname{78.6}
\expandafter\def\csname v@ifa/ft-ts-auxwp-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-auxwp/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-auxwp/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-auxwp/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-auxwp/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-auxwp/clean/w20\endcsname{78.7}
\expandafter\def\csname v@ifa/ft-ts-auxwp/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-dec/clean/mae\endcsname{16.6}
\expandafter\def\csname v@ifa/ft-ts-dec/clean/median\endcsname{10.3}
\expandafter\def\csname v@ifa/ft-ts-dec/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-dec/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-dec/clean/w20\endcsname{74.7}
\expandafter\def\csname v@ifa/ft-ts-dec/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-full/clean/mae\endcsname{15.1}
\expandafter\def\csname v@ifa/ft-ts-full/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-full/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-full/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-full/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-full/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-lora-argmax/clean/mae\endcsname{16.6}
\expandafter\def\csname v@ifa/ft-ts-lora-argmax/clean/median\endcsname{10.0}
\expandafter\def\csname v@ifa/ft-ts-lora-argmax/clean/over500\endcsname{0.14}
\expandafter\def\csname v@ifa/ft-ts-lora-argmax/clean/w100\endcsname{98.9}
\expandafter\def\csname v@ifa/ft-ts-lora-argmax/clean/w20\endcsname{75.4}
\expandafter\def\csname v@ifa/ft-ts-lora-argmax/clean/w50\endcsname{95.8}
\expandafter\def\csname v@ifa/ft-ts-lora-en-nolang/clean/mae\endcsname{26.1}
\expandafter\def\csname v@ifa/ft-ts-lora-en-nolang/clean/median\endcsname{10.6}
\expandafter\def\csname v@ifa/ft-ts-lora-en-nolang/clean/over500\endcsname{0.72}
\expandafter\def\csname v@ifa/ft-ts-lora-en-nolang/clean/w100\endcsname{97.6}
\expandafter\def\csname v@ifa/ft-ts-lora-en-nolang/clean/w20\endcsname{71.5}
\expandafter\def\csname v@ifa/ft-ts-lora-en-nolang/clean/w50\endcsname{92.0}
\expandafter\def\csname v@ifa/ft-ts-lora-en/clean/mae\endcsname{22.2}
\expandafter\def\csname v@ifa/ft-ts-lora-en/clean/median\endcsname{10.5}
\expandafter\def\csname v@ifa/ft-ts-lora-en/clean/over500\endcsname{0.38}
\expandafter\def\csname v@ifa/ft-ts-lora-en/clean/w100\endcsname{98.1}
\expandafter\def\csname v@ifa/ft-ts-lora-en/clean/w20\endcsname{71.7}
\expandafter\def\csname v@ifa/ft-ts-lora-en/clean/w50\endcsname{92.4}
\expandafter\def\csname v@ifa/ft-ts-lora-full/clean/mae\endcsname{18.4}
\expandafter\def\csname v@ifa/ft-ts-lora-full/clean/median\endcsname{11.3}
\expandafter\def\csname v@ifa/ft-ts-lora-full/clean/over500\endcsname{0.22}
\expandafter\def\csname v@ifa/ft-ts-lora-full/clean/w100\endcsname{98.9}
\expandafter\def\csname v@ifa/ft-ts-lora-full/clean/w20\endcsname{72.0}
\expandafter\def\csname v@ifa/ft-ts-lora-full/clean/w50\endcsname{95.9}
\expandafter\def\csname v@ifa/ft-ts-lora-nolang/clean/mae\endcsname{15.5}
\expandafter\def\csname v@ifa/ft-ts-lora-nolang/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-lora-nolang/clean/over500\endcsname{0.16}
\expandafter\def\csname v@ifa/ft-ts-lora-nolang/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-lora-nolang/clean/w20\endcsname{78.5}
\expandafter\def\csname v@ifa/ft-ts-lora-nolang/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-lora-r1/clean/mae\endcsname{15.4}
\expandafter\def\csname v@ifa/ft-ts-lora-r1/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-lora-r1/clean/over500\endcsname{0.14}
\expandafter\def\csname v@ifa/ft-ts-lora-r1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@ifa/ft-ts-lora-r1/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-lora-r1/clean/w50\endcsname{96.1}
\expandafter\def\csname v@ifa/ft-ts-lora-r5/clean/mae\endcsname{15.3}
\expandafter\def\csname v@ifa/ft-ts-lora-r5/clean/median\endcsname{8.9}
\expandafter\def\csname v@ifa/ft-ts-lora-r5/clean/over500\endcsname{0.14}
\expandafter\def\csname v@ifa/ft-ts-lora-r5/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-lora-r5/clean/w20\endcsname{77.7}
\expandafter\def\csname v@ifa/ft-ts-lora-r5/clean/w50\endcsname{96.9}
\expandafter\def\csname v@ifa/ft-ts-lora/clean/mae\endcsname{15.3}
\expandafter\def\csname v@ifa/ft-ts-lora/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-lora/clean/over500\endcsname{0.14}
\expandafter\def\csname v@ifa/ft-ts-lora/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-lora/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-lora/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-lr1e4/clean/mae\endcsname{14.8}
\expandafter\def\csname v@ifa/ft-ts-lr1e4/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-lr1e4/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-lr1e4/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-lr1e4/clean/w20\endcsname{78.9}
\expandafter\def\csname v@ifa/ft-ts-lr1e4/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-lr5e4/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-lr5e4/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-lr5e4/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-lr5e4/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-lr5e4/clean/w20\endcsname{78.7}
\expandafter\def\csname v@ifa/ft-ts-lr5e4/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-4k/clean/mae\endcsname{15.1}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-4k/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-4k/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-4k/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-4k/clean/w20\endcsname{77.8}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-4k/clean/w50\endcsname{96.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr2e4/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr2e4/clean/median\endcsname{8.3}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr2e4/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr2e4/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr2e4/clean/w20\endcsname{78.1}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr2e4/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr5e3/clean/mae\endcsname{14.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr5e3/clean/median\endcsname{8.3}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr5e3/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr5e3/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr5e3/clean/w20\endcsname{79.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-lr5e3/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-r64/clean/mae\endcsname{14.8}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-r64/clean/median\endcsname{8.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-r64/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-r64/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-r64/clean/w20\endcsname{78.0}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-r64/clean/w50\endcsname{96.1}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-rand/clean/mae\endcsname{14.8}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-rand/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-rand/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-rand/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-rand/clean/w20\endcsname{77.9}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-rand/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-round/clean/mae\endcsname{15.0}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-round/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-round/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-round/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-round/clean/w20\endcsname{78.0}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-round/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s1/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s1/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s1/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s2/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s2/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s2/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s2/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s2/clean/w20\endcsname{78.3}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s2/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s3/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s3/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s3/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s3/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s3/clean/w20\endcsname{78.9}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s3/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s4/clean/mae\endcsname{14.8}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s4/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s4/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s4/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s4/clean/w20\endcsname{78.0}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-s4/clean/w50\endcsname{96.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-tn10/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-tn10/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-tn10/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-tn10/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-tn10/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms-tn10/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-post-10ms/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-post-10ms/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-10ms/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-10ms/clean/w20\endcsname{78.7}
\expandafter\def\csname v@ifa/ft-ts-post-10ms/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-post-5ms/clean/mae\endcsname{14.8}
\expandafter\def\csname v@ifa/ft-ts-post-5ms/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-post-5ms/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-5ms/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-5ms/clean/w20\endcsname{77.7}
\expandafter\def\csname v@ifa/ft-ts-post-5ms/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-post-s1/clean/mae\endcsname{15.3}
\expandafter\def\csname v@ifa/ft-ts-post-s1/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-post-s1/clean/over500\endcsname{0.14}
\expandafter\def\csname v@ifa/ft-ts-post-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-s1/clean/w20\endcsname{78.3}
\expandafter\def\csname v@ifa/ft-ts-post-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-post-s2/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-post-s2/clean/median\endcsname{9.0}
\expandafter\def\csname v@ifa/ft-ts-post-s2/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-s2/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-post-s2/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-post-s2/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-post-s3/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-post-s3/clean/median\endcsname{8.8}
\expandafter\def\csname v@ifa/ft-ts-post-s3/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-s3/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-s3/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-post-s3/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-post-s4/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-post-s4/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-post-s4/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-post-s4/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-post-s4/clean/w20\endcsname{78.5}
\expandafter\def\csname v@ifa/ft-ts-post-s4/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-post-sidon-s1/clean/mae\endcsname{14.8}
\expandafter\def\csname v@ifa/ft-ts-post-sidon-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-post-sidon-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-sidon-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-sidon-s1/clean/w20\endcsname{78.0}
\expandafter\def\csname v@ifa/ft-ts-post-sidon-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-post-sidon/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-post-sidon/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-post-sidon/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-sidon/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-sidon/clean/w20\endcsname{78.1}
\expandafter\def\csname v@ifa/ft-ts-post-sidon/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-post-tn10-s1/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-post-tn10-s1/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-post-tn10-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-tn10-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post-tn10-s1/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-post-tn10-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-post-tn10/clean/mae\endcsname{14.5}
\expandafter\def\csname v@ifa/ft-ts-post-tn10/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-post-tn10/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post-tn10/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-post-tn10/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-post-tn10/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-post/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-post/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-post/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-post/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-post/clean/w20\endcsname{78.3}
\expandafter\def\csname v@ifa/ft-ts-post/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-r128/clean/mae\endcsname{15.0}
\expandafter\def\csname v@ifa/ft-ts-r128/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-r128/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-r128/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-r128/clean/w20\endcsname{78.0}
\expandafter\def\csname v@ifa/ft-ts-r128/clean/w50\endcsname{96.2}
\expandafter\def\csname v@ifa/ft-ts-r16/clean/mae\endcsname{14.8}
\expandafter\def\csname v@ifa/ft-ts-r16/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-r16/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-r16/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-r16/clean/w20\endcsname{78.9}
\expandafter\def\csname v@ifa/ft-ts-r16/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-r64/clean/mae\endcsname{15.0}
\expandafter\def\csname v@ifa/ft-ts-r64/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-r64/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-r64/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-r64/clean/w20\endcsname{78.1}
\expandafter\def\csname v@ifa/ft-ts-r64/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-r8/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-r8/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-r8/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-r8/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-r8/clean/w20\endcsname{78.6}
\expandafter\def\csname v@ifa/ft-ts-r8/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-round-s1/clean/mae\endcsname{15.6}
\expandafter\def\csname v@ifa/ft-ts-round-s1/clean/median\endcsname{8.8}
\expandafter\def\csname v@ifa/ft-ts-round-s1/clean/over500\endcsname{0.16}
\expandafter\def\csname v@ifa/ft-ts-round-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-round-s1/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-round-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-round/clean/mae\endcsname{15.0}
\expandafter\def\csname v@ifa/ft-ts-round/clean/median\endcsname{8.9}
\expandafter\def\csname v@ifa/ft-ts-round/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-round/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-round/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-round/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-s6-final-s1/clean/mae\endcsname{14.4}
\expandafter\def\csname v@ifa/ft-ts-s6-final-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-s6-final-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-s6-final-s1/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-s6-final-s1/clean/w20\endcsname{78.6}
\expandafter\def\csname v@ifa/ft-ts-s6-final-s1/clean/w50\endcsname{96.9}
\expandafter\def\csname v@ifa/ft-ts-s6-final/clean/mae\endcsname{14.5}
\expandafter\def\csname v@ifa/ft-ts-s6-final/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-s6-final/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-s6-final/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-s6-final/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-s6-final/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-s6-post-s1/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-s6-post-s1/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-s6-post-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-s6-post-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-s6-post-s1/clean/w20\endcsname{78.3}
\expandafter\def\csname v@ifa/ft-ts-s6-post-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-s6-post/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-s6-post/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-s6-post/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-s6-post/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-s6-post/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-s6-post/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon-s1/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon-s1/clean/w20\endcsname{78.2}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon/clean/w20\endcsname{78.5}
\expandafter\def\csname v@ifa/ft-ts-s6-sidon/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-seed1/clean/mae\endcsname{15.3}
\expandafter\def\csname v@ifa/ft-ts-seed1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-seed1/clean/over500\endcsname{0.14}
\expandafter\def\csname v@ifa/ft-ts-seed1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-seed1/clean/w20\endcsname{78.7}
\expandafter\def\csname v@ifa/ft-ts-seed1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-seed2/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-seed2/clean/median\endcsname{8.8}
\expandafter\def\csname v@ifa/ft-ts-seed2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-seed2/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-seed2/clean/w20\endcsname{78.7}
\expandafter\def\csname v@ifa/ft-ts-seed2/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-seed3/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-seed3/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-seed3/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-seed3/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-seed3/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-seed3/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-seed4/clean/mae\endcsname{15.5}
\expandafter\def\csname v@ifa/ft-ts-seed4/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-seed4/clean/over500\endcsname{0.16}
\expandafter\def\csname v@ifa/ft-ts-seed4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-seed4/clean/w20\endcsname{78.5}
\expandafter\def\csname v@ifa/ft-ts-seed4/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-tn10-s1/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-tn10-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-tn10-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-tn10-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-tn10-s1/clean/w20\endcsname{79.3}
\expandafter\def\csname v@ifa/ft-ts-tn10-s1/clean/w50\endcsname{96.7}
\expandafter\def\csname v@ifa/ft-ts-tn10/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-tn10/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-tn10/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-tn10/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-tn10/clean/w20\endcsname{79.2}
\expandafter\def\csname v@ifa/ft-ts-tn10/clean/w50\endcsname{96.7}
\expandafter\def\csname v@ifa/ft-ts-tn20/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-tn20/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-tn20/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-tn20/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-tn20/clean/w20\endcsname{79.3}
\expandafter\def\csname v@ifa/ft-ts-tn20/clean/w50\endcsname{96.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-final-s1/clean/mae\endcsname{14.5}
\expandafter\def\csname v@ifa/ft-ts-turbo-final-s1/clean/median\endcsname{8.8}
\expandafter\def\csname v@ifa/ft-ts-turbo-final-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-final-s1/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-turbo-final-s1/clean/w20\endcsname{79.0}
\expandafter\def\csname v@ifa/ft-ts-turbo-final-s1/clean/w50\endcsname{96.8}
\expandafter\def\csname v@ifa/ft-ts-turbo-final/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-final/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-turbo-final/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-final/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-final/clean/w20\endcsname{79.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-final/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-10ms/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-10ms/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-10ms/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-10ms/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-10ms/clean/w20\endcsname{79.0}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-10ms/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-s1/clean/mae\endcsname{15.1}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-s1/clean/median\endcsname{8.9}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-s1/clean/over500\endcsname{0.12}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-s1/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-s1/clean/w20\endcsname{78.1}
\expandafter\def\csname v@ifa/ft-ts-turbo-post-s1/clean/w50\endcsname{96.9}
\expandafter\def\csname v@ifa/ft-ts-turbo-post/clean/mae\endcsname{14.5}
\expandafter\def\csname v@ifa/ft-ts-turbo-post/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-post/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-post/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-post/clean/w20\endcsname{79.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-post/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-s1/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-s1/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-turbo-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-s1/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-turbo-s1/clean/w20\endcsname{78.9}
\expandafter\def\csname v@ifa/ft-ts-turbo-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-s2/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-s2/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-s2/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-s2/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-turbo-s2/clean/w20\endcsname{79.7}
\expandafter\def\csname v@ifa/ft-ts-turbo-s2/clean/w50\endcsname{96.7}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10-s1/clean/mae\endcsname{14.3}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10-s1/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10-s1/clean/w20\endcsname{79.4}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10-s1/clean/w50\endcsname{96.9}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10/clean/w20\endcsname{79.2}
\expandafter\def\csname v@ifa/ft-ts-turbo-tn10/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-turbo/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-turbo/clean/median\endcsname{8.7}
\expandafter\def\csname v@ifa/ft-ts-turbo/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-turbo/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-turbo/clean/w20\endcsname{79.4}
\expandafter\def\csname v@ifa/ft-ts-turbo/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-v3-final-s1/clean/mae\endcsname{14.4}
\expandafter\def\csname v@ifa/ft-ts-v3-final-s1/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-v3-final-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-v3-final-s1/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-v3-final-s1/clean/w20\endcsname{79.1}
\expandafter\def\csname v@ifa/ft-ts-v3-final-s1/clean/w50\endcsname{96.7}
\expandafter\def\csname v@ifa/ft-ts-v3-final/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-v3-final/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-v3-final/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-v3-final/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-v3-final/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-v3-final/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-v3-post-10ms/clean/mae\endcsname{14.5}
\expandafter\def\csname v@ifa/ft-ts-v3-post-10ms/clean/median\endcsname{8.4}
\expandafter\def\csname v@ifa/ft-ts-v3-post-10ms/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-v3-post-10ms/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-v3-post-10ms/clean/w20\endcsname{78.8}
\expandafter\def\csname v@ifa/ft-ts-v3-post-10ms/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-v3-post-s1/clean/mae\endcsname{14.5}
\expandafter\def\csname v@ifa/ft-ts-v3-post-s1/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-v3-post-s1/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-v3-post-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-v3-post-s1/clean/w20\endcsname{79.0}
\expandafter\def\csname v@ifa/ft-ts-v3-post-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-v3-post/clean/mae\endcsname{14.6}
\expandafter\def\csname v@ifa/ft-ts-v3-post/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-v3-post/clean/over500\endcsname{0.08}
\expandafter\def\csname v@ifa/ft-ts-v3-post/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-v3-post/clean/w20\endcsname{78.4}
\expandafter\def\csname v@ifa/ft-ts-v3-post/clean/w50\endcsname{96.3}
\expandafter\def\csname v@ifa/ft-ts-v3-s1/clean/mae\endcsname{16.8}
\expandafter\def\csname v@ifa/ft-ts-v3-s1/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-v3-s1/clean/over500\endcsname{0.28}
\expandafter\def\csname v@ifa/ft-ts-v3-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@ifa/ft-ts-v3-s1/clean/w20\endcsname{78.3}
\expandafter\def\csname v@ifa/ft-ts-v3-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@ifa/ft-ts-v3-s2/clean/mae\endcsname{14.9}
\expandafter\def\csname v@ifa/ft-ts-v3-s2/clean/median\endcsname{8.6}
\expandafter\def\csname v@ifa/ft-ts-v3-s2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-v3-s2/clean/w100\endcsname{99.3}
\expandafter\def\csname v@ifa/ft-ts-v3-s2/clean/w20\endcsname{78.7}
\expandafter\def\csname v@ifa/ft-ts-v3-s2/clean/w50\endcsname{96.6}
\expandafter\def\csname v@ifa/ft-ts-v3/clean/mae\endcsname{14.7}
\expandafter\def\csname v@ifa/ft-ts-v3/clean/median\endcsname{8.5}
\expandafter\def\csname v@ifa/ft-ts-v3/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-v3/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-v3/clean/w20\endcsname{79.2}
\expandafter\def\csname v@ifa/ft-ts-v3/clean/w50\endcsname{96.4}
\expandafter\def\csname v@ifa/ft-ts-wt-s1/clean/mae\endcsname{15.6}
\expandafter\def\csname v@ifa/ft-ts-wt-s1/clean/median\endcsname{9.1}
\expandafter\def\csname v@ifa/ft-ts-wt-s1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-wt-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-wt-s1/clean/w20\endcsname{77.7}
\expandafter\def\csname v@ifa/ft-ts-wt-s1/clean/w50\endcsname{96.1}
\expandafter\def\csname v@ifa/ft-ts-wt/clean/mae\endcsname{15.7}
\expandafter\def\csname v@ifa/ft-ts-wt/clean/median\endcsname{9.1}
\expandafter\def\csname v@ifa/ft-ts-wt/clean/over500\endcsname{0.10}
\expandafter\def\csname v@ifa/ft-ts-wt/clean/w100\endcsname{99.2}
\expandafter\def\csname v@ifa/ft-ts-wt/clean/w20\endcsname{77.1}
\expandafter\def\csname v@ifa/ft-ts-wt/clean/w50\endcsname{96.1}
\expandafter\def\csname v@ifa/mfa-dutch/clean/mae\endcsname{335.4}
\expandafter\def\csname v@ifa/mfa-dutch/clean/median\endcsname{28.3}
\expandafter\def\csname v@ifa/mfa-dutch/clean/over500\endcsname{5.27}
\expandafter\def\csname v@ifa/mfa-dutch/clean/w100\endcsname{91.9}
\expandafter\def\csname v@ifa/mfa-dutch/clean/w20\endcsname{38.1}
\expandafter\def\csname v@ifa/mfa-dutch/clean/w50\endcsname{76.7}
\expandafter\def\csname v@ifa/whisper-tm-cal/clean/mae\endcsname{167.3}
\expandafter\def\csname v@ifa/whisper-tm-cal/clean/median\endcsname{51.0}
\expandafter\def\csname v@ifa/whisper-tm-cal/clean/over500\endcsname{10.28}
\expandafter\def\csname v@ifa/whisper-tm-cal/clean/w100\endcsname{61.4}
\expandafter\def\csname v@ifa/whisper-tm-cal/clean/w20\endcsname{27.7}
\expandafter\def\csname v@ifa/whisper-tm-cal/clean/w50\endcsname{49.4}
\expandafter\def\csname v@long/cfa-edges/clean/ebias\endcsname{18}
\expandafter\def\csname v@long/cfa-edges/clean/ebias-signed\endcsname{$+18$}
\expandafter\def\csname v@long/cfa-edges/clean/fail\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/clean/mae\endcsname{45.3}
\expandafter\def\csname v@long/cfa-edges/clean/median\endcsname{24.7}
\expandafter\def\csname v@long/cfa-edges/clean/over500\endcsname{0.3}
\expandafter\def\csname v@long/cfa-edges/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@long/cfa-edges/clean/sbias\endcsname{8}
\expandafter\def\csname v@long/cfa-edges/clean/sbias-signed\endcsname{$+8$}
\expandafter\def\csname v@long/cfa-edges/clean/w10\endcsname{21.4}
\expandafter\def\csname v@long/cfa-edges/clean/w100\endcsname{88.5}
\expandafter\def\csname v@long/cfa-edges/clean/w20\endcsname{41.4}
\expandafter\def\csname v@long/cfa-edges/clean/w50\endcsname{78.4}
\expandafter\def\csname v@long/cfa-edges/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/cfa-edges/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/cfa-edges/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@long/cfa-edges/g711u/ebias\endcsname{19}
\expandafter\def\csname v@long/cfa-edges/g711u/ebias-signed\endcsname{$+19$}
\expandafter\def\csname v@long/cfa-edges/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/cfa-edges/g711u/mae\endcsname{45.7}
\expandafter\def\csname v@long/cfa-edges/g711u/median\endcsname{25.1}
\expandafter\def\csname v@long/cfa-edges/g711u/over500\endcsname{0.3}
\expandafter\def\csname v@long/cfa-edges/g711u/rtf\endcsname{0.004}
\expandafter\def\csname v@long/cfa-edges/g711u/sbias\endcsname{8}
\expandafter\def\csname v@long/cfa-edges/g711u/sbias-signed\endcsname{$+8$}
\expandafter\def\csname v@long/cfa-edges/g711u/w10\endcsname{21.0}
\expandafter\def\csname v@long/cfa-edges/g711u/w100\endcsname{88.5}
\expandafter\def\csname v@long/cfa-edges/g711u/w20\endcsname{40.7}
\expandafter\def\csname v@long/cfa-edges/g711u/w50\endcsname{78.0}
\expandafter\def\csname v@long/ft-ctcm-full/clean/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcm-full/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ctcm-full/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/clean/mae\endcsname{16.9}
\expandafter\def\csname v@long/ft-ctcm-full/clean/median\endcsname{9.5}
\expandafter\def\csname v@long/ft-ctcm-full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcm-full/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcm-full/clean/sbias\endcsname{2}
\expandafter\def\csname v@long/ft-ctcm-full/clean/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@long/ft-ctcm-full/clean/w10\endcsname{51.8}
\expandafter\def\csname v@long/ft-ctcm-full/clean/w100\endcsname{98.8}
\expandafter\def\csname v@long/ft-ctcm-full/clean/w20\endcsname{74.2}
\expandafter\def\csname v@long/ft-ctcm-full/clean/w50\endcsname{92.9}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/dmae\endcsname{-0.2}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/dw20\endcsname{-0.2}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/dw50\endcsname{-0.3}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/mae\endcsname{16.8}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/median\endcsname{9.5}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/sbias\endcsname{3}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/w10\endcsname{51.6}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/w100\endcsname{98.8}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/w20\endcsname{74.4}
\expandafter\def\csname v@long/ft-ctcm-full/g711u/w50\endcsname{93.1}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/mae\endcsname{17.4}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/median\endcsname{9.8}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/sbias\endcsname{3}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/w10\endcsname{50.7}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/w100\endcsname{98.8}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/w20\endcsname{73.7}
\expandafter\def\csname v@long/ft-ctcm-lora/clean/w50\endcsname{92.4}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/dmae\endcsname{-0.2}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/dw20\endcsname{0.2}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/dw50\endcsname{-0.5}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/mae\endcsname{17.2}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/median\endcsname{9.9}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/sbias\endcsname{3}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/w10\endcsname{50.5}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/w100\endcsname{98.7}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/w20\endcsname{73.5}
\expandafter\def\csname v@long/ft-ctcm-lora/g711u/w50\endcsname{92.9}
\expandafter\def\csname v@long/ft-ctcw-full/clean/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-full/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ctcw-full/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/clean/mae\endcsname{15.7}
\expandafter\def\csname v@long/ft-ctcw-full/clean/median\endcsname{8.5}
\expandafter\def\csname v@long/ft-ctcw-full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcw-full/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcw-full/clean/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-full/clean/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/ft-ctcw-full/clean/w10\endcsname{56.0}
\expandafter\def\csname v@long/ft-ctcw-full/clean/w100\endcsname{98.8}
\expandafter\def\csname v@long/ft-ctcw-full/clean/w20\endcsname{78.3}
\expandafter\def\csname v@long/ft-ctcw-full/clean/w50\endcsname{93.6}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/dmae\endcsname{-0.1}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/dw20\endcsname{0.3}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/dw50\endcsname{-0.1}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/mae\endcsname{15.6}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/median\endcsname{8.5}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/w10\endcsname{55.8}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/w100\endcsname{98.8}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/w20\endcsname{78.0}
\expandafter\def\csname v@long/ft-ctcw-full/g711u/w50\endcsname{93.7}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/mae\endcsname{15.6}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/median\endcsname{8.4}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/w10\endcsname{56.1}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/w100\endcsname{98.8}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/w20\endcsname{78.1}
\expandafter\def\csname v@long/ft-ctcw-lora/clean/w50\endcsname{93.5}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/dmae\endcsname{-0.1}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/dw20\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/dw50\endcsname{-0.3}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/mae\endcsname{15.5}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/median\endcsname{8.5}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/w10\endcsname{56.1}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/w100\endcsname{98.9}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/w20\endcsname{78.1}
\expandafter\def\csname v@long/ft-ctcw-lora/g711u/w50\endcsname{93.7}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/w10\endcsname{71.6}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/w20\endcsname{88.3}
\expandafter\def\csname v@long/ft-ts-1k-s1/clean/w50\endcsname{96.0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/w10\endcsname{70.5}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/w20\endcsname{87.7}
\expandafter\def\csname v@long/ft-ts-1k-s1/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@long/ft-ts-1k/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/clean/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-1k/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-1k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-1k/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-1k/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k/clean/w10\endcsname{72.0}
\expandafter\def\csname v@long/ft-ts-1k/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-1k/clean/w20\endcsname{88.2}
\expandafter\def\csname v@long/ft-ts-1k/clean/w50\endcsname{96.0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-1k/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-1k/g711u/dw50\endcsname{-0.1}
\expandafter\def\csname v@long/ft-ts-1k/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-1k/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-1k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-1k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-1k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-1k/g711u/w10\endcsname{70.6}
\expandafter\def\csname v@long/ft-ts-1k/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-1k/g711u/w20\endcsname{87.6}
\expandafter\def\csname v@long/ft-ts-1k/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@long/ft-ts-4k/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-4k/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/clean/mae\endcsname{10.3}
\expandafter\def\csname v@long/ft-ts-4k/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-4k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-4k/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-4k/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-4k/clean/w10\endcsname{73.6}
\expandafter\def\csname v@long/ft-ts-4k/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-4k/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-4k/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-4k/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-4k/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-4k/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-4k/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-4k/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-4k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-4k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-4k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-4k/g711u/w10\endcsname{72.4}
\expandafter\def\csname v@long/ft-ts-4k/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-4k/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-4k/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-6k/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-6k/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-6k/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-6k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-6k/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-6k/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-6k/clean/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-6k/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-6k/clean/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-6k/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-6k/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-6k/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-6k/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-6k/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-6k/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-6k/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-6k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-6k/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-6k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-6k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-6k/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@long/ft-ts-6k/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-6k/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-6k/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-a02/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-a02/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/clean/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-a02/clean/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-a02/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-a02/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-a02/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-a02/clean/w10\endcsname{71.1}
\expandafter\def\csname v@long/ft-ts-a02/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-a02/clean/w20\endcsname{87.8}
\expandafter\def\csname v@long/ft-ts-a02/clean/w50\endcsname{95.7}
\expandafter\def\csname v@long/ft-ts-a02/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-a02/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-a02/g711u/dw50\endcsname{-0.1}
\expandafter\def\csname v@long/ft-ts-a02/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-a02/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/g711u/mae\endcsname{11.6}
\expandafter\def\csname v@long/ft-ts-a02/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-a02/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-a02/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-a02/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-a02/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-a02/g711u/w10\endcsname{69.9}
\expandafter\def\csname v@long/ft-ts-a02/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-a02/g711u/w20\endcsname{87.2}
\expandafter\def\csname v@long/ft-ts-a02/g711u/w50\endcsname{95.7}
\expandafter\def\csname v@long/ft-ts-attn/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-attn/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-attn/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-attn/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-attn/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-attn/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-attn/clean/w10\endcsname{72.1}
\expandafter\def\csname v@long/ft-ts-attn/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-attn/clean/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-attn/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-attn/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-attn/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-attn/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-attn/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-attn/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-attn/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-attn/g711u/w10\endcsname{71.0}
\expandafter\def\csname v@long/ft-ts-attn/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-attn/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@long/ft-ts-attn/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/w10\endcsname{74.3}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-aug0-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/dmae\endcsname{4.7}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/dw20\endcsname{11.7}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/dw50\endcsname{2.4}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/ebias\endcsname{2}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/mae\endcsname{15.2}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/median\endcsname{8.3}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/w10\endcsname{56.6}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/w20\endcsname{77.8}
\expandafter\def\csname v@long/ft-ts-aug0-s1/g711u/w50\endcsname{94.0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/w10\endcsname{74.1}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-aug0-s2/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/dmae\endcsname{6.0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/dw20\endcsname{13.8}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/dw50\endcsname{3.2}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/ebias\endcsname{2}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/mae\endcsname{16.2}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/median\endcsname{9.1}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/sbias\endcsname{2}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/w10\endcsname{53.5}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/w20\endcsname{75.6}
\expandafter\def\csname v@long/ft-ts-aug0-s2/g711u/w50\endcsname{93.3}
\expandafter\def\csname v@long/ft-ts-aug0/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug0/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-aug0/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-aug0/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug0/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug0/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug0/clean/w10\endcsname{73.8}
\expandafter\def\csname v@long/ft-ts-aug0/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug0/clean/w20\endcsname{89.7}
\expandafter\def\csname v@long/ft-ts-aug0/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/dmae\endcsname{5.8}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/dw20\endcsname{13.9}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/dw50\endcsname{3.2}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/ebias\endcsname{3}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/mae\endcsname{16.0}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/median\endcsname{9.0}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/w10\endcsname{53.8}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/w20\endcsname{75.8}
\expandafter\def\csname v@long/ft-ts-aug0/g711u/w50\endcsname{93.5}
\expandafter\def\csname v@long/ft-ts-aug100/clean/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-aug100/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-aug100/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-aug100/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-aug100/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug100/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug100/clean/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-aug100/clean/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/ft-ts-aug100/clean/w10\endcsname{71.9}
\expandafter\def\csname v@long/ft-ts-aug100/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug100/clean/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-aug100/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/dmae\endcsname{-0.1}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/dw20\endcsname{-0.2}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-aug100/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/w10\endcsname{74.2}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/w20\endcsname{89.7}
\expandafter\def\csname v@long/ft-ts-aug25-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-aug25-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/mae\endcsname{10.1}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/w10\endcsname{73.9}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/w20\endcsname{89.6}
\expandafter\def\csname v@long/ft-ts-aug25-s2/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-aug25-s2/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-aug25/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-aug25/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-aug25/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug25/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug25/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25/clean/w10\endcsname{73.8}
\expandafter\def\csname v@long/ft-ts-aug25/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug25/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-aug25/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-aug25/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-aug75/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug75/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-aug75/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-aug75/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug75/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-aug75/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug75/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-aug75/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-aug75/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-aug75/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-aug75/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/w10\endcsname{74.1}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/w20\endcsname{89.7}
\expandafter\def\csname v@long/ft-ts-augamr-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-augamr-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-augamr/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/clean/mae\endcsname{10.3}
\expandafter\def\csname v@long/ft-ts-augamr/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-augamr/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-augamr/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-augamr/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-augamr/clean/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-augamr/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-augamr/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-augamr/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/w10\endcsname{73.7}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/w20\endcsname{89.6}
\expandafter\def\csname v@long/ft-ts-auxw-s1/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-auxw-s1/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-auxw/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-auxw/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-auxw/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxw/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-auxw/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw/clean/w10\endcsname{73.5}
\expandafter\def\csname v@long/ft-ts-auxw/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-auxw/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-auxw/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-auxw/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/mae\endcsname{10.3}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/w10\endcsname{74.3}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/w20\endcsname{89.8}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/w10\endcsname{73.3}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-auxwp-s1/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/w10\endcsname{73.8}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/w20\endcsname{89.6}
\expandafter\def\csname v@long/ft-ts-auxwp/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/w10\endcsname{73.1}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-auxwp/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-dec/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-dec/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/clean/mae\endcsname{12.0}
\expandafter\def\csname v@long/ft-ts-dec/clean/median\endcsname{6.7}
\expandafter\def\csname v@long/ft-ts-dec/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-dec/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-dec/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-dec/clean/w10\endcsname{65.4}
\expandafter\def\csname v@long/ft-ts-dec/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-dec/clean/w20\endcsname{85.7}
\expandafter\def\csname v@long/ft-ts-dec/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-dec/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-dec/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-dec/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-dec/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/mae\endcsname{12.1}
\expandafter\def\csname v@long/ft-ts-dec/g711u/median\endcsname{6.8}
\expandafter\def\csname v@long/ft-ts-dec/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-dec/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-dec/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-dec/g711u/w10\endcsname{64.1}
\expandafter\def\csname v@long/ft-ts-dec/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-dec/g711u/w20\endcsname{85.3}
\expandafter\def\csname v@long/ft-ts-dec/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-full/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-full/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-full/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-full/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-full/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-full/clean/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-full/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-full/clean/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-full/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-full/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-full/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-full/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-full/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-full/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-full/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-full/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-full/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-full/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-full/g711u/w10\endcsname{71.7}
\expandafter\def\csname v@long/ft-ts-full/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-full/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@long/ft-ts-full/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/w10\endcsname{73.7}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-lora-en/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/w10\endcsname{72.4}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-lora-en/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-lora/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/clean/mae\endcsname{10.3}
\expandafter\def\csname v@long/ft-ts-lora/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-lora/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lora/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora/clean/w10\endcsname{73.7}
\expandafter\def\csname v@long/ft-ts-lora/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lora/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-lora/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-lora/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-lora/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-lora/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lora/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-lora/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-lora/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lora/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora/g711u/w10\endcsname{72.6}
\expandafter\def\csname v@long/ft-ts-lora/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lora/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-lora/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/mae\endcsname{12.0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/median\endcsname{7.4}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/w10\endcsname{64.3}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/w20\endcsname{87.9}
\expandafter\def\csname v@long/ft-ts-lora@argmax/clean/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/mae\endcsname{12.3}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/median\endcsname{7.5}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/w10\endcsname{63.4}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/w20\endcsname{87.0}
\expandafter\def\csname v@long/ft-ts-lora@argmax/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/mae\endcsname{11.3}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/median\endcsname{5.8}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/w10\endcsname{68.5}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/w100\endcsname{99.3}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/w20\endcsname{85.7}
\expandafter\def\csname v@long/ft-ts-lora@full/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/dmae\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/mae\endcsname{11.4}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/median\endcsname{6.0}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/sbias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/w10\endcsname{67.7}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/w100\endcsname{99.3}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/w20\endcsname{85.2}
\expandafter\def\csname v@long/ft-ts-lora@full/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/mae\endcsname{10.3}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/w10\endcsname{74.1}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-lora@r1/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/w10\endcsname{73.0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-lora@r1/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/w10\endcsname{71.8}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/w20\endcsname{88.3}
\expandafter\def\csname v@long/ft-ts-lora@r5/clean/w50\endcsname{97.1}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/w10\endcsname{70.6}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@long/ft-ts-lora@r5/g711u/w50\endcsname{97.0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/w20\endcsname{88.6}
\expandafter\def\csname v@long/ft-ts-lr1e4/clean/w50\endcsname{96.1}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/w10\endcsname{71.7}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/w20\endcsname{88.0}
\expandafter\def\csname v@long/ft-ts-lr1e4/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/mae\endcsname{10.0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/w10\endcsname{74.2}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/w20\endcsname{90.0}
\expandafter\def\csname v@long/ft-ts-lr5e4/clean/w50\endcsname{96.9}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/w10\endcsname{73.0}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/w20\endcsname{89.6}
\expandafter\def\csname v@long/ft-ts-lr5e4/g711u/w50\endcsname{96.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/w10\endcsname{73.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/w10\endcsname{72.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-4k/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/w10\endcsname{73.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr2e4/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/w10\endcsname{71.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/w10\endcsname{70.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/w20\endcsname{87.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-lr5e3/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/w10\endcsname{73.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-r64/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/w10\endcsname{73.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-rand/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/w10\endcsname{70.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/w20\endcsname{88.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/clean/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/mae\endcsname{11.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/median\endcsname{5.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/w10\endcsname{69.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/w20\endcsname{87.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-round/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/w10\endcsname{71.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/w10\endcsname{72.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/w10\endcsname{71.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-s2/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/w10\endcsname{71.7}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-s3/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/w10\endcsname{71.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-s4/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/w10\endcsname{72.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/w10\endcsname{71.1}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@long/ft-ts-post-10ms-tn10/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/w20\endcsname{88.7}
\expandafter\def\csname v@long/ft-ts-post-10ms/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/w10\endcsname{71.8}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/w20\endcsname{88.0}
\expandafter\def\csname v@long/ft-ts-post-10ms/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/w10\endcsname{71.6}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/w20\endcsname{88.1}
\expandafter\def\csname v@long/ft-ts-post-5ms/clean/w50\endcsname{96.1}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/w10\endcsname{70.5}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/w20\endcsname{87.3}
\expandafter\def\csname v@long/ft-ts-post-5ms/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/w10\endcsname{73.2}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-post-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/w20\endcsname{88.7}
\expandafter\def\csname v@long/ft-ts-post-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-post-s2/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-post-s2/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-post-s3/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@long/ft-ts-post-s3/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/w10\endcsname{73.1}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/w20\endcsname{89.3}
\expandafter\def\csname v@long/ft-ts-post-s4/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/w10\endcsname{71.8}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-post-s4/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/w10\endcsname{72.6}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/median\endcsname{5.8}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/w10\endcsname{70.2}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/w20\endcsname{88.0}
\expandafter\def\csname v@long/ft-ts-post-sidon-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-post-sidon/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/rtf\endcsname{0.004}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/w10\endcsname{71.4}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@long/ft-ts-post-sidon/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/w10\endcsname{71.8}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-post-tn10-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/w10\endcsname{72.6}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-post-tn10/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/dmae\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/w10\endcsname{71.7}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@long/ft-ts-post-tn10/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-post/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-post/clean/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-post/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-post/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-post/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-post/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-post/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-post/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-post/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-post/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-post/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-post/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-post/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-r128/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r128/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/clean/mae\endcsname{10.1}
\expandafter\def\csname v@long/ft-ts-r128/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-r128/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r128/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-r128/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r128/clean/w10\endcsname{73.7}
\expandafter\def\csname v@long/ft-ts-r128/clean/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-r128/clean/w20\endcsname{89.8}
\expandafter\def\csname v@long/ft-ts-r128/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-r128/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-r128/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-r128/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-r128/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r128/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/g711u/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-r128/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-r128/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r128/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-r128/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r128/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r128/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-r128/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-r128/g711u/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-r128/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-r16/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r16/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-r16/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-r16/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r16/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-r16/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r16/clean/w10\endcsname{73.1}
\expandafter\def\csname v@long/ft-ts-r16/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-r16/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-r16/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-r16/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-r16/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-r16/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r16/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-r16/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-r16/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-r16/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r16/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r16/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-r16/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-r16/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-r16/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-r64/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r64/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/clean/mae\endcsname{10.1}
\expandafter\def\csname v@long/ft-ts-r64/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-r64/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r64/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-r64/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r64/clean/w10\endcsname{74.1}
\expandafter\def\csname v@long/ft-ts-r64/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-r64/clean/w20\endcsname{89.7}
\expandafter\def\csname v@long/ft-ts-r64/clean/w50\endcsname{96.8}
\expandafter\def\csname v@long/ft-ts-r64/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-r64/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-r64/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-r64/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r64/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/g711u/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-r64/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-r64/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r64/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-r64/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r64/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r64/g711u/w10\endcsname{73.1}
\expandafter\def\csname v@long/ft-ts-r64/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-r64/g711u/w20\endcsname{89.3}
\expandafter\def\csname v@long/ft-ts-r64/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-r8/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r8/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/clean/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-r8/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-r8/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r8/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-r8/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r8/clean/w10\endcsname{72.6}
\expandafter\def\csname v@long/ft-ts-r8/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-r8/clean/w20\endcsname{88.7}
\expandafter\def\csname v@long/ft-ts-r8/clean/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-r8/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-r8/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-r8/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-r8/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r8/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@long/ft-ts-r8/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-r8/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-r8/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-r8/g711u/w10\endcsname{71.6}
\expandafter\def\csname v@long/ft-ts-r8/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-r8/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@long/ft-ts-r8/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/w10\endcsname{72.1}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-round-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/median\endcsname{5.8}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/w10\endcsname{70.9}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@long/ft-ts-round-s1/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-round/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-round/clean/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-round/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-round/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-round/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round/clean/w10\endcsname{71.6}
\expandafter\def\csname v@long/ft-ts-round/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-round/clean/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-round/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-round/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-round/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-round/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@long/ft-ts-round/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-round/g711u/median\endcsname{5.8}
\expandafter\def\csname v@long/ft-ts-round/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-round/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-round/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-round/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-round/g711u/w10\endcsname{70.8}
\expandafter\def\csname v@long/ft-ts-round/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-round/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-round/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/w10\endcsname{72.4}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/dw20\endcsname{1.3}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/median\endcsname{5.9}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/w10\endcsname{69.9}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/w20\endcsname{87.6}
\expandafter\def\csname v@long/ft-ts-s6-final-s1/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-s6-final/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/median\endcsname{5.8}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/w10\endcsname{70.1}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/w20\endcsname{87.7}
\expandafter\def\csname v@long/ft-ts-s6-final/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/w10\endcsname{73.2}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-s6-post-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-s6-post/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/w10\endcsname{71.7}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-s6-post/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/w10\endcsname{72.1}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/median\endcsname{5.8}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/w10\endcsname{70.5}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@long/ft-ts-s6-sidon-s1/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/dw20\endcsname{1.4}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/median\endcsname{5.9}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/w10\endcsname{69.7}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/w20\endcsname{87.6}
\expandafter\def\csname v@long/ft-ts-s6-sidon/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-seed1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-seed1/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-seed1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-seed1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed1/clean/w10\endcsname{73.9}
\expandafter\def\csname v@long/ft-ts-seed1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-seed1/clean/w20\endcsname{89.6}
\expandafter\def\csname v@long/ft-ts-seed1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-seed1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-seed2/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed2/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-seed2/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-seed2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed2/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-seed2/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed2/clean/w10\endcsname{73.7}
\expandafter\def\csname v@long/ft-ts-seed2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-seed2/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-seed2/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-seed2/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-seed3/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed3/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-seed3/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-seed3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed3/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-seed3/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed3/clean/w10\endcsname{73.6}
\expandafter\def\csname v@long/ft-ts-seed3/clean/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-seed3/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-seed3/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-seed3/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-seed4/clean/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-seed4/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-seed4/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-seed4/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-seed4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed4/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-seed4/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed4/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-seed4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-seed4/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-seed4/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-seed4/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/w10\endcsname{73.3}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/w20\endcsname{89.3}
\expandafter\def\csname v@long/ft-ts-tn10-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-tn10-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-tn10/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-tn10/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-tn10/clean/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-tn10/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-tn10/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-tn20/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn20/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-tn20/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-tn20/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-tn20/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn20/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-tn20/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-tn20/clean/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-tn20/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/w10\endcsname{71.7}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@long/ft-ts-tn20/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/clean/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/w10\endcsname{70.9}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/w20\endcsname{87.8}
\expandafter\def\csname v@long/ft-ts-turbo-final-s1/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-turbo-final/clean/w50\endcsname{96.1}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/w10\endcsname{70.8}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/w20\endcsname{87.7}
\expandafter\def\csname v@long/ft-ts-turbo-final/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/w10\endcsname{72.4}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/clean/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/w10\endcsname{71.2}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@long/ft-ts-turbo-post-10ms/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/w10\endcsname{71.8}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@long/ft-ts-turbo-post-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/w20\endcsname{89.3}
\expandafter\def\csname v@long/ft-ts-turbo-post/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/w10\endcsname{72.1}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@long/ft-ts-turbo-post/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/w10\endcsname{73.6}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/w20\endcsname{89.6}
\expandafter\def\csname v@long/ft-ts-turbo-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/w10\endcsname{72.0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-turbo-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/w10\endcsname{73.6}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-turbo-s2/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/w10\endcsname{72.6}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@long/ft-ts-turbo-s2/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/w20\endcsname{89.2}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/w10\endcsname{71.5}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-turbo-tn10-s1/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/w10\endcsname{72.4}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/clean/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/median\endcsname{5.6}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/w10\endcsname{71.3}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@long/ft-ts-turbo-tn10/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-turbo/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-turbo/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-turbo/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo/clean/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo/clean/w10\endcsname{73.5}
\expandafter\def\csname v@long/ft-ts-turbo/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-turbo/clean/w20\endcsname{89.4}
\expandafter\def\csname v@long/ft-ts-turbo/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/median\endcsname{5.5}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/w10\endcsname{72.3}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/w20\endcsname{88.7}
\expandafter\def\csname v@long/ft-ts-turbo/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/w20\endcsname{89.6}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/w10\endcsname{71.0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-v3-final-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-v3-final/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/median\endcsname{5.7}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/w10\endcsname{70.5}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@long/ft-ts-v3-final/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/w10\endcsname{73.4}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/clean/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@long/ft-ts-v3-post-10ms/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/w10\endcsname{73.8}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/w20\endcsname{89.7}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/rtf\endcsname{0.004}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-v3-post-s1/g711u/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/mae\endcsname{10.3}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/w10\endcsname{73.8}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/w20\endcsname{89.3}
\expandafter\def\csname v@long/ft-ts-v3-post/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/median\endcsname{5.4}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-v3-post/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/w10\endcsname{74.0}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/w20\endcsname{89.7}
\expandafter\def\csname v@long/ft-ts-v3-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/w10\endcsname{73.2}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/w20\endcsname{89.0}
\expandafter\def\csname v@long/ft-ts-v3-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/mae\endcsname{10.1}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/w10\endcsname{74.1}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/w20\endcsname{89.7}
\expandafter\def\csname v@long/ft-ts-v3-s2/clean/w50\endcsname{96.7}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/mae\endcsname{10.4}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/w10\endcsname{72.9}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/w20\endcsname{89.1}
\expandafter\def\csname v@long/ft-ts-v3-s2/g711u/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-v3/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/clean/mae\endcsname{10.2}
\expandafter\def\csname v@long/ft-ts-v3/clean/median\endcsname{5.1}
\expandafter\def\csname v@long/ft-ts-v3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@long/ft-ts-v3/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3/clean/w10\endcsname{73.9}
\expandafter\def\csname v@long/ft-ts-v3/clean/w100\endcsname{99.2}
\expandafter\def\csname v@long/ft-ts-v3/clean/w20\endcsname{89.5}
\expandafter\def\csname v@long/ft-ts-v3/clean/w50\endcsname{96.6}
\expandafter\def\csname v@long/ft-ts-v3/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-v3/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-v3/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-v3/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@long/ft-ts-v3/g711u/median\endcsname{5.3}
\expandafter\def\csname v@long/ft-ts-v3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-v3/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@long/ft-ts-v3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-v3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-v3/g711u/w10\endcsname{72.8}
\expandafter\def\csname v@long/ft-ts-v3/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-v3/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@long/ft-ts-v3/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/median\endcsname{6.4}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/rtf\endcsname{0.040}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/w10\endcsname{68.1}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/w20\endcsname{88.0}
\expandafter\def\csname v@long/ft-ts-wt-s1/clean/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/mae\endcsname{11.8}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/median\endcsname{6.6}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/rtf\endcsname{0.038}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/w10\endcsname{67.3}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/w20\endcsname{87.4}
\expandafter\def\csname v@long/ft-ts-wt-s1/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@long/ft-ts-wt/clean/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt/clean/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/clean/mae\endcsname{11.5}
\expandafter\def\csname v@long/ft-ts-wt/clean/median\endcsname{6.4}
\expandafter\def\csname v@long/ft-ts-wt/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-wt/clean/rtf\endcsname{0.040}
\expandafter\def\csname v@long/ft-ts-wt/clean/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt/clean/w10\endcsname{68.2}
\expandafter\def\csname v@long/ft-ts-wt/clean/w100\endcsname{99.1}
\expandafter\def\csname v@long/ft-ts-wt/clean/w20\endcsname{88.1}
\expandafter\def\csname v@long/ft-ts-wt/clean/w50\endcsname{96.2}
\expandafter\def\csname v@long/ft-ts-wt/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@long/ft-ts-wt/g711u/dw20\endcsname{0.4}
\expandafter\def\csname v@long/ft-ts-wt/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@long/ft-ts-wt/g711u/ebias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/mae\endcsname{11.7}
\expandafter\def\csname v@long/ft-ts-wt/g711u/median\endcsname{6.5}
\expandafter\def\csname v@long/ft-ts-wt/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/rtf\endcsname{0.038}
\expandafter\def\csname v@long/ft-ts-wt/g711u/sbias\endcsname{0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@long/ft-ts-wt/g711u/w10\endcsname{67.3}
\expandafter\def\csname v@long/ft-ts-wt/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@long/ft-ts-wt/g711u/w20\endcsname{87.7}
\expandafter\def\csname v@long/ft-ts-wt/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@long/hours\endcsname{1.13}
\expandafter\def\csname v@long/lag/g711u\endcsname{0.000}
\expandafter\def\csname v@long/mfa-arpa/clean/ebias\endcsname{2}
\expandafter\def\csname v@long/mfa-arpa/clean/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@long/mfa-arpa/clean/fail\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/clean/mae\endcsname{19.5}
\expandafter\def\csname v@long/mfa-arpa/clean/median\endcsname{11.6}
\expandafter\def\csname v@long/mfa-arpa/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/mfa-arpa/clean/rtf\endcsname{0.021}
\expandafter\def\csname v@long/mfa-arpa/clean/sbias\endcsname{3}
\expandafter\def\csname v@long/mfa-arpa/clean/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@long/mfa-arpa/clean/w10\endcsname{45.3}
\expandafter\def\csname v@long/mfa-arpa/clean/w100\endcsname{98.2}
\expandafter\def\csname v@long/mfa-arpa/clean/w20\endcsname{68.1}
\expandafter\def\csname v@long/mfa-arpa/clean/w50\endcsname{91.9}
\expandafter\def\csname v@long/mfa-arpa/g711u/dmae\endcsname{6.1}
\expandafter\def\csname v@long/mfa-arpa/g711u/dw20\endcsname{4.7}
\expandafter\def\csname v@long/mfa-arpa/g711u/dw50\endcsname{5.3}
\expandafter\def\csname v@long/mfa-arpa/g711u/ebias\endcsname{1}
\expandafter\def\csname v@long/mfa-arpa/g711u/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/mfa-arpa/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/mfa-arpa/g711u/mae\endcsname{25.6}
\expandafter\def\csname v@long/mfa-arpa/g711u/median\endcsname{13.1}
\expandafter\def\csname v@long/mfa-arpa/g711u/over500\endcsname{0.1}
\expandafter\def\csname v@long/mfa-arpa/g711u/rtf\endcsname{0.021}
\expandafter\def\csname v@long/mfa-arpa/g711u/sbias\endcsname{2}
\expandafter\def\csname v@long/mfa-arpa/g711u/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@long/mfa-arpa/g711u/w10\endcsname{41.6}
\expandafter\def\csname v@long/mfa-arpa/g711u/w100\endcsname{95.1}
\expandafter\def\csname v@long/mfa-arpa/g711u/w20\endcsname{63.4}
\expandafter\def\csname v@long/mfa-arpa/g711u/w50\endcsname{86.6}
\expandafter\def\csname v@long/mms-torchaudio/clean/ebias\endcsname{18}
\expandafter\def\csname v@long/mms-torchaudio/clean/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@long/mms-torchaudio/clean/fail\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/clean/mae\endcsname{38.0}
\expandafter\def\csname v@long/mms-torchaudio/clean/median\endcsname{31.5}
\expandafter\def\csname v@long/mms-torchaudio/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/mms-torchaudio/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@long/mms-torchaudio/clean/sbias\endcsname{41}
\expandafter\def\csname v@long/mms-torchaudio/clean/sbias-signed\endcsname{$+41$}
\expandafter\def\csname v@long/mms-torchaudio/clean/w10\endcsname{18.1}
\expandafter\def\csname v@long/mms-torchaudio/clean/w100\endcsname{96.2}
\expandafter\def\csname v@long/mms-torchaudio/clean/w20\endcsname{34.4}
\expandafter\def\csname v@long/mms-torchaudio/clean/w50\endcsname{70.6}
\expandafter\def\csname v@long/mms-torchaudio/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@long/mms-torchaudio/g711u/dw20\endcsname{-0.1}
\expandafter\def\csname v@long/mms-torchaudio/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@long/mms-torchaudio/g711u/ebias\endcsname{17}
\expandafter\def\csname v@long/mms-torchaudio/g711u/ebias-signed\endcsname{$-17$}
\expandafter\def\csname v@long/mms-torchaudio/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/mms-torchaudio/g711u/mae\endcsname{38.6}
\expandafter\def\csname v@long/mms-torchaudio/g711u/median\endcsname{31.5}
\expandafter\def\csname v@long/mms-torchaudio/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@long/mms-torchaudio/g711u/rtf\endcsname{0.004}
\expandafter\def\csname v@long/mms-torchaudio/g711u/sbias\endcsname{41}
\expandafter\def\csname v@long/mms-torchaudio/g711u/sbias-signed\endcsname{$+41$}
\expandafter\def\csname v@long/mms-torchaudio/g711u/w10\endcsname{18.1}
\expandafter\def\csname v@long/mms-torchaudio/g711u/w100\endcsname{95.7}
\expandafter\def\csname v@long/mms-torchaudio/g711u/w20\endcsname{34.6}
\expandafter\def\csname v@long/mms-torchaudio/g711u/w50\endcsname{70.3}
\expandafter\def\csname v@long/n-utt\endcsname{168}
\expandafter\def\csname v@long/n-words\endcsname{10{,}930}
\expandafter\def\csname v@long/qwen3fa/clean/ebias\endcsname{2}
\expandafter\def\csname v@long/qwen3fa/clean/ebias-signed\endcsname{$-2$}
\expandafter\def\csname v@long/qwen3fa/clean/fail\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/clean/mae\endcsname{29.9}
\expandafter\def\csname v@long/qwen3fa/clean/median\endcsname{24.3}
\expandafter\def\csname v@long/qwen3fa/clean/over500\endcsname{0.0}
\expandafter\def\csname v@long/qwen3fa/clean/rtf\endcsname{0.006}
\expandafter\def\csname v@long/qwen3fa/clean/sbias\endcsname{6}
\expandafter\def\csname v@long/qwen3fa/clean/sbias-signed\endcsname{$-6$}
\expandafter\def\csname v@long/qwen3fa/clean/w10\endcsname{20.9}
\expandafter\def\csname v@long/qwen3fa/clean/w100\endcsname{97.6}
\expandafter\def\csname v@long/qwen3fa/clean/w20\endcsname{41.6}
\expandafter\def\csname v@long/qwen3fa/clean/w50\endcsname{84.6}
\expandafter\def\csname v@long/qwen3fa/g711u/dmae\endcsname{19.7}
\expandafter\def\csname v@long/qwen3fa/g711u/dw20\endcsname{10.6}
\expandafter\def\csname v@long/qwen3fa/g711u/dw50\endcsname{18.2}
\expandafter\def\csname v@long/qwen3fa/g711u/ebias\endcsname{30}
\expandafter\def\csname v@long/qwen3fa/g711u/ebias-signed\endcsname{$-30$}
\expandafter\def\csname v@long/qwen3fa/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/qwen3fa/g711u/mae\endcsname{49.7}
\expandafter\def\csname v@long/qwen3fa/g711u/median\endcsname{33.3}
\expandafter\def\csname v@long/qwen3fa/g711u/over500\endcsname{0.1}
\expandafter\def\csname v@long/qwen3fa/g711u/rtf\endcsname{0.006}
\expandafter\def\csname v@long/qwen3fa/g711u/sbias\endcsname{17}
\expandafter\def\csname v@long/qwen3fa/g711u/sbias-signed\endcsname{$+17$}
\expandafter\def\csname v@long/qwen3fa/g711u/w10\endcsname{15.4}
\expandafter\def\csname v@long/qwen3fa/g711u/w100\endcsname{88.3}
\expandafter\def\csname v@long/qwen3fa/g711u/w20\endcsname{30.9}
\expandafter\def\csname v@long/qwen3fa/g711u/w50\endcsname{66.5}
\expandafter\def\csname v@long/whisper-tm-cal/clean/ebias\endcsname{10}
\expandafter\def\csname v@long/whisper-tm-cal/clean/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@long/whisper-tm-cal/clean/fail\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/clean/mae\endcsname{50.4}
\expandafter\def\csname v@long/whisper-tm-cal/clean/median\endcsname{26.8}
\expandafter\def\csname v@long/whisper-tm-cal/clean/over500\endcsname{0.6}
\expandafter\def\csname v@long/whisper-tm-cal/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@long/whisper-tm-cal/clean/sbias\endcsname{2}
\expandafter\def\csname v@long/whisper-tm-cal/clean/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@long/whisper-tm-cal/clean/w10\endcsname{20.8}
\expandafter\def\csname v@long/whisper-tm-cal/clean/w100\endcsname{89.4}
\expandafter\def\csname v@long/whisper-tm-cal/clean/w20\endcsname{39.2}
\expandafter\def\csname v@long/whisper-tm-cal/clean/w50\endcsname{73.7}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/ebias\endcsname{11}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/ebias-signed\endcsname{$+11$}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/mae\endcsname{50.9}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/median\endcsname{27.2}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/over500\endcsname{0.6}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/rtf\endcsname{0.003}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/sbias\endcsname{1}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/w10\endcsname{20.3}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/w100\endcsname{89.5}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/w20\endcsname{38.6}
\expandafter\def\csname v@long/whisper-tm-cal/g711u/w50\endcsname{73.4}
\expandafter\def\csname v@long/whisper-tm-oai/clean/ebias\endcsname{138}
\expandafter\def\csname v@long/whisper-tm-oai/clean/ebias-signed\endcsname{$-138$}
\expandafter\def\csname v@long/whisper-tm-oai/clean/fail\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/clean/fail-other\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/clean/mae\endcsname{180.6}
\expandafter\def\csname v@long/whisper-tm-oai/clean/median\endcsname{139.9}
\expandafter\def\csname v@long/whisper-tm-oai/clean/over500\endcsname{4.1}
\expandafter\def\csname v@long/whisper-tm-oai/clean/rtf\endcsname{0.005}
\expandafter\def\csname v@long/whisper-tm-oai/clean/sbias\endcsname{142}
\expandafter\def\csname v@long/whisper-tm-oai/clean/sbias-signed\endcsname{$-142$}
\expandafter\def\csname v@long/whisper-tm-oai/clean/w10\endcsname{0.8}
\expandafter\def\csname v@long/whisper-tm-oai/clean/w100\endcsname{29.9}
\expandafter\def\csname v@long/whisper-tm-oai/clean/w20\endcsname{1.9}
\expandafter\def\csname v@long/whisper-tm-oai/clean/w50\endcsname{8.4}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/dmae\endcsname{-0.1}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/dw20\endcsname{0.0}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/dw50\endcsname{-0.2}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/ebias\endcsname{137}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/ebias-signed\endcsname{$-137$}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/fail\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/mae\endcsname{180.4}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/median\endcsname{139.6}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/over500\endcsname{4.2}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/rtf\endcsname{0.004}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/sbias\endcsname{142}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/sbias-signed\endcsname{$-142$}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/w10\endcsname{0.8}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/w100\endcsname{30.1}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/w20\endcsname{1.9}
\expandafter\def\csname v@long/whisper-tm-oai/g711u/w50\endcsname{8.6}
\expandafter\def\csname v@longseoul/cfa-segment/clean/mae\endcsname{51.6}
\expandafter\def\csname v@longseoul/cfa-segment/clean/median\endcsname{26.6}
\expandafter\def\csname v@longseoul/cfa-segment/clean/over500\endcsname{0.64}
\expandafter\def\csname v@longseoul/cfa-segment/clean/rtf\endcsname{0.005}
\expandafter\def\csname v@longseoul/cfa-segment/clean/w100\endcsname{87.8}
\expandafter\def\csname v@longseoul/cfa-segment/clean/w20\endcsname{38.0}
\expandafter\def\csname v@longseoul/cfa-segment/clean/w50\endcsname{74.3}
\expandafter\def\csname v@longseoul/ft-ctcm-lora/clean/mae\endcsname{15.6}
\expandafter\def\csname v@longseoul/ft-ctcm-lora/clean/median\endcsname{7.9}
\expandafter\def\csname v@longseoul/ft-ctcm-lora/clean/over500\endcsname{0.19}
\expandafter\def\csname v@longseoul/ft-ctcm-lora/clean/rtf\endcsname{0.003}
\expandafter\def\csname v@longseoul/ft-ctcm-lora/clean/w100\endcsname{98.6}
\expandafter\def\csname v@longseoul/ft-ctcm-lora/clean/w20\endcsname{82.9}
\expandafter\def\csname v@longseoul/ft-ctcm-lora/clean/w50\endcsname{95.9}
\expandafter\def\csname v@longseoul/ft-ctcw-lora-long/clean/mae\endcsname{13.9}
\expandafter\def\csname v@longseoul/ft-ctcw-lora-long/clean/median\endcsname{7.0}
\expandafter\def\csname v@longseoul/ft-ctcw-lora-long/clean/over500\endcsname{0.18}
\expandafter\def\csname v@longseoul/ft-ctcw-lora-long/clean/rtf\endcsname{0.006}
\expandafter\def\csname v@longseoul/ft-ctcw-lora-long/clean/w100\endcsname{98.8}
\expandafter\def\csname v@longseoul/ft-ctcw-lora-long/clean/w20\endcsname{86.3}
\expandafter\def\csname v@longseoul/ft-ctcw-lora-long/clean/w50\endcsname{96.7}
\expandafter\def\csname v@longseoul/ft-ts-lora-long/clean/mae\endcsname{12.2}
\expandafter\def\csname v@longseoul/ft-ts-lora-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-lora-long/clean/over500\endcsname{0.19}
\expandafter\def\csname v@longseoul/ft-ts-lora-long/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@longseoul/ft-ts-lora-long/clean/w100\endcsname{98.8}
\expandafter\def\csname v@longseoul/ft-ts-lora-long/clean/w20\endcsname{90.0}
\expandafter\def\csname v@longseoul/ft-ts-lora-long/clean/w50\endcsname{97.1}
\expandafter\def\csname v@longseoul/ft-ts-s6-final-long/clean/mae\endcsname{11.1}
\expandafter\def\csname v@longseoul/ft-ts-s6-final-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-s6-final-long/clean/over500\endcsname{0.08}
\expandafter\def\csname v@longseoul/ft-ts-s6-final-long/clean/rtf\endcsname{0.013}
\expandafter\def\csname v@longseoul/ft-ts-s6-final-long/clean/w100\endcsname{99.1}
\expandafter\def\csname v@longseoul/ft-ts-s6-final-long/clean/w20\endcsname{90.4}
\expandafter\def\csname v@longseoul/ft-ts-s6-final-long/clean/w50\endcsname{97.5}
\expandafter\def\csname v@longseoul/ft-ts-seed1-long/clean/mae\endcsname{11.6}
\expandafter\def\csname v@longseoul/ft-ts-seed1-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-seed1-long/clean/over500\endcsname{0.15}
\expandafter\def\csname v@longseoul/ft-ts-seed1-long/clean/rtf\endcsname{0.007}
\expandafter\def\csname v@longseoul/ft-ts-seed1-long/clean/w100\endcsname{98.9}
\expandafter\def\csname v@longseoul/ft-ts-seed1-long/clean/w20\endcsname{90.0}
\expandafter\def\csname v@longseoul/ft-ts-seed1-long/clean/w50\endcsname{97.2}
\expandafter\def\csname v@longseoul/ft-ts-seed2-long/clean/mae\endcsname{11.8}
\expandafter\def\csname v@longseoul/ft-ts-seed2-long/clean/median\endcsname{5.3}
\expandafter\def\csname v@longseoul/ft-ts-seed2-long/clean/over500\endcsname{0.16}
\expandafter\def\csname v@longseoul/ft-ts-seed2-long/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@longseoul/ft-ts-seed2-long/clean/w100\endcsname{98.9}
\expandafter\def\csname v@longseoul/ft-ts-seed2-long/clean/w20\endcsname{89.9}
\expandafter\def\csname v@longseoul/ft-ts-seed2-long/clean/w50\endcsname{97.1}
\expandafter\def\csname v@longseoul/ft-ts-tn10-long/clean/mae\endcsname{11.8}
\expandafter\def\csname v@longseoul/ft-ts-tn10-long/clean/median\endcsname{5.3}
\expandafter\def\csname v@longseoul/ft-ts-tn10-long/clean/over500\endcsname{0.14}
\expandafter\def\csname v@longseoul/ft-ts-tn10-long/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@longseoul/ft-ts-tn10-long/clean/w100\endcsname{98.9}
\expandafter\def\csname v@longseoul/ft-ts-tn10-long/clean/w20\endcsname{90.0}
\expandafter\def\csname v@longseoul/ft-ts-tn10-long/clean/w50\endcsname{97.2}
\expandafter\def\csname v@longseoul/ft-ts-tn10-s1-long/clean/mae\endcsname{11.7}
\expandafter\def\csname v@longseoul/ft-ts-tn10-s1-long/clean/median\endcsname{5.3}
\expandafter\def\csname v@longseoul/ft-ts-tn10-s1-long/clean/over500\endcsname{0.14}
\expandafter\def\csname v@longseoul/ft-ts-tn10-s1-long/clean/rtf\endcsname{0.005}
\expandafter\def\csname v@longseoul/ft-ts-tn10-s1-long/clean/w100\endcsname{98.8}
\expandafter\def\csname v@longseoul/ft-ts-tn10-s1-long/clean/w20\endcsname{89.8}
\expandafter\def\csname v@longseoul/ft-ts-tn10-s1-long/clean/w50\endcsname{97.2}
\expandafter\def\csname v@longseoul/ft-ts-turbo-final-long/clean/mae\endcsname{10.6}
\expandafter\def\csname v@longseoul/ft-ts-turbo-final-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-turbo-final-long/clean/over500\endcsname{0.05}
\expandafter\def\csname v@longseoul/ft-ts-turbo-final-long/clean/rtf\endcsname{0.011}
\expandafter\def\csname v@longseoul/ft-ts-turbo-final-long/clean/w100\endcsname{99.0}
\expandafter\def\csname v@longseoul/ft-ts-turbo-final-long/clean/w20\endcsname{89.8}
\expandafter\def\csname v@longseoul/ft-ts-turbo-final-long/clean/w50\endcsname{97.3}
\expandafter\def\csname v@longseoul/ft-ts-turbo-long/clean/mae\endcsname{11.8}
\expandafter\def\csname v@longseoul/ft-ts-turbo-long/clean/median\endcsname{5.3}
\expandafter\def\csname v@longseoul/ft-ts-turbo-long/clean/over500\endcsname{0.15}
\expandafter\def\csname v@longseoul/ft-ts-turbo-long/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@longseoul/ft-ts-turbo-long/clean/w100\endcsname{98.9}
\expandafter\def\csname v@longseoul/ft-ts-turbo-long/clean/w20\endcsname{89.6}
\expandafter\def\csname v@longseoul/ft-ts-turbo-long/clean/w50\endcsname{97.2}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s1-long/clean/mae\endcsname{12.1}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s1-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s1-long/clean/over500\endcsname{0.17}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s1-long/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s1-long/clean/w100\endcsname{98.9}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s1-long/clean/w20\endcsname{89.8}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s1-long/clean/w50\endcsname{97.0}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s2-long/clean/mae\endcsname{11.9}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s2-long/clean/median\endcsname{5.3}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s2-long/clean/over500\endcsname{0.15}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s2-long/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s2-long/clean/w100\endcsname{98.9}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s2-long/clean/w20\endcsname{89.8}
\expandafter\def\csname v@longseoul/ft-ts-turbo-s2-long/clean/w50\endcsname{97.0}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-long/clean/mae\endcsname{11.9}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-long/clean/over500\endcsname{0.16}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-long/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-long/clean/w100\endcsname{98.9}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-long/clean/w20\endcsname{89.4}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-long/clean/w50\endcsname{97.2}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-s1-long/clean/mae\endcsname{12.1}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-s1-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-s1-long/clean/over500\endcsname{0.17}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-s1-long/clean/rtf\endcsname{0.004}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-s1-long/clean/w100\endcsname{98.8}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-s1-long/clean/w20\endcsname{89.7}
\expandafter\def\csname v@longseoul/ft-ts-turbo-tn10-s1-long/clean/w50\endcsname{97.0}
\expandafter\def\csname v@longseoul/ft-ts-v3-final-long/clean/mae\endcsname{10.1}
\expandafter\def\csname v@longseoul/ft-ts-v3-final-long/clean/median\endcsname{5.4}
\expandafter\def\csname v@longseoul/ft-ts-v3-final-long/clean/over500\endcsname{0.05}
\expandafter\def\csname v@longseoul/ft-ts-v3-final-long/clean/rtf\endcsname{0.013}
\expandafter\def\csname v@longseoul/ft-ts-v3-final-long/clean/w100\endcsname{99.2}
\expandafter\def\csname v@longseoul/ft-ts-v3-final-long/clean/w20\endcsname{90.5}
\expandafter\def\csname v@longseoul/ft-ts-v3-final-long/clean/w50\endcsname{97.7}
\expandafter\def\csname v@longseoul/hours\endcsname{0.93}
\expandafter\def\csname v@longseoul/max-s\endcsname{105}
\expandafter\def\csname v@longseoul/mfa-korean/clean/mae\endcsname{19.0}
\expandafter\def\csname v@longseoul/mfa-korean/clean/median\endcsname{10.7}
\expandafter\def\csname v@longseoul/mfa-korean/clean/over500\endcsname{0.11}
\expandafter\def\csname v@longseoul/mfa-korean/clean/rtf\endcsname{0.013}
\expandafter\def\csname v@longseoul/mfa-korean/clean/w100\endcsname{98.2}
\expandafter\def\csname v@longseoul/mfa-korean/clean/w20\endcsname{71.2}
\expandafter\def\csname v@longseoul/mfa-korean/clean/w50\endcsname{94.1}
\expandafter\def\csname v@longseoul/n-items\endcsname{61}
\expandafter\def\csname v@longseoul/n-words\endcsname{6{,}450}
\expandafter\def\csname v@longseoul/ts-seeds/mae-hi\endcsname{12.2}
\expandafter\def\csname v@longseoul/ts-seeds/mae-lo\endcsname{11.6}
\expandafter\def\csname v@longseoul/ts-seeds/w20-hi\endcsname{90.0}
\expandafter\def\csname v@longseoul/ts-seeds/w20-lo\endcsname{89.9}
\expandafter\def\csname v@peaky/clean/blank\endcsname{67}
\expandafter\def\csname v@peaky/clean/blank-mean\endcsname{63}
\expandafter\def\csname v@peaky/clean/first\endcsname{33}
\expandafter\def\csname v@peaky/clean/first-q25\endcsname{10}
\expandafter\def\csname v@peaky/clean/first-q75\endcsname{53}
\expandafter\def\csname v@peaky/clean/last\endcsname{26}
\expandafter\def\csname v@peaky/clean/n-words\endcsname{11{,}025}
\expandafter\def\csname v@peaky/g711u/blank\endcsname{67}
\expandafter\def\csname v@peaky/g711u/blank-mean\endcsname{63}
\expandafter\def\csname v@peaky/g711u/first\endcsname{33}
\expandafter\def\csname v@peaky/g711u/first-q25\endcsname{10}
\expandafter\def\csname v@peaky/g711u/first-q75\endcsname{54}
\expandafter\def\csname v@peaky/g711u/last\endcsname{25}
\expandafter\def\csname v@peaky/g711u/n-words\endcsname{11{,}025}
\expandafter\def\csname v@peaky/gsm/blank\endcsname{67}
\expandafter\def\csname v@peaky/gsm/blank-mean\endcsname{64}
\expandafter\def\csname v@peaky/gsm/first\endcsname{32}
\expandafter\def\csname v@peaky/gsm/first-q25\endcsname{9}
\expandafter\def\csname v@peaky/gsm/first-q75\endcsname{53}
\expandafter\def\csname v@peaky/gsm/last\endcsname{24}
\expandafter\def\csname v@peaky/gsm/n-words\endcsname{11{,}025}
\expandafter\def\csname v@prior/gap-any-max\endcsname{99.99}
\expandafter\def\csname v@prior/gap-any-min\endcsname{99.95}
\expandafter\def\csname v@prior/gap01-max\endcsname{54}
\expandafter\def\csname v@prior/gap01-min\endcsname{44}
\expandafter\def\csname v@prior/mfa-gap-any-max\endcsname{23}
\expandafter\def\csname v@prior/mfa-gap-any-min\endcsname{12}
\expandafter\def\csname v@prior/mfa-gap01-all\endcsname{14}
\expandafter\def\csname v@prior/mid-speech-max\endcsname{92}
\expandafter\def\csname v@prior/mid-speech-min\endcsname{85}
\expandafter\def\csname v@prior/per-real-max\endcsname{6}
\expandafter\def\csname v@prior/per-real-min\endcsname{4}
\expandafter\def\csname v@prior/precision-max\endcsname{23}
\expandafter\def\csname v@prior/precision-min\endcsname{15}
\expandafter\def\csname v@prior/words-m\endcsname{32.3}
\expandafter\def\csname v@prog/aug/ce\endcsname{16.6}
\expandafter\def\csname v@prog/aug/clean\endcsname{10.5}
\expandafter\def\csname v@prog/aug/codecs\endcsname{11.2}
\expandafter\def\csname v@prog/aug/n\endcsname{5}
\expandafter\def\csname v@prog/aug/seven\endcsname{14.0}
\expandafter\def\csname v@prog/aug/swb\endcsname{23.2}
\expandafter\def\csname v@prog/ctc/ce\endcsname{19.9}
\expandafter\def\csname v@prog/ctc/clean\endcsname{16.4}
\expandafter\def\csname v@prog/ctc/codecs\endcsname{16.4}
\expandafter\def\csname v@prog/ctc/n\endcsname{1}
\expandafter\def\csname v@prog/ctc/seven\endcsname{17.0}
\expandafter\def\csname v@prog/ctc/swb\endcsname{22.3}
\expandafter\def\csname v@prog/degrader/ce\endcsname{13.4}
\expandafter\def\csname v@prog/degrader/clean\endcsname{10.6}
\expandafter\def\csname v@prog/degrader/codecs\endcsname{11.8}
\expandafter\def\csname v@prog/degrader/n\endcsname{2}
\expandafter\def\csname v@prog/degrader/seven\endcsname{12.7}
\expandafter\def\csname v@prog/degrader/swb\endcsname{15.9}
\expandafter\def\csname v@prog/noise/ce\endcsname{16.4}
\expandafter\def\csname v@prog/noise/clean\endcsname{10.7}
\expandafter\def\csname v@prog/noise/codecs\endcsname{11.3}
\expandafter\def\csname v@prog/noise/n\endcsname{2}
\expandafter\def\csname v@prog/noise/seven\endcsname{12.7}
\expandafter\def\csname v@prog/noise/swb\endcsname{16.4}
\expandafter\def\csname v@prog/post/ce\endcsname{16.3}
\expandafter\def\csname v@prog/post/clean\endcsname{10.5}
\expandafter\def\csname v@prog/post/codecs\endcsname{11.2}
\expandafter\def\csname v@prog/post/n\endcsname{5}
\expandafter\def\csname v@prog/post/seven\endcsname{13.0}
\expandafter\def\csname v@prog/post/swb\endcsname{18.4}
\expandafter\def\csname v@prog/stack/ce\endcsname{58.1}
\expandafter\def\csname v@prog/stack/clean\endcsname{46.8}
\expandafter\def\csname v@prog/stack/codecs\endcsname{47.5}
\expandafter\def\csname v@prog/stack/n\endcsname{1}
\expandafter\def\csname v@prog/stack/swb\endcsname{71.6}
\expandafter\def\csname v@prog/ts/ce\endcsname{20.9}
\expandafter\def\csname v@prog/ts/clean\endcsname{10.4}
\expandafter\def\csname v@prog/ts/codecs\endcsname{17.1}
\expandafter\def\csname v@prog/ts/n\endcsname{3}
\expandafter\def\csname v@prog/ts/seven\endcsname{14.2}
\expandafter\def\csname v@prog/ts/swb\endcsname{24.5}
\expandafter\def\csname v@res10/best/mae\endcsname{12.68}
\expandafter\def\csname v@res10/best/median\endcsname{6.51}
\expandafter\def\csname v@res10/best/n\endcsname{2}
\expandafter\def\csname v@res10/best/w10\endcsname{65.9}
\expandafter\def\csname v@res10/best/w20\endcsname{85.2}
\expandafter\def\csname v@res10/best10/mae\endcsname{12.74}
\expandafter\def\csname v@res10/best10/median\endcsname{6.41}
\expandafter\def\csname v@res10/best10/n\endcsname{1}
\expandafter\def\csname v@res10/best10/w10\endcsname{66.1}
\expandafter\def\csname v@res10/best10/w20\endcsname{84.6}
\expandafter\def\csname v@res10/buckeye/d\endcsname{$-0.08$}
\expandafter\def\csname v@res10/buckeye/se\endcsname{0.10}
\expandafter\def\csname v@res10/buckeye/z\endcsname{0.8}
\expandafter\def\csname v@res10/d-mae\endcsname{$-0.04$}
\expandafter\def\csname v@res10/d-median\endcsname{$-0.09$}
\expandafter\def\csname v@res10/d-w10\endcsname{0.2}
\expandafter\def\csname v@res10/d-w20\endcsname{$-0.2$}
\expandafter\def\csname v@res10/ifa/d\endcsname{$-0.05$}
\expandafter\def\csname v@res10/ifa/se\endcsname{0.15}
\expandafter\def\csname v@res10/ifa/z\endcsname{0.3}
\expandafter\def\csname v@res10/long/d\endcsname{0.17}
\expandafter\def\csname v@res10/long/se\endcsname{0.05}
\expandafter\def\csname v@res10/long/z\endcsname{3.5}
\expandafter\def\csname v@res10/ms10/mae\endcsname{12.99}
\expandafter\def\csname v@res10/ms10/median\endcsname{6.47}
\expandafter\def\csname v@res10/ms10/n\endcsname{5}
\expandafter\def\csname v@res10/ms10/w10\endcsname{66.0}
\expandafter\def\csname v@res10/ms10/w20\endcsname{84.8}
\expandafter\def\csname v@res10/post/hi\endcsname{13.22}
\expandafter\def\csname v@res10/post/lo\endcsname{12.86}
\expandafter\def\csname v@res10/post/mae\endcsname{13.02}
\expandafter\def\csname v@res10/post/median\endcsname{6.56}
\expandafter\def\csname v@res10/post/n\endcsname{5}
\expandafter\def\csname v@res10/post/w10\endcsname{65.8}
\expandafter\def\csname v@res10/post/w20\endcsname{85.0}
\expandafter\def\csname v@res10/se-mae\endcsname{0.07}
\expandafter\def\csname v@res10/se-median\endcsname{0.03}
\expandafter\def\csname v@res10/se-w10\endcsname{0.1}
\expandafter\def\csname v@res10/se-w20\endcsname{0.1}
\expandafter\def\csname v@res10/seoul/d\endcsname{$-0.07$}
\expandafter\def\csname v@res10/seoul/se\endcsname{0.08}
\expandafter\def\csname v@res10/seoul/z\endcsname{0.8}
\expandafter\def\csname v@res10/sw/4k/mae\endcsname{13.04}
\expandafter\def\csname v@res10/sw/4k/median\endcsname{6.50}
\expandafter\def\csname v@res10/sw/4k/w10\endcsname{66.1}
\expandafter\def\csname v@res10/sw/4k/w20\endcsname{84.8}
\expandafter\def\csname v@res10/sw/lr2e4/mae\endcsname{12.94}
\expandafter\def\csname v@res10/sw/lr2e4/median\endcsname{6.36}
\expandafter\def\csname v@res10/sw/lr2e4/w10\endcsname{66.3}
\expandafter\def\csname v@res10/sw/lr2e4/w20\endcsname{84.8}
\expandafter\def\csname v@res10/sw/lr5e3/mae\endcsname{12.87}
\expandafter\def\csname v@res10/sw/lr5e3/median\endcsname{6.50}
\expandafter\def\csname v@res10/sw/lr5e3/w10\endcsname{66.0}
\expandafter\def\csname v@res10/sw/lr5e3/w20\endcsname{84.8}
\expandafter\def\csname v@res10/sw/ms5/mae\endcsname{13.14}
\expandafter\def\csname v@res10/sw/ms5/median\endcsname{6.47}
\expandafter\def\csname v@res10/sw/ms5/w10\endcsname{65.6}
\expandafter\def\csname v@res10/sw/ms5/w20\endcsname{84.4}
\expandafter\def\csname v@res10/sw/r64/mae\endcsname{12.86}
\expandafter\def\csname v@res10/sw/r64/median\endcsname{6.33}
\expandafter\def\csname v@res10/sw/r64/w10\endcsname{66.4}
\expandafter\def\csname v@res10/sw/r64/w20\endcsname{85.0}
\expandafter\def\csname v@res10/sw/rand/mae\endcsname{13.03}
\expandafter\def\csname v@res10/sw/rand/median\endcsname{6.33}
\expandafter\def\csname v@res10/sw/rand/w10\endcsname{66.5}
\expandafter\def\csname v@res10/sw/rand/w20\endcsname{84.9}
\expandafter\def\csname v@res10/sw/round/mae\endcsname{13.08}
\expandafter\def\csname v@res10/sw/round/median\endcsname{6.57}
\expandafter\def\csname v@res10/sw/round/w10\endcsname{65.2}
\expandafter\def\csname v@res10/sw/round/w20\endcsname{84.4}
\expandafter\def\csname v@res10/sw/turbo-10/mae\endcsname{12.93}
\expandafter\def\csname v@res10/sw/turbo-10/median\endcsname{6.54}
\expandafter\def\csname v@res10/sw/turbo-10/w10\endcsname{65.9}
\expandafter\def\csname v@res10/sw/turbo-10/w20\endcsname{84.6}
\expandafter\def\csname v@res10/sw/turbo-20/mae\endcsname{12.99}
\expandafter\def\csname v@res10/sw/turbo-20/median\endcsname{6.54}
\expandafter\def\csname v@res10/sw/turbo-20/w10\endcsname{65.9}
\expandafter\def\csname v@res10/sw/turbo-20/w20\endcsname{84.9}
\expandafter\def\csname v@res10/sw/v3-10/mae\endcsname{12.71}
\expandafter\def\csname v@res10/sw/v3-10/median\endcsname{6.36}
\expandafter\def\csname v@res10/sw/v3-10/w10\endcsname{66.5}
\expandafter\def\csname v@res10/sw/v3-10/w20\endcsname{85.2}
\expandafter\def\csname v@res10/sw/v3-20/mae\endcsname{12.88}
\expandafter\def\csname v@res10/sw/v3-20/median\endcsname{6.48}
\expandafter\def\csname v@res10/sw/v3-20/w10\endcsname{66.2}
\expandafter\def\csname v@res10/sw/v3-20/w20\endcsname{85.2}
\expandafter\def\csname v@res10/swb/d\endcsname{$-0.44$}
\expandafter\def\csname v@res10/swb/se\endcsname{0.38}
\expandafter\def\csname v@res10/swb/z\endcsname{1.2}
\expandafter\def\csname v@res10/timit/d\endcsname{0.07}
\expandafter\def\csname v@res10/timit/se\endcsname{0.04}
\expandafter\def\csname v@res10/timit/z\endcsname{1.9}
\expandafter\def\csname v@res10/vox/d\endcsname{0.12}
\expandafter\def\csname v@res10/vox/se\endcsname{0.12}
\expandafter\def\csname v@res10/vox/z\endcsname{1.0}
\expandafter\def\csname v@res10/z-mae\endcsname{0.6}
\expandafter\def\csname v@res10/z-median\endcsname{2.9}
\expandafter\def\csname v@res10/z-w10\endcsname{3.4}
\expandafter\def\csname v@res10/z-w20\endcsname{3.0}
\expandafter\def\csname v@s2/bar/buckeye-codecs/mae\endcsname{26.6}
\expandafter\def\csname v@s2/bar/buckeye-codecs/w20\endcsname{64.5}
\expandafter\def\csname v@s2/bar/buckeye/mae\endcsname{21.5}
\expandafter\def\csname v@s2/bar/buckeye/w20\endcsname{70.7}
\expandafter\def\csname v@s2/bar/ifa/mae\endcsname{335.4}
\expandafter\def\csname v@s2/bar/ifa/w20\endcsname{38.1}
\expandafter\def\csname v@s2/bar/long/mae\endcsname{19.5}
\expandafter\def\csname v@s2/bar/long/w20\endcsname{68.1}
\expandafter\def\csname v@s2/bar/seoul/mae\endcsname{21.3}
\expandafter\def\csname v@s2/bar/seoul/w20\endcsname{70.2}
\expandafter\def\csname v@s2/bar/swb/mae\endcsname{36.5}
\expandafter\def\csname v@s2/bar/swb/w20\endcsname{64.2}
\expandafter\def\csname v@s2/bar/timit-codecs/mae\endcsname{25.7}
\expandafter\def\csname v@s2/bar/timit-codecs/w20\endcsname{62.7}
\expandafter\def\csname v@s2/bar/timit/mae\endcsname{19.1}
\expandafter\def\csname v@s2/bar/timit/w20\endcsname{68.2}
\expandafter\def\csname v@s2/ctcm-full/beats\endcsname{16}
\expandafter\def\csname v@s2/ctcm-full/buckeye-codecs/mae\endcsname{15.9}
\expandafter\def\csname v@s2/ctcm-full/buckeye-codecs/w20\endcsname{77.1}
\expandafter\def\csname v@s2/ctcm-full/buckeye/mae\endcsname{15.4}
\expandafter\def\csname v@s2/ctcm-full/buckeye/w20\endcsname{77.6}
\expandafter\def\csname v@s2/ctcm-full/ifa/mae\endcsname{17.8}
\expandafter\def\csname v@s2/ctcm-full/ifa/w20\endcsname{73.5}
\expandafter\def\csname v@s2/ctcm-full/long/mae\endcsname{16.9}
\expandafter\def\csname v@s2/ctcm-full/long/w20\endcsname{74.2}
\expandafter\def\csname v@s2/ctcm-full/seoul/mae\endcsname{15.6}
\expandafter\def\csname v@s2/ctcm-full/seoul/w20\endcsname{81.7}
\expandafter\def\csname v@s2/ctcm-full/swb/mae\endcsname{21.8}
\expandafter\def\csname v@s2/ctcm-full/swb/w20\endcsname{75.2}
\expandafter\def\csname v@s2/ctcm-full/timit-codecs/mae\endcsname{16.9}
\expandafter\def\csname v@s2/ctcm-full/timit-codecs/w20\endcsname{74.2}
\expandafter\def\csname v@s2/ctcm-full/timit/mae\endcsname{16.9}
\expandafter\def\csname v@s2/ctcm-full/timit/w20\endcsname{74.0}
\expandafter\def\csname v@s2/ctcm-full/vox/mae\endcsname{20.7}
\expandafter\def\csname v@s2/ctcm-full/vox/w20\endcsname{66.9}
\expandafter\def\csname v@s2/ctcm-lora/beats\endcsname{16}
\expandafter\def\csname v@s2/ctcm-lora/buckeye-codecs/mae\endcsname{16.2}
\expandafter\def\csname v@s2/ctcm-lora/buckeye-codecs/w20\endcsname{76.0}
\expandafter\def\csname v@s2/ctcm-lora/buckeye/mae\endcsname{15.7}
\expandafter\def\csname v@s2/ctcm-lora/buckeye/w20\endcsname{77.9}
\expandafter\def\csname v@s2/ctcm-lora/ifa/mae\endcsname{18.6}
\expandafter\def\csname v@s2/ctcm-lora/ifa/w20\endcsname{73.1}
\expandafter\def\csname v@s2/ctcm-lora/long/mae\endcsname{17.4}
\expandafter\def\csname v@s2/ctcm-lora/long/w20\endcsname{73.7}
\expandafter\def\csname v@s2/ctcm-lora/seoul/mae\endcsname{16.2}
\expandafter\def\csname v@s2/ctcm-lora/seoul/w20\endcsname{81.0}
\expandafter\def\csname v@s2/ctcm-lora/swb/mae\endcsname{22.6}
\expandafter\def\csname v@s2/ctcm-lora/swb/w20\endcsname{74.7}
\expandafter\def\csname v@s2/ctcm-lora/timit-codecs/mae\endcsname{17.2}
\expandafter\def\csname v@s2/ctcm-lora/timit-codecs/w20\endcsname{73.6}
\expandafter\def\csname v@s2/ctcm-lora/timit/mae\endcsname{17.2}
\expandafter\def\csname v@s2/ctcm-lora/timit/w20\endcsname{74.0}
\expandafter\def\csname v@s2/ctcm-lora/vox/mae\endcsname{20.3}
\expandafter\def\csname v@s2/ctcm-lora/vox/w20\endcsname{67.4}
\expandafter\def\csname v@s2/ctcw-full/beats\endcsname{16}
\expandafter\def\csname v@s2/ctcw-full/buckeye-codecs/mae\endcsname{14.6}
\expandafter\def\csname v@s2/ctcw-full/buckeye-codecs/w20\endcsname{79.5}
\expandafter\def\csname v@s2/ctcw-full/buckeye/mae\endcsname{13.9}
\expandafter\def\csname v@s2/ctcw-full/buckeye/w20\endcsname{80.5}
\expandafter\def\csname v@s2/ctcw-full/ifa/mae\endcsname{17.4}
\expandafter\def\csname v@s2/ctcw-full/ifa/w20\endcsname{75.5}
\expandafter\def\csname v@s2/ctcw-full/long/mae\endcsname{15.7}
\expandafter\def\csname v@s2/ctcw-full/long/w20\endcsname{78.3}
\expandafter\def\csname v@s2/ctcw-full/seoul/mae\endcsname{14.0}
\expandafter\def\csname v@s2/ctcw-full/seoul/w20\endcsname{85.7}
\expandafter\def\csname v@s2/ctcw-full/swb/mae\endcsname{22.4}
\expandafter\def\csname v@s2/ctcw-full/swb/w20\endcsname{78.0}
\expandafter\def\csname v@s2/ctcw-full/timit-codecs/mae\endcsname{16.4}
\expandafter\def\csname v@s2/ctcw-full/timit-codecs/w20\endcsname{75.7}
\expandafter\def\csname v@s2/ctcw-full/timit/mae\endcsname{16.2}
\expandafter\def\csname v@s2/ctcw-full/timit/w20\endcsname{76.5}
\expandafter\def\csname v@s2/ctcw-full/vox/mae\endcsname{18.5}
\expandafter\def\csname v@s2/ctcw-full/vox/w20\endcsname{73.5}
\expandafter\def\csname v@s2/ctcw-lora/beats\endcsname{16}
\expandafter\def\csname v@s2/ctcw-lora/buckeye-codecs/mae\endcsname{14.7}
\expandafter\def\csname v@s2/ctcw-lora/buckeye-codecs/w20\endcsname{78.9}
\expandafter\def\csname v@s2/ctcw-lora/buckeye/mae\endcsname{14.0}
\expandafter\def\csname v@s2/ctcw-lora/buckeye/w20\endcsname{80.6}
\expandafter\def\csname v@s2/ctcw-lora/ifa/mae\endcsname{18.1}
\expandafter\def\csname v@s2/ctcw-lora/ifa/w20\endcsname{74.9}
\expandafter\def\csname v@s2/ctcw-lora/long/mae\endcsname{15.6}
\expandafter\def\csname v@s2/ctcw-lora/long/w20\endcsname{78.1}
\expandafter\def\csname v@s2/ctcw-lora/seoul/mae\endcsname{13.5}
\expandafter\def\csname v@s2/ctcw-lora/seoul/w20\endcsname{86.0}
\expandafter\def\csname v@s2/ctcw-lora/swb/mae\endcsname{22.3}
\expandafter\def\csname v@s2/ctcw-lora/swb/w20\endcsname{78.0}
\expandafter\def\csname v@s2/ctcw-lora/timit-codecs/mae\endcsname{16.4}
\expandafter\def\csname v@s2/ctcw-lora/timit-codecs/w20\endcsname{75.8}
\expandafter\def\csname v@s2/ctcw-lora/timit/mae\endcsname{16.4}
\expandafter\def\csname v@s2/ctcw-lora/timit/w20\endcsname{76.0}
\expandafter\def\csname v@s2/ctcw-lora/vox/mae\endcsname{18.8}
\expandafter\def\csname v@s2/ctcw-lora/vox/w20\endcsname{73.1}
\expandafter\def\csname v@s2/full-max-abs\endcsname{0.8}
\expandafter\def\csname v@s2/head-gain-max\endcsname{13.2}
\expandafter\def\csname v@s2/head-gain-min\endcsname{2.7}
\expandafter\def\csname v@s2/min-beats\endcsname{16}
\expandafter\def\csname v@s2/n-bar\endcsname{16}
\expandafter\def\csname v@s2/swb/best-ctc-mae\endcsname{21.8}
\expandafter\def\csname v@s2/swb/best-ctc-w20\endcsname{78.0}
\expandafter\def\csname v@s2/ts-full/beats\endcsname{16}
\expandafter\def\csname v@s2/ts-full/buckeye-codecs/mae\endcsname{13.3}
\expandafter\def\csname v@s2/ts-full/buckeye-codecs/w20\endcsname{84.5}
\expandafter\def\csname v@s2/ts-full/buckeye/mae\endcsname{12.4}
\expandafter\def\csname v@s2/ts-full/buckeye/w20\endcsname{85.5}
\expandafter\def\csname v@s2/ts-full/ifa/mae\endcsname{15.1}
\expandafter\def\csname v@s2/ts-full/ifa/w20\endcsname{78.2}
\expandafter\def\csname v@s2/ts-full/long/mae\endcsname{10.5}
\expandafter\def\csname v@s2/ts-full/long/w20\endcsname{88.9}
\expandafter\def\csname v@s2/ts-full/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s2/ts-full/seoul/w20\endcsname{89.9}
\expandafter\def\csname v@s2/ts-full/swb/mae\endcsname{22.7}
\expandafter\def\csname v@s2/ts-full/swb/w20\endcsname{80.5}
\expandafter\def\csname v@s2/ts-full/timit-codecs/mae\endcsname{11.4}
\expandafter\def\csname v@s2/ts-full/timit-codecs/w20\endcsname{87.4}
\expandafter\def\csname v@s2/ts-full/timit/mae\endcsname{10.7}
\expandafter\def\csname v@s2/ts-full/timit/w20\endcsname{88.7}
\expandafter\def\csname v@s2/ts-full/vox/mae\endcsname{15.5}
\expandafter\def\csname v@s2/ts-full/vox/w20\endcsname{80.5}
\expandafter\def\csname v@s2/ts-lead-max\endcsname{12.6}
\expandafter\def\csname v@s2/ts-lead-min\endcsname{2.7}
\expandafter\def\csname v@s2/ts-lora/beats\endcsname{16}
\expandafter\def\csname v@s2/ts-lora/buckeye-codecs/mae\endcsname{13.0}
\expandafter\def\csname v@s2/ts-lora/buckeye-codecs/w20\endcsname{84.6}
\expandafter\def\csname v@s2/ts-lora/buckeye/mae\endcsname{12.1}
\expandafter\def\csname v@s2/ts-lora/buckeye/w20\endcsname{85.8}
\expandafter\def\csname v@s2/ts-lora/ifa/mae\endcsname{15.3}
\expandafter\def\csname v@s2/ts-lora/ifa/w20\endcsname{78.4}
\expandafter\def\csname v@s2/ts-lora/long/mae\endcsname{10.3}
\expandafter\def\csname v@s2/ts-lora/long/w20\endcsname{89.5}
\expandafter\def\csname v@s2/ts-lora/seoul/mae\endcsname{11.3}
\expandafter\def\csname v@s2/ts-lora/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s2/ts-lora/swb/mae\endcsname{23.0}
\expandafter\def\csname v@s2/ts-lora/swb/w20\endcsname{80.7}
\expandafter\def\csname v@s2/ts-lora/timit-codecs/mae\endcsname{11.1}
\expandafter\def\csname v@s2/ts-lora/timit-codecs/w20\endcsname{88.0}
\expandafter\def\csname v@s2/ts-lora/timit/mae\endcsname{10.5}
\expandafter\def\csname v@s2/ts-lora/timit/w20\endcsname{89.1}
\expandafter\def\csname v@s2/ts-lora/vox/mae\endcsname{15.9}
\expandafter\def\csname v@s2/ts-lora/vox/w20\endcsname{80.2}
\expandafter\def\csname v@s2/wenc-gain-max\endcsname{6.6}
\expandafter\def\csname v@s2/wenc-gain-min\endcsname{1.5}
\expandafter\def\csname v@s3/best/mae\endcsname{13.97}
\expandafter\def\csname v@s3/best/name\endcsname{rank 128}
\expandafter\def\csname v@s3/best/z\endcsname{0.3}
\expandafter\def\csname v@s3/dec/dmae-max\endcsname{1.9}
\expandafter\def\csname v@s3/dec/dmae-min\endcsname{1.2}
\expandafter\def\csname v@s3/dec/dw20-max\endcsname{4.9}
\expandafter\def\csname v@s3/dec/dw20-min\endcsname{1.7}
\expandafter\def\csname v@s3/epochs-1k\endcsname{0.33}
\expandafter\def\csname v@s3/epochs-2k\endcsname{0.65}
\expandafter\def\csname v@s3/epochs-4k\endcsname{1.30}
\expandafter\def\csname v@s3/epochs-6k\endcsname{1.95}
\expandafter\def\csname v@s3/max-z-w20\endcsname{$+0.8$}
\expandafter\def\csname v@s3/min-beats\endcsname{16}
\expandafter\def\csname v@s3/n-bar\endcsname{16}
\expandafter\def\csname v@s3/n-better-mae\endcsname{0}
\expandafter\def\csname v@s3/n-better-w20\endcsname{0}
\expandafter\def\csname v@s3/n-changed\endcsname{12}
\expandafter\def\csname v@s3/n-changed-done\endcsname{12}
\expandafter\def\csname v@s3/n-done\endcsname{16}
\expandafter\def\csname v@s3/n-runs\endcsname{16}
\expandafter\def\csname v@s3/n-seeds\endcsname{5}
\expandafter\def\csname v@s3/rank/mean-hi\endcsname{14.19}
\expandafter\def\csname v@s3/rank/mean-lo\endcsname{13.97}
\expandafter\def\csname v@s3/rank/params-hi\endcsname{231}
\expandafter\def\csname v@s3/rank/params-lo\endcsname{14}
\expandafter\def\csname v@s3/rank/swb/hi\endcsname{24.8}
\expandafter\def\csname v@s3/rank/swb/lo\endcsname{22.6}
\expandafter\def\csname v@s3/rank/timit-codecs/hi\endcsname{11.8}
\expandafter\def\csname v@s3/rank/timit-codecs/lo\endcsname{10.8}
\expandafter\def\csname v@s3/rank/timit/hi\endcsname{11.0}
\expandafter\def\csname v@s3/rank/timit/lo\endcsname{10.2}
\expandafter\def\csname v@s3/seed-dev-mae-max\endcsname{13.6}
\expandafter\def\csname v@s3/seed-dev-mae-min\endcsname{13.2}
\expandafter\def\csname v@s3/seed-dev-w20-max\endcsname{85.3}
\expandafter\def\csname v@s3/seed-dev-w20-min\endcsname{84.5}
\expandafter\def\csname v@s3/seed-mae-hi\endcsname{14.15}
\expandafter\def\csname v@s3/seed-mae-lo\endcsname{13.82}
\expandafter\def\csname v@s3/seed-mean-mae\endcsname{14.00}
\expandafter\def\csname v@s3/seed-mean-w20\endcsname{84.91}
\expandafter\def\csname v@s3/seed-range/buckeye-codecs/hi\endcsname{13.0}
\expandafter\def\csname v@s3/seed-range/buckeye-codecs/lo\endcsname{12.7}
\expandafter\def\csname v@s3/seed-range/buckeye-codecs/width\endcsname{0.4}
\expandafter\def\csname v@s3/seed-range/buckeye/hi\endcsname{12.2}
\expandafter\def\csname v@s3/seed-range/buckeye/lo\endcsname{11.9}
\expandafter\def\csname v@s3/seed-range/buckeye/width\endcsname{0.3}
\expandafter\def\csname v@s3/seed-range/ifa/hi\endcsname{15.5}
\expandafter\def\csname v@s3/seed-range/ifa/lo\endcsname{14.9}
\expandafter\def\csname v@s3/seed-range/ifa/width\endcsname{0.7}
\expandafter\def\csname v@s3/seed-range/long/hi\endcsname{10.5}
\expandafter\def\csname v@s3/seed-range/long/lo\endcsname{10.2}
\expandafter\def\csname v@s3/seed-range/long/width\endcsname{0.3}
\expandafter\def\csname v@s3/seed-range/seoul/hi\endcsname{11.5}
\expandafter\def\csname v@s3/seed-range/seoul/lo\endcsname{11.3}
\expandafter\def\csname v@s3/seed-range/seoul/width\endcsname{0.2}
\expandafter\def\csname v@s3/seed-range/swb/hi\endcsname{23.6}
\expandafter\def\csname v@s3/seed-range/swb/lo\endcsname{23.0}
\expandafter\def\csname v@s3/seed-range/swb/width\endcsname{0.6}
\expandafter\def\csname v@s3/seed-range/timit-codecs/hi\endcsname{11.3}
\expandafter\def\csname v@s3/seed-range/timit-codecs/lo\endcsname{11.1}
\expandafter\def\csname v@s3/seed-range/timit-codecs/width\endcsname{0.3}
\expandafter\def\csname v@s3/seed-range/timit/hi\endcsname{10.6}
\expandafter\def\csname v@s3/seed-range/timit/lo\endcsname{10.4}
\expandafter\def\csname v@s3/seed-range/timit/width\endcsname{0.2}
\expandafter\def\csname v@s3/seed-range/vox/hi\endcsname{15.9}
\expandafter\def\csname v@s3/seed-range/vox/lo\endcsname{14.8}
\expandafter\def\csname v@s3/seed-range/vox/width\endcsname{1.1}
\expandafter\def\csname v@s3/seed-sd-mae\endcsname{0.12}
\expandafter\def\csname v@s3/seed-sd-w20\endcsname{0.11}
\expandafter\def\csname v@s3/seeds\endcsname{5}
\expandafter\def\csname v@s3/stronger/mean-hi\endcsname{14.28}
\expandafter\def\csname v@s3/stronger/mean-lo\endcsname{13.97}
\expandafter\def\csname v@s3/stronger/params-hi\endcsname{231}
\expandafter\def\csname v@s3/stronger/params-lo\endcsname{58}
\expandafter\def\csname v@s3/stronger/swb/hi\endcsname{24.8}
\expandafter\def\csname v@s3/stronger/swb/lo\endcsname{23.9}
\expandafter\def\csname v@s3/stronger/timit-codecs/hi\endcsname{10.9}
\expandafter\def\csname v@s3/stronger/timit-codecs/lo\endcsname{10.7}
\expandafter\def\csname v@s3/stronger/timit/hi\endcsname{10.4}
\expandafter\def\csname v@s3/stronger/timit/lo\endcsname{10.1}
\expandafter\def\csname v@s3/ts-1k/buckeye-codecs/mae\endcsname{12.9}
\expandafter\def\csname v@s3/ts-1k/buckeye-codecs/w20\endcsname{84.6}
\expandafter\def\csname v@s3/ts-1k/buckeye/mae\endcsname{12.2}
\expandafter\def\csname v@s3/ts-1k/buckeye/w20\endcsname{85.2}
\expandafter\def\csname v@s3/ts-1k/d-mae\endcsname{0.1}
\expandafter\def\csname v@s3/ts-1k/d-w20\endcsname{0.4}
\expandafter\def\csname v@s3/ts-1k/dev-mae\endcsname{14.1}
\expandafter\def\csname v@s3/ts-1k/dev-w20\endcsname{84.1}
\expandafter\def\csname v@s3/ts-1k/ifa/mae\endcsname{14.7}
\expandafter\def\csname v@s3/ts-1k/ifa/w20\endcsname{79.2}
\expandafter\def\csname v@s3/ts-1k/long/mae\endcsname{10.9}
\expandafter\def\csname v@s3/ts-1k/long/w20\endcsname{88.2}
\expandafter\def\csname v@s3/ts-1k/mean-mae\endcsname{14.11}
\expandafter\def\csname v@s3/ts-1k/mean-w20\endcsname{84.49}
\expandafter\def\csname v@s3/ts-1k/params\endcsname{58}
\expandafter\def\csname v@s3/ts-1k/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s3/ts-1k/seoul/w20\endcsname{89.8}
\expandafter\def\csname v@s3/ts-1k/swb/mae\endcsname{22.7}
\expandafter\def\csname v@s3/ts-1k/swb/w20\endcsname{81.1}
\expandafter\def\csname v@s3/ts-1k/timit-codecs/mae\endcsname{12.0}
\expandafter\def\csname v@s3/ts-1k/timit-codecs/w20\endcsname{86.0}
\expandafter\def\csname v@s3/ts-1k/timit/mae\endcsname{11.0}
\expandafter\def\csname v@s3/ts-1k/timit/w20\endcsname{87.8}
\expandafter\def\csname v@s3/ts-1k/vox/mae\endcsname{15.9}
\expandafter\def\csname v@s3/ts-1k/vox/w20\endcsname{80.0}
\expandafter\def\csname v@s3/ts-1k/z-mae\endcsname{0.9}
\expandafter\def\csname v@s3/ts-1k/z-w20\endcsname{3.8}
\expandafter\def\csname v@s3/ts-4k/buckeye-codecs/mae\endcsname{13.0}
\expandafter\def\csname v@s3/ts-4k/buckeye-codecs/w20\endcsname{84.4}
\expandafter\def\csname v@s3/ts-4k/buckeye/mae\endcsname{12.2}
\expandafter\def\csname v@s3/ts-4k/buckeye/w20\endcsname{85.4}
\expandafter\def\csname v@s3/ts-4k/d-mae\endcsname{0.3}
\expandafter\def\csname v@s3/ts-4k/d-w20\endcsname{0.6}
\expandafter\def\csname v@s3/ts-4k/dev-mae\endcsname{13.6}
\expandafter\def\csname v@s3/ts-4k/dev-w20\endcsname{84.2}
\expandafter\def\csname v@s3/ts-4k/ifa/mae\endcsname{15.1}
\expandafter\def\csname v@s3/ts-4k/ifa/w20\endcsname{78.0}
\expandafter\def\csname v@s3/ts-4k/long/mae\endcsname{10.3}
\expandafter\def\csname v@s3/ts-4k/long/w20\endcsname{89.5}
\expandafter\def\csname v@s3/ts-4k/mean-mae\endcsname{14.28}
\expandafter\def\csname v@s3/ts-4k/mean-w20\endcsname{84.36}
\expandafter\def\csname v@s3/ts-4k/params\endcsname{58}
\expandafter\def\csname v@s3/ts-4k/seoul/mae\endcsname{11.8}
\expandafter\def\csname v@s3/ts-4k/seoul/w20\endcsname{89.5}
\expandafter\def\csname v@s3/ts-4k/swb/mae\endcsname{24.5}
\expandafter\def\csname v@s3/ts-4k/swb/w20\endcsname{79.2}
\expandafter\def\csname v@s3/ts-4k/timit-codecs/mae\endcsname{10.8}
\expandafter\def\csname v@s3/ts-4k/timit-codecs/w20\endcsname{88.5}
\expandafter\def\csname v@s3/ts-4k/timit/mae\endcsname{10.4}
\expandafter\def\csname v@s3/ts-4k/timit/w20\endcsname{89.5}
\expandafter\def\csname v@s3/ts-4k/vox/mae\endcsname{15.6}
\expandafter\def\csname v@s3/ts-4k/vox/w20\endcsname{79.5}
\expandafter\def\csname v@s3/ts-4k/z-mae\endcsname{2.4}
\expandafter\def\csname v@s3/ts-4k/z-w20\endcsname{5.0}
\expandafter\def\csname v@s3/ts-6k/buckeye-codecs/mae\endcsname{13.1}
\expandafter\def\csname v@s3/ts-6k/buckeye-codecs/w20\endcsname{84.3}
\expandafter\def\csname v@s3/ts-6k/buckeye/mae\endcsname{12.3}
\expandafter\def\csname v@s3/ts-6k/buckeye/w20\endcsname{84.5}
\expandafter\def\csname v@s3/ts-6k/d-mae\endcsname{0.4}
\expandafter\def\csname v@s3/ts-6k/d-w20\endcsname{1.0}
\expandafter\def\csname v@s3/ts-6k/dev-mae\endcsname{14.0}
\expandafter\def\csname v@s3/ts-6k/dev-w20\endcsname{84.3}
\expandafter\def\csname v@s3/ts-6k/ifa/mae\endcsname{15.7}
\expandafter\def\csname v@s3/ts-6k/ifa/w20\endcsname{77.0}
\expandafter\def\csname v@s3/ts-6k/long/mae\endcsname{10.4}
\expandafter\def\csname v@s3/ts-6k/long/w20\endcsname{89.1}
\expandafter\def\csname v@s3/ts-6k/mean-mae\endcsname{14.43}
\expandafter\def\csname v@s3/ts-6k/mean-w20\endcsname{83.87}
\expandafter\def\csname v@s3/ts-6k/params\endcsname{58}
\expandafter\def\csname v@s3/ts-6k/seoul/mae\endcsname{12.0}
\expandafter\def\csname v@s3/ts-6k/seoul/w20\endcsname{88.9}
\expandafter\def\csname v@s3/ts-6k/swb/mae\endcsname{24.7}
\expandafter\def\csname v@s3/ts-6k/swb/w20\endcsname{79.0}
\expandafter\def\csname v@s3/ts-6k/timit-codecs/mae\endcsname{10.9}
\expandafter\def\csname v@s3/ts-6k/timit-codecs/w20\endcsname{88.0}
\expandafter\def\csname v@s3/ts-6k/timit/mae\endcsname{10.3}
\expandafter\def\csname v@s3/ts-6k/timit/w20\endcsname{88.9}
\expandafter\def\csname v@s3/ts-6k/vox/mae\endcsname{15.6}
\expandafter\def\csname v@s3/ts-6k/vox/w20\endcsname{79.7}
\expandafter\def\csname v@s3/ts-6k/z-mae\endcsname{3.6}
\expandafter\def\csname v@s3/ts-6k/z-w20\endcsname{9.4}
\expandafter\def\csname v@s3/ts-a02/buckeye-codecs/mae\endcsname{13.2}
\expandafter\def\csname v@s3/ts-a02/buckeye-codecs/w20\endcsname{83.9}
\expandafter\def\csname v@s3/ts-a02/buckeye/mae\endcsname{12.4}
\expandafter\def\csname v@s3/ts-a02/buckeye/w20\endcsname{84.9}
\expandafter\def\csname v@s3/ts-a02/d-mae\endcsname{0.4}
\expandafter\def\csname v@s3/ts-a02/d-w20\endcsname{0.9}
\expandafter\def\csname v@s3/ts-a02/dev-mae\endcsname{14.3}
\expandafter\def\csname v@s3/ts-a02/dev-w20\endcsname{84.2}
\expandafter\def\csname v@s3/ts-a02/ifa/mae\endcsname{15.3}
\expandafter\def\csname v@s3/ts-a02/ifa/w20\endcsname{78.8}
\expandafter\def\csname v@s3/ts-a02/long/mae\endcsname{11.2}
\expandafter\def\csname v@s3/ts-a02/long/w20\endcsname{87.8}
\expandafter\def\csname v@s3/ts-a02/mean-mae\endcsname{14.44}
\expandafter\def\csname v@s3/ts-a02/mean-w20\endcsname{84.00}
\expandafter\def\csname v@s3/ts-a02/params\endcsname{58}
\expandafter\def\csname v@s3/ts-a02/seoul/mae\endcsname{11.6}
\expandafter\def\csname v@s3/ts-a02/seoul/w20\endcsname{89.6}
\expandafter\def\csname v@s3/ts-a02/swb/mae\endcsname{22.2}
\expandafter\def\csname v@s3/ts-a02/swb/w20\endcsname{81.1}
\expandafter\def\csname v@s3/ts-a02/timit-codecs/mae\endcsname{12.3}
\expandafter\def\csname v@s3/ts-a02/timit-codecs/w20\endcsname{85.4}
\expandafter\def\csname v@s3/ts-a02/timit/mae\endcsname{11.5}
\expandafter\def\csname v@s3/ts-a02/timit/w20\endcsname{87.3}
\expandafter\def\csname v@s3/ts-a02/vox/mae\endcsname{16.9}
\expandafter\def\csname v@s3/ts-a02/vox/w20\endcsname{78.3}
\expandafter\def\csname v@s3/ts-a02/z-mae\endcsname{3.7}
\expandafter\def\csname v@s3/ts-a02/z-w20\endcsname{8.2}
\expandafter\def\csname v@s3/ts-attn/buckeye-codecs/mae\endcsname{13.0}
\expandafter\def\csname v@s3/ts-attn/buckeye-codecs/w20\endcsname{84.5}
\expandafter\def\csname v@s3/ts-attn/buckeye/mae\endcsname{12.0}
\expandafter\def\csname v@s3/ts-attn/buckeye/w20\endcsname{85.5}
\expandafter\def\csname v@s3/ts-attn/d-mae\endcsname{0.2}
\expandafter\def\csname v@s3/ts-attn/d-w20\endcsname{0.4}
\expandafter\def\csname v@s3/ts-attn/dev-mae\endcsname{13.9}
\expandafter\def\csname v@s3/ts-attn/dev-w20\endcsname{84.3}
\expandafter\def\csname v@s3/ts-attn/ifa/mae\endcsname{14.9}
\expandafter\def\csname v@s3/ts-attn/ifa/w20\endcsname{78.8}
\expandafter\def\csname v@s3/ts-attn/long/mae\endcsname{10.7}
\expandafter\def\csname v@s3/ts-attn/long/w20\endcsname{88.8}
\expandafter\def\csname v@s3/ts-attn/mean-mae\endcsname{14.17}
\expandafter\def\csname v@s3/ts-attn/mean-w20\endcsname{84.52}
\expandafter\def\csname v@s3/ts-attn/params\endcsname{31}
\expandafter\def\csname v@s3/ts-attn/seoul/mae\endcsname{11.3}
\expandafter\def\csname v@s3/ts-attn/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s3/ts-attn/swb/mae\endcsname{23.1}
\expandafter\def\csname v@s3/ts-attn/swb/w20\endcsname{80.9}
\expandafter\def\csname v@s3/ts-attn/timit-codecs/mae\endcsname{11.5}
\expandafter\def\csname v@s3/ts-attn/timit-codecs/w20\endcsname{87.2}
\expandafter\def\csname v@s3/ts-attn/timit/mae\endcsname{11.0}
\expandafter\def\csname v@s3/ts-attn/timit/w20\endcsname{88.5}
\expandafter\def\csname v@s3/ts-attn/vox/mae\endcsname{16.2}
\expandafter\def\csname v@s3/ts-attn/vox/w20\endcsname{79.2}
\expandafter\def\csname v@s3/ts-attn/z-mae\endcsname{1.4}
\expandafter\def\csname v@s3/ts-attn/z-w20\endcsname{3.6}
\expandafter\def\csname v@s3/ts-dec/buckeye-codecs/mae\endcsname{13.9}
\expandafter\def\csname v@s3/ts-dec/buckeye-codecs/w20\endcsname{81.7}
\expandafter\def\csname v@s3/ts-dec/buckeye/mae\endcsname{13.3}
\expandafter\def\csname v@s3/ts-dec/buckeye/w20\endcsname{82.8}
\expandafter\def\csname v@s3/ts-dec/d-mae\endcsname{1.5}
\expandafter\def\csname v@s3/ts-dec/d-w20\endcsname{3.4}
\expandafter\def\csname v@s3/ts-dec/dev-mae\endcsname{15.0}
\expandafter\def\csname v@s3/ts-dec/dev-w20\endcsname{81.8}
\expandafter\def\csname v@s3/ts-dec/ifa/mae\endcsname{16.6}
\expandafter\def\csname v@s3/ts-dec/ifa/w20\endcsname{74.7}
\expandafter\def\csname v@s3/ts-dec/long/mae\endcsname{12.0}
\expandafter\def\csname v@s3/ts-dec/long/w20\endcsname{85.7}
\expandafter\def\csname v@s3/ts-dec/mean-mae\endcsname{15.53}
\expandafter\def\csname v@s3/ts-dec/mean-w20\endcsname{81.49}
\expandafter\def\csname v@s3/ts-dec/params\endcsname{34}
\expandafter\def\csname v@s3/ts-dec/seoul/mae\endcsname{12.7}
\expandafter\def\csname v@s3/ts-dec/seoul/w20\endcsname{87.5}
\expandafter\def\csname v@s3/ts-dec/swb/mae\endcsname{24.2}
\expandafter\def\csname v@s3/ts-dec/swb/w20\endcsname{79.0}
\expandafter\def\csname v@s3/ts-dec/timit-codecs/mae\endcsname{12.9}
\expandafter\def\csname v@s3/ts-dec/timit-codecs/w20\endcsname{84.0}
\expandafter\def\csname v@s3/ts-dec/timit/mae\endcsname{12.3}
\expandafter\def\csname v@s3/ts-dec/timit/w20\endcsname{85.5}
\expandafter\def\csname v@s3/ts-dec/vox/mae\endcsname{17.6}
\expandafter\def\csname v@s3/ts-dec/vox/w20\endcsname{75.3}
\expandafter\def\csname v@s3/ts-dec/z-mae\endcsname{12.8}
\expandafter\def\csname v@s3/ts-dec/z-w20\endcsname{30.6}
\expandafter\def\csname v@s3/ts-lora/buckeye-codecs/mae\endcsname{13.0}
\expandafter\def\csname v@s3/ts-lora/buckeye-codecs/w20\endcsname{84.6}
\expandafter\def\csname v@s3/ts-lora/buckeye/mae\endcsname{12.1}
\expandafter\def\csname v@s3/ts-lora/buckeye/w20\endcsname{85.8}
\expandafter\def\csname v@s3/ts-lora/d-mae\endcsname{0.1}
\expandafter\def\csname v@s3/ts-lora/d-w20\endcsname{0.1}
\expandafter\def\csname v@s3/ts-lora/dev-mae\endcsname{13.4}
\expandafter\def\csname v@s3/ts-lora/dev-w20\endcsname{85.0}
\expandafter\def\csname v@s3/ts-lora/ifa/mae\endcsname{15.3}
\expandafter\def\csname v@s3/ts-lora/ifa/w20\endcsname{78.4}
\expandafter\def\csname v@s3/ts-lora/long/mae\endcsname{10.3}
\expandafter\def\csname v@s3/ts-lora/long/w20\endcsname{89.5}
\expandafter\def\csname v@s3/ts-lora/mean-mae\endcsname{14.06}
\expandafter\def\csname v@s3/ts-lora/mean-w20\endcsname{84.82}
\expandafter\def\csname v@s3/ts-lora/params\endcsname{58}
\expandafter\def\csname v@s3/ts-lora/seoul/mae\endcsname{11.3}
\expandafter\def\csname v@s3/ts-lora/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s3/ts-lora/swb/mae\endcsname{23.0}
\expandafter\def\csname v@s3/ts-lora/swb/w20\endcsname{80.7}
\expandafter\def\csname v@s3/ts-lora/timit-codecs/mae\endcsname{11.1}
\expandafter\def\csname v@s3/ts-lora/timit-codecs/w20\endcsname{88.0}
\expandafter\def\csname v@s3/ts-lora/timit/mae\endcsname{10.5}
\expandafter\def\csname v@s3/ts-lora/timit/w20\endcsname{89.1}
\expandafter\def\csname v@s3/ts-lora/vox/mae\endcsname{15.9}
\expandafter\def\csname v@s3/ts-lora/vox/w20\endcsname{80.2}
\expandafter\def\csname v@s3/ts-lora/z-mae\endcsname{0.5}
\expandafter\def\csname v@s3/ts-lora/z-w20\endcsname{0.9}
\expandafter\def\csname v@s3/ts-lr1e4/buckeye-codecs/mae\endcsname{13.2}
\expandafter\def\csname v@s3/ts-lr1e4/buckeye-codecs/w20\endcsname{84.1}
\expandafter\def\csname v@s3/ts-lr1e4/buckeye/mae\endcsname{12.2}
\expandafter\def\csname v@s3/ts-lr1e4/buckeye/w20\endcsname{85.4}
\expandafter\def\csname v@s3/ts-lr1e4/d-mae\endcsname{0.1}
\expandafter\def\csname v@s3/ts-lr1e4/d-w20\endcsname{0.4}
\expandafter\def\csname v@s3/ts-lr1e4/dev-mae\endcsname{13.9}
\expandafter\def\csname v@s3/ts-lr1e4/dev-w20\endcsname{84.6}
\expandafter\def\csname v@s3/ts-lr1e4/ifa/mae\endcsname{14.8}
\expandafter\def\csname v@s3/ts-lr1e4/ifa/w20\endcsname{78.9}
\expandafter\def\csname v@s3/ts-lr1e4/long/mae\endcsname{10.8}
\expandafter\def\csname v@s3/ts-lr1e4/long/w20\endcsname{88.6}
\expandafter\def\csname v@s3/ts-lr1e4/mean-mae\endcsname{14.14}
\expandafter\def\csname v@s3/ts-lr1e4/mean-w20\endcsname{84.51}
\expandafter\def\csname v@s3/ts-lr1e4/params\endcsname{58}
\expandafter\def\csname v@s3/ts-lr1e4/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s3/ts-lr1e4/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s3/ts-lr1e4/swb/mae\endcsname{22.9}
\expandafter\def\csname v@s3/ts-lr1e4/swb/w20\endcsname{80.8}
\expandafter\def\csname v@s3/ts-lr1e4/timit-codecs/mae\endcsname{11.7}
\expandafter\def\csname v@s3/ts-lr1e4/timit-codecs/w20\endcsname{87.0}
\expandafter\def\csname v@s3/ts-lr1e4/timit/mae\endcsname{10.9}
\expandafter\def\csname v@s3/ts-lr1e4/timit/w20\endcsname{88.3}
\expandafter\def\csname v@s3/ts-lr1e4/vox/mae\endcsname{16.0}
\expandafter\def\csname v@s3/ts-lr1e4/vox/w20\endcsname{79.8}
\expandafter\def\csname v@s3/ts-lr1e4/z-mae\endcsname{1.2}
\expandafter\def\csname v@s3/ts-lr1e4/z-w20\endcsname{3.6}
\expandafter\def\csname v@s3/ts-lr5e4/buckeye-codecs/mae\endcsname{13.2}
\expandafter\def\csname v@s3/ts-lr5e4/buckeye-codecs/w20\endcsname{85.1}
\expandafter\def\csname v@s3/ts-lr5e4/buckeye/mae\endcsname{12.1}
\expandafter\def\csname v@s3/ts-lr5e4/buckeye/w20\endcsname{86.5}
\expandafter\def\csname v@s3/ts-lr5e4/d-mae\endcsname{0.0}
\expandafter\def\csname v@s3/ts-lr5e4/d-w20\endcsname{0.1}
\expandafter\def\csname v@s3/ts-lr5e4/dev-mae\endcsname{13.5}
\expandafter\def\csname v@s3/ts-lr5e4/dev-w20\endcsname{84.7}
\expandafter\def\csname v@s3/ts-lr5e4/ifa/mae\endcsname{14.9}
\expandafter\def\csname v@s3/ts-lr5e4/ifa/w20\endcsname{78.7}
\expandafter\def\csname v@s3/ts-lr5e4/long/mae\endcsname{10.0}
\expandafter\def\csname v@s3/ts-lr5e4/long/w20\endcsname{90.0}
\expandafter\def\csname v@s3/ts-lr5e4/mean-mae\endcsname{14.04}
\expandafter\def\csname v@s3/ts-lr5e4/mean-w20\endcsname{85.00}
\expandafter\def\csname v@s3/ts-lr5e4/params\endcsname{58}
\expandafter\def\csname v@s3/ts-lr5e4/seoul/mae\endcsname{11.6}
\expandafter\def\csname v@s3/ts-lr5e4/seoul/w20\endcsname{89.7}
\expandafter\def\csname v@s3/ts-lr5e4/swb/mae\endcsname{24.0}
\expandafter\def\csname v@s3/ts-lr5e4/swb/w20\endcsname{80.6}
\expandafter\def\csname v@s3/ts-lr5e4/timit-codecs/mae\endcsname{10.7}
\expandafter\def\csname v@s3/ts-lr5e4/timit-codecs/w20\endcsname{88.8}
\expandafter\def\csname v@s3/ts-lr5e4/timit/mae\endcsname{10.1}
\expandafter\def\csname v@s3/ts-lr5e4/timit/w20\endcsname{89.9}
\expandafter\def\csname v@s3/ts-lr5e4/vox/mae\endcsname{15.7}
\expandafter\def\csname v@s3/ts-lr5e4/vox/w20\endcsname{79.6}
\expandafter\def\csname v@s3/ts-lr5e4/z-mae\endcsname{0.3}
\expandafter\def\csname v@s3/ts-lr5e4/z-w20\endcsname{0.8}
\expandafter\def\csname v@s3/ts-r128/buckeye-codecs/mae\endcsname{12.9}
\expandafter\def\csname v@s3/ts-r128/buckeye-codecs/w20\endcsname{84.9}
\expandafter\def\csname v@s3/ts-r128/buckeye/mae\endcsname{12.2}
\expandafter\def\csname v@s3/ts-r128/buckeye/w20\endcsname{86.3}
\expandafter\def\csname v@s3/ts-r128/d-mae\endcsname{0.0}
\expandafter\def\csname v@s3/ts-r128/d-w20\endcsname{0.0}
\expandafter\def\csname v@s3/ts-r128/dev-mae\endcsname{13.6}
\expandafter\def\csname v@s3/ts-r128/dev-w20\endcsname{85.1}
\expandafter\def\csname v@s3/ts-r128/ifa/mae\endcsname{15.0}
\expandafter\def\csname v@s3/ts-r128/ifa/w20\endcsname{78.0}
\expandafter\def\csname v@s3/ts-r128/long/mae\endcsname{10.1}
\expandafter\def\csname v@s3/ts-r128/long/w20\endcsname{89.8}
\expandafter\def\csname v@s3/ts-r128/mean-mae\endcsname{13.97}
\expandafter\def\csname v@s3/ts-r128/mean-w20\endcsname{84.87}
\expandafter\def\csname v@s3/ts-r128/params\endcsname{231}
\expandafter\def\csname v@s3/ts-r128/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s3/ts-r128/seoul/w20\endcsname{89.7}
\expandafter\def\csname v@s3/ts-r128/swb/mae\endcsname{23.9}
\expandafter\def\csname v@s3/ts-r128/swb/w20\endcsname{80.1}
\expandafter\def\csname v@s3/ts-r128/timit-codecs/mae\endcsname{10.8}
\expandafter\def\csname v@s3/ts-r128/timit-codecs/w20\endcsname{88.7}
\expandafter\def\csname v@s3/ts-r128/timit/mae\endcsname{10.2}
\expandafter\def\csname v@s3/ts-r128/timit/w20\endcsname{89.8}
\expandafter\def\csname v@s3/ts-r128/vox/mae\endcsname{15.1}
\expandafter\def\csname v@s3/ts-r128/vox/w20\endcsname{80.3}
\expandafter\def\csname v@s3/ts-r128/z-mae\endcsname{0.3}
\expandafter\def\csname v@s3/ts-r128/z-w20\endcsname{0.4}
\expandafter\def\csname v@s3/ts-r16/buckeye-codecs/mae\endcsname{12.8}
\expandafter\def\csname v@s3/ts-r16/buckeye-codecs/w20\endcsname{84.6}
\expandafter\def\csname v@s3/ts-r16/buckeye/mae\endcsname{12.1}
\expandafter\def\csname v@s3/ts-r16/buckeye/w20\endcsname{85.6}
\expandafter\def\csname v@s3/ts-r16/d-mae\endcsname{0.1}
\expandafter\def\csname v@s3/ts-r16/d-w20\endcsname{0.2}
\expandafter\def\csname v@s3/ts-r16/dev-mae\endcsname{13.5}
\expandafter\def\csname v@s3/ts-r16/dev-w20\endcsname{84.5}
\expandafter\def\csname v@s3/ts-r16/ifa/mae\endcsname{14.8}
\expandafter\def\csname v@s3/ts-r16/ifa/w20\endcsname{78.9}
\expandafter\def\csname v@s3/ts-r16/long/mae\endcsname{10.5}
\expandafter\def\csname v@s3/ts-r16/long/w20\endcsname{89.2}
\expandafter\def\csname v@s3/ts-r16/mean-mae\endcsname{14.08}
\expandafter\def\csname v@s3/ts-r16/mean-w20\endcsname{84.73}
\expandafter\def\csname v@s3/ts-r16/params\endcsname{29}
\expandafter\def\csname v@s3/ts-r16/seoul/mae\endcsname{11.3}
\expandafter\def\csname v@s3/ts-r16/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s3/ts-r16/swb/mae\endcsname{23.1}
\expandafter\def\csname v@s3/ts-r16/swb/w20\endcsname{80.9}
\expandafter\def\csname v@s3/ts-r16/timit-codecs/mae\endcsname{11.4}
\expandafter\def\csname v@s3/ts-r16/timit-codecs/w20\endcsname{87.5}
\expandafter\def\csname v@s3/ts-r16/timit/mae\endcsname{10.8}
\expandafter\def\csname v@s3/ts-r16/timit/w20\endcsname{88.7}
\expandafter\def\csname v@s3/ts-r16/vox/mae\endcsname{16.0}
\expandafter\def\csname v@s3/ts-r16/vox/w20\endcsname{80.0}
\expandafter\def\csname v@s3/ts-r16/z-mae\endcsname{0.7}
\expandafter\def\csname v@s3/ts-r16/z-w20\endcsname{1.6}
\expandafter\def\csname v@s3/ts-r64/buckeye-codecs/mae\endcsname{12.9}
\expandafter\def\csname v@s3/ts-r64/buckeye-codecs/w20\endcsname{84.8}
\expandafter\def\csname v@s3/ts-r64/buckeye/mae\endcsname{12.3}
\expandafter\def\csname v@s3/ts-r64/buckeye/w20\endcsname{85.6}
\expandafter\def\csname v@s3/ts-r64/d-mae\endcsname{0.1}
\expandafter\def\csname v@s3/ts-r64/d-w20\endcsname{0.2}
\expandafter\def\csname v@s3/ts-r64/dev-mae\endcsname{13.1}
\expandafter\def\csname v@s3/ts-r64/dev-w20\endcsname{85.0}
\expandafter\def\csname v@s3/ts-r64/ifa/mae\endcsname{15.0}
\expandafter\def\csname v@s3/ts-r64/ifa/w20\endcsname{78.1}
\expandafter\def\csname v@s3/ts-r64/long/mae\endcsname{10.1}
\expandafter\def\csname v@s3/ts-r64/long/w20\endcsname{89.7}
\expandafter\def\csname v@s3/ts-r64/mean-mae\endcsname{14.13}
\expandafter\def\csname v@s3/ts-r64/mean-w20\endcsname{84.75}
\expandafter\def\csname v@s3/ts-r64/params\endcsname{115}
\expandafter\def\csname v@s3/ts-r64/seoul/mae\endcsname{11.1}
\expandafter\def\csname v@s3/ts-r64/seoul/w20\endcsname{89.9}
\expandafter\def\csname v@s3/ts-r64/swb/mae\endcsname{24.8}
\expandafter\def\csname v@s3/ts-r64/swb/w20\endcsname{80.2}
\expandafter\def\csname v@s3/ts-r64/timit-codecs/mae\endcsname{10.9}
\expandafter\def\csname v@s3/ts-r64/timit-codecs/w20\endcsname{88.4}
\expandafter\def\csname v@s3/ts-r64/timit/mae\endcsname{10.3}
\expandafter\def\csname v@s3/ts-r64/timit/w20\endcsname{89.5}
\expandafter\def\csname v@s3/ts-r64/vox/mae\endcsname{15.3}
\expandafter\def\csname v@s3/ts-r64/vox/w20\endcsname{80.3}
\expandafter\def\csname v@s3/ts-r64/z-mae\endcsname{1.1}
\expandafter\def\csname v@s3/ts-r64/z-w20\endcsname{1.4}
\expandafter\def\csname v@s3/ts-r8/buckeye-codecs/mae\endcsname{13.2}
\expandafter\def\csname v@s3/ts-r8/buckeye-codecs/w20\endcsname{84.4}
\expandafter\def\csname v@s3/ts-r8/buckeye/mae\endcsname{12.3}
\expandafter\def\csname v@s3/ts-r8/buckeye/w20\endcsname{85.3}
\expandafter\def\csname v@s3/ts-r8/d-mae\endcsname{0.2}
\expandafter\def\csname v@s3/ts-r8/d-w20\endcsname{0.5}
\expandafter\def\csname v@s3/ts-r8/dev-mae\endcsname{13.9}
\expandafter\def\csname v@s3/ts-r8/dev-w20\endcsname{84.6}
\expandafter\def\csname v@s3/ts-r8/ifa/mae\endcsname{14.7}
\expandafter\def\csname v@s3/ts-r8/ifa/w20\endcsname{78.6}
\expandafter\def\csname v@s3/ts-r8/long/mae\endcsname{10.8}
\expandafter\def\csname v@s3/ts-r8/long/w20\endcsname{88.7}
\expandafter\def\csname v@s3/ts-r8/mean-mae\endcsname{14.19}
\expandafter\def\csname v@s3/ts-r8/mean-w20\endcsname{84.44}
\expandafter\def\csname v@s3/ts-r8/params\endcsname{14}
\expandafter\def\csname v@s3/ts-r8/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s3/ts-r8/seoul/w20\endcsname{89.9}
\expandafter\def\csname v@s3/ts-r8/swb/mae\endcsname{22.6}
\expandafter\def\csname v@s3/ts-r8/swb/w20\endcsname{81.0}
\expandafter\def\csname v@s3/ts-r8/timit-codecs/mae\endcsname{11.8}
\expandafter\def\csname v@s3/ts-r8/timit-codecs/w20\endcsname{86.9}
\expandafter\def\csname v@s3/ts-r8/timit/mae\endcsname{11.0}
\expandafter\def\csname v@s3/ts-r8/timit/w20\endcsname{88.3}
\expandafter\def\csname v@s3/ts-r8/vox/mae\endcsname{16.6}
\expandafter\def\csname v@s3/ts-r8/vox/w20\endcsname{79.2}
\expandafter\def\csname v@s3/ts-r8/z-mae\endcsname{1.6}
\expandafter\def\csname v@s3/ts-r8/z-w20\endcsname{4.3}
\expandafter\def\csname v@s3/ts-seed1/buckeye-codecs/mae\endcsname{12.9}
\expandafter\def\csname v@s3/ts-seed1/buckeye-codecs/w20\endcsname{84.9}
\expandafter\def\csname v@s3/ts-seed1/buckeye/mae\endcsname{12.1}
\expandafter\def\csname v@s3/ts-seed1/buckeye/w20\endcsname{86.2}
\expandafter\def\csname v@s3/ts-seed1/d-mae\endcsname{0.1}
\expandafter\def\csname v@s3/ts-seed1/d-w20\endcsname{0.0}
\expandafter\def\csname v@s3/ts-seed1/dev-mae\endcsname{13.6}
\expandafter\def\csname v@s3/ts-seed1/dev-w20\endcsname{84.7}
\expandafter\def\csname v@s3/ts-seed1/ifa/mae\endcsname{15.3}
\expandafter\def\csname v@s3/ts-seed1/ifa/w20\endcsname{78.7}
\expandafter\def\csname v@s3/ts-seed1/long/mae\endcsname{10.5}
\expandafter\def\csname v@s3/ts-seed1/long/w20\endcsname{89.6}
\expandafter\def\csname v@s3/ts-seed1/mean-mae\endcsname{14.15}
\expandafter\def\csname v@s3/ts-seed1/mean-w20\endcsname{84.91}
\expandafter\def\csname v@s3/ts-seed1/params\endcsname{58}
\expandafter\def\csname v@s3/ts-seed1/seoul/mae\endcsname{11.5}
\expandafter\def\csname v@s3/ts-seed1/seoul/w20\endcsname{89.9}
\expandafter\def\csname v@s3/ts-seed1/swb/mae\endcsname{23.6}
\expandafter\def\csname v@s3/ts-seed1/swb/w20\endcsname{80.4}
\expandafter\def\csname v@s3/ts-seed1/timit-codecs/mae\endcsname{11.2}
\expandafter\def\csname v@s3/ts-seed1/timit-codecs/w20\endcsname{88.0}
\expandafter\def\csname v@s3/ts-seed1/timit/mae\endcsname{10.5}
\expandafter\def\csname v@s3/ts-seed1/timit/w20\endcsname{89.3}
\expandafter\def\csname v@s3/ts-seed1/vox/mae\endcsname{15.5}
\expandafter\def\csname v@s3/ts-seed1/vox/w20\endcsname{80.3}
\expandafter\def\csname v@s3/ts-seed1/z-mae\endcsname{1.2}
\expandafter\def\csname v@s3/ts-seed1/z-w20\endcsname{0.0}
\expandafter\def\csname v@s3/ts-seed2/buckeye-codecs/mae\endcsname{13.0}
\expandafter\def\csname v@s3/ts-seed2/buckeye-codecs/w20\endcsname{85.1}
\expandafter\def\csname v@s3/ts-seed2/buckeye/mae\endcsname{12.2}
\expandafter\def\csname v@s3/ts-seed2/buckeye/w20\endcsname{86.1}
\expandafter\def\csname v@s3/ts-seed2/d-mae\endcsname{0.0}
\expandafter\def\csname v@s3/ts-seed2/d-w20\endcsname{0.2}
\expandafter\def\csname v@s3/ts-seed2/dev-mae\endcsname{13.2}
\expandafter\def\csname v@s3/ts-seed2/dev-w20\endcsname{85.3}
\expandafter\def\csname v@s3/ts-seed2/ifa/mae\endcsname{14.9}
\expandafter\def\csname v@s3/ts-seed2/ifa/w20\endcsname{78.7}
\expandafter\def\csname v@s3/ts-seed2/long/mae\endcsname{10.2}
\expandafter\def\csname v@s3/ts-seed2/long/w20\endcsname{89.5}
\expandafter\def\csname v@s3/ts-seed2/mean-mae\endcsname{13.97}
\expandafter\def\csname v@s3/ts-seed2/mean-w20\endcsname{85.07}
\expandafter\def\csname v@s3/ts-seed2/params\endcsname{58}
\expandafter\def\csname v@s3/ts-seed2/seoul/mae\endcsname{11.5}
\expandafter\def\csname v@s3/ts-seed2/seoul/w20\endcsname{89.9}
\expandafter\def\csname v@s3/ts-seed2/swb/mae\endcsname{23.2}
\expandafter\def\csname v@s3/ts-seed2/swb/w20\endcsname{80.9}
\expandafter\def\csname v@s3/ts-seed2/timit-codecs/mae\endcsname{11.2}
\expandafter\def\csname v@s3/ts-seed2/timit-codecs/w20\endcsname{88.0}
\expandafter\def\csname v@s3/ts-seed2/timit/mae\endcsname{10.5}
\expandafter\def\csname v@s3/ts-seed2/timit/w20\endcsname{89.2}
\expandafter\def\csname v@s3/ts-seed2/vox/mae\endcsname{15.3}
\expandafter\def\csname v@s3/ts-seed2/vox/w20\endcsname{81.1}
\expandafter\def\csname v@s3/ts-seed2/z-mae\endcsname{0.2}
\expandafter\def\csname v@s3/ts-seed2/z-w20\endcsname{1.4}
\expandafter\def\csname v@s3/ts-seed3/buckeye-codecs/mae\endcsname{12.7}
\expandafter\def\csname v@s3/ts-seed3/buckeye-codecs/w20\endcsname{85.2}
\expandafter\def\csname v@s3/ts-seed3/buckeye/mae\endcsname{11.9}
\expandafter\def\csname v@s3/ts-seed3/buckeye/w20\endcsname{86.6}
\expandafter\def\csname v@s3/ts-seed3/d-mae\endcsname{0.2}
\expandafter\def\csname v@s3/ts-seed3/d-w20\endcsname{0.1}
\expandafter\def\csname v@s3/ts-seed3/dev-mae\endcsname{13.5}
\expandafter\def\csname v@s3/ts-seed3/dev-w20\endcsname{84.7}
\expandafter\def\csname v@s3/ts-seed3/ifa/mae\endcsname{14.9}
\expandafter\def\csname v@s3/ts-seed3/ifa/w20\endcsname{78.4}
\expandafter\def\csname v@s3/ts-seed3/long/mae\endcsname{10.2}
\expandafter\def\csname v@s3/ts-seed3/long/w20\endcsname{89.4}
\expandafter\def\csname v@s3/ts-seed3/mean-mae\endcsname{13.82}
\expandafter\def\csname v@s3/ts-seed3/mean-w20\endcsname{84.97}
\expandafter\def\csname v@s3/ts-seed3/params\endcsname{58}
\expandafter\def\csname v@s3/ts-seed3/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s3/ts-seed3/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s3/ts-seed3/swb/mae\endcsname{23.1}
\expandafter\def\csname v@s3/ts-seed3/swb/w20\endcsname{80.9}
\expandafter\def\csname v@s3/ts-seed3/timit-codecs/mae\endcsname{11.1}
\expandafter\def\csname v@s3/ts-seed3/timit-codecs/w20\endcsname{88.1}
\expandafter\def\csname v@s3/ts-seed3/timit/mae\endcsname{10.4}
\expandafter\def\csname v@s3/ts-seed3/timit/w20\endcsname{89.2}
\expandafter\def\csname v@s3/ts-seed3/vox/mae\endcsname{14.8}
\expandafter\def\csname v@s3/ts-seed3/vox/w20\endcsname{80.4}
\expandafter\def\csname v@s3/ts-seed3/z-mae\endcsname{1.5}
\expandafter\def\csname v@s3/ts-seed3/z-w20\endcsname{0.5}
\expandafter\def\csname v@s3/ts-seed4/buckeye-codecs/mae\endcsname{12.7}
\expandafter\def\csname v@s3/ts-seed4/buckeye-codecs/w20\endcsname{84.7}
\expandafter\def\csname v@s3/ts-seed4/buckeye/mae\endcsname{12.0}
\expandafter\def\csname v@s3/ts-seed4/buckeye/w20\endcsname{85.9}
\expandafter\def\csname v@s3/ts-seed4/d-mae\endcsname{0.0}
\expandafter\def\csname v@s3/ts-seed4/d-w20\endcsname{0.1}
\expandafter\def\csname v@s3/ts-seed4/dev-mae\endcsname{13.2}
\expandafter\def\csname v@s3/ts-seed4/dev-w20\endcsname{84.5}
\expandafter\def\csname v@s3/ts-seed4/ifa/mae\endcsname{15.5}
\expandafter\def\csname v@s3/ts-seed4/ifa/w20\endcsname{78.5}
\expandafter\def\csname v@s3/ts-seed4/long/mae\endcsname{10.2}
\expandafter\def\csname v@s3/ts-seed4/long/w20\endcsname{89.4}
\expandafter\def\csname v@s3/ts-seed4/mean-mae\endcsname{14.00}
\expandafter\def\csname v@s3/ts-seed4/mean-w20\endcsname{84.80}
\expandafter\def\csname v@s3/ts-seed4/params\endcsname{58}
\expandafter\def\csname v@s3/ts-seed4/seoul/mae\endcsname{11.5}
\expandafter\def\csname v@s3/ts-seed4/seoul/w20\endcsname{89.9}
\expandafter\def\csname v@s3/ts-seed4/swb/mae\endcsname{23.1}
\expandafter\def\csname v@s3/ts-seed4/swb/w20\endcsname{80.8}
\expandafter\def\csname v@s3/ts-seed4/timit-codecs/mae\endcsname{11.3}
\expandafter\def\csname v@s3/ts-seed4/timit-codecs/w20\endcsname{87.8}
\expandafter\def\csname v@s3/ts-seed4/timit/mae\endcsname{10.6}
\expandafter\def\csname v@s3/ts-seed4/timit/w20\endcsname{88.9}
\expandafter\def\csname v@s3/ts-seed4/vox/mae\endcsname{15.1}
\expandafter\def\csname v@s3/ts-seed4/vox/w20\endcsname{80.2}
\expandafter\def\csname v@s3/ts-seed4/z-mae\endcsname{0.0}
\expandafter\def\csname v@s3/ts-seed4/z-w20\endcsname{1.0}
\expandafter\def\csname v@s3/weaker/mean-hi\endcsname{14.44}
\expandafter\def\csname v@s3/weaker/mean-lo\endcsname{14.11}
\expandafter\def\csname v@s3/weaker/params-hi\endcsname{58}
\expandafter\def\csname v@s3/weaker/params-lo\endcsname{14}
\expandafter\def\csname v@s3/weaker/swb/hi\endcsname{22.9}
\expandafter\def\csname v@s3/weaker/swb/lo\endcsname{22.2}
\expandafter\def\csname v@s3/weaker/timit-codecs/hi\endcsname{12.3}
\expandafter\def\csname v@s3/weaker/timit-codecs/lo\endcsname{11.7}
\expandafter\def\csname v@s3/weaker/timit/hi\endcsname{11.5}
\expandafter\def\csname v@s3/weaker/timit/lo\endcsname{10.9}
\expandafter\def\csname v@s4/aux/none/mean-mae\endcsname{14.00}
\expandafter\def\csname v@s4/aux/none/mean-w20\endcsname{84.91}
\expandafter\def\csname v@s4/aux/none/runs\endcsname{5}
\expandafter\def\csname v@s4/aux/word/d-mae\endcsname{$+0.15$}
\expandafter\def\csname v@s4/aux/word/d-w20\endcsname{$-0.12$}
\expandafter\def\csname v@s4/aux/word/mean-mae\endcsname{14.15}
\expandafter\def\csname v@s4/aux/word/mean-w20\endcsname{84.79}
\expandafter\def\csname v@s4/aux/word/runs\endcsname{2}
\expandafter\def\csname v@s4/aux/word/se-mae\endcsname{0.10}
\expandafter\def\csname v@s4/aux/word/se-w20\endcsname{0.06}
\expandafter\def\csname v@s4/aux/wordphone/d-mae\endcsname{$+0.01$}
\expandafter\def\csname v@s4/aux/wordphone/d-w20\endcsname{$+0.04$}
\expandafter\def\csname v@s4/aux/wordphone/mean-mae\endcsname{14.01}
\expandafter\def\csname v@s4/aux/wordphone/mean-w20\endcsname{84.96}
\expandafter\def\csname v@s4/aux/wordphone/runs\endcsname{2}
\expandafter\def\csname v@s4/aux/wordphone/se-mae\endcsname{0.06}
\expandafter\def\csname v@s4/aux/wordphone/se-w20\endcsname{0.06}
\expandafter\def\csname v@s4/dec/argmax/mae\endcsname{15.5}
\expandafter\def\csname v@s4/dec/argmax/median\endcsname{8.4}
\expandafter\def\csname v@s4/dec/argmax/w10\endcsname{58.4}
\expandafter\def\csname v@s4/dec/argmax/w20\endcsname{82.5}
\expandafter\def\csname v@s4/dec/full/mae\endcsname{17.0}
\expandafter\def\csname v@s4/dec/full/median\endcsname{9.5}
\expandafter\def\csname v@s4/dec/full/w10\endcsname{52.6}
\expandafter\def\csname v@s4/dec/full/w20\endcsname{76.1}
\expandafter\def\csname v@s4/dec/grid-cost/mae\endcsname{1.5}
\expandafter\def\csname v@s4/dec/grid-cost/median\endcsname{1.9}
\expandafter\def\csname v@s4/dec/grid-cost/w10\endcsname{7.7}
\expandafter\def\csname v@s4/dec/grid-cost/w20\endcsname{2.3}
\expandafter\def\csname v@s4/dec/r1/mae\endcsname{14.1}
\expandafter\def\csname v@s4/dec/r1/median\endcsname{6.3}
\expandafter\def\csname v@s4/dec/r1/w10\endcsname{66.7}
\expandafter\def\csname v@s4/dec/r1/w20\endcsname{84.7}
\expandafter\def\csname v@s4/dec/r2/mae\endcsname{14.1}
\expandafter\def\csname v@s4/dec/r2/median\endcsname{6.5}
\expandafter\def\csname v@s4/dec/r2/w10\endcsname{66.1}
\expandafter\def\csname v@s4/dec/r2/w20\endcsname{84.8}
\expandafter\def\csname v@s4/dec/r5/mae\endcsname{14.1}
\expandafter\def\csname v@s4/dec/r5/median\endcsname{6.8}
\expandafter\def\csname v@s4/dec/r5/w10\endcsname{64.2}
\expandafter\def\csname v@s4/dec/r5/w20\endcsname{83.7}
\expandafter\def\csname v@s5/augamr/buckeye/amrnb\endcsname{13.0}
\expandafter\def\csname v@s5/augamr/buckeye/amrnb-hi\endcsname{13.0}
\expandafter\def\csname v@s5/augamr/buckeye/amrnb-lo\endcsname{12.9}
\expandafter\def\csname v@s5/augamr/buckeye/clean\endcsname{12.0}
\expandafter\def\csname v@s5/augamr/buckeye/g711u\endcsname{12.5}
\expandafter\def\csname v@s5/augamr/buckeye/g723\endcsname{13.4}
\expandafter\def\csname v@s5/augamr/buckeye/gsm\endcsname{13.0}
\expandafter\def\csname v@s5/augamr/buckeye/opus\endcsname{12.8}
\expandafter\def\csname v@s5/augamr/timit/amrnb\endcsname{12.6}
\expandafter\def\csname v@s5/augamr/timit/amrnb-hi\endcsname{12.6}
\expandafter\def\csname v@s5/augamr/timit/amrnb-lo\endcsname{12.6}
\expandafter\def\csname v@s5/augamr/timit/clean\endcsname{10.4}
\expandafter\def\csname v@s5/augamr/timit/codec-hi\endcsname{11.6}
\expandafter\def\csname v@s5/augamr/timit/codec-lo\endcsname{11.0}
\expandafter\def\csname v@s5/augamr/timit/cost-hi\endcsname{1.1}
\expandafter\def\csname v@s5/augamr/timit/cost-lo\endcsname{0.5}
\expandafter\def\csname v@s5/augamr/timit/cost-pct\endcsname{8}
\expandafter\def\csname v@s5/augamr/timit/g711u\endcsname{11.0}
\expandafter\def\csname v@s5/augamr/timit/g723\endcsname{11.4}
\expandafter\def\csname v@s5/augamr/timit/g726\endcsname{11.4}
\expandafter\def\csname v@s5/augamr/timit/gsm\endcsname{11.6}
\expandafter\def\csname v@s5/augamr/timit/mp3\endcsname{11.5}
\expandafter\def\csname v@s5/augamr/timit/opus\endcsname{11.1}
\expandafter\def\csname v@s5/augamr/timit/pcm\endcsname{11.0}
\expandafter\def\csname v@s5/augamr/timit/pcm-cost\endcsname{0.5}
\expandafter\def\csname v@s5/diff/buckeye-clean/mae\endcsname{$-0.2$}
\expandafter\def\csname v@s5/diff/buckeye-clean/mae-abs\endcsname{0.2}
\expandafter\def\csname v@s5/diff/buckeye-clean/mae-se\endcsname{0.06}
\expandafter\def\csname v@s5/diff/buckeye-clean/w20\endcsname{0.6}
\expandafter\def\csname v@s5/diff/buckeye-clean/w20-abs\endcsname{0.6}
\expandafter\def\csname v@s5/diff/buckeye-clean/w20-se\endcsname{0.24}
\expandafter\def\csname v@s5/diff/buckeye-seen/mae\endcsname{$-2.6$}
\expandafter\def\csname v@s5/diff/buckeye-seen/mae-abs\endcsname{2.6}
\expandafter\def\csname v@s5/diff/buckeye-seen/mae-se\endcsname{0.19}
\expandafter\def\csname v@s5/diff/buckeye-seen/w20\endcsname{3.7}
\expandafter\def\csname v@s5/diff/buckeye-seen/w20-abs\endcsname{3.7}
\expandafter\def\csname v@s5/diff/buckeye-seen/w20-se\endcsname{0.43}
\expandafter\def\csname v@s5/diff/buckeye-unseen/mae\endcsname{$-2.6$}
\expandafter\def\csname v@s5/diff/buckeye-unseen/mae-abs\endcsname{2.6}
\expandafter\def\csname v@s5/diff/buckeye-unseen/mae-se\endcsname{0.18}
\expandafter\def\csname v@s5/diff/buckeye-unseen/w20\endcsname{3.8}
\expandafter\def\csname v@s5/diff/buckeye-unseen/w20-abs\endcsname{3.8}
\expandafter\def\csname v@s5/diff/buckeye-unseen/w20-se\endcsname{0.30}
\expandafter\def\csname v@s5/diff/clean/mae\endcsname{$-0.1$}
\expandafter\def\csname v@s5/diff/clean/mae-abs\endcsname{0.1}
\expandafter\def\csname v@s5/diff/clean/mae-se\endcsname{0.07}
\expandafter\def\csname v@s5/diff/clean/w20\endcsname{0.2}
\expandafter\def\csname v@s5/diff/clean/w20-abs\endcsname{0.2}
\expandafter\def\csname v@s5/diff/clean/w20-se\endcsname{0.07}
\expandafter\def\csname v@s5/diff/ifa/mae\endcsname{$-0.3$}
\expandafter\def\csname v@s5/diff/ifa/mae-abs\endcsname{0.3}
\expandafter\def\csname v@s5/diff/ifa/mae-se\endcsname{0.25}
\expandafter\def\csname v@s5/diff/ifa/w20\endcsname{0.7}
\expandafter\def\csname v@s5/diff/ifa/w20-abs\endcsname{0.7}
\expandafter\def\csname v@s5/diff/ifa/w20-se\endcsname{0.13}
\expandafter\def\csname v@s5/diff/long-clean/mae\endcsname{0.0}
\expandafter\def\csname v@s5/diff/long-clean/mae-abs\endcsname{0.0}
\expandafter\def\csname v@s5/diff/long-clean/mae-se\endcsname{0.09}
\expandafter\def\csname v@s5/diff/long-clean/w20\endcsname{$-0.1$}
\expandafter\def\csname v@s5/diff/long-clean/w20-abs\endcsname{0.1}
\expandafter\def\csname v@s5/diff/long-clean/w20-se\endcsname{0.10}
\expandafter\def\csname v@s5/diff/long-g711/mae\endcsname{$-5.2$}
\expandafter\def\csname v@s5/diff/long-g711/mae-abs\endcsname{5.2}
\expandafter\def\csname v@s5/diff/long-g711/mae-se\endcsname{0.32}
\expandafter\def\csname v@s5/diff/long-g711/w20\endcsname{12.5}
\expandafter\def\csname v@s5/diff/long-g711/w20-abs\endcsname{12.5}
\expandafter\def\csname v@s5/diff/long-g711/w20-se\endcsname{0.72}
\expandafter\def\csname v@s5/diff/seen/mae\endcsname{$-4.6$}
\expandafter\def\csname v@s5/diff/seen/mae-abs\endcsname{4.6}
\expandafter\def\csname v@s5/diff/seen/mae-se\endcsname{0.29}
\expandafter\def\csname v@s5/diff/seen/w20\endcsname{9.8}
\expandafter\def\csname v@s5/diff/seen/w20-abs\endcsname{9.8}
\expandafter\def\csname v@s5/diff/seen/w20-se\endcsname{0.52}
\expandafter\def\csname v@s5/diff/seoul/mae\endcsname{$-0.1$}
\expandafter\def\csname v@s5/diff/seoul/mae-abs\endcsname{0.1}
\expandafter\def\csname v@s5/diff/seoul/mae-se\endcsname{0.08}
\expandafter\def\csname v@s5/diff/seoul/w20\endcsname{0.2}
\expandafter\def\csname v@s5/diff/seoul/w20-abs\endcsname{0.2}
\expandafter\def\csname v@s5/diff/seoul/w20-se\endcsname{0.06}
\expandafter\def\csname v@s5/diff/swb-col/mae\endcsname{$-1.3$}
\expandafter\def\csname v@s5/diff/swb-col/mae-abs\endcsname{1.3}
\expandafter\def\csname v@s5/diff/swb-col/mae-se\endcsname{0.42}
\expandafter\def\csname v@s5/diff/swb-col/w20\endcsname{0.8}
\expandafter\def\csname v@s5/diff/swb-col/w20-abs\endcsname{0.8}
\expandafter\def\csname v@s5/diff/swb-col/w20-se\endcsname{0.20}
\expandafter\def\csname v@s5/diff/swb/mae\endcsname{$-1.3$}
\expandafter\def\csname v@s5/diff/swb/mae-abs\endcsname{1.3}
\expandafter\def\csname v@s5/diff/swb/mae-se\endcsname{0.42}
\expandafter\def\csname v@s5/diff/swb/w20\endcsname{0.8}
\expandafter\def\csname v@s5/diff/swb/w20-abs\endcsname{0.8}
\expandafter\def\csname v@s5/diff/swb/w20-se\endcsname{0.20}
\expandafter\def\csname v@s5/diff/timit-clean/mae\endcsname{0.1}
\expandafter\def\csname v@s5/diff/timit-clean/mae-abs\endcsname{0.1}
\expandafter\def\csname v@s5/diff/timit-clean/mae-se\endcsname{0.05}
\expandafter\def\csname v@s5/diff/timit-clean/w20\endcsname{$-0.2$}
\expandafter\def\csname v@s5/diff/timit-clean/w20-abs\endcsname{0.2}
\expandafter\def\csname v@s5/diff/timit-clean/w20-se\endcsname{0.07}
\expandafter\def\csname v@s5/diff/timit-seen/mae\endcsname{$-6.0$}
\expandafter\def\csname v@s5/diff/timit-seen/mae-abs\endcsname{6.0}
\expandafter\def\csname v@s5/diff/timit-seen/mae-se\endcsname{0.41}
\expandafter\def\csname v@s5/diff/timit-seen/w20\endcsname{13.4}
\expandafter\def\csname v@s5/diff/timit-seen/w20-abs\endcsname{13.4}
\expandafter\def\csname v@s5/diff/timit-seen/w20-se\endcsname{0.53}
\expandafter\def\csname v@s5/diff/timit-unseen/mae\endcsname{$-5.4$}
\expandafter\def\csname v@s5/diff/timit-unseen/mae-abs\endcsname{5.4}
\expandafter\def\csname v@s5/diff/timit-unseen/mae-se\endcsname{0.30}
\expandafter\def\csname v@s5/diff/timit-unseen/w20\endcsname{12.7}
\expandafter\def\csname v@s5/diff/timit-unseen/w20-abs\endcsname{12.7}
\expandafter\def\csname v@s5/diff/timit-unseen/w20-se\endcsname{0.34}
\expandafter\def\csname v@s5/diff/unseen/mae\endcsname{$-4.0$}
\expandafter\def\csname v@s5/diff/unseen/mae-abs\endcsname{4.0}
\expandafter\def\csname v@s5/diff/unseen/mae-se\endcsname{0.21}
\expandafter\def\csname v@s5/diff/unseen/w20\endcsname{8.3}
\expandafter\def\csname v@s5/diff/unseen/w20-abs\endcsname{8.3}
\expandafter\def\csname v@s5/diff/unseen/w20-se\endcsname{0.24}
\expandafter\def\csname v@s5/diff/vox/mae\endcsname{0.1}
\expandafter\def\csname v@s5/diff/vox/mae-abs\endcsname{0.1}
\expandafter\def\csname v@s5/diff/vox/mae-se\endcsname{0.21}
\expandafter\def\csname v@s5/diff/vox/w20\endcsname{$-0.2$}
\expandafter\def\csname v@s5/diff/vox/w20-abs\endcsname{0.2}
\expandafter\def\csname v@s5/diff/vox/w20-se\endcsname{0.21}
\expandafter\def\csname v@s5/p0/buckeye-clean/mae\endcsname{12.3}
\expandafter\def\csname v@s5/p0/buckeye-clean/w20\endcsname{85.5}
\expandafter\def\csname v@s5/p0/buckeye-seen/mae\endcsname{15.4}
\expandafter\def\csname v@s5/p0/buckeye-seen/w20\endcsname{81.3}
\expandafter\def\csname v@s5/p0/buckeye-unseen/mae\endcsname{15.8}
\expandafter\def\csname v@s5/p0/buckeye-unseen/w20\endcsname{80.4}
\expandafter\def\csname v@s5/p0/buckeye/amrnb\endcsname{15.7}
\expandafter\def\csname v@s5/p0/buckeye/amrnb-hi\endcsname{16.0}
\expandafter\def\csname v@s5/p0/buckeye/amrnb-lo\endcsname{15.3}
\expandafter\def\csname v@s5/p0/buckeye/clean\endcsname{12.3}
\expandafter\def\csname v@s5/p0/buckeye/g711u\endcsname{14.9}
\expandafter\def\csname v@s5/p0/buckeye/g723\endcsname{15.9}
\expandafter\def\csname v@s5/p0/buckeye/gsm\endcsname{15.9}
\expandafter\def\csname v@s5/p0/buckeye/opus\endcsname{15.5}
\expandafter\def\csname v@s5/p0/clean/mae\endcsname{12.5}
\expandafter\def\csname v@s5/p0/clean/w20\endcsname{85.4}
\expandafter\def\csname v@s5/p0/ifa/mae\endcsname{15.5}
\expandafter\def\csname v@s5/p0/ifa/w20\endcsname{77.9}
\expandafter\def\csname v@s5/p0/long-clean/mae\endcsname{10.3}
\expandafter\def\csname v@s5/p0/long-clean/w20\endcsname{89.5}
\expandafter\def\csname v@s5/p0/long-g711/mae\endcsname{15.8}
\expandafter\def\csname v@s5/p0/long-g711/w20\endcsname{76.4}
\expandafter\def\csname v@s5/p0/seen/mae\endcsname{16.1}
\expandafter\def\csname v@s5/p0/seen/w20\endcsname{77.4}
\expandafter\def\csname v@s5/p0/seoul/mae\endcsname{11.5}
\expandafter\def\csname v@s5/p0/seoul/w20\endcsname{89.8}
\expandafter\def\csname v@s5/p0/swb-col/mae\endcsname{24.5}
\expandafter\def\csname v@s5/p0/swb-col/w20\endcsname{80.0}
\expandafter\def\csname v@s5/p0/swb/mae\endcsname{24.5}
\expandafter\def\csname v@s5/p0/swb/w20\endcsname{80.0}
\expandafter\def\csname v@s5/p0/timit-clean/mae\endcsname{10.4}
\expandafter\def\csname v@s5/p0/timit-clean/w20\endcsname{89.3}
\expandafter\def\csname v@s5/p0/timit-seen/mae\endcsname{17.1}
\expandafter\def\csname v@s5/p0/timit-seen/w20\endcsname{74.6}
\expandafter\def\csname v@s5/p0/timit-unseen/mae\endcsname{17.6}
\expandafter\def\csname v@s5/p0/timit-unseen/w20\endcsname{73.8}
\expandafter\def\csname v@s5/p0/timit/amrnb\endcsname{18.1}
\expandafter\def\csname v@s5/p0/timit/amrnb-hi\endcsname{18.5}
\expandafter\def\csname v@s5/p0/timit/amrnb-lo\endcsname{17.8}
\expandafter\def\csname v@s5/p0/timit/clean\endcsname{10.4}
\expandafter\def\csname v@s5/p0/timit/codec-hi\endcsname{17.8}
\expandafter\def\csname v@s5/p0/timit/codec-lo\endcsname{16.5}
\expandafter\def\csname v@s5/p0/timit/cost-hi\endcsname{7.4}
\expandafter\def\csname v@s5/p0/timit/cost-lo\endcsname{6.1}
\expandafter\def\csname v@s5/p0/timit/cost-pct\endcsname{65}
\expandafter\def\csname v@s5/p0/timit/g711u\endcsname{17.4}
\expandafter\def\csname v@s5/p0/timit/g723\endcsname{17.1}
\expandafter\def\csname v@s5/p0/timit/g726\endcsname{17.0}
\expandafter\def\csname v@s5/p0/timit/gsm\endcsname{17.8}
\expandafter\def\csname v@s5/p0/timit/mp3\endcsname{17.5}
\expandafter\def\csname v@s5/p0/timit/opus\endcsname{16.5}
\expandafter\def\csname v@s5/p0/timit/pcm\endcsname{16.5}
\expandafter\def\csname v@s5/p0/timit/pcm-cost\endcsname{6.1}
\expandafter\def\csname v@s5/p0/unseen/mae\endcsname{16.7}
\expandafter\def\csname v@s5/p0/unseen/w20\endcsname{77.1}
\expandafter\def\csname v@s5/p0/vox/mae\endcsname{15.2}
\expandafter\def\csname v@s5/p0/vox/w20\endcsname{80.7}
\expandafter\def\csname v@s5/p025/buckeye-clean/mae\endcsname{12.0}
\expandafter\def\csname v@s5/p025/buckeye-clean/w20\endcsname{85.8}
\expandafter\def\csname v@s5/p025/buckeye-seen/mae\endcsname{13.0}
\expandafter\def\csname v@s5/p025/buckeye-seen/w20\endcsname{84.8}
\expandafter\def\csname v@s5/p025/buckeye-unseen/mae\endcsname{13.3}
\expandafter\def\csname v@s5/p025/buckeye-unseen/w20\endcsname{84.1}
\expandafter\def\csname v@s5/p025/clean/mae\endcsname{12.4}
\expandafter\def\csname v@s5/p025/clean/w20\endcsname{85.6}
\expandafter\def\csname v@s5/p025/ifa/mae\endcsname{15.1}
\expandafter\def\csname v@s5/p025/ifa/w20\endcsname{78.1}
\expandafter\def\csname v@s5/p025/long-clean/mae\endcsname{10.2}
\expandafter\def\csname v@s5/p025/long-clean/w20\endcsname{89.6}
\expandafter\def\csname v@s5/p025/long-g711/mae\endcsname{10.5}
\expandafter\def\csname v@s5/p025/long-g711/w20\endcsname{88.9}
\expandafter\def\csname v@s5/p025/seen/mae\endcsname{11.6}
\expandafter\def\csname v@s5/p025/seen/w20\endcsname{87.2}
\expandafter\def\csname v@s5/p025/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s5/p025/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s5/p025/swb-col/mae\endcsname{23.3}
\expandafter\def\csname v@s5/p025/swb-col/w20\endcsname{80.5}
\expandafter\def\csname v@s5/p025/swb/mae\endcsname{23.3}
\expandafter\def\csname v@s5/p025/swb/w20\endcsname{80.5}
\expandafter\def\csname v@s5/p025/timit-clean/mae\endcsname{10.3}
\expandafter\def\csname v@s5/p025/timit-clean/w20\endcsname{89.4}
\expandafter\def\csname v@s5/p025/timit-seen/mae\endcsname{11.2}
\expandafter\def\csname v@s5/p025/timit-seen/w20\endcsname{87.8}
\expandafter\def\csname v@s5/p025/timit-unseen/mae\endcsname{12.3}
\expandafter\def\csname v@s5/p025/timit-unseen/w20\endcsname{86.3}
\expandafter\def\csname v@s5/p025/unseen/mae\endcsname{12.8}
\expandafter\def\csname v@s5/p025/unseen/w20\endcsname{85.2}
\expandafter\def\csname v@s5/p025/vox/mae\endcsname{15.4}
\expandafter\def\csname v@s5/p025/vox/w20\endcsname{80.6}
\expandafter\def\csname v@s5/p05/buckeye-clean/mae\endcsname{12.0}
\expandafter\def\csname v@s5/p05/buckeye-clean/w20\endcsname{86.1}
\expandafter\def\csname v@s5/p05/buckeye-seen/mae\endcsname{12.9}
\expandafter\def\csname v@s5/p05/buckeye-seen/w20\endcsname{84.9}
\expandafter\def\csname v@s5/p05/buckeye-unseen/mae\endcsname{13.2}
\expandafter\def\csname v@s5/p05/buckeye-unseen/w20\endcsname{84.3}
\expandafter\def\csname v@s5/p05/buckeye/amrnb\endcsname{13.0}
\expandafter\def\csname v@s5/p05/buckeye/amrnb-hi\endcsname{13.1}
\expandafter\def\csname v@s5/p05/buckeye/amrnb-lo\endcsname{12.8}
\expandafter\def\csname v@s5/p05/buckeye/clean\endcsname{12.0}
\expandafter\def\csname v@s5/p05/buckeye/g711u\endcsname{12.6}
\expandafter\def\csname v@s5/p05/buckeye/g723\endcsname{13.4}
\expandafter\def\csname v@s5/p05/buckeye/gsm\endcsname{13.1}
\expandafter\def\csname v@s5/p05/buckeye/opus\endcsname{12.8}
\expandafter\def\csname v@s5/p05/clean/mae\endcsname{12.5}
\expandafter\def\csname v@s5/p05/clean/w20\endcsname{85.6}
\expandafter\def\csname v@s5/p05/ifa/mae\endcsname{15.2}
\expandafter\def\csname v@s5/p05/ifa/w20\endcsname{78.5}
\expandafter\def\csname v@s5/p05/long-clean/mae\endcsname{10.3}
\expandafter\def\csname v@s5/p05/long-clean/w20\endcsname{89.5}
\expandafter\def\csname v@s5/p05/long-g711/mae\endcsname{10.6}
\expandafter\def\csname v@s5/p05/long-g711/w20\endcsname{88.9}
\expandafter\def\csname v@s5/p05/seen/mae\endcsname{11.5}
\expandafter\def\csname v@s5/p05/seen/w20\endcsname{87.2}
\expandafter\def\csname v@s5/p05/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s5/p05/seoul/w20\endcsname{89.9}
\expandafter\def\csname v@s5/p05/swb-col/mae\endcsname{23.2}
\expandafter\def\csname v@s5/p05/swb-col/w20\endcsname{80.8}
\expandafter\def\csname v@s5/p05/swb/mae\endcsname{23.2}
\expandafter\def\csname v@s5/p05/swb/w20\endcsname{80.8}
\expandafter\def\csname v@s5/p05/timit-clean/mae\endcsname{10.5}
\expandafter\def\csname v@s5/p05/timit-clean/w20\endcsname{89.1}
\expandafter\def\csname v@s5/p05/timit-seen/mae\endcsname{11.2}
\expandafter\def\csname v@s5/p05/timit-seen/w20\endcsname{88.0}
\expandafter\def\csname v@s5/p05/timit-unseen/mae\endcsname{12.2}
\expandafter\def\csname v@s5/p05/timit-unseen/w20\endcsname{86.4}
\expandafter\def\csname v@s5/p05/timit/amrnb\endcsname{12.9}
\expandafter\def\csname v@s5/p05/timit/amrnb-hi\endcsname{13.2}
\expandafter\def\csname v@s5/p05/timit/amrnb-lo\endcsname{12.7}
\expandafter\def\csname v@s5/p05/timit/clean\endcsname{10.5}
\expandafter\def\csname v@s5/p05/timit/codec-hi\endcsname{11.4}
\expandafter\def\csname v@s5/p05/timit/codec-lo\endcsname{10.9}
\expandafter\def\csname v@s5/p05/timit/cost-hi\endcsname{0.9}
\expandafter\def\csname v@s5/p05/timit/cost-lo\endcsname{0.4}
\expandafter\def\csname v@s5/p05/timit/cost-pct\endcsname{6}
\expandafter\def\csname v@s5/p05/timit/g711u\endcsname{11.0}
\expandafter\def\csname v@s5/p05/timit/g723\endcsname{11.4}
\expandafter\def\csname v@s5/p05/timit/g726\endcsname{11.2}
\expandafter\def\csname v@s5/p05/timit/gsm\endcsname{11.4}
\expandafter\def\csname v@s5/p05/timit/mp3\endcsname{11.4}
\expandafter\def\csname v@s5/p05/timit/opus\endcsname{11.1}
\expandafter\def\csname v@s5/p05/timit/pcm\endcsname{10.9}
\expandafter\def\csname v@s5/p05/timit/pcm-cost\endcsname{0.4}
\expandafter\def\csname v@s5/p05/unseen/mae\endcsname{12.7}
\expandafter\def\csname v@s5/p05/unseen/w20\endcsname{85.4}
\expandafter\def\csname v@s5/p05/vox/mae\endcsname{15.4}
\expandafter\def\csname v@s5/p05/vox/w20\endcsname{80.5}
\expandafter\def\csname v@s5/p075/buckeye-clean/mae\endcsname{12.2}
\expandafter\def\csname v@s5/p075/buckeye-clean/w20\endcsname{85.3}
\expandafter\def\csname v@s5/p075/buckeye-seen/mae\endcsname{13.1}
\expandafter\def\csname v@s5/p075/buckeye-seen/w20\endcsname{84.3}
\expandafter\def\csname v@s5/p075/buckeye-unseen/mae\endcsname{13.3}
\expandafter\def\csname v@s5/p075/buckeye-unseen/w20\endcsname{83.9}
\expandafter\def\csname v@s5/p075/clean/mae\endcsname{12.6}
\expandafter\def\csname v@s5/p075/clean/w20\endcsname{85.1}
\expandafter\def\csname v@s5/p075/ifa/mae\endcsname{14.7}
\expandafter\def\csname v@s5/p075/ifa/w20\endcsname{78.6}
\expandafter\def\csname v@s5/p075/long-clean/mae\endcsname{10.4}
\expandafter\def\csname v@s5/p075/long-clean/w20\endcsname{89.2}
\expandafter\def\csname v@s5/p075/long-g711/mae\endcsname{10.7}
\expandafter\def\csname v@s5/p075/long-g711/w20\endcsname{88.8}
\expandafter\def\csname v@s5/p075/seen/mae\endcsname{11.6}
\expandafter\def\csname v@s5/p075/seen/w20\endcsname{87.1}
\expandafter\def\csname v@s5/p075/seoul/mae\endcsname{11.4}
\expandafter\def\csname v@s5/p075/seoul/w20\endcsname{90.0}
\expandafter\def\csname v@s5/p075/swb-col/mae\endcsname{23.0}
\expandafter\def\csname v@s5/p075/swb-col/w20\endcsname{80.7}
\expandafter\def\csname v@s5/p075/swb/mae\endcsname{23.0}
\expandafter\def\csname v@s5/p075/swb/w20\endcsname{80.7}
\expandafter\def\csname v@s5/p075/timit-clean/mae\endcsname{10.6}
\expandafter\def\csname v@s5/p075/timit-clean/w20\endcsname{89.0}
\expandafter\def\csname v@s5/p075/timit-seen/mae\endcsname{11.0}
\expandafter\def\csname v@s5/p075/timit-seen/w20\endcsname{88.1}
\expandafter\def\csname v@s5/p075/timit-unseen/mae\endcsname{12.1}
\expandafter\def\csname v@s5/p075/timit-unseen/w20\endcsname{86.8}
\expandafter\def\csname v@s5/p075/unseen/mae\endcsname{12.7}
\expandafter\def\csname v@s5/p075/unseen/w20\endcsname{85.3}
\expandafter\def\csname v@s5/p075/vox/mae\endcsname{16.4}
\expandafter\def\csname v@s5/p075/vox/w20\endcsname{78.7}
\expandafter\def\csname v@s5/p1/buckeye-clean/mae\endcsname{12.5}
\expandafter\def\csname v@s5/p1/buckeye-clean/w20\endcsname{85.7}
\expandafter\def\csname v@s5/p1/buckeye-seen/mae\endcsname{13.1}
\expandafter\def\csname v@s5/p1/buckeye-seen/w20\endcsname{84.6}
\expandafter\def\csname v@s5/p1/buckeye-unseen/mae\endcsname{13.4}
\expandafter\def\csname v@s5/p1/buckeye-unseen/w20\endcsname{83.9}
\expandafter\def\csname v@s5/p1/clean/mae\endcsname{13.0}
\expandafter\def\csname v@s5/p1/clean/w20\endcsname{84.8}
\expandafter\def\csname v@s5/p1/ifa/mae\endcsname{15.2}
\expandafter\def\csname v@s5/p1/ifa/w20\endcsname{78.1}
\expandafter\def\csname v@s5/p1/long-clean/mae\endcsname{10.7}
\expandafter\def\csname v@s5/p1/long-clean/w20\endcsname{88.5}
\expandafter\def\csname v@s5/p1/long-g711/mae\endcsname{10.6}
\expandafter\def\csname v@s5/p1/long-g711/w20\endcsname{88.8}
\expandafter\def\csname v@s5/p1/seen/mae\endcsname{11.6}
\expandafter\def\csname v@s5/p1/seen/w20\endcsname{87.2}
\expandafter\def\csname v@s5/p1/seoul/mae\endcsname{11.7}
\expandafter\def\csname v@s5/p1/seoul/w20\endcsname{89.5}
\expandafter\def\csname v@s5/p1/swb-col/mae\endcsname{23.0}
\expandafter\def\csname v@s5/p1/swb-col/w20\endcsname{80.5}
\expandafter\def\csname v@s5/p1/swb/mae\endcsname{23.0}
\expandafter\def\csname v@s5/p1/swb/w20\endcsname{80.5}
\expandafter\def\csname v@s5/p1/timit-clean/mae\endcsname{11.0}
\expandafter\def\csname v@s5/p1/timit-clean/w20\endcsname{88.2}
\expandafter\def\csname v@s5/p1/timit-seen/mae\endcsname{11.1}
\expandafter\def\csname v@s5/p1/timit-seen/w20\endcsname{88.2}
\expandafter\def\csname v@s5/p1/timit-unseen/mae\endcsname{12.1}
\expandafter\def\csname v@s5/p1/timit-unseen/w20\endcsname{86.9}
\expandafter\def\csname v@s5/p1/unseen/mae\endcsname{12.7}
\expandafter\def\csname v@s5/p1/unseen/w20\endcsname{85.4}
\expandafter\def\csname v@s5/p1/vox/mae\endcsname{16.7}
\expandafter\def\csname v@s5/p1/vox/w20\endcsname{79.0}
\expandafter\def\csname v@seoul/ft-ctcm-full/clean/mae\endcsname{15.6}
\expandafter\def\csname v@seoul/ft-ctcm-full/clean/median\endcsname{8.0}
\expandafter\def\csname v@seoul/ft-ctcm-full/clean/over500\endcsname{0.14}
\expandafter\def\csname v@seoul/ft-ctcm-full/clean/w100\endcsname{98.6}
\expandafter\def\csname v@seoul/ft-ctcm-full/clean/w20\endcsname{81.7}
\expandafter\def\csname v@seoul/ft-ctcm-full/clean/w50\endcsname{95.7}
\expandafter\def\csname v@seoul/ft-ctcm-lora/clean/mae\endcsname{16.2}
\expandafter\def\csname v@seoul/ft-ctcm-lora/clean/median\endcsname{8.3}
\expandafter\def\csname v@seoul/ft-ctcm-lora/clean/over500\endcsname{0.13}
\expandafter\def\csname v@seoul/ft-ctcm-lora/clean/w100\endcsname{98.5}
\expandafter\def\csname v@seoul/ft-ctcm-lora/clean/w20\endcsname{81.0}
\expandafter\def\csname v@seoul/ft-ctcm-lora/clean/w50\endcsname{95.6}
\expandafter\def\csname v@seoul/ft-ctcw-full/clean/mae\endcsname{14.0}
\expandafter\def\csname v@seoul/ft-ctcw-full/clean/median\endcsname{7.4}
\expandafter\def\csname v@seoul/ft-ctcw-full/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ctcw-full/clean/w100\endcsname{98.6}
\expandafter\def\csname v@seoul/ft-ctcw-full/clean/w20\endcsname{85.7}
\expandafter\def\csname v@seoul/ft-ctcw-full/clean/w50\endcsname{96.2}
\expandafter\def\csname v@seoul/ft-ctcw-lora/clean/mae\endcsname{13.5}
\expandafter\def\csname v@seoul/ft-ctcw-lora/clean/median\endcsname{7.3}
\expandafter\def\csname v@seoul/ft-ctcw-lora/clean/over500\endcsname{0.06}
\expandafter\def\csname v@seoul/ft-ctcw-lora/clean/w100\endcsname{98.7}
\expandafter\def\csname v@seoul/ft-ctcw-lora/clean/w20\endcsname{86.0}
\expandafter\def\csname v@seoul/ft-ctcw-lora/clean/w50\endcsname{96.3}
\expandafter\def\csname v@seoul/ft-ts-1k-s1/clean/mae\endcsname{11.7}
\expandafter\def\csname v@seoul/ft-ts-1k-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-1k-s1/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-1k-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-1k-s1/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-1k-s1/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-1k/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-1k/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-1k/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-1k/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-1k/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-1k/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-4k/clean/mae\endcsname{11.8}
\expandafter\def\csname v@seoul/ft-ts-4k/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-4k/clean/over500\endcsname{0.12}
\expandafter\def\csname v@seoul/ft-ts-4k/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-4k/clean/w20\endcsname{89.5}
\expandafter\def\csname v@seoul/ft-ts-4k/clean/w50\endcsname{97.0}
\expandafter\def\csname v@seoul/ft-ts-6k/clean/mae\endcsname{12.0}
\expandafter\def\csname v@seoul/ft-ts-6k/clean/median\endcsname{5.6}
\expandafter\def\csname v@seoul/ft-ts-6k/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-6k/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-6k/clean/w20\endcsname{88.9}
\expandafter\def\csname v@seoul/ft-ts-6k/clean/w50\endcsname{97.0}
\expandafter\def\csname v@seoul/ft-ts-a02/clean/mae\endcsname{11.6}
\expandafter\def\csname v@seoul/ft-ts-a02/clean/median\endcsname{5.5}
\expandafter\def\csname v@seoul/ft-ts-a02/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-a02/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-a02/clean/w20\endcsname{89.6}
\expandafter\def\csname v@seoul/ft-ts-a02/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-attn/clean/mae\endcsname{11.3}
\expandafter\def\csname v@seoul/ft-ts-attn/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-attn/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-attn/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-attn/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-attn/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-aug0-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-aug0-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@seoul/ft-ts-aug0-s1/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-aug0-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-aug0-s1/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-aug0-s1/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-aug0-s2/clean/mae\endcsname{11.6}
\expandafter\def\csname v@seoul/ft-ts-aug0-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-aug0-s2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-aug0-s2/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-aug0-s2/clean/w20\endcsname{89.6}
\expandafter\def\csname v@seoul/ft-ts-aug0-s2/clean/w50\endcsname{97.0}
\expandafter\def\csname v@seoul/ft-ts-aug0/clean/mae\endcsname{11.5}
\expandafter\def\csname v@seoul/ft-ts-aug0/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-aug0/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-aug0/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-aug0/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-aug0/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-aug100/clean/mae\endcsname{11.7}
\expandafter\def\csname v@seoul/ft-ts-aug100/clean/median\endcsname{5.8}
\expandafter\def\csname v@seoul/ft-ts-aug100/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-aug100/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-aug100/clean/w20\endcsname{89.5}
\expandafter\def\csname v@seoul/ft-ts-aug100/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-aug25-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-aug25-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-aug25-s1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-aug25-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-aug25-s1/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-aug25-s1/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-aug25-s2/clean/mae\endcsname{11.6}
\expandafter\def\csname v@seoul/ft-ts-aug25-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-aug25-s2/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-aug25-s2/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-aug25-s2/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-aug25-s2/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-aug25/clean/mae\endcsname{11.3}
\expandafter\def\csname v@seoul/ft-ts-aug25/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-aug25/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-aug25/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-aug25/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-aug25/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-aug75/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-aug75/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-aug75/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-aug75/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-aug75/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-aug75/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-augamr-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-augamr-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-augamr-s1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-augamr-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-augamr-s1/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-augamr-s1/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-augamr/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-augamr/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-augamr/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-augamr/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-augamr/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-augamr/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-auxw-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-auxw-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-auxw-s1/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-auxw-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-auxw-s1/clean/w20\endcsname{90.2}
\expandafter\def\csname v@seoul/ft-ts-auxw-s1/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-auxw/clean/mae\endcsname{11.3}
\expandafter\def\csname v@seoul/ft-ts-auxw/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-auxw/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-auxw/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-auxw/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-auxw/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-auxwp-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-auxwp-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-auxwp-s1/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-auxwp-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-auxwp-s1/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-auxwp-s1/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-auxwp/clean/mae\endcsname{11.2}
\expandafter\def\csname v@seoul/ft-ts-auxwp/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-auxwp/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-auxwp/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-auxwp/clean/w20\endcsname{90.2}
\expandafter\def\csname v@seoul/ft-ts-auxwp/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-dec/clean/mae\endcsname{12.7}
\expandafter\def\csname v@seoul/ft-ts-dec/clean/median\endcsname{6.6}
\expandafter\def\csname v@seoul/ft-ts-dec/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-dec/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-dec/clean/w20\endcsname{87.5}
\expandafter\def\csname v@seoul/ft-ts-dec/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-full/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-full/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-full/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-full/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-full/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-full/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-lora-argmax/clean/mae\endcsname{12.9}
\expandafter\def\csname v@seoul/ft-ts-lora-argmax/clean/median\endcsname{7.1}
\expandafter\def\csname v@seoul/ft-ts-lora-argmax/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-lora-argmax/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-lora-argmax/clean/w20\endcsname{87.9}
\expandafter\def\csname v@seoul/ft-ts-lora-argmax/clean/w50\endcsname{96.9}
\expandafter\def\csname v@seoul/ft-ts-lora-en-nolang/clean/mae\endcsname{24.8}
\expandafter\def\csname v@seoul/ft-ts-lora-en-nolang/clean/median\endcsname{8.1}
\expandafter\def\csname v@seoul/ft-ts-lora-en-nolang/clean/over500\endcsname{0.70}
\expandafter\def\csname v@seoul/ft-ts-lora-en-nolang/clean/w100\endcsname{97.6}
\expandafter\def\csname v@seoul/ft-ts-lora-en-nolang/clean/w20\endcsname{79.2}
\expandafter\def\csname v@seoul/ft-ts-lora-en-nolang/clean/w50\endcsname{92.7}
\expandafter\def\csname v@seoul/ft-ts-lora-en/clean/mae\endcsname{24.2}
\expandafter\def\csname v@seoul/ft-ts-lora-en/clean/median\endcsname{8.2}
\expandafter\def\csname v@seoul/ft-ts-lora-en/clean/over500\endcsname{0.70}
\expandafter\def\csname v@seoul/ft-ts-lora-en/clean/w100\endcsname{97.7}
\expandafter\def\csname v@seoul/ft-ts-lora-en/clean/w20\endcsname{79.1}
\expandafter\def\csname v@seoul/ft-ts-lora-en/clean/w50\endcsname{92.7}
\expandafter\def\csname v@seoul/ft-ts-lora-full/clean/mae\endcsname{14.4}
\expandafter\def\csname v@seoul/ft-ts-lora-full/clean/median\endcsname{6.9}
\expandafter\def\csname v@seoul/ft-ts-lora-full/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-lora-full/clean/w100\endcsname{98.7}
\expandafter\def\csname v@seoul/ft-ts-lora-full/clean/w20\endcsname{82.6}
\expandafter\def\csname v@seoul/ft-ts-lora-full/clean/w50\endcsname{95.4}
\expandafter\def\csname v@seoul/ft-ts-lora-nolang/clean/mae\endcsname{11.2}
\expandafter\def\csname v@seoul/ft-ts-lora-nolang/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-lora-nolang/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-lora-nolang/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-lora-nolang/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-lora-nolang/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-lora-r1/clean/mae\endcsname{11.3}
\expandafter\def\csname v@seoul/ft-ts-lora-r1/clean/median\endcsname{5.2}
\expandafter\def\csname v@seoul/ft-ts-lora-r1/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-lora-r1/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-lora-r1/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-lora-r1/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-lora-r5/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-lora-r5/clean/median\endcsname{5.6}
\expandafter\def\csname v@seoul/ft-ts-lora-r5/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-lora-r5/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-lora-r5/clean/w20\endcsname{89.1}
\expandafter\def\csname v@seoul/ft-ts-lora-r5/clean/w50\endcsname{97.6}
\expandafter\def\csname v@seoul/ft-ts-lora/clean/mae\endcsname{11.3}
\expandafter\def\csname v@seoul/ft-ts-lora/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-lora/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-lora/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-lora/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-lora/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-lr1e4/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-lr1e4/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-lr1e4/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-lr1e4/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-lr1e4/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-lr1e4/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-lr5e4/clean/mae\endcsname{11.6}
\expandafter\def\csname v@seoul/ft-ts-lr5e4/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-lr5e4/clean/over500\endcsname{0.12}
\expandafter\def\csname v@seoul/ft-ts-lr5e4/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-lr5e4/clean/w20\endcsname{89.7}
\expandafter\def\csname v@seoul/ft-ts-lr5e4/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-4k/clean/mae\endcsname{10.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-4k/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-4k/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-4k/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-4k/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-4k/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr2e4/clean/mae\endcsname{10.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr2e4/clean/median\endcsname{5.2}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr2e4/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr2e4/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr2e4/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr2e4/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr5e3/clean/mae\endcsname{10.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr5e3/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr5e3/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr5e3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr5e3/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-lr5e3/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-r64/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-r64/clean/median\endcsname{5.2}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-r64/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-r64/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-r64/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-r64/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-rand/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-rand/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-rand/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-rand/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-rand/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-rand/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-round/clean/mae\endcsname{10.6}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-round/clean/median\endcsname{5.5}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-round/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-round/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-round/clean/w20\endcsname{89.5}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-round/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s1/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s1/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s1/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s2/clean/mae\endcsname{10.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s2/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s2/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s2/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s2/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s3/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s3/clean/median\endcsname{5.2}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s3/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s3/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s3/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s3/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s4/clean/mae\endcsname{10.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s4/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s4/clean/over500\endcsname{0.01}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s4/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-s4/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-tn10/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-tn10/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-tn10/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-tn10/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-tn10/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-post-10ms-tn10/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms/clean/mae\endcsname{10.2}
\expandafter\def\csname v@seoul/ft-ts-post-10ms/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-10ms/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-10ms/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-post-10ms/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-5ms/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-5ms/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-5ms/clean/over500\endcsname{0.01}
\expandafter\def\csname v@seoul/ft-ts-post-5ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-5ms/clean/w20\endcsname{89.5}
\expandafter\def\csname v@seoul/ft-ts-post-5ms/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-post-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-s1/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-s1/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-post-s1/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-s2/clean/mae\endcsname{10.6}
\expandafter\def\csname v@seoul/ft-ts-post-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-s2/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-post-s2/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-s2/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-post-s2/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-post-s3/clean/mae\endcsname{10.2}
\expandafter\def\csname v@seoul/ft-ts-post-s3/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-s3/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-s3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-s3/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-post-s3/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-s4/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-s4/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-s4/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-s4/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-s4/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-post-s4/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-sidon-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-sidon-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-post-sidon-s1/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-sidon-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-sidon-s1/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-post-sidon-s1/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-sidon/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-sidon/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-sidon/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post-sidon/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-sidon/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-post-sidon/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-tn10-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-post-tn10-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-tn10-s1/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-post-tn10-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post-tn10-s1/clean/w20\endcsname{90.2}
\expandafter\def\csname v@seoul/ft-ts-post-tn10-s1/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post-tn10/clean/mae\endcsname{10.3}
\expandafter\def\csname v@seoul/ft-ts-post-tn10/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post-tn10/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-post-tn10/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-post-tn10/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-post-tn10/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-post/clean/mae\endcsname{10.3}
\expandafter\def\csname v@seoul/ft-ts-post/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-post/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-post/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-post/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-post/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-r128/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-r128/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-r128/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-r128/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-r128/clean/w20\endcsname{89.7}
\expandafter\def\csname v@seoul/ft-ts-r128/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-r16/clean/mae\endcsname{11.3}
\expandafter\def\csname v@seoul/ft-ts-r16/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-r16/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-r16/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-r16/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-r16/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-r64/clean/mae\endcsname{11.1}
\expandafter\def\csname v@seoul/ft-ts-r64/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-r64/clean/over500\endcsname{0.09}
\expandafter\def\csname v@seoul/ft-ts-r64/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-r64/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-r64/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-r8/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-r8/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-r8/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-r8/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-r8/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-r8/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-round-s1/clean/mae\endcsname{12.0}
\expandafter\def\csname v@seoul/ft-ts-round-s1/clean/median\endcsname{5.6}
\expandafter\def\csname v@seoul/ft-ts-round-s1/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-round-s1/clean/w100\endcsname{98.7}
\expandafter\def\csname v@seoul/ft-ts-round-s1/clean/w20\endcsname{89.5}
\expandafter\def\csname v@seoul/ft-ts-round-s1/clean/w50\endcsname{97.0}
\expandafter\def\csname v@seoul/ft-ts-round/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-round/clean/median\endcsname{5.6}
\expandafter\def\csname v@seoul/ft-ts-round/clean/over500\endcsname{0.08}
\expandafter\def\csname v@seoul/ft-ts-round/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-round/clean/w20\endcsname{89.6}
\expandafter\def\csname v@seoul/ft-ts-round/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-s6-final-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@seoul/ft-ts-s6-final-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-s6-final-s1/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-s6-final-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-s6-final-s1/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-s6-final-s1/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-s6-final/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-s6-final/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-s6-final/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-s6-final/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-s6-final/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-s6-final/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-s6-post-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-s6-post-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-s6-post-s1/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-s6-post-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-s6-post-s1/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-s6-post-s1/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-s6-post/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-s6-post/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-s6-post/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-s6-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-s6-post/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-s6-post/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon-s1/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon-s1/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon-s1/clean/w50\endcsname{97.4}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon/clean/w20\endcsname{90.2}
\expandafter\def\csname v@seoul/ft-ts-s6-sidon/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-seed1/clean/mae\endcsname{11.5}
\expandafter\def\csname v@seoul/ft-ts-seed1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-seed1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-seed1/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-seed1/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-seed1/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-seed2/clean/mae\endcsname{11.5}
\expandafter\def\csname v@seoul/ft-ts-seed2/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-seed2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-seed2/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-seed2/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-seed2/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-seed3/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-seed3/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-seed3/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-seed3/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-seed3/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-seed3/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-seed4/clean/mae\endcsname{11.5}
\expandafter\def\csname v@seoul/ft-ts-seed4/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-seed4/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-seed4/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-seed4/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-seed4/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-tn10-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-tn10-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-tn10-s1/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-tn10-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-tn10-s1/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-tn10-s1/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-tn10/clean/mae\endcsname{11.5}
\expandafter\def\csname v@seoul/ft-ts-tn10/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-tn10/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-tn10/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-tn10/clean/w20\endcsname{90.0}
\expandafter\def\csname v@seoul/ft-ts-tn10/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-tn20/clean/mae\endcsname{11.5}
\expandafter\def\csname v@seoul/ft-ts-tn20/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-tn20/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-tn20/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-tn20/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-tn20/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-turbo-final-s1/clean/mae\endcsname{10.8}
\expandafter\def\csname v@seoul/ft-ts-turbo-final-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-turbo-final-s1/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-turbo-final-s1/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-turbo-final-s1/clean/w20\endcsname{89.5}
\expandafter\def\csname v@seoul/ft-ts-turbo-final-s1/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-turbo-final/clean/mae\endcsname{10.6}
\expandafter\def\csname v@seoul/ft-ts-turbo-final/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-turbo-final/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-turbo-final/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-turbo-final/clean/w20\endcsname{89.7}
\expandafter\def\csname v@seoul/ft-ts-turbo-final/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-10ms/clean/mae\endcsname{10.7}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-10ms/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-10ms/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-10ms/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-10ms/clean/w20\endcsname{89.4}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-10ms/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-s1/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-s1/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-turbo-post-s1/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-post/clean/mae\endcsname{10.7}
\expandafter\def\csname v@seoul/ft-ts-turbo-post/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-post/clean/over500\endcsname{0.03}
\expandafter\def\csname v@seoul/ft-ts-turbo-post/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-turbo-post/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-turbo-post/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-turbo-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-s1/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-turbo-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-turbo-s1/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-turbo-s1/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-turbo-s2/clean/mae\endcsname{11.7}
\expandafter\def\csname v@seoul/ft-ts-turbo-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-s2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-turbo-s2/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-turbo-s2/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-turbo-s2/clean/w50\endcsname{97.0}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10-s1/clean/mae\endcsname{12.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10-s1/clean/over500\endcsname{0.14}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10-s1/clean/w100\endcsname{98.7}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10-s1/clean/w20\endcsname{89.7}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10-s1/clean/w50\endcsname{97.0}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10/clean/mae\endcsname{11.7}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10/clean/w20\endcsname{89.6}
\expandafter\def\csname v@seoul/ft-ts-turbo-tn10/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-turbo/clean/mae\endcsname{11.5}
\expandafter\def\csname v@seoul/ft-ts-turbo/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-turbo/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-turbo/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-turbo/clean/w20\endcsname{89.8}
\expandafter\def\csname v@seoul/ft-ts-turbo/clean/w50\endcsname{97.1}
\expandafter\def\csname v@seoul/ft-ts-v3-final-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@seoul/ft-ts-v3-final-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-v3-final-s1/clean/over500\endcsname{0.04}
\expandafter\def\csname v@seoul/ft-ts-v3-final-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@seoul/ft-ts-v3-final-s1/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-v3-final-s1/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-v3-final/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-v3-final/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-v3-final/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-v3-final/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-v3-final/clean/w20\endcsname{90.1}
\expandafter\def\csname v@seoul/ft-ts-v3-final/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-v3-post-10ms/clean/mae\endcsname{10.4}
\expandafter\def\csname v@seoul/ft-ts-v3-post-10ms/clean/median\endcsname{5.2}
\expandafter\def\csname v@seoul/ft-ts-v3-post-10ms/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-v3-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-v3-post-10ms/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-v3-post-10ms/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-v3-post-s1/clean/mae\endcsname{10.2}
\expandafter\def\csname v@seoul/ft-ts-v3-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-v3-post-s1/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-v3-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-v3-post-s1/clean/w20\endcsname{90.3}
\expandafter\def\csname v@seoul/ft-ts-v3-post-s1/clean/w50\endcsname{97.6}
\expandafter\def\csname v@seoul/ft-ts-v3-post/clean/mae\endcsname{10.5}
\expandafter\def\csname v@seoul/ft-ts-v3-post/clean/median\endcsname{5.2}
\expandafter\def\csname v@seoul/ft-ts-v3-post/clean/over500\endcsname{0.02}
\expandafter\def\csname v@seoul/ft-ts-v3-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@seoul/ft-ts-v3-post/clean/w20\endcsname{90.4}
\expandafter\def\csname v@seoul/ft-ts-v3-post/clean/w50\endcsname{97.5}
\expandafter\def\csname v@seoul/ft-ts-v3-s1/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-v3-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-v3-s1/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-v3-s1/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-v3-s1/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-v3-s1/clean/w50\endcsname{97.2}
\expandafter\def\csname v@seoul/ft-ts-v3-s2/clean/mae\endcsname{11.3}
\expandafter\def\csname v@seoul/ft-ts-v3-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-v3-s2/clean/over500\endcsname{0.10}
\expandafter\def\csname v@seoul/ft-ts-v3-s2/clean/w100\endcsname{98.9}
\expandafter\def\csname v@seoul/ft-ts-v3-s2/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-v3-s2/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-v3/clean/mae\endcsname{11.4}
\expandafter\def\csname v@seoul/ft-ts-v3/clean/median\endcsname{5.3}
\expandafter\def\csname v@seoul/ft-ts-v3/clean/over500\endcsname{0.11}
\expandafter\def\csname v@seoul/ft-ts-v3/clean/w100\endcsname{98.8}
\expandafter\def\csname v@seoul/ft-ts-v3/clean/w20\endcsname{89.9}
\expandafter\def\csname v@seoul/ft-ts-v3/clean/w50\endcsname{97.3}
\expandafter\def\csname v@seoul/ft-ts-wt-s1/clean/mae\endcsname{23.8}
\expandafter\def\csname v@seoul/ft-ts-wt-s1/clean/median\endcsname{6.2}
\expandafter\def\csname v@seoul/ft-ts-wt-s1/clean/over500\endcsname{0.34}
\expandafter\def\csname v@seoul/ft-ts-wt-s1/clean/w100\endcsname{98.5}
\expandafter\def\csname v@seoul/ft-ts-wt-s1/clean/w20\endcsname{88.3}
\expandafter\def\csname v@seoul/ft-ts-wt-s1/clean/w50\endcsname{96.7}
\expandafter\def\csname v@seoul/ft-ts-wt/clean/mae\endcsname{21.7}
\expandafter\def\csname v@seoul/ft-ts-wt/clean/median\endcsname{6.2}
\expandafter\def\csname v@seoul/ft-ts-wt/clean/over500\endcsname{0.29}
\expandafter\def\csname v@seoul/ft-ts-wt/clean/w100\endcsname{98.6}
\expandafter\def\csname v@seoul/ft-ts-wt/clean/w20\endcsname{88.4}
\expandafter\def\csname v@seoul/ft-ts-wt/clean/w50\endcsname{96.8}
\expandafter\def\csname v@seoul/mfa-korean/clean/mae\endcsname{21.3}
\expandafter\def\csname v@seoul/mfa-korean/clean/median\endcsname{10.9}
\expandafter\def\csname v@seoul/mfa-korean/clean/over500\endcsname{0.21}
\expandafter\def\csname v@seoul/mfa-korean/clean/w100\endcsname{97.6}
\expandafter\def\csname v@seoul/mfa-korean/clean/w20\endcsname{70.2}
\expandafter\def\csname v@seoul/mfa-korean/clean/w50\endcsname{93.0}
\expandafter\def\csname v@seoul/whisper-tm-cal/clean/mae\endcsname{87.2}
\expandafter\def\csname v@seoul/whisper-tm-cal/clean/median\endcsname{28.2}
\expandafter\def\csname v@seoul/whisper-tm-cal/clean/over500\endcsname{3.53}
\expandafter\def\csname v@seoul/whisper-tm-cal/clean/w100\endcsname{81.4}
\expandafter\def\csname v@seoul/whisper-tm-cal/clean/w20\endcsname{37.8}
\expandafter\def\csname v@seoul/whisper-tm-cal/clean/w50\endcsname{68.9}
\expandafter\def\csname v@sub/ms10/0/frame\endcsname{100.0}
\expandafter\def\csname v@sub/ms10/0/mae\endcsname{10.65}
\expandafter\def\csname v@sub/ms10/0/near\endcsname{100.0}
\expandafter\def\csname v@sub/ms10/0/shift\endcsname{0.0}
\expandafter\def\csname v@sub/ms10/10/frame\endcsname{2.2}
\expandafter\def\csname v@sub/ms10/10/mae\endcsname{10.63}
\expandafter\def\csname v@sub/ms10/10/near\endcsname{67.6}
\expandafter\def\csname v@sub/ms10/10/shift\endcsname{9.9}
\expandafter\def\csname v@sub/ms10/15/frame\endcsname{16.0}
\expandafter\def\csname v@sub/ms10/15/mae\endcsname{10.60}
\expandafter\def\csname v@sub/ms10/15/near\endcsname{63.1}
\expandafter\def\csname v@sub/ms10/15/shift\endcsname{15.0}
\expandafter\def\csname v@sub/ms10/20/frame\endcsname{70.4}
\expandafter\def\csname v@sub/ms10/20/mae\endcsname{10.63}
\expandafter\def\csname v@sub/ms10/20/near\endcsname{70.3}
\expandafter\def\csname v@sub/ms10/20/shift\endcsname{20.0}
\expandafter\def\csname v@sub/ms10/5/frame\endcsname{10.3}
\expandafter\def\csname v@sub/ms10/5/mae\endcsname{10.59}
\expandafter\def\csname v@sub/ms10/5/near\endcsname{77.5}
\expandafter\def\csname v@sub/ms10/5/shift\endcsname{4.8}
\expandafter\def\csname v@sub/n\endcsname{22{,}050}
\expandafter\def\csname v@sub/post/0/frame\endcsname{100.0}
\expandafter\def\csname v@sub/post/0/mae\endcsname{10.51}
\expandafter\def\csname v@sub/post/0/near\endcsname{100.0}
\expandafter\def\csname v@sub/post/0/shift\endcsname{0.0}
\expandafter\def\csname v@sub/post/10/frame\endcsname{1.3}
\expandafter\def\csname v@sub/post/10/mae\endcsname{10.57}
\expandafter\def\csname v@sub/post/10/near\endcsname{72.0}
\expandafter\def\csname v@sub/post/10/shift\endcsname{10.0}
\expandafter\def\csname v@sub/post/15/frame\endcsname{12.2}
\expandafter\def\csname v@sub/post/15/mae\endcsname{10.58}
\expandafter\def\csname v@sub/post/15/near\endcsname{73.1}
\expandafter\def\csname v@sub/post/15/shift\endcsname{15.1}
\expandafter\def\csname v@sub/post/20/frame\endcsname{87.3}
\expandafter\def\csname v@sub/post/20/mae\endcsname{10.52}
\expandafter\def\csname v@sub/post/20/near\endcsname{87.2}
\expandafter\def\csname v@sub/post/20/shift\endcsname{20.0}
\expandafter\def\csname v@sub/post/5/frame\endcsname{8.7}
\expandafter\def\csname v@sub/post/5/mae\endcsname{10.54}
\expandafter\def\csname v@sub/post/5/near\endcsname{80.1}
\expandafter\def\csname v@sub/post/5/shift\endcsname{4.8}
\expandafter\def\csname v@survey/n-evalsets\endcsname{38}
\expandafter\def\csname v@survey/n-models\endcsname{72}
\expandafter\def\csname v@swb/cfa-edges/tel/ebias\endcsname{10}
\expandafter\def\csname v@swb/cfa-edges/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/cfa-edges/tel/mae\endcsname{56.4}
\expandafter\def\csname v@swb/cfa-edges/tel/over500\endcsname{1.3}
\expandafter\def\csname v@swb/cfa-edges/tel/sbias\endcsname{14}
\expandafter\def\csname v@swb/cfa-edges/tel/w100\endcsname{87.2}
\expandafter\def\csname v@swb/cfa-edges/tel/w20\endcsname{39.7}
\expandafter\def\csname v@swb/cfa-edges/tel/w50\endcsname{75.6}
\expandafter\def\csname v@swb/cfa-segment/tel/ebias\endcsname{12}
\expandafter\def\csname v@swb/cfa-segment/tel/fail\endcsname{1}
\expandafter\def\csname v@swb/cfa-segment/tel/mae\endcsname{71.6}
\expandafter\def\csname v@swb/cfa-segment/tel/over500\endcsname{2.0}
\expandafter\def\csname v@swb/cfa-segment/tel/sbias\endcsname{36}
\expandafter\def\csname v@swb/cfa-segment/tel/w100\endcsname{83.5}
\expandafter\def\csname v@swb/cfa-segment/tel/w20\endcsname{29.7}
\expandafter\def\csname v@swb/cfa-segment/tel/w50\endcsname{64.7}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/mae\endcsname{21.8}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/over500\endcsname{0.4}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/w100\endcsname{97.3}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/w20\endcsname{75.2}
\expandafter\def\csname v@swb/ft-ctcm-full/tel/w50\endcsname{93.9}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/mae\endcsname{22.6}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/over500\endcsname{0.5}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/w100\endcsname{97.2}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/w20\endcsname{74.7}
\expandafter\def\csname v@swb/ft-ctcm-lora/tel/w50\endcsname{93.4}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/ebias\endcsname{0}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/mae\endcsname{22.4}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/over500\endcsname{0.4}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/w100\endcsname{96.5}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/w20\endcsname{78.0}
\expandafter\def\csname v@swb/ft-ctcw-full/tel/w50\endcsname{93.5}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/ebias\endcsname{0}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/mae\endcsname{22.3}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/over500\endcsname{0.4}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/w100\endcsname{96.9}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/w20\endcsname{78.0}
\expandafter\def\csname v@swb/ft-ctcw-lora/tel/w50\endcsname{93.5}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/mae\endcsname{21.9}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/w100\endcsname{96.9}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/w20\endcsname{81.4}
\expandafter\def\csname v@swb/ft-ts-1k-s1/tel/w50\endcsname{94.2}
\expandafter\def\csname v@swb/ft-ts-1k/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-1k/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-1k/tel/mae\endcsname{22.7}
\expandafter\def\csname v@swb/ft-ts-1k/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-1k/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-1k/tel/w100\endcsname{96.9}
\expandafter\def\csname v@swb/ft-ts-1k/tel/w20\endcsname{81.1}
\expandafter\def\csname v@swb/ft-ts-1k/tel/w50\endcsname{94.0}
\expandafter\def\csname v@swb/ft-ts-4k/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-4k/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-4k/tel/mae\endcsname{24.5}
\expandafter\def\csname v@swb/ft-ts-4k/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-4k/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-4k/tel/w100\endcsname{96.5}
\expandafter\def\csname v@swb/ft-ts-4k/tel/w20\endcsname{79.2}
\expandafter\def\csname v@swb/ft-ts-4k/tel/w50\endcsname{93.3}
\expandafter\def\csname v@swb/ft-ts-6k/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-6k/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-6k/tel/mae\endcsname{24.7}
\expandafter\def\csname v@swb/ft-ts-6k/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-6k/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-6k/tel/w100\endcsname{96.4}
\expandafter\def\csname v@swb/ft-ts-6k/tel/w20\endcsname{79.0}
\expandafter\def\csname v@swb/ft-ts-6k/tel/w50\endcsname{93.3}
\expandafter\def\csname v@swb/ft-ts-a02/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-a02/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-a02/tel/mae\endcsname{22.2}
\expandafter\def\csname v@swb/ft-ts-a02/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-a02/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-a02/tel/w100\endcsname{97.0}
\expandafter\def\csname v@swb/ft-ts-a02/tel/w20\endcsname{81.1}
\expandafter\def\csname v@swb/ft-ts-a02/tel/w50\endcsname{94.2}
\expandafter\def\csname v@swb/ft-ts-attn/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-attn/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-attn/tel/mae\endcsname{23.1}
\expandafter\def\csname v@swb/ft-ts-attn/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-attn/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-attn/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-attn/tel/w20\endcsname{80.9}
\expandafter\def\csname v@swb/ft-ts-attn/tel/w50\endcsname{94.2}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/mae\endcsname{24.1}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/w100\endcsname{96.5}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/w20\endcsname{80.0}
\expandafter\def\csname v@swb/ft-ts-aug0-s1/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/mae\endcsname{25.3}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/w100\endcsname{96.3}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/w20\endcsname{79.6}
\expandafter\def\csname v@swb/ft-ts-aug0-s2/tel/w50\endcsname{93.4}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/mae\endcsname{24.0}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/w20\endcsname{80.2}
\expandafter\def\csname v@swb/ft-ts-aug0/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/mae\endcsname{23.0}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/w20\endcsname{80.5}
\expandafter\def\csname v@swb/ft-ts-aug100/tel/w50\endcsname{93.6}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/mae\endcsname{24.1}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/w100\endcsname{96.5}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/w20\endcsname{80.1}
\expandafter\def\csname v@swb/ft-ts-aug25-s1/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/mae\endcsname{23.2}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/w20\endcsname{80.6}
\expandafter\def\csname v@swb/ft-ts-aug25-s2/tel/w50\endcsname{93.9}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/mae\endcsname{22.7}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/w20\endcsname{80.9}
\expandafter\def\csname v@swb/ft-ts-aug25/tel/w50\endcsname{94.0}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/mae\endcsname{23.0}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/w20\endcsname{80.7}
\expandafter\def\csname v@swb/ft-ts-aug75/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/mae\endcsname{23.9}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/w20\endcsname{80.2}
\expandafter\def\csname v@swb/ft-ts-augamr-s1/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/mae\endcsname{23.0}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/w100\endcsname{96.9}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/w20\endcsname{80.7}
\expandafter\def\csname v@swb/ft-ts-augamr/tel/w50\endcsname{94.0}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/mae\endcsname{24.9}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/w100\endcsname{96.4}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/w20\endcsname{80.2}
\expandafter\def\csname v@swb/ft-ts-auxw-s1/tel/w50\endcsname{93.5}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/mae\endcsname{23.5}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/w20\endcsname{80.6}
\expandafter\def\csname v@swb/ft-ts-auxw/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/mae\endcsname{24.0}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/w20\endcsname{80.2}
\expandafter\def\csname v@swb/ft-ts-auxwp-s1/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/mae\endcsname{22.8}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/w20\endcsname{81.0}
\expandafter\def\csname v@swb/ft-ts-auxwp/tel/w50\endcsname{94.0}
\expandafter\def\csname v@swb/ft-ts-dec/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-dec/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-dec/tel/mae\endcsname{24.2}
\expandafter\def\csname v@swb/ft-ts-dec/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-dec/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-dec/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-dec/tel/w20\endcsname{79.0}
\expandafter\def\csname v@swb/ft-ts-dec/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-full/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-full/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-full/tel/mae\endcsname{22.7}
\expandafter\def\csname v@swb/ft-ts-full/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-full/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-full/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-full/tel/w20\endcsname{80.5}
\expandafter\def\csname v@swb/ft-ts-full/tel/w50\endcsname{93.9}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/mae\endcsname{27.1}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/over500\endcsname{0.8}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/w100\endcsname{95.9}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/w20\endcsname{78.5}
\expandafter\def\csname v@swb/ft-ts-lora-en/tel/w50\endcsname{92.7}
\expandafter\def\csname v@swb/ft-ts-lora/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lora/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora/tel/mae\endcsname{23.0}
\expandafter\def\csname v@swb/ft-ts-lora/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-lora/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lora/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-lora/tel/w20\endcsname{80.7}
\expandafter\def\csname v@swb/ft-ts-lora/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/ebias\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/mae\endcsname{24.1}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/sbias\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/w20\endcsname{77.9}
\expandafter\def\csname v@swb/ft-ts-lora@argmax/tel/w50\endcsname{93.3}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/ebias\endcsname{6}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/mae\endcsname{25.6}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/over500\endcsname{0.5}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/sbias\endcsname{3}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/w20\endcsname{72.7}
\expandafter\def\csname v@swb/ft-ts-lora@full/tel/w50\endcsname{92.7}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/mae\endcsname{23.0}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/w20\endcsname{80.6}
\expandafter\def\csname v@swb/ft-ts-lora@r1/tel/w50\endcsname{93.6}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/mae\endcsname{23.2}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/w20\endcsname{79.1}
\expandafter\def\csname v@swb/ft-ts-lora@r5/tel/w50\endcsname{94.2}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/mae\endcsname{22.9}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/w100\endcsname{96.9}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/w20\endcsname{80.8}
\expandafter\def\csname v@swb/ft-ts-lr1e4/tel/w50\endcsname{93.9}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/mae\endcsname{24.0}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/w100\endcsname{96.5}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/w20\endcsname{80.6}
\expandafter\def\csname v@swb/ft-ts-lr5e4/tel/w50\endcsname{93.6}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/mae\endcsname{19.0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/w100\endcsname{98.0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/w20\endcsname{80.9}
\expandafter\def\csname v@swb/ft-ts-post-10ms-4k/tel/w50\endcsname{94.8}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/mae\endcsname{17.8}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/w20\endcsname{81.8}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr2e4/tel/w50\endcsname{95.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/mae\endcsname{16.7}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/w100\endcsname{98.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/w20\endcsname{81.7}
\expandafter\def\csname v@swb/ft-ts-post-10ms-lr5e3/tel/w50\endcsname{95.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/mae\endcsname{17.8}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/w20\endcsname{81.8}
\expandafter\def\csname v@swb/ft-ts-post-10ms-r64/tel/w50\endcsname{95.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/mae\endcsname{18.0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/w100\endcsname{98.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/w20\endcsname{81.9}
\expandafter\def\csname v@swb/ft-ts-post-10ms-rand/tel/w50\endcsname{95.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/mae\endcsname{17.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/w20\endcsname{81.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-round/tel/w50\endcsname{95.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/mae\endcsname{17.8}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/w100\endcsname{98.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/w20\endcsname{81.5}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s1/tel/w50\endcsname{95.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/mae\endcsname{17.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/w100\endcsname{98.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/w20\endcsname{81.6}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s2/tel/w50\endcsname{95.0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/mae\endcsname{17.7}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/w20\endcsname{81.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s3/tel/w50\endcsname{95.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/mae\endcsname{18.7}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/w100\endcsname{98.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/w20\endcsname{81.0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-s4/tel/w50\endcsname{95.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/mae\endcsname{15.7}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/w100\endcsname{98.5}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/w20\endcsname{82.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms-tn10/tel/w50\endcsname{95.6}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/mae\endcsname{18.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/w100\endcsname{98.1}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/w20\endcsname{81.7}
\expandafter\def\csname v@swb/ft-ts-post-10ms/tel/w50\endcsname{95.1}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/mae\endcsname{17.3}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/w20\endcsname{81.2}
\expandafter\def\csname v@swb/ft-ts-post-5ms/tel/w50\endcsname{94.9}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/mae\endcsname{19.2}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/over500\endcsname{0.4}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/w100\endcsname{98.0}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/w20\endcsname{81.4}
\expandafter\def\csname v@swb/ft-ts-post-s1/tel/w50\endcsname{95.1}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/mae\endcsname{18.7}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/over500\endcsname{0.4}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/w100\endcsname{98.0}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/w20\endcsname{81.7}
\expandafter\def\csname v@swb/ft-ts-post-s2/tel/w50\endcsname{95.2}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/mae\endcsname{18.6}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/w100\endcsname{98.0}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/w20\endcsname{81.7}
\expandafter\def\csname v@swb/ft-ts-post-s3/tel/w50\endcsname{95.2}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/mae\endcsname{17.5}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/w100\endcsname{98.4}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/w20\endcsname{82.1}
\expandafter\def\csname v@swb/ft-ts-post-s4/tel/w50\endcsname{95.5}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/mae\endcsname{18.7}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/w100\endcsname{98.1}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/w20\endcsname{81.5}
\expandafter\def\csname v@swb/ft-ts-post-sidon-s1/tel/w50\endcsname{95.5}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/mae\endcsname{16.8}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/w100\endcsname{98.4}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/w20\endcsname{82.2}
\expandafter\def\csname v@swb/ft-ts-post-sidon/tel/w50\endcsname{95.6}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/mae\endcsname{16.5}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/w100\endcsname{98.5}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/w20\endcsname{82.3}
\expandafter\def\csname v@swb/ft-ts-post-tn10-s1/tel/w50\endcsname{95.7}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/mae\endcsname{16.3}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/w100\endcsname{98.5}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/w20\endcsname{82.2}
\expandafter\def\csname v@swb/ft-ts-post-tn10/tel/w50\endcsname{95.8}
\expandafter\def\csname v@swb/ft-ts-post/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-post/tel/mae\endcsname{18.0}
\expandafter\def\csname v@swb/ft-ts-post/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-post/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-post/tel/w100\endcsname{98.1}
\expandafter\def\csname v@swb/ft-ts-post/tel/w20\endcsname{81.9}
\expandafter\def\csname v@swb/ft-ts-post/tel/w50\endcsname{95.2}
\expandafter\def\csname v@swb/ft-ts-r128/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-r128/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-r128/tel/mae\endcsname{23.9}
\expandafter\def\csname v@swb/ft-ts-r128/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-r128/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-r128/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-r128/tel/w20\endcsname{80.1}
\expandafter\def\csname v@swb/ft-ts-r128/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-r16/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-r16/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-r16/tel/mae\endcsname{23.1}
\expandafter\def\csname v@swb/ft-ts-r16/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-r16/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-r16/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-r16/tel/w20\endcsname{80.9}
\expandafter\def\csname v@swb/ft-ts-r16/tel/w50\endcsname{93.9}
\expandafter\def\csname v@swb/ft-ts-r64/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-r64/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-r64/tel/mae\endcsname{24.8}
\expandafter\def\csname v@swb/ft-ts-r64/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-r64/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-r64/tel/w100\endcsname{96.3}
\expandafter\def\csname v@swb/ft-ts-r64/tel/w20\endcsname{80.2}
\expandafter\def\csname v@swb/ft-ts-r64/tel/w50\endcsname{93.4}
\expandafter\def\csname v@swb/ft-ts-r8/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-r8/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-r8/tel/mae\endcsname{22.6}
\expandafter\def\csname v@swb/ft-ts-r8/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-r8/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-r8/tel/w100\endcsname{97.0}
\expandafter\def\csname v@swb/ft-ts-r8/tel/w20\endcsname{81.0}
\expandafter\def\csname v@swb/ft-ts-r8/tel/w50\endcsname{94.0}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/mae\endcsname{23.9}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/w20\endcsname{79.9}
\expandafter\def\csname v@swb/ft-ts-round-s1/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-round/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-round/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-round/tel/mae\endcsname{23.2}
\expandafter\def\csname v@swb/ft-ts-round/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-round/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-round/tel/w100\endcsname{96.9}
\expandafter\def\csname v@swb/ft-ts-round/tel/w20\endcsname{80.2}
\expandafter\def\csname v@swb/ft-ts-round/tel/w50\endcsname{94.0}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/mae\endcsname{16.1}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/w100\endcsname{98.7}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/w20\endcsname{82.9}
\expandafter\def\csname v@swb/ft-ts-s6-final-s1/tel/w50\endcsname{96.0}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/mae\endcsname{16.2}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/w100\endcsname{98.7}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/w20\endcsname{82.8}
\expandafter\def\csname v@swb/ft-ts-s6-final/tel/w50\endcsname{96.0}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/mae\endcsname{19.0}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/w100\endcsname{98.0}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/w20\endcsname{81.4}
\expandafter\def\csname v@swb/ft-ts-s6-post-s1/tel/w50\endcsname{95.0}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/mae\endcsname{18.2}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/w20\endcsname{81.7}
\expandafter\def\csname v@swb/ft-ts-s6-post/tel/w50\endcsname{95.3}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/mae\endcsname{19.3}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/over500\endcsname{0.4}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/w100\endcsname{98.0}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/w20\endcsname{81.6}
\expandafter\def\csname v@swb/ft-ts-s6-sidon-s1/tel/w50\endcsname{95.4}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/mae\endcsname{16.1}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/w100\endcsname{98.5}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/w20\endcsname{82.4}
\expandafter\def\csname v@swb/ft-ts-s6-sidon/tel/w50\endcsname{95.7}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/mae\endcsname{23.6}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/w20\endcsname{80.4}
\expandafter\def\csname v@swb/ft-ts-seed1/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/mae\endcsname{23.2}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/w20\endcsname{80.9}
\expandafter\def\csname v@swb/ft-ts-seed2/tel/w50\endcsname{93.9}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/mae\endcsname{23.1}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/w20\endcsname{80.9}
\expandafter\def\csname v@swb/ft-ts-seed3/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/mae\endcsname{23.1}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/w100\endcsname{96.7}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/w20\endcsname{80.8}
\expandafter\def\csname v@swb/ft-ts-seed4/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/mae\endcsname{21.8}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/w100\endcsname{97.0}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/w20\endcsname{80.6}
\expandafter\def\csname v@swb/ft-ts-tn10-s1/tel/w50\endcsname{94.2}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/mae\endcsname{22.0}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/w100\endcsname{97.0}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/w20\endcsname{81.3}
\expandafter\def\csname v@swb/ft-ts-tn10/tel/w50\endcsname{94.3}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/mae\endcsname{22.4}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/w100\endcsname{97.0}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/w20\endcsname{81.2}
\expandafter\def\csname v@swb/ft-ts-tn20/tel/w50\endcsname{94.1}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/mae\endcsname{15.8}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/w100\endcsname{98.6}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/w20\endcsname{82.1}
\expandafter\def\csname v@swb/ft-ts-turbo-final-s1/tel/w50\endcsname{95.7}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/mae\endcsname{16.7}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/w100\endcsname{98.5}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/w20\endcsname{81.9}
\expandafter\def\csname v@swb/ft-ts-turbo-final/tel/w50\endcsname{95.6}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/mae\endcsname{16.6}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/w100\endcsname{98.4}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/w20\endcsname{81.4}
\expandafter\def\csname v@swb/ft-ts-turbo-post-10ms/tel/w50\endcsname{95.4}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/mae\endcsname{18.2}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/w100\endcsname{97.9}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/w20\endcsname{81.4}
\expandafter\def\csname v@swb/ft-ts-turbo-post-s1/tel/w50\endcsname{95.0}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/mae\endcsname{17.3}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/w20\endcsname{81.9}
\expandafter\def\csname v@swb/ft-ts-turbo-post/tel/w50\endcsname{95.3}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/mae\endcsname{23.2}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/w20\endcsname{80.3}
\expandafter\def\csname v@swb/ft-ts-turbo-s1/tel/w50\endcsname{93.9}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/mae\endcsname{23.7}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/w20\endcsname{80.4}
\expandafter\def\csname v@swb/ft-ts-turbo-s2/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/mae\endcsname{22.4}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/w100\endcsname{97.0}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/w20\endcsname{80.5}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10-s1/tel/w50\endcsname{94.1}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/mae\endcsname{22.2}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/w20\endcsname{80.9}
\expandafter\def\csname v@swb/ft-ts-turbo-tn10/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/mae\endcsname{22.5}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/over500\endcsname{0.6}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/w100\endcsname{96.8}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/w20\endcsname{80.7}
\expandafter\def\csname v@swb/ft-ts-turbo/tel/w50\endcsname{94.1}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/mae\endcsname{15.8}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/w100\endcsname{98.7}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/w20\endcsname{82.8}
\expandafter\def\csname v@swb/ft-ts-v3-final-s1/tel/w50\endcsname{96.1}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/mae\endcsname{16.0}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/over500\endcsname{0.1}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/w100\endcsname{98.7}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/w20\endcsname{82.6}
\expandafter\def\csname v@swb/ft-ts-v3-final/tel/w50\endcsname{95.9}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/mae\endcsname{17.0}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/w100\endcsname{98.2}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/w20\endcsname{81.9}
\expandafter\def\csname v@swb/ft-ts-v3-post-10ms/tel/w50\endcsname{95.4}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/mae\endcsname{19.7}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/w100\endcsname{97.8}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/w20\endcsname{81.1}
\expandafter\def\csname v@swb/ft-ts-v3-post-s1/tel/w50\endcsname{95.0}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/mae\endcsname{16.9}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/over500\endcsname{0.2}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/w100\endcsname{98.3}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/w20\endcsname{82.1}
\expandafter\def\csname v@swb/ft-ts-v3-post/tel/w50\endcsname{95.5}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/mae\endcsname{24.1}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/w20\endcsname{80.3}
\expandafter\def\csname v@swb/ft-ts-v3-s1/tel/w50\endcsname{93.6}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/mae\endcsname{24.9}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/w100\endcsname{96.4}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/w20\endcsname{80.4}
\expandafter\def\csname v@swb/ft-ts-v3-s2/tel/w50\endcsname{93.7}
\expandafter\def\csname v@swb/ft-ts-v3/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-v3/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-v3/tel/mae\endcsname{23.5}
\expandafter\def\csname v@swb/ft-ts-v3/tel/over500\endcsname{0.7}
\expandafter\def\csname v@swb/ft-ts-v3/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-v3/tel/w100\endcsname{96.6}
\expandafter\def\csname v@swb/ft-ts-v3/tel/w20\endcsname{80.4}
\expandafter\def\csname v@swb/ft-ts-v3/tel/w50\endcsname{93.8}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/ebias\endcsname{1}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/mae\endcsname{31.9}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/over500\endcsname{1.2}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/w100\endcsname{94.7}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/w20\endcsname{77.6}
\expandafter\def\csname v@swb/ft-ts-wt-s1/tel/w50\endcsname{91.7}
\expandafter\def\csname v@swb/ft-ts-wt/tel/ebias\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-wt/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/ft-ts-wt/tel/mae\endcsname{31.0}
\expandafter\def\csname v@swb/ft-ts-wt/tel/over500\endcsname{1.0}
\expandafter\def\csname v@swb/ft-ts-wt/tel/sbias\endcsname{2}
\expandafter\def\csname v@swb/ft-ts-wt/tel/w100\endcsname{94.9}
\expandafter\def\csname v@swb/ft-ts-wt/tel/w20\endcsname{77.9}
\expandafter\def\csname v@swb/ft-ts-wt/tel/w50\endcsname{91.8}
\expandafter\def\csname v@swb/hours\endcsname{0.61}
\expandafter\def\csname v@swb/mfa-arpa/tel/ebias\endcsname{0}
\expandafter\def\csname v@swb/mfa-arpa/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/mfa-arpa/tel/mae\endcsname{36.5}
\expandafter\def\csname v@swb/mfa-arpa/tel/over500\endcsname{1.1}
\expandafter\def\csname v@swb/mfa-arpa/tel/sbias\endcsname{0}
\expandafter\def\csname v@swb/mfa-arpa/tel/w100\endcsname{93.3}
\expandafter\def\csname v@swb/mfa-arpa/tel/w20\endcsname{64.2}
\expandafter\def\csname v@swb/mfa-arpa/tel/w50\endcsname{86.2}
\expandafter\def\csname v@swb/mfa-english/tel/ebias\endcsname{0}
\expandafter\def\csname v@swb/mfa-english/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/mfa-english/tel/mae\endcsname{40.5}
\expandafter\def\csname v@swb/mfa-english/tel/over500\endcsname{1.2}
\expandafter\def\csname v@swb/mfa-english/tel/sbias\endcsname{0}
\expandafter\def\csname v@swb/mfa-english/tel/w100\endcsname{91.7}
\expandafter\def\csname v@swb/mfa-english/tel/w20\endcsname{60.6}
\expandafter\def\csname v@swb/mfa-english/tel/w50\endcsname{83.5}
\expandafter\def\csname v@swb/mms-torchaudio/tel/ebias\endcsname{12}
\expandafter\def\csname v@swb/mms-torchaudio/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/mms-torchaudio/tel/mae\endcsname{47.8}
\expandafter\def\csname v@swb/mms-torchaudio/tel/over500\endcsname{0.5}
\expandafter\def\csname v@swb/mms-torchaudio/tel/sbias\endcsname{36}
\expandafter\def\csname v@swb/mms-torchaudio/tel/w100\endcsname{91.2}
\expandafter\def\csname v@swb/mms-torchaudio/tel/w20\endcsname{33.8}
\expandafter\def\csname v@swb/mms-torchaudio/tel/w50\endcsname{70.9}
\expandafter\def\csname v@swb/n-utt\endcsname{932}
\expandafter\def\csname v@swb/n-words\endcsname{6{,}828}
\expandafter\def\csname v@swb/qwen3fa/tel/ebias\endcsname{14}
\expandafter\def\csname v@swb/qwen3fa/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/qwen3fa/tel/mae\endcsname{42.3}
\expandafter\def\csname v@swb/qwen3fa/tel/over500\endcsname{0.3}
\expandafter\def\csname v@swb/qwen3fa/tel/sbias\endcsname{9}
\expandafter\def\csname v@swb/qwen3fa/tel/w100\endcsname{92.3}
\expandafter\def\csname v@swb/qwen3fa/tel/w20\endcsname{36.9}
\expandafter\def\csname v@swb/qwen3fa/tel/w50\endcsname{76.4}
\expandafter\def\csname v@swb/stablets/tel/ebias\endcsname{30}
\expandafter\def\csname v@swb/stablets/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/stablets/tel/mae\endcsname{67.2}
\expandafter\def\csname v@swb/stablets/tel/over500\endcsname{0.8}
\expandafter\def\csname v@swb/stablets/tel/sbias\endcsname{13}
\expandafter\def\csname v@swb/stablets/tel/w100\endcsname{82.3}
\expandafter\def\csname v@swb/stablets/tel/w20\endcsname{27.6}
\expandafter\def\csname v@swb/stablets/tel/w50\endcsname{58.9}
\expandafter\def\csname v@swb/sttapi/tel/ebias\endcsname{13}
\expandafter\def\csname v@swb/sttapi/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/sttapi/tel/mae\endcsname{46.9}
\expandafter\def\csname v@swb/sttapi/tel/over500\endcsname{0.4}
\expandafter\def\csname v@swb/sttapi/tel/sbias\endcsname{27}
\expandafter\def\csname v@swb/sttapi/tel/w100\endcsname{90.5}
\expandafter\def\csname v@swb/sttapi/tel/w20\endcsname{35.9}
\expandafter\def\csname v@swb/sttapi/tel/w50\endcsname{73.3}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/ebias\endcsname{7}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/mae\endcsname{54.6}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/over500\endcsname{0.8}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/sbias\endcsname{1}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/w100\endcsname{88.1}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/w20\endcsname{39.4}
\expandafter\def\csname v@swb/whisper-tm-cal/tel/w50\endcsname{75.2}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/ebias\endcsname{865}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/mae\endcsname{1342.6}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/over500\endcsname{72.1}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/sbias\endcsname{850}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/w100\endcsname{5.8}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/w20\endcsname{1.0}
\expandafter\def\csname v@swb/whisper-tm-cfg/tel/w50\endcsname{2.6}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/ebias\endcsname{112}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/mae\endcsname{147.3}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/over500\endcsname{2.3}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/sbias\endcsname{113}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/w100\endcsname{43.7}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/w20\endcsname{4.1}
\expandafter\def\csname v@swb/whisper-tm-oai/tel/w50\endcsname{15.1}
\expandafter\def\csname v@swb/whisperx/tel/ebias\endcsname{2}
\expandafter\def\csname v@swb/whisperx/tel/fail\endcsname{0}
\expandafter\def\csname v@swb/whisperx/tel/mae\endcsname{53.7}
\expandafter\def\csname v@swb/whisperx/tel/over500\endcsname{0.5}
\expandafter\def\csname v@swb/whisperx/tel/sbias\endcsname{51}
\expandafter\def\csname v@swb/whisperx/tel/w100\endcsname{90.6}
\expandafter\def\csname v@swb/whisperx/tel/w20\endcsname{28.2}
\expandafter\def\csname v@swb/whisperx/tel/w50\endcsname{62.5}
\expandafter\def\csname v@tel/clean/above4k\endcsname{64}
\expandafter\def\csname v@tel/clean/bw99\endcsname{2{,}266}
\expandafter\def\csname v@tel/clean/crest\endcsname{16.4}
\expandafter\def\csname v@tel/clean/dur\endcsname{2.5}
\expandafter\def\csname v@tel/clean/edge\endcsname{4{,}578}
\expandafter\def\csname v@tel/clean/edge-p10\endcsname{3{,}031}
\expandafter\def\csname v@tel/clean/floor\endcsname{$-$58}
\expandafter\def\csname v@tel/clean/inband-hi\endcsname{3{,}438}
\expandafter\def\csname v@tel/clean/inband-lo\endcsname{219}
\expandafter\def\csname v@tel/clean/level\endcsname{$-$30}
\expandafter\def\csname v@tel/clean/lf\endcsname{62}
\expandafter\def\csname v@tel/clean/ltas-dev\endcsname{2.2}
\expandafter\def\csname v@tel/clean/snr\endcsname{30.5}
\expandafter\def\csname v@tel/clean/snr-p10\endcsname{19.3}
\expandafter\def\csname v@tel/clean/snr-p90\endcsname{42.6}
\expandafter\def\csname v@tel/clean/speech\endcsname{82}
\expandafter\def\csname v@tel/clean/tilt\endcsname{$-$9.1}
\expandafter\def\csname v@tel/codecs/above4k\endcsname{3}
\expandafter\def\csname v@tel/codecs/bw99\endcsname{2{,}281}
\expandafter\def\csname v@tel/codecs/crest\endcsname{17.8}
\expandafter\def\csname v@tel/codecs/dur\endcsname{2.5}
\expandafter\def\csname v@tel/codecs/edge\endcsname{3{,}312}
\expandafter\def\csname v@tel/codecs/edge-p10\endcsname{2{,}841}
\expandafter\def\csname v@tel/codecs/floor\endcsname{$-$63}
\expandafter\def\csname v@tel/codecs/inband-hi\endcsname{3{,}938}
\expandafter\def\csname v@tel/codecs/inband-lo\endcsname{312}
\expandafter\def\csname v@tel/codecs/level\endcsname{$-$33}
\expandafter\def\csname v@tel/codecs/lf\endcsname{250}
\expandafter\def\csname v@tel/codecs/ltas-dev\endcsname{2.1}
\expandafter\def\csname v@tel/codecs/snr\endcsname{31.5}
\expandafter\def\csname v@tel/codecs/snr-p10\endcsname{19.0}
\expandafter\def\csname v@tel/codecs/snr-p90\endcsname{45.3}
\expandafter\def\csname v@tel/codecs/speech\endcsname{77}
\expandafter\def\csname v@tel/codecs/tilt\endcsname{$-$9.1}
\expandafter\def\csname v@tel/lag/dropped-pct\endcsname{3.8}
\expandafter\def\csname v@tel/lag/kept\endcsname{47{,}287}
\expandafter\def\csname v@tel/lag/late-pct\endcsname{37}
\expandafter\def\csname v@tel/lag/max\endcsname{136.5}
\expandafter\def\csname v@tel/lag/median\endcsname{0}
\expandafter\def\csname v@tel/lag/over5-pct\endcsname{8.3}
\expandafter\def\csname v@tel/lag/p99\endcsname{33}
\expandafter\def\csname v@tel/lag/residual-n\endcsname{7}
\expandafter\def\csname v@tel/lag/rows\endcsname{49{,}170}
\expandafter\def\csname v@tel/ltas-dev-hi\endcsname{2.3}
\expandafter\def\csname v@tel/ltas-dev-lo\endcsname{2.1}
\expandafter\def\csname v@tel/n-windows\endcsname{1{,}000}
\expandafter\def\csname v@tel/real/above4k\endcsname{0}
\expandafter\def\csname v@tel/real/bw99\endcsname{1{,}844}
\expandafter\def\csname v@tel/real/crest\endcsname{18.9}
\expandafter\def\csname v@tel/real/dur\endcsname{29.9}
\expandafter\def\csname v@tel/real/edge\endcsname{3{,}281}
\expandafter\def\csname v@tel/real/edge-p10\endcsname{2{,}656}
\expandafter\def\csname v@tel/real/floor\endcsname{$-$81}
\expandafter\def\csname v@tel/real/level\endcsname{$-$26}
\expandafter\def\csname v@tel/real/lf\endcsname{94}
\expandafter\def\csname v@tel/real/n-calls\endcsname{58}
\expandafter\def\csname v@tel/real/n-legs\endcsname{116}
\expandafter\def\csname v@tel/real/snr\endcsname{50.9}
\expandafter\def\csname v@tel/real/snr-p10\endcsname{38.6}
\expandafter\def\csname v@tel/real/snr-p90\endcsname{65.2}
\expandafter\def\csname v@tel/real/speech\endcsname{38}
\expandafter\def\csname v@tel/real/tilt\endcsname{$-$10.7}
\expandafter\def\csname v@tel/sidon/above4k\endcsname{8}
\expandafter\def\csname v@tel/sidon/bw99\endcsname{1{,}844}
\expandafter\def\csname v@tel/sidon/crest\endcsname{17.1}
\expandafter\def\csname v@tel/sidon/dur\endcsname{2.5}
\expandafter\def\csname v@tel/sidon/edge\endcsname{3{,}000}
\expandafter\def\csname v@tel/sidon/edge-p10\endcsname{2{,}188}
\expandafter\def\csname v@tel/sidon/floor\endcsname{$-$50}
\expandafter\def\csname v@tel/sidon/floor-rise\endcsname{7}
\expandafter\def\csname v@tel/sidon/inband-hi\endcsname{3{,}844}
\expandafter\def\csname v@tel/sidon/inband-lo\endcsname{250}
\expandafter\def\csname v@tel/sidon/level\endcsname{$-$19}
\expandafter\def\csname v@tel/sidon/level-rise\endcsname{11}
\expandafter\def\csname v@tel/sidon/lf\endcsname{156}
\expandafter\def\csname v@tel/sidon/ltas-dev\endcsname{2.3}
\expandafter\def\csname v@tel/sidon/n\endcsname{959}
\expandafter\def\csname v@tel/sidon/snr\endcsname{33.2}
\expandafter\def\csname v@tel/sidon/snr-p10\endcsname{19.6}
\expandafter\def\csname v@tel/sidon/snr-p90\endcsname{46.1}
\expandafter\def\csname v@tel/sidon/speech\endcsname{78}
\expandafter\def\csname v@tel/sidon/tilt\endcsname{$-$10.4}
\expandafter\def\csname v@timit/cfa-edges/clean/ebias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/clean/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/clean/mae\endcsname{29.2}
\expandafter\def\csname v@timit/cfa-edges/clean/median\endcsname{22.5}
\expandafter\def\csname v@timit/cfa-edges/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-edges/clean/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-edges/clean/sbias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/clean/sbias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/clean/w10\endcsname{23.3}
\expandafter\def\csname v@timit/cfa-edges/clean/w100\endcsname{97.1}
\expandafter\def\csname v@timit/cfa-edges/clean/w20\endcsname{45.5}
\expandafter\def\csname v@timit/cfa-edges/clean/w50\endcsname{85.9}
\expandafter\def\csname v@timit/cfa-edges/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/cfa-edges/g711u/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/cfa-edges/g711u/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/cfa-edges/g711u/ebias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/g711u/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g711u/mae\endcsname{29.8}
\expandafter\def\csname v@timit/cfa-edges/g711u/median\endcsname{22.5}
\expandafter\def\csname v@timit/cfa-edges/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-edges/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-edges/g711u/sbias\endcsname{11}
\expandafter\def\csname v@timit/cfa-edges/g711u/sbias-signed\endcsname{$+11$}
\expandafter\def\csname v@timit/cfa-edges/g711u/w10\endcsname{23.2}
\expandafter\def\csname v@timit/cfa-edges/g711u/w100\endcsname{96.6}
\expandafter\def\csname v@timit/cfa-edges/g711u/w20\endcsname{45.4}
\expandafter\def\csname v@timit/cfa-edges/g711u/w50\endcsname{85.3}
\expandafter\def\csname v@timit/cfa-edges/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/cfa-edges/g726/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/cfa-edges/g726/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/cfa-edges/g726/ebias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/g726/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/g726/mae\endcsname{29.8}
\expandafter\def\csname v@timit/cfa-edges/g726/median\endcsname{22.5}
\expandafter\def\csname v@timit/cfa-edges/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-edges/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-edges/g726/sbias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/g726/sbias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/g726/w10\endcsname{23.4}
\expandafter\def\csname v@timit/cfa-edges/g726/w100\endcsname{96.6}
\expandafter\def\csname v@timit/cfa-edges/g726/w20\endcsname{45.4}
\expandafter\def\csname v@timit/cfa-edges/g726/w50\endcsname{85.4}
\expandafter\def\csname v@timit/cfa-edges/gsm/dmae\endcsname{1.7}
\expandafter\def\csname v@timit/cfa-edges/gsm/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/cfa-edges/gsm/dw50\endcsname{1.5}
\expandafter\def\csname v@timit/cfa-edges/gsm/ebias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/gsm/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/gsm/mae\endcsname{30.9}
\expandafter\def\csname v@timit/cfa-edges/gsm/median\endcsname{22.5}
\expandafter\def\csname v@timit/cfa-edges/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-edges/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-edges/gsm/sbias\endcsname{11}
\expandafter\def\csname v@timit/cfa-edges/gsm/sbias-signed\endcsname{$+11$}
\expandafter\def\csname v@timit/cfa-edges/gsm/w10\endcsname{22.7}
\expandafter\def\csname v@timit/cfa-edges/gsm/w100\endcsname{96.2}
\expandafter\def\csname v@timit/cfa-edges/gsm/w20\endcsname{44.5}
\expandafter\def\csname v@timit/cfa-edges/gsm/w50\endcsname{84.3}
\expandafter\def\csname v@timit/cfa-edges/mp3/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/cfa-edges/mp3/dw20\endcsname{0.3}
\expandafter\def\csname v@timit/cfa-edges/mp3/dw50\endcsname{0.9}
\expandafter\def\csname v@timit/cfa-edges/mp3/ebias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/mp3/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/mp3/mae\endcsname{30.4}
\expandafter\def\csname v@timit/cfa-edges/mp3/median\endcsname{22.5}
\expandafter\def\csname v@timit/cfa-edges/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-edges/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-edges/mp3/sbias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/mp3/sbias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/mp3/w10\endcsname{23.2}
\expandafter\def\csname v@timit/cfa-edges/mp3/w100\endcsname{96.4}
\expandafter\def\csname v@timit/cfa-edges/mp3/w20\endcsname{45.2}
\expandafter\def\csname v@timit/cfa-edges/mp3/w50\endcsname{84.9}
\expandafter\def\csname v@timit/cfa-edges/opus/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/cfa-edges/opus/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/cfa-edges/opus/dw50\endcsname{0.9}
\expandafter\def\csname v@timit/cfa-edges/opus/ebias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/opus/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/opus/mae\endcsname{30.2}
\expandafter\def\csname v@timit/cfa-edges/opus/median\endcsname{22.5}
\expandafter\def\csname v@timit/cfa-edges/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-edges/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-edges/opus/sbias\endcsname{11}
\expandafter\def\csname v@timit/cfa-edges/opus/sbias-signed\endcsname{$+11$}
\expandafter\def\csname v@timit/cfa-edges/opus/w10\endcsname{22.9}
\expandafter\def\csname v@timit/cfa-edges/opus/w100\endcsname{96.4}
\expandafter\def\csname v@timit/cfa-edges/opus/w20\endcsname{45.0}
\expandafter\def\csname v@timit/cfa-edges/opus/w50\endcsname{84.9}
\expandafter\def\csname v@timit/cfa-edges/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/cfa-edges/pcm/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/cfa-edges/pcm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-edges/pcm/ebias\endcsname{10}
\expandafter\def\csname v@timit/cfa-edges/pcm/ebias-signed\endcsname{$+10$}
\expandafter\def\csname v@timit/cfa-edges/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-edges/pcm/mae\endcsname{29.8}
\expandafter\def\csname v@timit/cfa-edges/pcm/median\endcsname{22.5}
\expandafter\def\csname v@timit/cfa-edges/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-edges/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-edges/pcm/sbias\endcsname{11}
\expandafter\def\csname v@timit/cfa-edges/pcm/sbias-signed\endcsname{$+11$}
\expandafter\def\csname v@timit/cfa-edges/pcm/w10\endcsname{23.1}
\expandafter\def\csname v@timit/cfa-edges/pcm/w100\endcsname{96.6}
\expandafter\def\csname v@timit/cfa-edges/pcm/w20\endcsname{45.3}
\expandafter\def\csname v@timit/cfa-edges/pcm/w50\endcsname{85.4}
\expandafter\def\csname v@timit/cfa-segment/ce/dmae\endcsname{11.3}
\expandafter\def\csname v@timit/cfa-segment/ce/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/cfa-segment/ce/dw50\endcsname{3.9}
\expandafter\def\csname v@timit/cfa-segment/ce/ebias\endcsname{20}
\expandafter\def\csname v@timit/cfa-segment/ce/ebias-signed\endcsname{$-20$}
\expandafter\def\csname v@timit/cfa-segment/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/ce/mae\endcsname{58.1}
\expandafter\def\csname v@timit/cfa-segment/ce/median\endcsname{36.4}
\expandafter\def\csname v@timit/cfa-segment/ce/over500\endcsname{1.0}
\expandafter\def\csname v@timit/cfa-segment/ce/rtf\endcsname{0.003}
\expandafter\def\csname v@timit/cfa-segment/ce/sbias\endcsname{37}
\expandafter\def\csname v@timit/cfa-segment/ce/sbias-signed\endcsname{$+37$}
\expandafter\def\csname v@timit/cfa-segment/ce/w10\endcsname{14.8}
\expandafter\def\csname v@timit/cfa-segment/ce/w100\endcsname{87.4}
\expandafter\def\csname v@timit/cfa-segment/ce/w20\endcsname{29.2}
\expandafter\def\csname v@timit/cfa-segment/ce/w50\endcsname{64.6}
\expandafter\def\csname v@timit/cfa-segment/clean/ebias\endcsname{22}
\expandafter\def\csname v@timit/cfa-segment/clean/ebias-signed\endcsname{$-22$}
\expandafter\def\csname v@timit/cfa-segment/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/clean/mae\endcsname{46.8}
\expandafter\def\csname v@timit/cfa-segment/clean/median\endcsname{33.1}
\expandafter\def\csname v@timit/cfa-segment/clean/over500\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-segment/clean/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-segment/clean/sbias\endcsname{34}
\expandafter\def\csname v@timit/cfa-segment/clean/sbias-signed\endcsname{$+34$}
\expandafter\def\csname v@timit/cfa-segment/clean/w10\endcsname{15.5}
\expandafter\def\csname v@timit/cfa-segment/clean/w100\endcsname{91.5}
\expandafter\def\csname v@timit/cfa-segment/clean/w20\endcsname{31.0}
\expandafter\def\csname v@timit/cfa-segment/clean/w50\endcsname{68.5}
\expandafter\def\csname v@timit/cfa-segment/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/cfa-segment/g711u/dw20\endcsname{-0.1}
\expandafter\def\csname v@timit/cfa-segment/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/cfa-segment/g711u/ebias\endcsname{21}
\expandafter\def\csname v@timit/cfa-segment/g711u/ebias-signed\endcsname{$-21$}
\expandafter\def\csname v@timit/cfa-segment/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g711u/mae\endcsname{47.2}
\expandafter\def\csname v@timit/cfa-segment/g711u/median\endcsname{33.1}
\expandafter\def\csname v@timit/cfa-segment/g711u/over500\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-segment/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-segment/g711u/sbias\endcsname{34}
\expandafter\def\csname v@timit/cfa-segment/g711u/sbias-signed\endcsname{$+34$}
\expandafter\def\csname v@timit/cfa-segment/g711u/w10\endcsname{15.7}
\expandafter\def\csname v@timit/cfa-segment/g711u/w100\endcsname{91.2}
\expandafter\def\csname v@timit/cfa-segment/g711u/w20\endcsname{31.1}
\expandafter\def\csname v@timit/cfa-segment/g711u/w50\endcsname{68.5}
\expandafter\def\csname v@timit/cfa-segment/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/cfa-segment/g726/dw20\endcsname{-0.2}
\expandafter\def\csname v@timit/cfa-segment/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/cfa-segment/g726/ebias\endcsname{21}
\expandafter\def\csname v@timit/cfa-segment/g726/ebias-signed\endcsname{$-21$}
\expandafter\def\csname v@timit/cfa-segment/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/g726/mae\endcsname{47.3}
\expandafter\def\csname v@timit/cfa-segment/g726/median\endcsname{33.0}
\expandafter\def\csname v@timit/cfa-segment/g726/over500\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-segment/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-segment/g726/sbias\endcsname{34}
\expandafter\def\csname v@timit/cfa-segment/g726/sbias-signed\endcsname{$+34$}
\expandafter\def\csname v@timit/cfa-segment/g726/w10\endcsname{15.6}
\expandafter\def\csname v@timit/cfa-segment/g726/w100\endcsname{91.1}
\expandafter\def\csname v@timit/cfa-segment/g726/w20\endcsname{31.2}
\expandafter\def\csname v@timit/cfa-segment/g726/w50\endcsname{68.3}
\expandafter\def\csname v@timit/cfa-segment/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/cfa-segment/gsm/dw20\endcsname{-0.3}
\expandafter\def\csname v@timit/cfa-segment/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/cfa-segment/gsm/ebias\endcsname{20}
\expandafter\def\csname v@timit/cfa-segment/gsm/ebias-signed\endcsname{$-20$}
\expandafter\def\csname v@timit/cfa-segment/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/gsm/mae\endcsname{48.0}
\expandafter\def\csname v@timit/cfa-segment/gsm/median\endcsname{33.1}
\expandafter\def\csname v@timit/cfa-segment/gsm/over500\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-segment/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-segment/gsm/sbias\endcsname{34}
\expandafter\def\csname v@timit/cfa-segment/gsm/sbias-signed\endcsname{$+34$}
\expandafter\def\csname v@timit/cfa-segment/gsm/w10\endcsname{15.7}
\expandafter\def\csname v@timit/cfa-segment/gsm/w100\endcsname{90.5}
\expandafter\def\csname v@timit/cfa-segment/gsm/w20\endcsname{31.4}
\expandafter\def\csname v@timit/cfa-segment/gsm/w50\endcsname{68.2}
\expandafter\def\csname v@timit/cfa-segment/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/cfa-segment/mp3/dw20\endcsname{-0.1}
\expandafter\def\csname v@timit/cfa-segment/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/cfa-segment/mp3/ebias\endcsname{21}
\expandafter\def\csname v@timit/cfa-segment/mp3/ebias-signed\endcsname{$-21$}
\expandafter\def\csname v@timit/cfa-segment/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/mp3/mae\endcsname{47.6}
\expandafter\def\csname v@timit/cfa-segment/mp3/median\endcsname{33.1}
\expandafter\def\csname v@timit/cfa-segment/mp3/over500\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-segment/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-segment/mp3/sbias\endcsname{34}
\expandafter\def\csname v@timit/cfa-segment/mp3/sbias-signed\endcsname{$+34$}
\expandafter\def\csname v@timit/cfa-segment/mp3/w10\endcsname{15.8}
\expandafter\def\csname v@timit/cfa-segment/mp3/w100\endcsname{90.8}
\expandafter\def\csname v@timit/cfa-segment/mp3/w20\endcsname{31.1}
\expandafter\def\csname v@timit/cfa-segment/mp3/w50\endcsname{68.3}
\expandafter\def\csname v@timit/cfa-segment/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/cfa-segment/opus/dw20\endcsname{-0.2}
\expandafter\def\csname v@timit/cfa-segment/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/cfa-segment/opus/ebias\endcsname{20}
\expandafter\def\csname v@timit/cfa-segment/opus/ebias-signed\endcsname{$-20$}
\expandafter\def\csname v@timit/cfa-segment/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/opus/mae\endcsname{47.6}
\expandafter\def\csname v@timit/cfa-segment/opus/median\endcsname{33.1}
\expandafter\def\csname v@timit/cfa-segment/opus/over500\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-segment/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-segment/opus/sbias\endcsname{34}
\expandafter\def\csname v@timit/cfa-segment/opus/sbias-signed\endcsname{$+34$}
\expandafter\def\csname v@timit/cfa-segment/opus/w10\endcsname{15.7}
\expandafter\def\csname v@timit/cfa-segment/opus/w100\endcsname{90.9}
\expandafter\def\csname v@timit/cfa-segment/opus/w20\endcsname{31.2}
\expandafter\def\csname v@timit/cfa-segment/opus/w50\endcsname{68.4}
\expandafter\def\csname v@timit/cfa-segment/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/cfa-segment/pcm/dw20\endcsname{-0.1}
\expandafter\def\csname v@timit/cfa-segment/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/cfa-segment/pcm/ebias\endcsname{21}
\expandafter\def\csname v@timit/cfa-segment/pcm/ebias-signed\endcsname{$-21$}
\expandafter\def\csname v@timit/cfa-segment/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/cfa-segment/pcm/mae\endcsname{47.1}
\expandafter\def\csname v@timit/cfa-segment/pcm/median\endcsname{32.9}
\expandafter\def\csname v@timit/cfa-segment/pcm/over500\endcsname{0.4}
\expandafter\def\csname v@timit/cfa-segment/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/cfa-segment/pcm/sbias\endcsname{34}
\expandafter\def\csname v@timit/cfa-segment/pcm/sbias-signed\endcsname{$+34$}
\expandafter\def\csname v@timit/cfa-segment/pcm/w10\endcsname{15.7}
\expandafter\def\csname v@timit/cfa-segment/pcm/w100\endcsname{91.2}
\expandafter\def\csname v@timit/cfa-segment/pcm/w20\endcsname{31.1}
\expandafter\def\csname v@timit/cfa-segment/pcm/w50\endcsname{68.5}
\expandafter\def\csname v@timit/clean/mae-max\endcsname{77.5}
\expandafter\def\csname v@timit/clean/mae-min\endcsname{19.1}
\expandafter\def\csname v@timit/clean/mms-mae-max\endcsname{46.8}
\expandafter\def\csname v@timit/clean/mms-mae-min\endcsname{29.2}
\expandafter\def\csname v@timit/clean/n-aligners\endcsname{9}
\expandafter\def\csname v@timit/clean/rtf-max\endcsname{0.044}
\expandafter\def\csname v@timit/clean/rtf-min\endcsname{0.007}
\expandafter\def\csname v@timit/clean/speedup-min\endcsname{23}
\expandafter\def\csname v@timit/clean/w20-max\endcsname{68.2}
\expandafter\def\csname v@timit/clean/w20-min\endcsname{20.6}
\expandafter\def\csname v@timit/clean/w50-max\endcsname{91.9}
\expandafter\def\csname v@timit/clean/w50-min\endcsname{47.3}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/mae\endcsname{17.7}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/median\endcsname{10.0}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/rtf\endcsname{0.002}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/w10\endcsname{49.9}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/w20\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ctcm-full/amrnb/w50\endcsname{92.5}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/mae\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/median\endcsname{9.6}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/w10\endcsname{51.4}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/w20\endcsname{74.0}
\expandafter\def\csname v@timit/ft-ctcm-full/clean/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/dmae\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/dw20\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/dw50\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/mae\endcsname{16.7}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/w10\endcsname{51.2}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/w20\endcsname{74.3}
\expandafter\def\csname v@timit/ft-ctcm-full/g711u/w50\endcsname{93.4}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/dw20\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/mae\endcsname{17.1}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/median\endcsname{9.9}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/w10\endcsname{50.3}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/w20\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ctcm-full/g723/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/dmae\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/dw20\endcsname{-1.3}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/mae\endcsname{16.6}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/median\endcsname{9.4}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/w10\endcsname{51.9}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/w20\endcsname{75.4}
\expandafter\def\csname v@timit/ft-ctcm-full/g726/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/dw50\endcsname{-0.4}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/mae\endcsname{17.0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/median\endcsname{10.0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/w10\endcsname{49.8}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/w20\endcsname{73.9}
\expandafter\def\csname v@timit/ft-ctcm-full/gsm/w50\endcsname{93.5}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/mae\endcsname{17.2}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/median\endcsname{10.1}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/w10\endcsname{49.6}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/w20\endcsname{73.2}
\expandafter\def\csname v@timit/ft-ctcm-full/mp3/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/dmae\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/dw20\endcsname{-0.4}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/mae\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/w10\endcsname{51.1}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/w20\endcsname{74.4}
\expandafter\def\csname v@timit/ft-ctcm-full/opus/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/dmae\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/dw20\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/mae\endcsname{16.8}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/median\endcsname{9.6}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/w10\endcsname{51.4}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/w20\endcsname{74.2}
\expandafter\def\csname v@timit/ft-ctcm-full/pcm/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/mae\endcsname{17.9}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/median\endcsname{10.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/rtf\endcsname{0.002}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/w10\endcsname{49.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/w20\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ctcm-lora/amrnb/w50\endcsname{92.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/mae\endcsname{17.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/rtf\endcsname{0.002}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/w10\endcsname{51.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/w20\endcsname{74.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/clean/w50\endcsname{92.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/dmae\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/mae\endcsname{17.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/median\endcsname{9.9}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/w10\endcsname{50.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/w20\endcsname{73.9}
\expandafter\def\csname v@timit/ft-ctcm-lora/g711u/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/mae\endcsname{17.5}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/median\endcsname{10.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/w10\endcsname{49.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/w20\endcsname{73.4}
\expandafter\def\csname v@timit/ft-ctcm-lora/g723/w50\endcsname{92.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/dmae\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/dw20\endcsname{-0.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/mae\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/w10\endcsname{51.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/w20\endcsname{74.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/g726/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/dw50\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/mae\endcsname{17.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/median\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/w10\endcsname{49.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/w20\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/gsm/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/mae\endcsname{17.6}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/median\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/w10\endcsname{48.8}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/w20\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ctcm-lora/mp3/w50\endcsname{92.9}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/mae\endcsname{17.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/median\endcsname{9.9}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/w10\endcsname{50.2}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/w20\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/opus/w50\endcsname{92.8}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/dmae\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/mae\endcsname{17.1}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/median\endcsname{9.8}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/rtf\endcsname{0.001}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/sbias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/w10\endcsname{50.5}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/w20\endcsname{73.8}
\expandafter\def\csname v@timit/ft-ctcm-lora/pcm/w50\endcsname{92.8}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/dmae\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/dw50\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/mae\endcsname{18.0}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/w10\endcsname{51.1}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/w100\endcsname{98.0}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/w20\endcsname{74.2}
\expandafter\def\csname v@timit/ft-ctcw-full/amrnb/w50\endcsname{92.2}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/mae\endcsname{16.2}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/median\endcsname{9.1}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/w10\endcsname{53.5}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/w20\endcsname{76.5}
\expandafter\def\csname v@timit/ft-ctcw-full/clean/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/mae\endcsname{16.4}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/median\endcsname{9.2}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/w10\endcsname{53.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/w20\endcsname{75.7}
\expandafter\def\csname v@timit/ft-ctcw-full/g711u/w50\endcsname{93.4}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/mae\endcsname{16.7}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/median\endcsname{9.3}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/w10\endcsname{52.5}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/w20\endcsname{75.8}
\expandafter\def\csname v@timit/ft-ctcw-full/g723/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/dmae\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/dw20\endcsname{-0.5}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/mae\endcsname{16.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/median\endcsname{8.7}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/w10\endcsname{55.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/w20\endcsname{77.0}
\expandafter\def\csname v@timit/ft-ctcw-full/g726/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/mae\endcsname{16.7}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/w10\endcsname{51.0}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/w20\endcsname{74.9}
\expandafter\def\csname v@timit/ft-ctcw-full/gsm/w50\endcsname{93.4}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/mae\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/median\endcsname{9.6}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/w10\endcsname{51.2}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/w20\endcsname{74.3}
\expandafter\def\csname v@timit/ft-ctcw-full/mp3/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/mae\endcsname{16.3}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/median\endcsname{9.2}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/w10\endcsname{52.8}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/w20\endcsname{76.3}
\expandafter\def\csname v@timit/ft-ctcw-full/opus/w50\endcsname{93.4}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/dw20\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/mae\endcsname{16.3}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/median\endcsname{9.1}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/w10\endcsname{53.3}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/w20\endcsname{76.1}
\expandafter\def\csname v@timit/ft-ctcw-full/pcm/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/dmae\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/dw50\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/mae\endcsname{17.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/median\endcsname{9.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/w10\endcsname{51.7}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/w100\endcsname{98.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/w20\endcsname{74.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/amrnb/w50\endcsname{92.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/dmae\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/dw20\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/dw50\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/mae\endcsname{19.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/median\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/rtf\endcsname{0.015}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/w10\endcsname{47.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/w100\endcsname{97.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/w20\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ctcw-lora/ce/w50\endcsname{90.7}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/mae\endcsname{16.4}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/median\endcsname{9.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/w10\endcsname{52.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/w20\endcsname{76.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/clean/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/dmae\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/dw20\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/mae\endcsname{16.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/median\endcsname{9.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/w10\endcsname{53.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/w20\endcsname{75.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/g711u/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/mae\endcsname{16.6}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/median\endcsname{9.4}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/w10\endcsname{52.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/w20\endcsname{75.7}
\expandafter\def\csname v@timit/ft-ctcw-lora/g723/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/dmae\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/dw20\endcsname{-0.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/mae\endcsname{16.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/median\endcsname{8.7}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/w10\endcsname{55.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/w20\endcsname{76.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/g726/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/mae\endcsname{16.6}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/median\endcsname{9.6}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/w10\endcsname{51.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/w20\endcsname{75.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/gsm/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/mae\endcsname{16.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/median\endcsname{9.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/w10\endcsname{51.7}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/w20\endcsname{74.4}
\expandafter\def\csname v@timit/ft-ctcw-lora/mp3/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/dmae\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/dw20\endcsname{-0.4}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/mae\endcsname{16.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/median\endcsname{9.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/w10\endcsname{53.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/w20\endcsname{76.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/opus/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/dmae\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/dw20\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/mae\endcsname{16.3}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/median\endcsname{9.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/w10\endcsname{53.5}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/w20\endcsname{76.1}
\expandafter\def\csname v@timit/ft-ctcw-lora/pcm/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/dw20\endcsname{4.6}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/mae\endcsname{13.8}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/w10\endcsname{64.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/w20\endcsname{83.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/amrnb/w50\endcsname{94.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/clean/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g711u/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/w10\endcsname{66.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g723/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/w20\endcsname{85.9}
\expandafter\def\csname v@timit/ft-ts-1k-s1/g726/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/dw20\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/w10\endcsname{65.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/w20\endcsname{84.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/gsm/w50\endcsname{95.5}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/dw20\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/mae\endcsname{12.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/w10\endcsname{65.9}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/w20\endcsname{85.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/mp3/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/w10\endcsname{68.6}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-1k-s1/opus/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-1k-s1/pcm/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/dmae\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/mae\endcsname{13.6}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/w10\endcsname{64.4}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/w20\endcsname{83.7}
\expandafter\def\csname v@timit/ft-ts-1k/amrnb/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-1k/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-1k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/clean/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-1k/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-1k/clean/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-1k/clean/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-1k/g711u/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-1k/g723/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-1k/g723/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-1k/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-1k/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g723/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-1k/g723/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-1k/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/g723/w10\endcsname{66.5}
\expandafter\def\csname v@timit/ft-ts-1k/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-1k/g723/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-1k/g723/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-1k/g726/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-1k/g726/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-1k/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-1k/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-1k/g726/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-1k/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/g726/w10\endcsname{67.7}
\expandafter\def\csname v@timit/ft-ts-1k/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/w20\endcsname{86.0}
\expandafter\def\csname v@timit/ft-ts-1k/g726/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/dw20\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/w10\endcsname{65.9}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-1k/gsm/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/dw20\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/w10\endcsname{65.4}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-1k/mp3/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-1k/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-1k/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-1k/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-1k/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-1k/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-1k/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/opus/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-1k/opus/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-1k/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/opus/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-1k/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-1k/opus/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-1k/opus/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-1k/pcm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-4k/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-4k/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-4k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-4k/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/clean/w10\endcsname{73.8}
\expandafter\def\csname v@timit/ft-ts-4k/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-4k/clean/w20\endcsname{89.5}
\expandafter\def\csname v@timit/ft-ts-4k/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-4k/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-4k/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-4k/g726/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-4k/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-4k/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g726/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-4k/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-4k/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-4k/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/g726/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-4k/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-4k/g726/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-4k/g726/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-4k/gsm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-4k/mp3/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-4k/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-4k/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-4k/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-4k/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-4k/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-4k/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/opus/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-4k/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-4k/opus/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-4k/opus/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/w10\endcsname{72.8}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-4k/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-6k/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-6k/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-6k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-6k/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-6k/clean/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-6k/clean/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-6k/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-6k/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-6k/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-6k/g726/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-6k/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-6k/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g726/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-6k/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-6k/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-6k/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/g726/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-6k/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-6k/g726/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-6k/g726/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-6k/gsm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-6k/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-6k/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-6k/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-6k/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-6k/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/opus/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-6k/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-6k/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-6k/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/opus/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-6k/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-6k/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-6k/opus/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/dw20\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-6k/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-a02/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-a02/clean/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-a02/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-a02/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/clean/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-a02/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-a02/clean/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-a02/clean/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/w20\endcsname{85.8}
\expandafter\def\csname v@timit/ft-ts-a02/g711u/w50\endcsname{95.5}
\expandafter\def\csname v@timit/ft-ts-a02/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-a02/g726/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-a02/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-a02/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-a02/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-a02/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g726/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-a02/g726/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-a02/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-a02/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/g726/w10\endcsname{66.9}
\expandafter\def\csname v@timit/ft-ts-a02/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-a02/g726/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-a02/g726/w50\endcsname{95.3}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/dw20\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/median\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/w10\endcsname{64.3}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/w20\endcsname{84.0}
\expandafter\def\csname v@timit/ft-ts-a02/gsm/w50\endcsname{95.2}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/dw20\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/mae\endcsname{12.6}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/median\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/w10\endcsname{64.6}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/w20\endcsname{84.3}
\expandafter\def\csname v@timit/ft-ts-a02/mp3/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-a02/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-a02/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-a02/opus/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-a02/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-a02/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-a02/opus/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-a02/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-a02/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/opus/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-a02/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-a02/opus/w20\endcsname{86.1}
\expandafter\def\csname v@timit/ft-ts-a02/opus/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-a02/pcm/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-attn/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-attn/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-attn/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/clean/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-attn/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-attn/clean/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-attn/clean/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-attn/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-attn/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-attn/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-attn/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-attn/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-attn/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-attn/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-attn/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/g726/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-attn/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-attn/g726/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-attn/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/w10\endcsname{68.6}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-attn/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-attn/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-attn/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-attn/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-attn/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-attn/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-attn/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/opus/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-attn/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-attn/opus/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-attn/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-attn/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/dmae\endcsname{7.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/dw20\endcsname{16.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/dw50\endcsname{4.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/mae\endcsname{18.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/median\endcsname{9.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/w10\endcsname{51.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/w20\endcsname{73.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/amrnb/w50\endcsname{92.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/dmae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/dw20\endcsname{19.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/dw50\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/mae\endcsname{20.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/median\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/w10\endcsname{48.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/w100\endcsname{97.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/w20\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/ce/w50\endcsname{90.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/w10\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/dmae\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/dw20\endcsname{14.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/mae\endcsname{17.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/median\endcsname{9.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/w10\endcsname{52.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/w20\endcsname{74.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g711u/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/dmae\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/dw20\endcsname{13.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/dw50\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/mae\endcsname{16.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/median\endcsname{9.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/w10\endcsname{53.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/w20\endcsname{75.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g723/w50\endcsname{93.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/dmae\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/dw20\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/dw50\endcsname{3.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/mae\endcsname{16.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/median\endcsname{8.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/w10\endcsname{54.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/w20\endcsname{76.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/g726/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/dmae\endcsname{7.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/dw20\endcsname{16.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/mae\endcsname{17.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/median\endcsname{10.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/w10\endcsname{49.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/w20\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/gsm/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/dmae\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/dw20\endcsname{15.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/dw50\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/mae\endcsname{17.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/w10\endcsname{51.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/w20\endcsname{73.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/mp3/w50\endcsname{93.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/dmae\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/dw20\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/dw50\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/mae\endcsname{15.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/median\endcsname{8.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/w10\endcsname{55.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/w20\endcsname{77.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/opus/w50\endcsname{94.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/dmae\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/dw20\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/dw50\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/mae\endcsname{15.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/median\endcsname{8.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/w10\endcsname{55.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/w20\endcsname{77.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s1/pcm/w50\endcsname{94.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/dmae\endcsname{8.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/dw20\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/dw50\endcsname{4.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/mae\endcsname{18.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/median\endcsname{10.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/w10\endcsname{50.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/w20\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/amrnb/w50\endcsname{91.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/dmae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/dw20\endcsname{20.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/dw50\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/mae\endcsname{21.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/median\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/rtf\endcsname{0.010}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/w10\endcsname{46.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/w100\endcsname{97.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/w20\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/ce/w50\endcsname{90.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/w10\endcsname{74.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/dmae\endcsname{7.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/dw20\endcsname{16.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/dw50\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/mae\endcsname{18.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/median\endcsname{9.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/w10\endcsname{51.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/w20\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g711u/w50\endcsname{92.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/dmae\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/dw20\endcsname{15.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/dw50\endcsname{3.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/mae\endcsname{17.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/median\endcsname{9.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/w10\endcsname{51.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/w20\endcsname{74.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g723/w50\endcsname{92.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/dmae\endcsname{7.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/dw20\endcsname{14.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/dw50\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/mae\endcsname{17.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/median\endcsname{9.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/w10\endcsname{53.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/w20\endcsname{74.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/g726/w50\endcsname{92.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/dmae\endcsname{7.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/dw20\endcsname{17.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/dw50\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/mae\endcsname{18.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/median\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/w10\endcsname{48.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/w20\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/gsm/w50\endcsname{92.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/dmae\endcsname{7.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/dw20\endcsname{17.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/mae\endcsname{18.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/median\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/w10\endcsname{48.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/w20\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/mp3/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/dmae\endcsname{7.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/dw20\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/dw50\endcsname{3.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/mae\endcsname{17.5}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/median\endcsname{9.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/w10\endcsname{52.8}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/w20\endcsname{75.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/opus/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/dmae\endcsname{7.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/dw20\endcsname{14.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/mae\endcsname{17.6}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/median\endcsname{9.2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/w10\endcsname{52.9}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/w20\endcsname{74.7}
\expandafter\def\csname v@timit/ft-ts-aug0-s2/pcm/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/dmae\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/dw20\endcsname{16.5}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/dw50\endcsname{4.3}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/mae\endcsname{17.8}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/median\endcsname{10.0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/w10\endcsname{50.0}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/w20\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-aug0/amrnb/w50\endcsname{92.2}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/dmae\endcsname{10.1}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/dw20\endcsname{19.0}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/dw50\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/mae\endcsname{20.4}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/median\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/w10\endcsname{48.2}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/w100\endcsname{97.8}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/w20\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-aug0/ce/w50\endcsname{90.9}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-aug0/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/dmae\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/dw20\endcsname{15.2}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/dw50\endcsname{3.4}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/mae\endcsname{17.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/median\endcsname{9.5}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/w10\endcsname{51.8}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/w20\endcsname{74.1}
\expandafter\def\csname v@timit/ft-ts-aug0/g711u/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/dmae\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/dw20\endcsname{14.5}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/mae\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/median\endcsname{9.5}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/w10\endcsname{52.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/w20\endcsname{74.8}
\expandafter\def\csname v@timit/ft-ts-aug0/g723/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/dmae\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/dw20\endcsname{14.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/dw50\endcsname{3.4}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/mae\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/median\endcsname{9.2}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/w10\endcsname{53.0}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/w20\endcsname{75.3}
\expandafter\def\csname v@timit/ft-ts-aug0/g726/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/dmae\endcsname{7.2}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/dw20\endcsname{16.4}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/dw50\endcsname{3.4}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/ebias\endcsname{4}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/ebias-signed\endcsname{$+4$}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/mae\endcsname{17.4}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/median\endcsname{10.2}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/w10\endcsname{49.3}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/w20\endcsname{73.0}
\expandafter\def\csname v@timit/ft-ts-aug0/gsm/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/dmae\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/dw20\endcsname{15.8}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/dw50\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/mae\endcsname{17.1}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/median\endcsname{9.9}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/w10\endcsname{50.4}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/w20\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-aug0/mp3/w50\endcsname{93.6}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/dmae\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/dw20\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/dw50\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/mae\endcsname{16.4}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/median\endcsname{9.1}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/w10\endcsname{53.3}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/w20\endcsname{76.2}
\expandafter\def\csname v@timit/ft-ts-aug0/opus/w50\endcsname{93.6}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/dmae\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/dw20\endcsname{13.2}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/dw50\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/ebias\endcsname{3}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/ebias-signed\endcsname{$+3$}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/mae\endcsname{16.3}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/median\endcsname{8.9}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/w10\endcsname{54.0}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/w20\endcsname{76.1}
\expandafter\def\csname v@timit/ft-ts-aug0/pcm/w50\endcsname{93.6}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/dmae\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/dw20\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/dw50\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/w20\endcsname{85.8}
\expandafter\def\csname v@timit/ft-ts-aug100/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-aug100/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/dmae\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/dw20\endcsname{-0.4}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-aug100/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-aug100/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/dmae\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/dw20\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-aug100/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-aug100/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-aug100/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/dmae\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-aug100/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/dmae\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/dw20\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-aug100/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/dw20\endcsname{4.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/dw50\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/w10\endcsname{67.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s1/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/dmae\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/dw20\endcsname{4.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/dw50\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/mae\endcsname{13.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/w10\endcsname{74.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/w20\endcsname{89.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/dw20\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/w10\endcsname{68.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/dw20\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-aug25-s2/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/dmae\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/w20\endcsname{85.3}
\expandafter\def\csname v@timit/ft-ts-aug25/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/w10\endcsname{73.8}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-aug25/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-aug25/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-aug25/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-aug25/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-aug25/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-aug25/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-aug25/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-aug25/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/dmae\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/dw20\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-aug75/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/w10\endcsname{73.2}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-aug75/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-aug75/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-aug75/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-aug75/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-aug75/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-aug75/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-aug75/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-aug75/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/dmae\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/dw50\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/mae\endcsname{12.6}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/amrnb/w50\endcsname{95.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-augamr-s1/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/dmae\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/dw20\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/dw50\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/mae\endcsname{12.6}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-augamr/amrnb/w50\endcsname{95.0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-augamr/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-augamr/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-augamr/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-augamr/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-augamr/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-augamr/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-augamr/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/dw20\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-augamr/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/dmae\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/w10\endcsname{73.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/gsm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/opus/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-auxw-s1/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/dmae\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/w10\endcsname{67.7}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-auxw/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/w10\endcsname{73.4}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-auxw/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-auxw/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-auxw/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-auxw/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-auxw/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-auxw/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-auxw/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-auxw/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/dw20\endcsname{4.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/w10\endcsname{67.6}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/w10\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/dw20\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-auxwp-s1/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/w10\endcsname{73.9}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-auxwp/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-auxwp/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-auxwp/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-dec/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-dec/clean/median\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-dec/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-dec/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/clean/w10\endcsname{65.0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-dec/clean/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-dec/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/w10\endcsname{63.4}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/w20\endcsname{84.5}
\expandafter\def\csname v@timit/ft-ts-dec/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-dec/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-dec/g726/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-dec/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-dec/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g726/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-dec/g726/median\endcsname{7.1}
\expandafter\def\csname v@timit/ft-ts-dec/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-dec/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-dec/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/g726/w10\endcsname{62.9}
\expandafter\def\csname v@timit/ft-ts-dec/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-dec/g726/w20\endcsname{83.9}
\expandafter\def\csname v@timit/ft-ts-dec/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/dw20\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/mae\endcsname{13.3}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/median\endcsname{7.4}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/w10\endcsname{61.2}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/w20\endcsname{82.9}
\expandafter\def\csname v@timit/ft-ts-dec/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/median\endcsname{7.3}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/w10\endcsname{61.2}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/w20\endcsname{83.5}
\expandafter\def\csname v@timit/ft-ts-dec/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-dec/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-dec/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-dec/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-dec/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-dec/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-dec/opus/median\endcsname{7.0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-dec/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/opus/w10\endcsname{63.1}
\expandafter\def\csname v@timit/ft-ts-dec/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-dec/opus/w20\endcsname{84.3}
\expandafter\def\csname v@timit/ft-ts-dec/opus/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/w10\endcsname{63.6}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/w20\endcsname{84.6}
\expandafter\def\csname v@timit/ft-ts-dec/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/w20\endcsname{85.0}
\expandafter\def\csname v@timit/ft-ts-full/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-full/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-full/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-full/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/clean/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-full/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-full/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-full/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-full/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-full/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-full/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-full/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-full/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-full/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/g711u/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-full/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-full/g711u/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-full/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-full/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-full/g723/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-full/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-full/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-full/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-full/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g723/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-full/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-full/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-full/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/g723/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-full/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-full/g723/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-full/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-full/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-full/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-full/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-full/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-full/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-full/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-full/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/g726/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-full/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-full/g726/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-full/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-full/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-full/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-full/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-full/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-full/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-full/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-full/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/gsm/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-full/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-full/gsm/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-full/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-full/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-full/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-full/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-full/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/mp3/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-full/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-full/mp3/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-full/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-full/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-full/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-full/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-full/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-full/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-full/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-full/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/opus/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-full/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-full/opus/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-full/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-full/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-full/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-full/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-full/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-full/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-full/pcm/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-full/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-full/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-full/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/w10\endcsname{73.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-lora-en/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-lora-en/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/dmae\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/dw20\endcsname{3.6}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/dw50\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-lora/amrnb/w50\endcsname{94.9}
\expandafter\def\csname v@timit/ft-ts-lora/ce/dmae\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-lora/ce/dw20\endcsname{10.0}
\expandafter\def\csname v@timit/ft-ts-lora/ce/dw50\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-lora/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-lora/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-lora/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/ce/mae\endcsname{16.1}
\expandafter\def\csname v@timit/ft-ts-lora/ce/median\endcsname{7.7}
\expandafter\def\csname v@timit/ft-ts-lora/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora/ce/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-lora/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/ce/w10\endcsname{58.7}
\expandafter\def\csname v@timit/ft-ts-lora/ce/w100\endcsname{98.1}
\expandafter\def\csname v@timit/ft-ts-lora/ce/w20\endcsname{79.1}
\expandafter\def\csname v@timit/ft-ts-lora/ce/w50\endcsname{93.4}
\expandafter\def\csname v@timit/ft-ts-lora/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-lora/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-lora/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lora/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/clean/w10\endcsname{73.2}
\expandafter\def\csname v@timit/ft-ts-lora/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lora/clean/w20\endcsname{89.1}
\expandafter\def\csname v@timit/ft-ts-lora/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-lora/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-lora/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-lora/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-lora/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/g723/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-lora/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora/g723/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-lora/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-lora/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lora/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-lora/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-lora/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/g726/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-lora/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora/g726/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-lora/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-lora/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-lora/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-lora/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lora/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-lora/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-lora/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/opus/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-lora/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora/opus/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-lora/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-lora/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/dmae\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/mae\endcsname{14.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/w10\endcsname{59.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/w20\endcsname{83.6}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/amrnb/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/mae\endcsname{12.2}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/w10\endcsname{64.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/clean/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/mae\endcsname{12.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/w10\endcsname{63.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g711u/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/w10\endcsname{61.8}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/w20\endcsname{86.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g723/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/w10\endcsname{62.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/g726/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/w10\endcsname{61.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/gsm/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/w10\endcsname{61.3}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/mp3/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/mae\endcsname{12.6}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/w10\endcsname{62.9}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/opus/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/median\endcsname{7.5}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/w10\endcsname{63.3}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-lora@argmax/pcm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/dw50\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/mae\endcsname{17.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/median\endcsname{10.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/sbias\endcsname{8}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/sbias-signed\endcsname{$+8$}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/w10\endcsname{49.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/w20\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/amrnb/w50\endcsname{93.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/mae\endcsname{15.8}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/median\endcsname{9.4}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/sbias\endcsname{7}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/w10\endcsname{52.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/w20\endcsname{74.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/clean/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/dmae\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/dw20\endcsname{-0.6}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/dw50\endcsname{-0.6}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/mae\endcsname{15.5}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/median\endcsname{9.5}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/sbias\endcsname{7}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/w10\endcsname{51.8}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/w20\endcsname{75.3}
\expandafter\def\csname v@timit/ft-ts-lora@full/g711u/w50\endcsname{95.5}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/dmae\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/dw20\endcsname{-1.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/dw50\endcsname{-0.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/mae\endcsname{15.5}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/sbias\endcsname{7}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/w10\endcsname{50.9}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/w20\endcsname{75.8}
\expandafter\def\csname v@timit/ft-ts-lora@full/g723/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/dw50\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/ebias\endcsname{5}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/ebias-signed\endcsname{$+5$}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/mae\endcsname{15.9}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/sbias\endcsname{7}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/w10\endcsname{51.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/w20\endcsname{74.5}
\expandafter\def\csname v@timit/ft-ts-lora@full/g726/w50\endcsname{95.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/dmae\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/dw20\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/dw50\endcsname{-0.5}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/mae\endcsname{15.6}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/median\endcsname{9.9}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/sbias\endcsname{7}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/w10\endcsname{50.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/w20\endcsname{75.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/gsm/w50\endcsname{95.4}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/dmae\endcsname{-0.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/dw20\endcsname{-0.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/dw50\endcsname{-0.6}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/mae\endcsname{15.6}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/sbias\endcsname{7}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/w10\endcsname{51.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/w20\endcsname{74.8}
\expandafter\def\csname v@timit/ft-ts-lora@full/mp3/w50\endcsname{95.4}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/dw20\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/dw50\endcsname{-0.4}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/mae\endcsname{15.8}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/median\endcsname{9.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/sbias\endcsname{8}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/sbias-signed\endcsname{$+8$}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/w10\endcsname{51.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/w20\endcsname{74.4}
\expandafter\def\csname v@timit/ft-ts-lora@full/opus/w50\endcsname{95.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/dmae\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/dw50\endcsname{-0.3}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/ebias\endcsname{6}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/ebias-signed\endcsname{$+6$}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/mae\endcsname{15.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/median\endcsname{9.5}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/sbias\endcsname{7}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/sbias-signed\endcsname{$+7$}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/w10\endcsname{51.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/w20\endcsname{74.7}
\expandafter\def\csname v@timit/ft-ts-lora@full/pcm/w50\endcsname{95.1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/dmae\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/dw20\endcsname{3.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/w10\endcsname{73.9}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g723/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-lora@r1/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/opus/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-lora@r1/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/dmae\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/dw20\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/dw50\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/w10\endcsname{66.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/w20\endcsname{84.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/amrnb/w50\endcsname{95.5}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/clean/w50\endcsname{96.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g711u/w50\endcsname{96.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/w10\endcsname{68.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g723/w50\endcsname{96.7}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/g726/w50\endcsname{96.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/w10\endcsname{67.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/w20\endcsname{86.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/gsm/w50\endcsname{96.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/w10\endcsname{67.7}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/w20\endcsname{86.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/mp3/w50\endcsname{96.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/opus/w50\endcsname{96.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-lora@r5/pcm/w50\endcsname{96.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-lr1e4/clean/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-lr1e4/g726/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-lr1e4/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/w10\endcsname{67.9}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-lr1e4/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-lr1e4/opus/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-lr1e4/pcm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/mae\endcsname{10.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/w10\endcsname{74.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/w20\endcsname{89.9}
\expandafter\def\csname v@timit/ft-ts-lr5e4/clean/w50\endcsname{96.7}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-lr5e4/g726/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/gsm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/opus/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-lr5e4/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/dw20\endcsname{3.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/mae\endcsname{12.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/w10\endcsname{68.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g723/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/g726/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/gsm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-4k/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/w20\endcsname{84.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/amrnb/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/w10\endcsname{71.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g723/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr2e4/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/w20\endcsname{84.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-lr5e3/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/w10\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-r64/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/w20\endcsname{85.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/w10\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/w20\endcsname{89.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-rand/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/mae\endcsname{13.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/w10\endcsname{67.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/w20\endcsname{84.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/amrnb/w50\endcsname{94.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g723/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/w10\endcsname{68.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/opus/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-round/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/dw20\endcsname{4.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/w20\endcsname{84.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/w10\endcsname{73.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/dw20\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/mp3/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s1/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/w10\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/w20\endcsname{88.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/w10\endcsname{71.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s2/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/dw20\endcsname{4.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/w20\endcsname{84.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/w10\endcsname{72.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s3/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/w20\endcsname{84.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/w10\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-s4/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/dmae\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/mae\endcsname{14.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/w10\endcsname{67.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/w100\endcsname{98.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/w20\endcsname{84.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/amrnb/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/clean/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g723/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/w10\endcsname{68.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/w20\endcsname{86.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/mp3/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms-tn10/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/w20\endcsname{84.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/w10\endcsname{73.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-10ms/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/dw20\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-post-10ms/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/mae\endcsname{13.2}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/w20\endcsname{84.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/amrnb/w50\endcsname{94.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-post-5ms/clean/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-5ms/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/w10\endcsname{67.6}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/w20\endcsname{85.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/dmae\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/dw20\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/mae\endcsname{16.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/median\endcsname{8.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/w10\endcsname{57.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/w100\endcsname{98.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/w20\endcsname{78.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/ce/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-s1/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-post-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/w10\endcsname{68.6}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-post-s1/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/dmae\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/dmae\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/dw20\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/dw50\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/mae\endcsname{16.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/median\endcsname{7.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/w10\endcsname{57.7}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/w100\endcsname{98.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/w20\endcsname{78.6}
\expandafter\def\csname v@timit/ft-ts-post-s2/ce/w50\endcsname{93.5}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-s2/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-s2/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post-s2/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/dmae\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/dw20\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/dw50\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/mae\endcsname{16.6}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/median\endcsname{8.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/rtf\endcsname{0.010}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/w10\endcsname{57.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/w100\endcsname{98.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/w20\endcsname{77.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/ce/w50\endcsname{92.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/w10\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/w20\endcsname{89.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/w10\endcsname{68.8}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-post-s3/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-post-s3/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/dw20\endcsname{4.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/w20\endcsname{84.8}
\expandafter\def\csname v@timit/ft-ts-post-s4/amrnb/w50\endcsname{94.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/dmae\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/dw20\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/dw50\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/mae\endcsname{16.7}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/median\endcsname{8.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/w10\endcsname{56.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/w100\endcsname{98.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/w20\endcsname{77.6}
\expandafter\def\csname v@timit/ft-ts-post-s4/ce/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/w10\endcsname{73.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/w20\endcsname{89.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-s4/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-post-s4/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-s4/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-s4/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-post-s4/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/dmae\endcsname{3.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/dw20\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/mae\endcsname{13.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/w10\endcsname{63.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/w20\endcsname{83.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/w20\endcsname{88.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/dmae\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/mae\endcsname{12.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/w10\endcsname{65.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g711u/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/dw20\endcsname{3.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/w10\endcsname{66.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/dmae\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/dw20\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/mae\endcsname{12.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/w10\endcsname{65.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/w20\endcsname{85.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/w10\endcsname{67.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon-s1/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/dmae\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/dw20\endcsname{5.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/mae\endcsname{13.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/median\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/rtf\endcsname{0.027}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/w10\endcsname{64.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/w20\endcsname{84.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/rtf\endcsname{0.027}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/w20\endcsname{89.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/dw20\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/rtf\endcsname{0.026}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/w10\endcsname{66.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/w20\endcsname{86.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g711u/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/rtf\endcsname{0.026}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/rtf\endcsname{0.027}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/dw20\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/rtf\endcsname{0.027}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/w20\endcsname{86.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/rtf\endcsname{0.027}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/w10\endcsname{68.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/rtf\endcsname{0.027}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-post-sidon/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/rtf\endcsname{0.027}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-sidon/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/dmae\endcsname{3.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/dw20\endcsname{4.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/mae\endcsname{13.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/w10\endcsname{66.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/w20\endcsname{84.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/dmae\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/dw20\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/dw50\endcsname{3.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/mae\endcsname{16.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/median\endcsname{8.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/w10\endcsname{56.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/w100\endcsname{98.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/w20\endcsname{78.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/ce/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/dw20\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10-s1/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/mae\endcsname{13.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/w10\endcsname{66.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/w20\endcsname{84.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/dmae\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/dw20\endcsname{10.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/dw50\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/mae\endcsname{16.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/median\endcsname{7.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/w10\endcsname{58.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/w100\endcsname{98.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/w20\endcsname{78.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/ce/w50\endcsname{93.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/w10\endcsname{68.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-post-tn10/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post-tn10/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-post-tn10/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/w20\endcsname{85.0}
\expandafter\def\csname v@timit/ft-ts-post/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-post/ce/dmae\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-post/ce/dw20\endcsname{10.1}
\expandafter\def\csname v@timit/ft-ts-post/ce/dw50\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-post/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-post/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-post/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/ce/mae\endcsname{15.9}
\expandafter\def\csname v@timit/ft-ts-post/ce/median\endcsname{7.8}
\expandafter\def\csname v@timit/ft-ts-post/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/ce/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-post/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/ce/w10\endcsname{58.4}
\expandafter\def\csname v@timit/ft-ts-post/ce/w100\endcsname{98.3}
\expandafter\def\csname v@timit/ft-ts-post/ce/w20\endcsname{79.0}
\expandafter\def\csname v@timit/ft-ts-post/ce/w50\endcsname{93.3}
\expandafter\def\csname v@timit/ft-ts-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-post/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/clean/w10\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ts-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-post/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-post/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-post/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-post/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/g711u/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-post/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-post/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-post/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-post/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/g723/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-post/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-post/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-post/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-post/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-post/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-post/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/g726/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-post/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-post/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-post/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/gsm/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-post/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-post/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-post/mp3/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-post/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-post/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-post/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/mp3/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-post/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post/mp3/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-post/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-post/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-post/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-post/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-post/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-post/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-post/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-post/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-post/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/opus/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-post/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post/opus/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-post/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-post/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-post/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-post/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-post/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-post/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-post/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-post/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-post/pcm/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-post/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-post/pcm/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-post/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-r128/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/clean/mae\endcsname{10.2}
\expandafter\def\csname v@timit/ft-ts-r128/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-r128/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r128/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-r128/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/clean/w10\endcsname{73.9}
\expandafter\def\csname v@timit/ft-ts-r128/clean/w100\endcsname{99.2}
\expandafter\def\csname v@timit/ft-ts-r128/clean/w20\endcsname{89.8}
\expandafter\def\csname v@timit/ft-ts-r128/clean/w50\endcsname{96.7}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-r128/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-r128/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r128/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-r128/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-r128/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g726/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-r128/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-r128/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r128/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r128/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/g726/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-r128/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r128/g726/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-r128/g726/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-r128/gsm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-r128/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-r128/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r128/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-r128/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-r128/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-r128/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-r128/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r128/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/opus/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-r128/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r128/opus/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-r128/opus/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-r128/pcm/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-r16/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-r16/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-r16/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-r16/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/clean/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-r16/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r16/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-r16/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-r16/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-r16/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-r16/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-r16/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-r16/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-r16/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-r16/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r16/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/g726/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-r16/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r16/g726/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-r16/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-r16/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-r16/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-r16/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-r16/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-r16/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r16/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r16/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r16/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/opus/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-r16/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-r16/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r16/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r16/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/opus/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-r16/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r16/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-r16/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-r16/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-r64/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-r64/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-r64/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r64/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-r64/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/clean/w10\endcsname{74.1}
\expandafter\def\csname v@timit/ft-ts-r64/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r64/clean/w20\endcsname{89.5}
\expandafter\def\csname v@timit/ft-ts-r64/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/w20\endcsname{88.8}
\expandafter\def\csname v@timit/ft-ts-r64/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-r64/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r64/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-r64/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-r64/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-r64/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r64/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/g726/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-r64/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r64/g726/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-r64/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-r64/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-r64/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-r64/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-r64/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-r64/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r64/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r64/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r64/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/opus/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-r64/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-r64/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r64/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r64/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/opus/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-r64/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r64/opus/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-r64/opus/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-r64/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-r8/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-r8/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-r8/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/clean/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-r8/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r8/clean/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-r8/clean/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-r8/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-r8/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-r8/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-r8/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r8/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/g726/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-r8/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r8/g726/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-r8/g726/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/w20\endcsname{86.2}
\expandafter\def\csname v@timit/ft-ts-r8/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-r8/mp3/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-r8/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r8/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-r8/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-r8/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-r8/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-r8/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/opus/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-r8/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-r8/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r8/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/opus/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-r8/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r8/opus/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-r8/opus/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-r8/pcm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/mae\endcsname{13.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/w10\endcsname{66.2}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/w20\endcsname{84.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-round-s1/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-round-s1/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-round-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-round-s1/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-round-s1/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-round-s1/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/dw20\endcsname{3.6}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/mae\endcsname{13.1}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/w10\endcsname{66.5}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/w20\endcsname{85.0}
\expandafter\def\csname v@timit/ft-ts-round/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-round/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/clean/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-round/clean/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-round/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-round/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/clean/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-round/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-round/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-round/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-round/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-round/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-round/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-round/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-round/g711u/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-round/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/g711u/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-round/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round/g711u/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-round/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-round/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-round/g723/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-round/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-round/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-round/g723/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-round/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/g723/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-round/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round/g723/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-round/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-round/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-round/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-round/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-round/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g726/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-round/g726/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-round/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/g726/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-round/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round/g726/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-round/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-round/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-round/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-round/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-round/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-round/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-round/gsm/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-round/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/gsm/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-round/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round/gsm/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-round/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-round/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-round/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-round/mp3/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-round/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/mp3/w10\endcsname{67.1}
\expandafter\def\csname v@timit/ft-ts-round/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-round/mp3/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-round/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-round/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-round/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-round/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-round/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/opus/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-round/opus/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-round/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/opus/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-round/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round/opus/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-round/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-round/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-round/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-round/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-round/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-round/pcm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-round/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-round/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-round/pcm/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-round/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-round/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/dmae\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/dw20\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/dw50\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/median\endcsname{7.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/w10\endcsname{62.2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/w20\endcsname{82.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/amrnb/w50\endcsname{94.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/mae\endcsname{12.2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/median\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/w10\endcsname{65.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/w20\endcsname{84.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/dw20\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/w20\endcsname{86.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/dmae\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/median\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/w10\endcsname{65.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/w20\endcsname{84.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/g726/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/dmae\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/dw20\endcsname{4.2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/mae\endcsname{12.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/w10\endcsname{64.2}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/w20\endcsname{84.3}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/dw20\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/w10\endcsname{66.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/w20\endcsname{85.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/mp3/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/w10\endcsname{68.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-s6-final-s1/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/dmae\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/dw20\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/w10\endcsname{63.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/w20\endcsname{83.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/amrnb/w50\endcsname{94.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/dmae\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/dw20\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/dw50\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/mae\endcsname{13.7}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/median\endcsname{7.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/w10\endcsname{62.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/w20\endcsname{82.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/ce/w50\endcsname{95.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-s6-final/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/dw20\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/w10\endcsname{66.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-s6-final/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/dw20\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/w10\endcsname{66.8}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/w20\endcsname{85.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/dmae\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/dw20\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/median\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/w10\endcsname{65.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/dw20\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/w20\endcsname{86.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/mp3/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-s6-final/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/w20\endcsname{89.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/w10\endcsname{68.8}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/w10\endcsname{68.8}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-s6-post-s1/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/w10\endcsname{67.6}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/w10\endcsname{73.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-s6-post/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-s6-post/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-s6-post/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-s6-post/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/rtf\endcsname{0.015}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-s6-post/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/dmae\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/dw20\endcsname{4.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/mae\endcsname{13.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/median\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/w10\endcsname{64.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/w20\endcsname{84.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/w10\endcsname{67.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/w10\endcsname{67.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/median\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/w10\endcsname{66.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/w10\endcsname{67.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon-s1/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/dmae\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/dw20\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/dw50\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/mae\endcsname{14.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/median\endcsname{7.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/w10\endcsname{62.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/w20\endcsname{82.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/dmae\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/w10\endcsname{64.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g711u/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/dmae\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/w10\endcsname{65.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/dmae\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/mae\endcsname{12.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/w10\endcsname{64.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/w20\endcsname{84.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/w10\endcsname{68.8}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-s6-sidon/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/mae\endcsname{13.2}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-seed1/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/dmae\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/dw20\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/dw50\endcsname{3.1}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/mae\endcsname{16.6}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/median\endcsname{7.8}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/w10\endcsname{58.0}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/w100\endcsname{98.2}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/w20\endcsname{78.8}
\expandafter\def\csname v@timit/ft-ts-seed1/ce/w50\endcsname{93.4}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/w10\endcsname{73.3}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-seed1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-seed1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/rtf\endcsname{0.011}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-seed1/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-seed1/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-seed1/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-seed1/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-seed1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-seed1/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/w10\endcsname{67.9}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-seed2/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/dmae\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/dw20\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/mae\endcsname{16.5}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/median\endcsname{7.8}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/w10\endcsname{58.1}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/w100\endcsname{98.1}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/w20\endcsname{78.8}
\expandafter\def\csname v@timit/ft-ts-seed2/ce/w50\endcsname{93.2}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/w10\endcsname{73.2}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-seed2/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/w10\endcsname{71.8}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-seed2/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-seed2/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-seed2/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-seed2/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-seed2/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-seed2/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-seed2/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/w10\endcsname{67.9}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/w20\endcsname{85.3}
\expandafter\def\csname v@timit/ft-ts-seed3/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/dmae\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/dw20\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/dw50\endcsname{3.4}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/mae\endcsname{16.7}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/median\endcsname{7.8}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/rtf\endcsname{0.010}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/w10\endcsname{58.1}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/w100\endcsname{98.1}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/w20\endcsname{78.4}
\expandafter\def\csname v@timit/ft-ts-seed3/ce/w50\endcsname{93.1}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/w10\endcsname{73.4}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-seed3/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-seed3/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-seed3/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-seed3/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-seed3/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-seed3/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-seed3/opus/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-seed3/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-seed4/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/dmae\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/dw20\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/dw50\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/mae\endcsname{17.1}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/median\endcsname{8.0}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/w10\endcsname{57.2}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/w100\endcsname{98.1}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/w20\endcsname{78.0}
\expandafter\def\csname v@timit/ft-ts-seed4/ce/w50\endcsname{93.0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/w10\endcsname{73.3}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-seed4/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-seed4/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-seed4/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-seed4/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-seed4/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-seed4/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-seed4/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-seed4/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/dmae\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/dw20\endcsname{4.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/dw50\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/mae\endcsname{14.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/w10\endcsname{66.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/w20\endcsname{84.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/amrnb/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/dw20\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-tn10-s1/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/dmae\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/dw50\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/mae\endcsname{13.9}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/w10\endcsname{67.1}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-tn10/amrnb/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-tn10/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-tn10/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-tn10/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/w10\endcsname{68.6}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-tn10/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-tn10/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-tn10/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-tn10/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/dmae\endcsname{3.5}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/dw20\endcsname{4.2}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/mae\endcsname{14.4}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/w10\endcsname{66.6}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/w20\endcsname{84.5}
\expandafter\def\csname v@timit/ft-ts-tn20/amrnb/w50\endcsname{94.3}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/w10\endcsname{72.7}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-tn20/clean/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-tn20/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-tn20/g723/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-tn20/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-tn20/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-tn20/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-tn20/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-tn20/pcm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/dmae\endcsname{2.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/dw20\endcsname{4.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/mae\endcsname{13.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/w10\endcsname{65.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/w20\endcsname{83.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/amrnb/w50\endcsname{94.3}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/dmae\endcsname{3.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/dw20\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/w10\endcsname{62.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/w20\endcsname{81.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/ce/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/clean/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/w20\endcsname{85.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g711u/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g723/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/g726/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/dw20\endcsname{3.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/mae\endcsname{12.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/w20\endcsname{85.3}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/gsm/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/w20\endcsname{85.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/mp3/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/opus/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final-s1/pcm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/dw20\endcsname{4.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/dw50\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/mae\endcsname{13.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/w10\endcsname{65.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/w20\endcsname{83.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/amrnb/w50\endcsname{94.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/dmae\endcsname{3.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/dw20\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/dw50\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/w10\endcsname{63.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/w20\endcsname{82.3}
\expandafter\def\csname v@timit/ft-ts-turbo-final/ce/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final/clean/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/w20\endcsname{85.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g711u/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/w10\endcsname{68.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g723/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/w10\endcsname{68.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/dmae\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/dw20\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/dw20\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/w10\endcsname{67.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/w20\endcsname{86.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/mp3/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/opus/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/w10\endcsname{70.4}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-turbo-final/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/mae\endcsname{13.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/w10\endcsname{67.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/w20\endcsname{84.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/w10\endcsname{73.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g711u/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/g726/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-10ms/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/w10\endcsname{68.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/w10\endcsname{73.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/w10\endcsname{71.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/sbias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/rtf\endcsname{0.017}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post-s1/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/w20\endcsname{85.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/dmae\endcsname{6.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/dw20\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/dw50\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/mae\endcsname{16.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/median\endcsname{8.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/w10\endcsname{56.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/w100\endcsname{98.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/w20\endcsname{77.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/ce/w50\endcsname{92.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/w10\endcsname{73.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/w20\endcsname{89.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/rtf\endcsname{0.016}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-turbo-post/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/dw20\endcsname{4.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/mae\endcsname{13.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/w10\endcsname{67.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/w10\endcsname{73.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/w10\endcsname{71.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/w20\endcsname{87.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/mp3/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/w10\endcsname{71.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s1/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/amrnb/w50\endcsname{94.9}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/w10\endcsname{73.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g723/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/w20\endcsname{88.8}
\expandafter\def\csname v@timit/ft-ts-turbo-s2/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/dmae\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/dw20\endcsname{4.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/dw50\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/mae\endcsname{13.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/w10\endcsname{66.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/w20\endcsname{84.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/amrnb/w50\endcsname{94.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/w10\endcsname{69.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/dw20\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/dw20\endcsname{2.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/w10\endcsname{70.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10-s1/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/dmae\endcsname{3.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/dw20\endcsname{4.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/dw50\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/over500\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/w10\endcsname{66.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/w100\endcsname{98.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/w20\endcsname{84.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/amrnb/w50\endcsname{94.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/clean/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/w10\endcsname{69.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/g726/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/w10\endcsname{68.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/w20\endcsname{86.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/w10\endcsname{71.2}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-turbo-tn10/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/w10\endcsname{68.3}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-turbo/amrnb/w50\endcsname{94.9}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-turbo/clean/w50\endcsname{96.6}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-turbo/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/w10\endcsname{70.6}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-turbo/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/w10\endcsname{71.4}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-turbo/g726/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-turbo/gsm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/w10\endcsname{69.7}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-turbo/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-turbo/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-turbo/pcm/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/dmae\endcsname{3.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/dw20\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/mae\endcsname{13.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/w10\endcsname{63.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/w20\endcsname{83.5}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/amrnb/w50\endcsname{94.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/dmae\endcsname{2.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/dw20\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/dw50\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/mae\endcsname{13.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/median\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/w10\endcsname{64.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/w100\endcsname{98.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/w20\endcsname{83.4}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/ce/w50\endcsname{95.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/w10\endcsname{72.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/w20\endcsname{89.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/dw20\endcsname{3.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/median\endcsname{6.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/w10\endcsname{66.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/w20\endcsname{86.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g711u/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/w10\endcsname{69.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/dw20\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/w10\endcsname{67.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/dmae\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/w10\endcsname{65.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/w20\endcsname{85.4}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/gsm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/dw20\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/median\endcsname{6.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/rtf\endcsname{0.018}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/w10\endcsname{69.5}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/opus/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-v3-final-s1/pcm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/dmae\endcsname{3.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/dw20\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/median\endcsname{7.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/w10\endcsname{63.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/w20\endcsname{83.2}
\expandafter\def\csname v@timit/ft-ts-v3-final/amrnb/w50\endcsname{94.6}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/dmae\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/dw20\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/dw50\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/mae\endcsname{13.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/median\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/w10\endcsname{63.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/w100\endcsname{98.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/w20\endcsname{83.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/ce/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/w10\endcsname{72.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/w20\endcsname{88.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/dmae\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/median\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/w10\endcsname{64.6}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/w20\endcsname{85.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g711u/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/w10\endcsname{68.2}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/w20\endcsname{86.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/g723/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/dmae\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/dw50\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/w10\endcsname{65.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/w20\endcsname{85.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/g726/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/dmae\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/dw50\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/ebias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/mae\endcsname{12.5}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/median\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/w10\endcsname{65.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/w20\endcsname{84.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/gsm/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/dw20\endcsname{2.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/mae\endcsname{11.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/median\endcsname{6.2}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/w10\endcsname{67.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/w20\endcsname{86.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/mp3/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/w10\endcsname{69.2}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-v3-final/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/w10\endcsname{69.4}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-v3-final/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/w20\endcsname{85.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/amrnb/w50\endcsname{94.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/mae\endcsname{10.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/w10\endcsname{73.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/w20\endcsname{89.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/clean/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g711u/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/w10\endcsname{70.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g723/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/g726/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/gsm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/w20\endcsname{87.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/mp3/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/w10\endcsname{71.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/opus/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-10ms/pcm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/dw20\endcsname{3.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/rtf\endcsname{0.026}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/rtf\endcsname{0.024}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g711u/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/rtf\endcsname{0.026}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/w10\endcsname{70.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/rtf\endcsname{0.026}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/rtf\endcsname{0.026}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/w10\endcsname{69.6}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/rtf\endcsname{0.026}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/w20\endcsname{88.8}
\expandafter\def\csname v@timit/ft-ts-v3-post-s1/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/dmae\endcsname{2.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/dw50\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/median\endcsname{6.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/w10\endcsname{68.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/w20\endcsname{85.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/median\endcsname{5.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/w10\endcsname{73.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-v3-post/g723/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/w10\endcsname{71.1}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/dw20\endcsname{1.9}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-v3-post/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/dw20\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/median\endcsname{5.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-v3-post/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/rtf\endcsname{0.019}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/w10\endcsname{72.4}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/w20\endcsname{88.5}
\expandafter\def\csname v@timit/ft-ts-v3-post/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/dmae\endcsname{2.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/dw20\endcsname{3.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/mae\endcsname{12.9}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/w10\endcsname{68.5}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/w20\endcsname{85.7}
\expandafter\def\csname v@timit/ft-ts-v3-s1/amrnb/w50\endcsname{94.9}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/mae\endcsname{10.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/w10\endcsname{74.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/clean/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/w10\endcsname{72.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g711u/w50\endcsname{96.5}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/w20\endcsname{87.9}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/w10\endcsname{71.5}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/w20\endcsname{88.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/g726/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/mae\endcsname{11.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/w20\endcsname{87.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/mae\endcsname{11.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/w10\endcsname{69.8}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-v3-s1/mp3/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/mae\endcsname{10.8}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/w10\endcsname{72.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/w20\endcsname{88.8}
\expandafter\def\csname v@timit/ft-ts-v3-s1/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/dmae\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/dw50\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/mae\endcsname{12.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/w10\endcsname{68.6}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/w100\endcsname{98.6}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/w20\endcsname{85.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/amrnb/w50\endcsname{94.9}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/mae\endcsname{10.6}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/w10\endcsname{73.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/w20\endcsname{89.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/w10\endcsname{72.5}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/w20\endcsname{88.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/w10\endcsname{70.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/w20\endcsname{88.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g723/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/w10\endcsname{71.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/w10\endcsname{70.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/w20\endcsname{87.6}
\expandafter\def\csname v@timit/ft-ts-v3-s2/gsm/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/mae\endcsname{11.5}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/median\endcsname{5.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/w10\endcsname{70.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/w20\endcsname{87.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/w10\endcsname{72.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/w20\endcsname{88.4}
\expandafter\def\csname v@timit/ft-ts-v3-s2/opus/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/dmae\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/dw50\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/mae\endcsname{10.7}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/median\endcsname{5.3}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/w10\endcsname{72.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/w20\endcsname{88.8}
\expandafter\def\csname v@timit/ft-ts-v3-s2/pcm/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/dw20\endcsname{3.7}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/dw50\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/median\endcsname{5.9}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/w10\endcsname{68.7}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/w100\endcsname{98.5}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-v3/amrnb/w50\endcsname{94.8}
\expandafter\def\csname v@timit/ft-ts-v3/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/clean/mae\endcsname{10.4}
\expandafter\def\csname v@timit/ft-ts-v3/clean/median\endcsname{5.1}
\expandafter\def\csname v@timit/ft-ts-v3/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/clean/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/clean/w10\endcsname{73.7}
\expandafter\def\csname v@timit/ft-ts-v3/clean/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-v3/clean/w20\endcsname{89.3}
\expandafter\def\csname v@timit/ft-ts-v3/clean/w50\endcsname{96.4}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/w10\endcsname{72.2}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-v3/g711u/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3/g723/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-v3/g723/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/mae\endcsname{11.4}
\expandafter\def\csname v@timit/ft-ts-v3/g723/median\endcsname{5.6}
\expandafter\def\csname v@timit/ft-ts-v3/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/g723/w10\endcsname{70.8}
\expandafter\def\csname v@timit/ft-ts-v3/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3/g723/w20\endcsname{88.2}
\expandafter\def\csname v@timit/ft-ts-v3/g723/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3/g726/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3/g726/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-v3/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/mae\endcsname{11.1}
\expandafter\def\csname v@timit/ft-ts-v3/g726/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/g726/w10\endcsname{71.6}
\expandafter\def\csname v@timit/ft-ts-v3/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3/g726/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-v3/g726/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/w10\endcsname{70.1}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-v3/gsm/w50\endcsname{96.1}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/dw20\endcsname{1.6}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/mae\endcsname{11.3}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/median\endcsname{5.8}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/w10\endcsname{69.9}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/w20\endcsname{87.7}
\expandafter\def\csname v@timit/ft-ts-v3/mp3/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-v3/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3/opus/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-v3/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-v3/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-v3/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/mae\endcsname{10.9}
\expandafter\def\csname v@timit/ft-ts-v3/opus/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/opus/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/opus/w10\endcsname{71.9}
\expandafter\def\csname v@timit/ft-ts-v3/opus/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3/opus/w20\endcsname{88.3}
\expandafter\def\csname v@timit/ft-ts-v3/opus/w50\endcsname{96.2}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/mae\endcsname{11.0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/median\endcsname{5.4}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/w10\endcsname{72.6}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/w20\endcsname{88.6}
\expandafter\def\csname v@timit/ft-ts-v3/pcm/w50\endcsname{96.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/dmae\endcsname{2.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/dw20\endcsname{4.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/median\endcsname{7.4}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/w10\endcsname{62.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/w100\endcsname{98.4}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/w20\endcsname{83.4}
\expandafter\def\csname v@timit/ft-ts-wt-s1/amrnb/w50\endcsname{94.2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/mae\endcsname{11.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/median\endcsname{6.6}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/rtf\endcsname{0.036}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/w10\endcsname{67.7}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/w20\endcsname{87.4}
\expandafter\def\csname v@timit/ft-ts-wt-s1/clean/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/w10\endcsname{65.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g711u/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/dw20\endcsname{1.5}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/mae\endcsname{12.5}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/median\endcsname{7.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/w10\endcsname{64.7}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/w20\endcsname{85.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g723/w50\endcsname{95.7}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/w10\endcsname{65.5}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/g726/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/median\endcsname{7.2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/w10\endcsname{64.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/w20\endcsname{85.5}
\expandafter\def\csname v@timit/ft-ts-wt-s1/gsm/w50\endcsname{95.6}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/dw20\endcsname{2.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/mae\endcsname{12.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/median\endcsname{7.2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/w10\endcsname{63.7}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/w100\endcsname{99.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/w20\endcsname{85.2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/mp3/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/dw20\endcsname{1.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/w10\endcsname{65.7}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/w20\endcsname{86.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/opus/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/w10\endcsname{66.1}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/w20\endcsname{86.7}
\expandafter\def\csname v@timit/ft-ts-wt-s1/pcm/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/dmae\endcsname{2.4}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/dw20\endcsname{3.9}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/dw50\endcsname{1.8}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/mae\endcsname{14.1}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/median\endcsname{7.4}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/sbias\endcsname{2}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/w10\endcsname{62.7}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/w100\endcsname{98.3}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/w20\endcsname{83.7}
\expandafter\def\csname v@timit/ft-ts-wt/amrnb/w50\endcsname{94.2}
\expandafter\def\csname v@timit/ft-ts-wt/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/mae\endcsname{11.7}
\expandafter\def\csname v@timit/ft-ts-wt/clean/median\endcsname{6.5}
\expandafter\def\csname v@timit/ft-ts-wt/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/rtf\endcsname{0.036}
\expandafter\def\csname v@timit/ft-ts-wt/clean/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/clean/w10\endcsname{68.0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt/clean/w20\endcsname{87.5}
\expandafter\def\csname v@timit/ft-ts-wt/clean/w50\endcsname{96.0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/dw20\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/mae\endcsname{12.1}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/median\endcsname{6.8}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/w10\endcsname{66.5}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/w20\endcsname{86.8}
\expandafter\def\csname v@timit/ft-ts-wt/g711u/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-wt/g723/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-wt/g723/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/ft-ts-wt/g723/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-wt/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-wt/g723/median\endcsname{7.0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/g723/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/g723/w10\endcsname{65.3}
\expandafter\def\csname v@timit/ft-ts-wt/g723/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt/g723/w20\endcsname{86.2}
\expandafter\def\csname v@timit/ft-ts-wt/g723/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt/g726/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/ft-ts-wt/g726/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-wt/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/mae\endcsname{12.3}
\expandafter\def\csname v@timit/ft-ts-wt/g726/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-wt/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/g726/w10\endcsname{66.0}
\expandafter\def\csname v@timit/ft-ts-wt/g726/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-wt/g726/w20\endcsname{86.5}
\expandafter\def\csname v@timit/ft-ts-wt/g726/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/mae\endcsname{12.4}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/median\endcsname{7.1}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/w10\endcsname{64.8}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/w20\endcsname{85.9}
\expandafter\def\csname v@timit/ft-ts-wt/gsm/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/dw20\endcsname{2.0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/mae\endcsname{12.5}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/median\endcsname{7.2}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/w10\endcsname{63.9}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/w20\endcsname{85.6}
\expandafter\def\csname v@timit/ft-ts-wt/mp3/w50\endcsname{95.9}
\expandafter\def\csname v@timit/ft-ts-wt/opus/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-wt/opus/dw20\endcsname{0.9}
\expandafter\def\csname v@timit/ft-ts-wt/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/ft-ts-wt/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/opus/mae\endcsname{12.2}
\expandafter\def\csname v@timit/ft-ts-wt/opus/median\endcsname{6.9}
\expandafter\def\csname v@timit/ft-ts-wt/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/opus/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/opus/sbias\endcsname{1}
\expandafter\def\csname v@timit/ft-ts-wt/opus/sbias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/ft-ts-wt/opus/w10\endcsname{66.0}
\expandafter\def\csname v@timit/ft-ts-wt/opus/w100\endcsname{98.9}
\expandafter\def\csname v@timit/ft-ts-wt/opus/w20\endcsname{86.6}
\expandafter\def\csname v@timit/ft-ts-wt/opus/w50\endcsname{95.8}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/dw20\endcsname{0.5}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/mae\endcsname{12.0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/median\endcsname{6.7}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/sbias\endcsname{0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/w10\endcsname{66.8}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/w100\endcsname{99.0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/w20\endcsname{87.0}
\expandafter\def\csname v@timit/ft-ts-wt/pcm/w50\endcsname{96.0}
\expandafter\def\csname v@timit/hours\endcsname{1.15}
\expandafter\def\csname v@timit/lag/amrnb\endcsname{5.000}
\expandafter\def\csname v@timit/lag/g711u\endcsname{0.000}
\expandafter\def\csname v@timit/lag/g723\endcsname{7.500}
\expandafter\def\csname v@timit/lag/g726\endcsname{0.000}
\expandafter\def\csname v@timit/lag/gsm\endcsname{0.000}
\expandafter\def\csname v@timit/lag/mp3\endcsname{138.125}
\expandafter\def\csname v@timit/lag/opus\endcsname{0.125}
\expandafter\def\csname v@timit/lag/pcm\endcsname{0.000}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/dmae\endcsname{6.1}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/dw20\endcsname{4.5}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/dw50\endcsname{5.3}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/mae\endcsname{25.2}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/median\endcsname{12.5}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/sbias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/w10\endcsname{41.9}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/w100\endcsname{95.1}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/w20\endcsname{63.6}
\expandafter\def\csname v@timit/mfa-arpa/amrnb/w50\endcsname{86.6}
\expandafter\def\csname v@timit/mfa-arpa/ce/dmae\endcsname{24.0}
\expandafter\def\csname v@timit/mfa-arpa/ce/dw20\endcsname{15.1}
\expandafter\def\csname v@timit/mfa-arpa/ce/dw50\endcsname{16.1}
\expandafter\def\csname v@timit/mfa-arpa/ce/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/ce/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/ce/fail\endcsname{37}
\expandafter\def\csname v@timit/mfa-arpa/ce/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/ce/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/ce/fail-other\endcsname{37}
\expandafter\def\csname v@timit/mfa-arpa/ce/mae\endcsname{43.1}
\expandafter\def\csname v@timit/mfa-arpa/ce/median\endcsname{17.5}
\expandafter\def\csname v@timit/mfa-arpa/ce/over500\endcsname{0.6}
\expandafter\def\csname v@timit/mfa-arpa/ce/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/mfa-arpa/ce/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/ce/sbias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/mfa-arpa/ce/w10\endcsname{33.7}
\expandafter\def\csname v@timit/mfa-arpa/ce/w100\endcsname{89.0}
\expandafter\def\csname v@timit/mfa-arpa/ce/w20\endcsname{53.0}
\expandafter\def\csname v@timit/mfa-arpa/ce/w50\endcsname{75.8}
\expandafter\def\csname v@timit/mfa-arpa/clean/ebias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/clean/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/mfa-arpa/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/clean/mae\endcsname{19.1}
\expandafter\def\csname v@timit/mfa-arpa/clean/median\endcsname{12.0}
\expandafter\def\csname v@timit/mfa-arpa/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/clean/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/mfa-arpa/clean/sbias\endcsname{3}
\expandafter\def\csname v@timit/mfa-arpa/clean/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/mfa-arpa/clean/w10\endcsname{45.4}
\expandafter\def\csname v@timit/mfa-arpa/clean/w100\endcsname{98.3}
\expandafter\def\csname v@timit/mfa-arpa/clean/w20\endcsname{68.2}
\expandafter\def\csname v@timit/mfa-arpa/clean/w50\endcsname{91.9}
\expandafter\def\csname v@timit/mfa-arpa/g711u/dmae\endcsname{6.2}
\expandafter\def\csname v@timit/mfa-arpa/g711u/dw20\endcsname{5.1}
\expandafter\def\csname v@timit/mfa-arpa/g711u/dw50\endcsname{5.3}
\expandafter\def\csname v@timit/mfa-arpa/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/mfa-arpa/g711u/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/mfa-arpa/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g711u/mae\endcsname{25.3}
\expandafter\def\csname v@timit/mfa-arpa/g711u/median\endcsname{12.5}
\expandafter\def\csname v@timit/mfa-arpa/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/g711u/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/mfa-arpa/g711u/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/g711u/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-arpa/g711u/w10\endcsname{41.6}
\expandafter\def\csname v@timit/mfa-arpa/g711u/w100\endcsname{95.0}
\expandafter\def\csname v@timit/mfa-arpa/g711u/w20\endcsname{63.1}
\expandafter\def\csname v@timit/mfa-arpa/g711u/w50\endcsname{86.6}
\expandafter\def\csname v@timit/mfa-arpa/g723/dmae\endcsname{6.4}
\expandafter\def\csname v@timit/mfa-arpa/g723/dw20\endcsname{5.6}
\expandafter\def\csname v@timit/mfa-arpa/g723/dw50\endcsname{5.6}
\expandafter\def\csname v@timit/mfa-arpa/g723/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g723/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g723/mae\endcsname{25.6}
\expandafter\def\csname v@timit/mfa-arpa/g723/median\endcsname{12.9}
\expandafter\def\csname v@timit/mfa-arpa/g723/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/g723/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/mfa-arpa/g723/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/g723/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-arpa/g723/w10\endcsname{40.3}
\expandafter\def\csname v@timit/mfa-arpa/g723/w100\endcsname{95.2}
\expandafter\def\csname v@timit/mfa-arpa/g723/w20\endcsname{62.6}
\expandafter\def\csname v@timit/mfa-arpa/g723/w50\endcsname{86.3}
\expandafter\def\csname v@timit/mfa-arpa/g726/dmae\endcsname{7.6}
\expandafter\def\csname v@timit/mfa-arpa/g726/dw20\endcsname{6.7}
\expandafter\def\csname v@timit/mfa-arpa/g726/dw50\endcsname{6.8}
\expandafter\def\csname v@timit/mfa-arpa/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/mfa-arpa/g726/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/mfa-arpa/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/g726/mae\endcsname{26.8}
\expandafter\def\csname v@timit/mfa-arpa/g726/median\endcsname{13.6}
\expandafter\def\csname v@timit/mfa-arpa/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/g726/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/mfa-arpa/g726/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/g726/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-arpa/g726/w10\endcsname{39.6}
\expandafter\def\csname v@timit/mfa-arpa/g726/w100\endcsname{94.7}
\expandafter\def\csname v@timit/mfa-arpa/g726/w20\endcsname{61.5}
\expandafter\def\csname v@timit/mfa-arpa/g726/w50\endcsname{85.0}
\expandafter\def\csname v@timit/mfa-arpa/gsm/dmae\endcsname{6.7}
\expandafter\def\csname v@timit/mfa-arpa/gsm/dw20\endcsname{5.5}
\expandafter\def\csname v@timit/mfa-arpa/gsm/dw50\endcsname{5.6}
\expandafter\def\csname v@timit/mfa-arpa/gsm/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/gsm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/gsm/mae\endcsname{25.8}
\expandafter\def\csname v@timit/mfa-arpa/gsm/median\endcsname{12.8}
\expandafter\def\csname v@timit/mfa-arpa/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/gsm/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/mfa-arpa/gsm/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/gsm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-arpa/gsm/w10\endcsname{40.3}
\expandafter\def\csname v@timit/mfa-arpa/gsm/w100\endcsname{94.8}
\expandafter\def\csname v@timit/mfa-arpa/gsm/w20\endcsname{62.7}
\expandafter\def\csname v@timit/mfa-arpa/gsm/w50\endcsname{86.3}
\expandafter\def\csname v@timit/mfa-arpa/mp3/dmae\endcsname{6.2}
\expandafter\def\csname v@timit/mfa-arpa/mp3/dw20\endcsname{5.3}
\expandafter\def\csname v@timit/mfa-arpa/mp3/dw50\endcsname{5.4}
\expandafter\def\csname v@timit/mfa-arpa/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/mp3/mae\endcsname{25.4}
\expandafter\def\csname v@timit/mfa-arpa/mp3/median\endcsname{12.7}
\expandafter\def\csname v@timit/mfa-arpa/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/mp3/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/mfa-arpa/mp3/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/mp3/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-arpa/mp3/w10\endcsname{40.9}
\expandafter\def\csname v@timit/mfa-arpa/mp3/w100\endcsname{95.1}
\expandafter\def\csname v@timit/mfa-arpa/mp3/w20\endcsname{62.9}
\expandafter\def\csname v@timit/mfa-arpa/mp3/w50\endcsname{86.5}
\expandafter\def\csname v@timit/mfa-arpa/opus/dmae\endcsname{6.3}
\expandafter\def\csname v@timit/mfa-arpa/opus/dw20\endcsname{5.1}
\expandafter\def\csname v@timit/mfa-arpa/opus/dw50\endcsname{5.6}
\expandafter\def\csname v@timit/mfa-arpa/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/opus/mae\endcsname{25.5}
\expandafter\def\csname v@timit/mfa-arpa/opus/median\endcsname{12.7}
\expandafter\def\csname v@timit/mfa-arpa/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/opus/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/mfa-arpa/opus/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/opus/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-arpa/opus/w10\endcsname{40.7}
\expandafter\def\csname v@timit/mfa-arpa/opus/w100\endcsname{95.1}
\expandafter\def\csname v@timit/mfa-arpa/opus/w20\endcsname{63.1}
\expandafter\def\csname v@timit/mfa-arpa/opus/w50\endcsname{86.3}
\expandafter\def\csname v@timit/mfa-arpa/pcm/dmae\endcsname{6.2}
\expandafter\def\csname v@timit/mfa-arpa/pcm/dw20\endcsname{5.0}
\expandafter\def\csname v@timit/mfa-arpa/pcm/dw50\endcsname{5.4}
\expandafter\def\csname v@timit/mfa-arpa/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-arpa/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-arpa/pcm/mae\endcsname{25.3}
\expandafter\def\csname v@timit/mfa-arpa/pcm/median\endcsname{12.5}
\expandafter\def\csname v@timit/mfa-arpa/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-arpa/pcm/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/mfa-arpa/pcm/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-arpa/pcm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-arpa/pcm/w10\endcsname{41.2}
\expandafter\def\csname v@timit/mfa-arpa/pcm/w100\endcsname{95.1}
\expandafter\def\csname v@timit/mfa-arpa/pcm/w20\endcsname{63.2}
\expandafter\def\csname v@timit/mfa-arpa/pcm/w50\endcsname{86.5}
\expandafter\def\csname v@timit/mfa-english/clean/ebias\endcsname{2}
\expandafter\def\csname v@timit/mfa-english/clean/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/mfa-english/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/clean/mae\endcsname{21.3}
\expandafter\def\csname v@timit/mfa-english/clean/median\endcsname{12.5}
\expandafter\def\csname v@timit/mfa-english/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-english/clean/rtf\endcsname{0.011}
\expandafter\def\csname v@timit/mfa-english/clean/sbias\endcsname{3}
\expandafter\def\csname v@timit/mfa-english/clean/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/mfa-english/clean/w10\endcsname{44.0}
\expandafter\def\csname v@timit/mfa-english/clean/w100\endcsname{97.9}
\expandafter\def\csname v@timit/mfa-english/clean/w20\endcsname{64.5}
\expandafter\def\csname v@timit/mfa-english/clean/w50\endcsname{90.2}
\expandafter\def\csname v@timit/mfa-english/g711u/dmae\endcsname{6.6}
\expandafter\def\csname v@timit/mfa-english/g711u/dw20\endcsname{5.9}
\expandafter\def\csname v@timit/mfa-english/g711u/dw50\endcsname{5.5}
\expandafter\def\csname v@timit/mfa-english/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/mfa-english/g711u/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/mfa-english/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g711u/mae\endcsname{27.9}
\expandafter\def\csname v@timit/mfa-english/g711u/median\endcsname{14.6}
\expandafter\def\csname v@timit/mfa-english/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-english/g711u/rtf\endcsname{0.012}
\expandafter\def\csname v@timit/mfa-english/g711u/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-english/g711u/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-english/g711u/w10\endcsname{40.1}
\expandafter\def\csname v@timit/mfa-english/g711u/w100\endcsname{94.5}
\expandafter\def\csname v@timit/mfa-english/g711u/w20\endcsname{58.6}
\expandafter\def\csname v@timit/mfa-english/g711u/w50\endcsname{84.7}
\expandafter\def\csname v@timit/mfa-english/g726/dmae\endcsname{15.9}
\expandafter\def\csname v@timit/mfa-english/g726/dw20\endcsname{11.7}
\expandafter\def\csname v@timit/mfa-english/g726/dw50\endcsname{12.9}
\expandafter\def\csname v@timit/mfa-english/g726/ebias\endcsname{3}
\expandafter\def\csname v@timit/mfa-english/g726/ebias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/mfa-english/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g726/mae\endcsname{37.2}
\expandafter\def\csname v@timit/mfa-english/g726/median\endcsname{17.5}
\expandafter\def\csname v@timit/mfa-english/g726/over500\endcsname{0.1}
\expandafter\def\csname v@timit/mfa-english/g726/rtf\endcsname{0.012}
\expandafter\def\csname v@timit/mfa-english/g726/sbias\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/g726/sbias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-english/g726/w10\endcsname{35.2}
\expandafter\def\csname v@timit/mfa-english/g726/w100\endcsname{90.9}
\expandafter\def\csname v@timit/mfa-english/g726/w20\endcsname{52.8}
\expandafter\def\csname v@timit/mfa-english/g726/w50\endcsname{77.3}
\expandafter\def\csname v@timit/mfa-english/gsm/dmae\endcsname{8.2}
\expandafter\def\csname v@timit/mfa-english/gsm/dw20\endcsname{7.1}
\expandafter\def\csname v@timit/mfa-english/gsm/dw50\endcsname{6.6}
\expandafter\def\csname v@timit/mfa-english/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/mfa-english/gsm/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/mfa-english/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/gsm/mae\endcsname{29.5}
\expandafter\def\csname v@timit/mfa-english/gsm/median\endcsname{15.4}
\expandafter\def\csname v@timit/mfa-english/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-english/gsm/rtf\endcsname{0.011}
\expandafter\def\csname v@timit/mfa-english/gsm/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-english/gsm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-english/gsm/w10\endcsname{38.3}
\expandafter\def\csname v@timit/mfa-english/gsm/w100\endcsname{93.7}
\expandafter\def\csname v@timit/mfa-english/gsm/w20\endcsname{57.3}
\expandafter\def\csname v@timit/mfa-english/gsm/w50\endcsname{83.6}
\expandafter\def\csname v@timit/mfa-english/mp3/dmae\endcsname{6.0}
\expandafter\def\csname v@timit/mfa-english/mp3/dw20\endcsname{5.9}
\expandafter\def\csname v@timit/mfa-english/mp3/dw50\endcsname{5.3}
\expandafter\def\csname v@timit/mfa-english/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/mfa-english/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/mp3/mae\endcsname{27.3}
\expandafter\def\csname v@timit/mfa-english/mp3/median\endcsname{14.6}
\expandafter\def\csname v@timit/mfa-english/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-english/mp3/rtf\endcsname{0.011}
\expandafter\def\csname v@timit/mfa-english/mp3/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-english/mp3/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-english/mp3/w10\endcsname{39.8}
\expandafter\def\csname v@timit/mfa-english/mp3/w100\endcsname{94.9}
\expandafter\def\csname v@timit/mfa-english/mp3/w20\endcsname{58.5}
\expandafter\def\csname v@timit/mfa-english/mp3/w50\endcsname{85.0}
\expandafter\def\csname v@timit/mfa-english/opus/dmae\endcsname{7.9}
\expandafter\def\csname v@timit/mfa-english/opus/dw20\endcsname{7.5}
\expandafter\def\csname v@timit/mfa-english/opus/dw50\endcsname{6.9}
\expandafter\def\csname v@timit/mfa-english/opus/ebias\endcsname{1}
\expandafter\def\csname v@timit/mfa-english/opus/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/mfa-english/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/opus/mae\endcsname{29.2}
\expandafter\def\csname v@timit/mfa-english/opus/median\endcsname{15.8}
\expandafter\def\csname v@timit/mfa-english/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-english/opus/rtf\endcsname{0.011}
\expandafter\def\csname v@timit/mfa-english/opus/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-english/opus/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-english/opus/w10\endcsname{37.5}
\expandafter\def\csname v@timit/mfa-english/opus/w100\endcsname{94.3}
\expandafter\def\csname v@timit/mfa-english/opus/w20\endcsname{57.0}
\expandafter\def\csname v@timit/mfa-english/opus/w50\endcsname{83.3}
\expandafter\def\csname v@timit/mfa-english/pcm/dmae\endcsname{6.8}
\expandafter\def\csname v@timit/mfa-english/pcm/dw20\endcsname{6.6}
\expandafter\def\csname v@timit/mfa-english/pcm/dw50\endcsname{6.1}
\expandafter\def\csname v@timit/mfa-english/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/mfa-english/pcm/ebias-signed\endcsname{$-1$}
\expandafter\def\csname v@timit/mfa-english/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mfa-english/pcm/mae\endcsname{28.1}
\expandafter\def\csname v@timit/mfa-english/pcm/median\endcsname{15.0}
\expandafter\def\csname v@timit/mfa-english/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mfa-english/pcm/rtf\endcsname{0.012}
\expandafter\def\csname v@timit/mfa-english/pcm/sbias\endcsname{2}
\expandafter\def\csname v@timit/mfa-english/pcm/sbias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/mfa-english/pcm/w10\endcsname{38.9}
\expandafter\def\csname v@timit/mfa-english/pcm/w100\endcsname{94.8}
\expandafter\def\csname v@timit/mfa-english/pcm/w20\endcsname{57.9}
\expandafter\def\csname v@timit/mfa-english/pcm/w50\endcsname{84.1}
\expandafter\def\csname v@timit/mms-torchaudio/clean/ebias\endcsname{18}
\expandafter\def\csname v@timit/mms-torchaudio/clean/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/mms-torchaudio/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/clean/mae\endcsname{37.5}
\expandafter\def\csname v@timit/mms-torchaudio/clean/median\endcsname{31.0}
\expandafter\def\csname v@timit/mms-torchaudio/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/clean/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/mms-torchaudio/clean/sbias\endcsname{40}
\expandafter\def\csname v@timit/mms-torchaudio/clean/sbias-signed\endcsname{$+40$}
\expandafter\def\csname v@timit/mms-torchaudio/clean/w10\endcsname{18.3}
\expandafter\def\csname v@timit/mms-torchaudio/clean/w100\endcsname{96.1}
\expandafter\def\csname v@timit/mms-torchaudio/clean/w20\endcsname{35.0}
\expandafter\def\csname v@timit/mms-torchaudio/clean/w50\endcsname{71.4}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/ebias\endcsname{18}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/mae\endcsname{37.9}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/median\endcsname{30.8}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/sbias\endcsname{40}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/sbias-signed\endcsname{$+40$}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/w10\endcsname{18.2}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/w100\endcsname{95.7}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/w20\endcsname{34.9}
\expandafter\def\csname v@timit/mms-torchaudio/g711u/w50\endcsname{71.3}
\expandafter\def\csname v@timit/mms-torchaudio/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/mms-torchaudio/g726/dw20\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/mms-torchaudio/g726/ebias\endcsname{18}
\expandafter\def\csname v@timit/mms-torchaudio/g726/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/mms-torchaudio/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/g726/mae\endcsname{37.9}
\expandafter\def\csname v@timit/mms-torchaudio/g726/median\endcsname{30.7}
\expandafter\def\csname v@timit/mms-torchaudio/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/g726/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/mms-torchaudio/g726/sbias\endcsname{40}
\expandafter\def\csname v@timit/mms-torchaudio/g726/sbias-signed\endcsname{$+40$}
\expandafter\def\csname v@timit/mms-torchaudio/g726/w10\endcsname{18.2}
\expandafter\def\csname v@timit/mms-torchaudio/g726/w100\endcsname{95.6}
\expandafter\def\csname v@timit/mms-torchaudio/g726/w20\endcsname{34.9}
\expandafter\def\csname v@timit/mms-torchaudio/g726/w50\endcsname{71.4}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/dw20\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/ebias\endcsname{17}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/ebias-signed\endcsname{$-17$}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/mae\endcsname{38.2}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/median\endcsname{30.8}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/sbias\endcsname{39}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/sbias-signed\endcsname{$+39$}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/w10\endcsname{18.1}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/w100\endcsname{95.4}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/w20\endcsname{35.0}
\expandafter\def\csname v@timit/mms-torchaudio/gsm/w50\endcsname{71.5}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/ebias\endcsname{18}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/mae\endcsname{38.1}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/median\endcsname{30.8}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/sbias\endcsname{39}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/sbias-signed\endcsname{$+39$}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/w10\endcsname{18.1}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/w100\endcsname{95.5}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/w20\endcsname{35.0}
\expandafter\def\csname v@timit/mms-torchaudio/mp3/w50\endcsname{71.2}
\expandafter\def\csname v@timit/mms-torchaudio/opus/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/mms-torchaudio/opus/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/mms-torchaudio/opus/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/mms-torchaudio/opus/ebias\endcsname{17}
\expandafter\def\csname v@timit/mms-torchaudio/opus/ebias-signed\endcsname{$-17$}
\expandafter\def\csname v@timit/mms-torchaudio/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/opus/mae\endcsname{38.1}
\expandafter\def\csname v@timit/mms-torchaudio/opus/median\endcsname{30.9}
\expandafter\def\csname v@timit/mms-torchaudio/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/opus/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/mms-torchaudio/opus/sbias\endcsname{40}
\expandafter\def\csname v@timit/mms-torchaudio/opus/sbias-signed\endcsname{$+40$}
\expandafter\def\csname v@timit/mms-torchaudio/opus/w10\endcsname{18.2}
\expandafter\def\csname v@timit/mms-torchaudio/opus/w100\endcsname{95.5}
\expandafter\def\csname v@timit/mms-torchaudio/opus/w20\endcsname{35.0}
\expandafter\def\csname v@timit/mms-torchaudio/opus/w50\endcsname{71.2}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/dw20\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/ebias\endcsname{18}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/mae\endcsname{37.9}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/median\endcsname{30.8}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/rtf\endcsname{0.007}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/sbias\endcsname{40}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/sbias-signed\endcsname{$+40$}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/w10\endcsname{18.2}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/w100\endcsname{95.7}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/w20\endcsname{35.0}
\expandafter\def\csname v@timit/mms-torchaudio/pcm/w50\endcsname{71.4}
\expandafter\def\csname v@timit/n-utt\endcsname{1{,}344}
\expandafter\def\csname v@timit/n-words\endcsname{11{,}025}
\expandafter\def\csname v@timit/qwen3fa/clean/ebias\endcsname{2}
\expandafter\def\csname v@timit/qwen3fa/clean/ebias-signed\endcsname{$-2$}
\expandafter\def\csname v@timit/qwen3fa/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/clean/mae\endcsname{30.1}
\expandafter\def\csname v@timit/qwen3fa/clean/median\endcsname{24.1}
\expandafter\def\csname v@timit/qwen3fa/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/qwen3fa/clean/rtf\endcsname{0.028}
\expandafter\def\csname v@timit/qwen3fa/clean/sbias\endcsname{4}
\expandafter\def\csname v@timit/qwen3fa/clean/sbias-signed\endcsname{$-4$}
\expandafter\def\csname v@timit/qwen3fa/clean/w10\endcsname{20.3}
\expandafter\def\csname v@timit/qwen3fa/clean/w100\endcsname{97.5}
\expandafter\def\csname v@timit/qwen3fa/clean/w20\endcsname{41.0}
\expandafter\def\csname v@timit/qwen3fa/clean/w50\endcsname{84.6}
\expandafter\def\csname v@timit/qwen3fa/g711u/dmae\endcsname{20.0}
\expandafter\def\csname v@timit/qwen3fa/g711u/dw20\endcsname{11.0}
\expandafter\def\csname v@timit/qwen3fa/g711u/dw50\endcsname{18.3}
\expandafter\def\csname v@timit/qwen3fa/g711u/ebias\endcsname{30}
\expandafter\def\csname v@timit/qwen3fa/g711u/ebias-signed\endcsname{$-30$}
\expandafter\def\csname v@timit/qwen3fa/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g711u/mae\endcsname{50.1}
\expandafter\def\csname v@timit/qwen3fa/g711u/median\endcsname{32.8}
\expandafter\def\csname v@timit/qwen3fa/g711u/over500\endcsname{0.1}
\expandafter\def\csname v@timit/qwen3fa/g711u/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/qwen3fa/g711u/sbias\endcsname{21}
\expandafter\def\csname v@timit/qwen3fa/g711u/sbias-signed\endcsname{$+21$}
\expandafter\def\csname v@timit/qwen3fa/g711u/w10\endcsname{14.6}
\expandafter\def\csname v@timit/qwen3fa/g711u/w100\endcsname{87.9}
\expandafter\def\csname v@timit/qwen3fa/g711u/w20\endcsname{30.0}
\expandafter\def\csname v@timit/qwen3fa/g711u/w50\endcsname{66.3}
\expandafter\def\csname v@timit/qwen3fa/g726/dmae\endcsname{24.4}
\expandafter\def\csname v@timit/qwen3fa/g726/dw20\endcsname{13.0}
\expandafter\def\csname v@timit/qwen3fa/g726/dw50\endcsname{21.9}
\expandafter\def\csname v@timit/qwen3fa/g726/ebias\endcsname{35}
\expandafter\def\csname v@timit/qwen3fa/g726/ebias-signed\endcsname{$-35$}
\expandafter\def\csname v@timit/qwen3fa/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/g726/mae\endcsname{54.4}
\expandafter\def\csname v@timit/qwen3fa/g726/median\endcsname{36.5}
\expandafter\def\csname v@timit/qwen3fa/g726/over500\endcsname{0.1}
\expandafter\def\csname v@timit/qwen3fa/g726/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/qwen3fa/g726/sbias\endcsname{23}
\expandafter\def\csname v@timit/qwen3fa/g726/sbias-signed\endcsname{$+23$}
\expandafter\def\csname v@timit/qwen3fa/g726/w10\endcsname{13.6}
\expandafter\def\csname v@timit/qwen3fa/g726/w100\endcsname{85.7}
\expandafter\def\csname v@timit/qwen3fa/g726/w20\endcsname{28.0}
\expandafter\def\csname v@timit/qwen3fa/g726/w50\endcsname{62.8}
\expandafter\def\csname v@timit/qwen3fa/gsm/dmae\endcsname{22.6}
\expandafter\def\csname v@timit/qwen3fa/gsm/dw20\endcsname{12.5}
\expandafter\def\csname v@timit/qwen3fa/gsm/dw50\endcsname{20.9}
\expandafter\def\csname v@timit/qwen3fa/gsm/ebias\endcsname{32}
\expandafter\def\csname v@timit/qwen3fa/gsm/ebias-signed\endcsname{$-32$}
\expandafter\def\csname v@timit/qwen3fa/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/gsm/mae\endcsname{52.6}
\expandafter\def\csname v@timit/qwen3fa/gsm/median\endcsname{35.3}
\expandafter\def\csname v@timit/qwen3fa/gsm/over500\endcsname{0.1}
\expandafter\def\csname v@timit/qwen3fa/gsm/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/qwen3fa/gsm/sbias\endcsname{22}
\expandafter\def\csname v@timit/qwen3fa/gsm/sbias-signed\endcsname{$+22$}
\expandafter\def\csname v@timit/qwen3fa/gsm/w10\endcsname{13.9}
\expandafter\def\csname v@timit/qwen3fa/gsm/w100\endcsname{86.5}
\expandafter\def\csname v@timit/qwen3fa/gsm/w20\endcsname{28.5}
\expandafter\def\csname v@timit/qwen3fa/gsm/w50\endcsname{63.8}
\expandafter\def\csname v@timit/qwen3fa/mp3/dmae\endcsname{34.7}
\expandafter\def\csname v@timit/qwen3fa/mp3/dw20\endcsname{15.4}
\expandafter\def\csname v@timit/qwen3fa/mp3/dw50\endcsname{26.9}
\expandafter\def\csname v@timit/qwen3fa/mp3/ebias\endcsname{42}
\expandafter\def\csname v@timit/qwen3fa/mp3/ebias-signed\endcsname{$-42$}
\expandafter\def\csname v@timit/qwen3fa/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/mp3/mae\endcsname{64.8}
\expandafter\def\csname v@timit/qwen3fa/mp3/median\endcsname{40.4}
\expandafter\def\csname v@timit/qwen3fa/mp3/over500\endcsname{0.3}
\expandafter\def\csname v@timit/qwen3fa/mp3/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/qwen3fa/mp3/sbias\endcsname{27}
\expandafter\def\csname v@timit/qwen3fa/mp3/sbias-signed\endcsname{$+27$}
\expandafter\def\csname v@timit/qwen3fa/mp3/w10\endcsname{12.5}
\expandafter\def\csname v@timit/qwen3fa/mp3/w100\endcsname{81.6}
\expandafter\def\csname v@timit/qwen3fa/mp3/w20\endcsname{25.6}
\expandafter\def\csname v@timit/qwen3fa/mp3/w50\endcsname{57.8}
\expandafter\def\csname v@timit/qwen3fa/opus/dmae\endcsname{22.2}
\expandafter\def\csname v@timit/qwen3fa/opus/dw20\endcsname{12.0}
\expandafter\def\csname v@timit/qwen3fa/opus/dw50\endcsname{20.0}
\expandafter\def\csname v@timit/qwen3fa/opus/ebias\endcsname{33}
\expandafter\def\csname v@timit/qwen3fa/opus/ebias-signed\endcsname{$-33$}
\expandafter\def\csname v@timit/qwen3fa/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/opus/mae\endcsname{52.3}
\expandafter\def\csname v@timit/qwen3fa/opus/median\endcsname{34.5}
\expandafter\def\csname v@timit/qwen3fa/opus/over500\endcsname{0.1}
\expandafter\def\csname v@timit/qwen3fa/opus/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/qwen3fa/opus/sbias\endcsname{22}
\expandafter\def\csname v@timit/qwen3fa/opus/sbias-signed\endcsname{$+22$}
\expandafter\def\csname v@timit/qwen3fa/opus/w10\endcsname{14.2}
\expandafter\def\csname v@timit/qwen3fa/opus/w100\endcsname{87.0}
\expandafter\def\csname v@timit/qwen3fa/opus/w20\endcsname{29.1}
\expandafter\def\csname v@timit/qwen3fa/opus/w50\endcsname{64.6}
\expandafter\def\csname v@timit/qwen3fa/pcm/dmae\endcsname{22.6}
\expandafter\def\csname v@timit/qwen3fa/pcm/dw20\endcsname{12.1}
\expandafter\def\csname v@timit/qwen3fa/pcm/dw50\endcsname{20.6}
\expandafter\def\csname v@timit/qwen3fa/pcm/ebias\endcsname{33}
\expandafter\def\csname v@timit/qwen3fa/pcm/ebias-signed\endcsname{$-33$}
\expandafter\def\csname v@timit/qwen3fa/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/qwen3fa/pcm/mae\endcsname{52.7}
\expandafter\def\csname v@timit/qwen3fa/pcm/median\endcsname{35.0}
\expandafter\def\csname v@timit/qwen3fa/pcm/over500\endcsname{0.1}
\expandafter\def\csname v@timit/qwen3fa/pcm/rtf\endcsname{0.020}
\expandafter\def\csname v@timit/qwen3fa/pcm/sbias\endcsname{21}
\expandafter\def\csname v@timit/qwen3fa/pcm/sbias-signed\endcsname{$+21$}
\expandafter\def\csname v@timit/qwen3fa/pcm/w10\endcsname{14.1}
\expandafter\def\csname v@timit/qwen3fa/pcm/w100\endcsname{86.4}
\expandafter\def\csname v@timit/qwen3fa/pcm/w20\endcsname{29.0}
\expandafter\def\csname v@timit/qwen3fa/pcm/w50\endcsname{64.0}
\expandafter\def\csname v@timit/stablets/clean/ebias\endcsname{51}
\expandafter\def\csname v@timit/stablets/clean/ebias-signed\endcsname{$-51$}
\expandafter\def\csname v@timit/stablets/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/stablets/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/stablets/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/stablets/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/stablets/clean/mae\endcsname{77.5}
\expandafter\def\csname v@timit/stablets/clean/median\endcsname{52.9}
\expandafter\def\csname v@timit/stablets/clean/over500\endcsname{0.5}
\expandafter\def\csname v@timit/stablets/clean/rtf\endcsname{0.041}
\expandafter\def\csname v@timit/stablets/clean/sbias\endcsname{22}
\expandafter\def\csname v@timit/stablets/clean/sbias-signed\endcsname{$-22$}
\expandafter\def\csname v@timit/stablets/clean/w10\endcsname{10.2}
\expandafter\def\csname v@timit/stablets/clean/w100\endcsname{74.0}
\expandafter\def\csname v@timit/stablets/clean/w20\endcsname{20.6}
\expandafter\def\csname v@timit/stablets/clean/w50\endcsname{47.3}
\expandafter\def\csname v@timit/stablets/g711u/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/stablets/g711u/dw20\endcsname{-0.7}
\expandafter\def\csname v@timit/stablets/g711u/dw50\endcsname{-0.5}
\expandafter\def\csname v@timit/stablets/g711u/ebias\endcsname{47}
\expandafter\def\csname v@timit/stablets/g711u/ebias-signed\endcsname{$-47$}
\expandafter\def\csname v@timit/stablets/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/stablets/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/stablets/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/stablets/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/stablets/g711u/mae\endcsname{78.3}
\expandafter\def\csname v@timit/stablets/g711u/median\endcsname{52.5}
\expandafter\def\csname v@timit/stablets/g711u/over500\endcsname{0.6}
\expandafter\def\csname v@timit/stablets/g711u/rtf\endcsname{0.040}
\expandafter\def\csname v@timit/stablets/g711u/sbias\endcsname{15}
\expandafter\def\csname v@timit/stablets/g711u/sbias-signed\endcsname{$-15$}
\expandafter\def\csname v@timit/stablets/g711u/w10\endcsname{10.7}
\expandafter\def\csname v@timit/stablets/g711u/w100\endcsname{74.1}
\expandafter\def\csname v@timit/stablets/g711u/w20\endcsname{21.3}
\expandafter\def\csname v@timit/stablets/g711u/w50\endcsname{47.9}
\expandafter\def\csname v@timit/stablets/g726/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/stablets/g726/dw20\endcsname{-0.6}
\expandafter\def\csname v@timit/stablets/g726/dw50\endcsname{-0.5}
\expandafter\def\csname v@timit/stablets/g726/ebias\endcsname{47}
\expandafter\def\csname v@timit/stablets/g726/ebias-signed\endcsname{$-47$}
\expandafter\def\csname v@timit/stablets/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/stablets/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/stablets/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/stablets/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/stablets/g726/mae\endcsname{78.1}
\expandafter\def\csname v@timit/stablets/g726/median\endcsname{52.5}
\expandafter\def\csname v@timit/stablets/g726/over500\endcsname{0.6}
\expandafter\def\csname v@timit/stablets/g726/rtf\endcsname{0.039}
\expandafter\def\csname v@timit/stablets/g726/sbias\endcsname{15}
\expandafter\def\csname v@timit/stablets/g726/sbias-signed\endcsname{$-15$}
\expandafter\def\csname v@timit/stablets/g726/w10\endcsname{10.7}
\expandafter\def\csname v@timit/stablets/g726/w100\endcsname{74.1}
\expandafter\def\csname v@timit/stablets/g726/w20\endcsname{21.3}
\expandafter\def\csname v@timit/stablets/g726/w50\endcsname{47.9}
\expandafter\def\csname v@timit/stablets/gsm/dmae\endcsname{0.2}
\expandafter\def\csname v@timit/stablets/gsm/dw20\endcsname{-0.7}
\expandafter\def\csname v@timit/stablets/gsm/dw50\endcsname{-0.5}
\expandafter\def\csname v@timit/stablets/gsm/ebias\endcsname{46}
\expandafter\def\csname v@timit/stablets/gsm/ebias-signed\endcsname{$-46$}
\expandafter\def\csname v@timit/stablets/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/stablets/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/stablets/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/stablets/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/stablets/gsm/mae\endcsname{77.8}
\expandafter\def\csname v@timit/stablets/gsm/median\endcsname{52.5}
\expandafter\def\csname v@timit/stablets/gsm/over500\endcsname{0.6}
\expandafter\def\csname v@timit/stablets/gsm/rtf\endcsname{0.040}
\expandafter\def\csname v@timit/stablets/gsm/sbias\endcsname{13}
\expandafter\def\csname v@timit/stablets/gsm/sbias-signed\endcsname{$-13$}
\expandafter\def\csname v@timit/stablets/gsm/w10\endcsname{10.9}
\expandafter\def\csname v@timit/stablets/gsm/w100\endcsname{74.2}
\expandafter\def\csname v@timit/stablets/gsm/w20\endcsname{21.3}
\expandafter\def\csname v@timit/stablets/gsm/w50\endcsname{47.8}
\expandafter\def\csname v@timit/stablets/mp3/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/stablets/mp3/dw20\endcsname{-0.5}
\expandafter\def\csname v@timit/stablets/mp3/dw50\endcsname{-0.4}
\expandafter\def\csname v@timit/stablets/mp3/ebias\endcsname{47}
\expandafter\def\csname v@timit/stablets/mp3/ebias-signed\endcsname{$-47$}
\expandafter\def\csname v@timit/stablets/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/stablets/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/stablets/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/stablets/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/stablets/mp3/mae\endcsname{78.2}
\expandafter\def\csname v@timit/stablets/mp3/median\endcsname{52.5}
\expandafter\def\csname v@timit/stablets/mp3/over500\endcsname{0.6}
\expandafter\def\csname v@timit/stablets/mp3/rtf\endcsname{0.040}
\expandafter\def\csname v@timit/stablets/mp3/sbias\endcsname{15}
\expandafter\def\csname v@timit/stablets/mp3/sbias-signed\endcsname{$-15$}
\expandafter\def\csname v@timit/stablets/mp3/w10\endcsname{10.7}
\expandafter\def\csname v@timit/stablets/mp3/w100\endcsname{74.0}
\expandafter\def\csname v@timit/stablets/mp3/w20\endcsname{21.2}
\expandafter\def\csname v@timit/stablets/mp3/w50\endcsname{47.8}
\expandafter\def\csname v@timit/stablets/opus/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/stablets/opus/dw20\endcsname{-0.7}
\expandafter\def\csname v@timit/stablets/opus/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/stablets/opus/ebias\endcsname{46}
\expandafter\def\csname v@timit/stablets/opus/ebias-signed\endcsname{$-46$}
\expandafter\def\csname v@timit/stablets/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/stablets/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/stablets/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/stablets/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/stablets/opus/mae\endcsname{78.7}
\expandafter\def\csname v@timit/stablets/opus/median\endcsname{52.7}
\expandafter\def\csname v@timit/stablets/opus/over500\endcsname{0.6}
\expandafter\def\csname v@timit/stablets/opus/rtf\endcsname{0.040}
\expandafter\def\csname v@timit/stablets/opus/sbias\endcsname{13}
\expandafter\def\csname v@timit/stablets/opus/sbias-signed\endcsname{$-13$}
\expandafter\def\csname v@timit/stablets/opus/w10\endcsname{10.7}
\expandafter\def\csname v@timit/stablets/opus/w100\endcsname{73.9}
\expandafter\def\csname v@timit/stablets/opus/w20\endcsname{21.3}
\expandafter\def\csname v@timit/stablets/opus/w50\endcsname{47.5}
\expandafter\def\csname v@timit/stablets/pcm/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/stablets/pcm/dw20\endcsname{-0.5}
\expandafter\def\csname v@timit/stablets/pcm/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/stablets/pcm/ebias\endcsname{47}
\expandafter\def\csname v@timit/stablets/pcm/ebias-signed\endcsname{$-47$}
\expandafter\def\csname v@timit/stablets/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/stablets/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/stablets/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/stablets/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/stablets/pcm/mae\endcsname{78.8}
\expandafter\def\csname v@timit/stablets/pcm/median\endcsname{52.7}
\expandafter\def\csname v@timit/stablets/pcm/over500\endcsname{0.6}
\expandafter\def\csname v@timit/stablets/pcm/rtf\endcsname{0.040}
\expandafter\def\csname v@timit/stablets/pcm/sbias\endcsname{15}
\expandafter\def\csname v@timit/stablets/pcm/sbias-signed\endcsname{$-15$}
\expandafter\def\csname v@timit/stablets/pcm/w10\endcsname{10.6}
\expandafter\def\csname v@timit/stablets/pcm/w100\endcsname{73.8}
\expandafter\def\csname v@timit/stablets/pcm/w20\endcsname{21.2}
\expandafter\def\csname v@timit/stablets/pcm/w50\endcsname{47.5}
\expandafter\def\csname v@timit/sttapi/clean/ebias\endcsname{18}
\expandafter\def\csname v@timit/sttapi/clean/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/sttapi/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/sttapi/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/sttapi/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/sttapi/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/sttapi/clean/mae\endcsname{35.6}
\expandafter\def\csname v@timit/sttapi/clean/median\endcsname{28.7}
\expandafter\def\csname v@timit/sttapi/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/clean/rtf\endcsname{0.044}
\expandafter\def\csname v@timit/sttapi/clean/sbias\endcsname{30}
\expandafter\def\csname v@timit/sttapi/clean/sbias-signed\endcsname{$+30$}
\expandafter\def\csname v@timit/sttapi/clean/w10\endcsname{17.6}
\expandafter\def\csname v@timit/sttapi/clean/w100\endcsname{96.2}
\expandafter\def\csname v@timit/sttapi/clean/w20\endcsname{35.4}
\expandafter\def\csname v@timit/sttapi/clean/w50\endcsname{76.4}
\expandafter\def\csname v@timit/sttapi/g711u/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/sttapi/g711u/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/sttapi/g711u/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/sttapi/g711u/ebias\endcsname{18}
\expandafter\def\csname v@timit/sttapi/g711u/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/sttapi/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g711u/mae\endcsname{36.4}
\expandafter\def\csname v@timit/sttapi/g711u/median\endcsname{28.8}
\expandafter\def\csname v@timit/sttapi/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/g711u/rtf\endcsname{0.038}
\expandafter\def\csname v@timit/sttapi/g711u/sbias\endcsname{29}
\expandafter\def\csname v@timit/sttapi/g711u/sbias-signed\endcsname{$+29$}
\expandafter\def\csname v@timit/sttapi/g711u/w10\endcsname{17.4}
\expandafter\def\csname v@timit/sttapi/g711u/w100\endcsname{95.7}
\expandafter\def\csname v@timit/sttapi/g711u/w20\endcsname{35.2}
\expandafter\def\csname v@timit/sttapi/g711u/w50\endcsname{75.9}
\expandafter\def\csname v@timit/sttapi/g726/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/sttapi/g726/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/sttapi/g726/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/sttapi/g726/ebias\endcsname{18}
\expandafter\def\csname v@timit/sttapi/g726/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/sttapi/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/sttapi/g726/mae\endcsname{36.6}
\expandafter\def\csname v@timit/sttapi/g726/median\endcsname{29.0}
\expandafter\def\csname v@timit/sttapi/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/g726/rtf\endcsname{0.038}
\expandafter\def\csname v@timit/sttapi/g726/sbias\endcsname{29}
\expandafter\def\csname v@timit/sttapi/g726/sbias-signed\endcsname{$+29$}
\expandafter\def\csname v@timit/sttapi/g726/w10\endcsname{17.5}
\expandafter\def\csname v@timit/sttapi/g726/w100\endcsname{95.6}
\expandafter\def\csname v@timit/sttapi/g726/w20\endcsname{35.2}
\expandafter\def\csname v@timit/sttapi/g726/w50\endcsname{76.1}
\expandafter\def\csname v@timit/sttapi/gsm/dmae\endcsname{1.6}
\expandafter\def\csname v@timit/sttapi/gsm/dw20\endcsname{-0.3}
\expandafter\def\csname v@timit/sttapi/gsm/dw50\endcsname{0.8}
\expandafter\def\csname v@timit/sttapi/gsm/ebias\endcsname{16}
\expandafter\def\csname v@timit/sttapi/gsm/ebias-signed\endcsname{$-16$}
\expandafter\def\csname v@timit/sttapi/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/sttapi/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/sttapi/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/sttapi/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/sttapi/gsm/mae\endcsname{37.2}
\expandafter\def\csname v@timit/sttapi/gsm/median\endcsname{28.7}
\expandafter\def\csname v@timit/sttapi/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/gsm/rtf\endcsname{0.038}
\expandafter\def\csname v@timit/sttapi/gsm/sbias\endcsname{29}
\expandafter\def\csname v@timit/sttapi/gsm/sbias-signed\endcsname{$+29$}
\expandafter\def\csname v@timit/sttapi/gsm/w10\endcsname{17.8}
\expandafter\def\csname v@timit/sttapi/gsm/w100\endcsname{94.9}
\expandafter\def\csname v@timit/sttapi/gsm/w20\endcsname{35.6}
\expandafter\def\csname v@timit/sttapi/gsm/w50\endcsname{75.7}
\expandafter\def\csname v@timit/sttapi/mp3/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/sttapi/mp3/dw20\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/mp3/dw50\endcsname{0.6}
\expandafter\def\csname v@timit/sttapi/mp3/ebias\endcsname{18}
\expandafter\def\csname v@timit/sttapi/mp3/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/sttapi/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/sttapi/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/sttapi/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/sttapi/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/sttapi/mp3/mae\endcsname{36.9}
\expandafter\def\csname v@timit/sttapi/mp3/median\endcsname{28.9}
\expandafter\def\csname v@timit/sttapi/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/mp3/rtf\endcsname{0.038}
\expandafter\def\csname v@timit/sttapi/mp3/sbias\endcsname{28}
\expandafter\def\csname v@timit/sttapi/mp3/sbias-signed\endcsname{$+28$}
\expandafter\def\csname v@timit/sttapi/mp3/w10\endcsname{17.5}
\expandafter\def\csname v@timit/sttapi/mp3/w100\endcsname{95.5}
\expandafter\def\csname v@timit/sttapi/mp3/w20\endcsname{35.4}
\expandafter\def\csname v@timit/sttapi/mp3/w50\endcsname{75.8}
\expandafter\def\csname v@timit/sttapi/opus/dmae\endcsname{1.5}
\expandafter\def\csname v@timit/sttapi/opus/dw20\endcsname{0.2}
\expandafter\def\csname v@timit/sttapi/opus/dw50\endcsname{0.8}
\expandafter\def\csname v@timit/sttapi/opus/ebias\endcsname{17}
\expandafter\def\csname v@timit/sttapi/opus/ebias-signed\endcsname{$-17$}
\expandafter\def\csname v@timit/sttapi/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/sttapi/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/sttapi/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/sttapi/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/sttapi/opus/mae\endcsname{37.1}
\expandafter\def\csname v@timit/sttapi/opus/median\endcsname{28.9}
\expandafter\def\csname v@timit/sttapi/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/opus/rtf\endcsname{0.038}
\expandafter\def\csname v@timit/sttapi/opus/sbias\endcsname{29}
\expandafter\def\csname v@timit/sttapi/opus/sbias-signed\endcsname{$+29$}
\expandafter\def\csname v@timit/sttapi/opus/w10\endcsname{17.4}
\expandafter\def\csname v@timit/sttapi/opus/w100\endcsname{95.3}
\expandafter\def\csname v@timit/sttapi/opus/w20\endcsname{35.2}
\expandafter\def\csname v@timit/sttapi/opus/w50\endcsname{75.7}
\expandafter\def\csname v@timit/sttapi/pcm/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/sttapi/pcm/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/sttapi/pcm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/sttapi/pcm/ebias\endcsname{18}
\expandafter\def\csname v@timit/sttapi/pcm/ebias-signed\endcsname{$-18$}
\expandafter\def\csname v@timit/sttapi/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/sttapi/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/sttapi/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/sttapi/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/sttapi/pcm/mae\endcsname{36.5}
\expandafter\def\csname v@timit/sttapi/pcm/median\endcsname{28.8}
\expandafter\def\csname v@timit/sttapi/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/sttapi/pcm/rtf\endcsname{0.038}
\expandafter\def\csname v@timit/sttapi/pcm/sbias\endcsname{29}
\expandafter\def\csname v@timit/sttapi/pcm/sbias-signed\endcsname{$+29$}
\expandafter\def\csname v@timit/sttapi/pcm/w10\endcsname{17.4}
\expandafter\def\csname v@timit/sttapi/pcm/w100\endcsname{95.7}
\expandafter\def\csname v@timit/sttapi/pcm/w20\endcsname{35.3}
\expandafter\def\csname v@timit/sttapi/pcm/w50\endcsname{75.9}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/dmae\endcsname{1.3}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/dw20\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/dw50\endcsname{1.1}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/ebias\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/mae\endcsname{42.5}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/median\endcsname{26.6}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/rtf\endcsname{0.009}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/sbias\endcsname{3}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/w10\endcsname{21.5}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/w100\endcsname{89.8}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/w20\endcsname{40.1}
\expandafter\def\csname v@timit/whisper-tm-cal/amrnb/w50\endcsname{75.3}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/ebias\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/mae\endcsname{41.2}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/median\endcsname{25.3}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/sbias\endcsname{5}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/sbias-signed\endcsname{$-5$}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/w10\endcsname{22.7}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/w100\endcsname{90.1}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/w20\endcsname{41.5}
\expandafter\def\csname v@timit/whisper-tm-cal/clean/w50\endcsname{76.3}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/dmae\endcsname{0.5}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/ebias\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/mae\endcsname{41.6}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/median\endcsname{25.5}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/sbias\endcsname{5}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/sbias-signed\endcsname{$-5$}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/w10\endcsname{22.1}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/w100\endcsname{90.0}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/w20\endcsname{40.9}
\expandafter\def\csname v@timit/whisper-tm-cal/g711u/w50\endcsname{76.0}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/dmae\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/dw20\endcsname{1.7}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/dw50\endcsname{1.3}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/ebias\endcsname{1}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/mae\endcsname{42.6}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/median\endcsname{26.8}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/rtf\endcsname{0.008}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/sbias\endcsname{3}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/w10\endcsname{21.4}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/w100\endcsname{89.7}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/w20\endcsname{39.8}
\expandafter\def\csname v@timit/whisper-tm-cal/g723/w50\endcsname{75.0}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/dmae\endcsname{0.8}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/dw50\endcsname{0.7}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/ebias\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/mae\endcsname{42.0}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/median\endcsname{25.9}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/sbias\endcsname{5}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/sbias-signed\endcsname{$-5$}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/w10\endcsname{21.7}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/w100\endcsname{89.9}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/w20\endcsname{40.6}
\expandafter\def\csname v@timit/whisper-tm-cal/g726/w50\endcsname{75.7}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/dmae\endcsname{1.1}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/dw20\endcsname{1.8}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/dw50\endcsname{0.9}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/ebias\endcsname{1}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/mae\endcsname{42.3}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/median\endcsname{26.6}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/sbias\endcsname{3}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/w10\endcsname{21.1}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/w100\endcsname{89.8}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/w20\endcsname{39.7}
\expandafter\def\csname v@timit/whisper-tm-cal/gsm/w50\endcsname{75.5}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/dmae\endcsname{1.0}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/dw20\endcsname{1.0}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/dw50\endcsname{1.1}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/ebias\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/mae\endcsname{42.2}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/median\endcsname{25.9}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/sbias\endcsname{5}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/sbias-signed\endcsname{$-5$}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/w10\endcsname{21.7}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/w100\endcsname{89.9}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/w20\endcsname{40.5}
\expandafter\def\csname v@timit/whisper-tm-cal/mp3/w50\endcsname{75.2}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/dmae\endcsname{0.9}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/dw20\endcsname{1.2}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/dw50\endcsname{0.8}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/ebias\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/mae\endcsname{42.1}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/median\endcsname{26.3}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/over500\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/sbias\endcsname{3}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/sbias-signed\endcsname{$-3$}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/w10\endcsname{21.7}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/w100\endcsname{89.9}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/w20\endcsname{40.3}
\expandafter\def\csname v@timit/whisper-tm-cal/opus/w50\endcsname{75.6}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/dw50\endcsname{0.4}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/ebias\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/ebias-signed\endcsname{$0$}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/mae\endcsname{41.7}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/median\endcsname{25.6}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/over500\endcsname{0.3}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/sbias\endcsname{5}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/sbias-signed\endcsname{$-5$}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/w10\endcsname{22.1}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/w100\endcsname{90.0}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/w20\endcsname{40.7}
\expandafter\def\csname v@timit/whisper-tm-cal/pcm/w50\endcsname{75.9}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/ebias\endcsname{750}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/ebias-signed\endcsname{$+750$}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/mae\endcsname{1204.3}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/median\endcsname{1027.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/over500\endcsname{76.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/sbias\endcsname{742}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/sbias-signed\endcsname{$+742$}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/w10\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/w100\endcsname{2.3}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/w20\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/clean/w50\endcsname{0.6}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/dmae\endcsname{8.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/ebias\endcsname{768}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/ebias-signed\endcsname{$+768$}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/mae\endcsname{1212.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/median\endcsname{1027.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/over500\endcsname{76.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/sbias\endcsname{760}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/sbias-signed\endcsname{$+760$}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/w10\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/w100\endcsname{2.6}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/w20\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/g711u/w50\endcsname{0.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/dmae\endcsname{-33.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/ebias\endcsname{623}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/ebias-signed\endcsname{$+623$}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/mae\endcsname{1170.6}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/median\endcsname{993.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/over500\endcsname{75.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/sbias\endcsname{606}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/sbias-signed\endcsname{$+606$}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/w10\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/w100\endcsname{2.6}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/w20\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/g726/w50\endcsname{0.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/dmae\endcsname{-34.3}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/ebias\endcsname{607}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/ebias-signed\endcsname{$+607$}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/mae\endcsname{1170.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/median\endcsname{992.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/over500\endcsname{75.3}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/sbias\endcsname{587}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/sbias-signed\endcsname{$+587$}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/w10\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/w100\endcsname{2.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/w20\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/gsm/w50\endcsname{0.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/dmae\endcsname{-5.4}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/ebias\endcsname{752}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/ebias-signed\endcsname{$+752$}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/mae\endcsname{1198.9}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/median\endcsname{1017.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/over500\endcsname{76.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/sbias\endcsname{742}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/sbias-signed\endcsname{$+742$}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/w10\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/w100\endcsname{2.6}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/w20\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/mp3/w50\endcsname{0.7}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/dmae\endcsname{13.8}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/dw50\endcsname{-0.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/ebias\endcsname{762}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/ebias-signed\endcsname{$+762$}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/mae\endcsname{1218.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/median\endcsname{1032.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/over500\endcsname{76.6}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/rtf\endcsname{0.022}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/sbias\endcsname{752}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/sbias-signed\endcsname{$+752$}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/w10\endcsname{0.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/w100\endcsname{2.4}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/w20\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/opus/w50\endcsname{0.6}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/dmae\endcsname{33.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/dw20\endcsname{-0.0}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/ebias\endcsname{822}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/ebias-signed\endcsname{$+822$}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/mae\endcsname{1237.4}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/median\endcsname{1057.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/over500\endcsname{77.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/rtf\endcsname{0.021}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/sbias\endcsname{813}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/sbias-signed\endcsname{$+813$}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/w10\endcsname{0.1}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/w100\endcsname{2.5}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/w20\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-cfg/pcm/w50\endcsname{0.7}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/ebias\endcsname{136}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/ebias-signed\endcsname{$-136$}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/mae\endcsname{156.3}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/median\endcsname{133.1}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/over500\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/rtf\endcsname{0.032}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/sbias\endcsname{132}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/sbias-signed\endcsname{$-132$}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/w10\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/w100\endcsname{32.3}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/w20\endcsname{2.9}
\expandafter\def\csname v@timit/whisper-tm-oai/clean/w50\endcsname{10.1}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/dmae\endcsname{-0.2}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/dw20\endcsname{-0.2}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/dw50\endcsname{-0.1}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/ebias\endcsname{136}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/ebias-signed\endcsname{$-136$}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/mae\endcsname{156.1}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/median\endcsname{132.7}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/over500\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/sbias\endcsname{132}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/sbias-signed\endcsname{$-132$}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/w10\endcsname{1.5}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/w100\endcsname{32.2}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/w20\endcsname{3.1}
\expandafter\def\csname v@timit/whisper-tm-oai/g711u/w50\endcsname{10.2}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/dmae\endcsname{-0.4}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/dw20\endcsname{-0.3}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/ebias\endcsname{136}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/ebias-signed\endcsname{$-136$}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/mae\endcsname{156.0}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/median\endcsname{132.7}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/over500\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/sbias\endcsname{132}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/sbias-signed\endcsname{$-132$}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/w10\endcsname{1.7}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/w100\endcsname{32.3}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/w20\endcsname{3.2}
\expandafter\def\csname v@timit/whisper-tm-oai/g726/w50\endcsname{9.9}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/dmae\endcsname{-1.7}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/dw20\endcsname{-0.4}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/dw50\endcsname{-0.6}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/ebias\endcsname{133}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/ebias-signed\endcsname{$-133$}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/mae\endcsname{154.6}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/median\endcsname{132.5}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/over500\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/rtf\endcsname{0.032}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/sbias\endcsname{132}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/sbias-signed\endcsname{$-132$}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/w10\endcsname{1.6}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/w100\endcsname{33.0}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/w20\endcsname{3.3}
\expandafter\def\csname v@timit/whisper-tm-oai/gsm/w50\endcsname{10.6}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/dmae\endcsname{-1.1}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/dw20\endcsname{-0.3}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/ebias\endcsname{135}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/ebias-signed\endcsname{$-135$}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/mae\endcsname{155.3}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/median\endcsname{132.5}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/over500\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/sbias\endcsname{132}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/sbias-signed\endcsname{$-132$}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/w10\endcsname{1.5}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/w100\endcsname{32.6}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/w20\endcsname{3.2}
\expandafter\def\csname v@timit/whisper-tm-oai/mp3/w50\endcsname{10.2}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/dmae\endcsname{-1.3}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/dw20\endcsname{-0.4}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/dw50\endcsname{-0.4}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/ebias\endcsname{135}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/ebias-signed\endcsname{$-135$}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/mae\endcsname{155.1}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/median\endcsname{132.5}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/over500\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/sbias\endcsname{132}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/sbias-signed\endcsname{$-132$}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/w10\endcsname{1.5}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/w100\endcsname{32.9}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/w20\endcsname{3.3}
\expandafter\def\csname v@timit/whisper-tm-oai/opus/w50\endcsname{10.5}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/dmae\endcsname{-0.2}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/dw20\endcsname{-0.2}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/dw50\endcsname{-0.2}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/ebias\endcsname{136}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/ebias-signed\endcsname{$-136$}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/mae\endcsname{156.2}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/median\endcsname{132.6}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/over500\endcsname{1.4}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/rtf\endcsname{0.031}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/sbias\endcsname{132}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/sbias-signed\endcsname{$-132$}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/w10\endcsname{1.5}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/w100\endcsname{32.2}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/w20\endcsname{3.1}
\expandafter\def\csname v@timit/whisper-tm-oai/pcm/w50\endcsname{10.3}
\expandafter\def\csname v@timit/whisperx/clean/ebias\endcsname{1}
\expandafter\def\csname v@timit/whisperx/clean/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/whisperx/clean/fail\endcsname{0}
\expandafter\def\csname v@timit/whisperx/clean/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisperx/clean/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisperx/clean/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisperx/clean/mae\endcsname{46.9}
\expandafter\def\csname v@timit/whisperx/clean/median\endcsname{37.9}
\expandafter\def\csname v@timit/whisperx/clean/over500\endcsname{0.0}
\expandafter\def\csname v@timit/whisperx/clean/rtf\endcsname{0.033}
\expandafter\def\csname v@timit/whisperx/clean/sbias\endcsname{60}
\expandafter\def\csname v@timit/whisperx/clean/sbias-signed\endcsname{$+60$}
\expandafter\def\csname v@timit/whisperx/clean/w10\endcsname{15.3}
\expandafter\def\csname v@timit/whisperx/clean/w100\endcsname{91.1}
\expandafter\def\csname v@timit/whisperx/clean/w20\endcsname{29.5}
\expandafter\def\csname v@timit/whisperx/clean/w50\endcsname{60.7}
\expandafter\def\csname v@timit/whisperx/g711u/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/whisperx/g711u/dw20\endcsname{0.1}
\expandafter\def\csname v@timit/whisperx/g711u/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/whisperx/g711u/ebias\endcsname{1}
\expandafter\def\csname v@timit/whisperx/g711u/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/whisperx/g711u/fail\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g711u/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g711u/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g711u/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g711u/mae\endcsname{47.3}
\expandafter\def\csname v@timit/whisperx/g711u/median\endcsname{38.3}
\expandafter\def\csname v@timit/whisperx/g711u/over500\endcsname{0.0}
\expandafter\def\csname v@timit/whisperx/g711u/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/whisperx/g711u/sbias\endcsname{60}
\expandafter\def\csname v@timit/whisperx/g711u/sbias-signed\endcsname{$+60$}
\expandafter\def\csname v@timit/whisperx/g711u/w10\endcsname{15.2}
\expandafter\def\csname v@timit/whisperx/g711u/w100\endcsname{91.0}
\expandafter\def\csname v@timit/whisperx/g711u/w20\endcsname{29.4}
\expandafter\def\csname v@timit/whisperx/g711u/w50\endcsname{60.4}
\expandafter\def\csname v@timit/whisperx/g726/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/whisperx/g726/dw20\endcsname{0.4}
\expandafter\def\csname v@timit/whisperx/g726/dw50\endcsname{0.1}
\expandafter\def\csname v@timit/whisperx/g726/ebias\endcsname{1}
\expandafter\def\csname v@timit/whisperx/g726/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/whisperx/g726/fail\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g726/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g726/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g726/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisperx/g726/mae\endcsname{47.3}
\expandafter\def\csname v@timit/whisperx/g726/median\endcsname{38.1}
\expandafter\def\csname v@timit/whisperx/g726/over500\endcsname{0.0}
\expandafter\def\csname v@timit/whisperx/g726/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/whisperx/g726/sbias\endcsname{59}
\expandafter\def\csname v@timit/whisperx/g726/sbias-signed\endcsname{$+59$}
\expandafter\def\csname v@timit/whisperx/g726/w10\endcsname{15.0}
\expandafter\def\csname v@timit/whisperx/g726/w100\endcsname{91.0}
\expandafter\def\csname v@timit/whisperx/g726/w20\endcsname{29.1}
\expandafter\def\csname v@timit/whisperx/g726/w50\endcsname{60.6}
\expandafter\def\csname v@timit/whisperx/gsm/dmae\endcsname{0.6}
\expandafter\def\csname v@timit/whisperx/gsm/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/whisperx/gsm/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/whisperx/gsm/ebias\endcsname{2}
\expandafter\def\csname v@timit/whisperx/gsm/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/whisperx/gsm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisperx/gsm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisperx/gsm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisperx/gsm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisperx/gsm/mae\endcsname{47.5}
\expandafter\def\csname v@timit/whisperx/gsm/median\endcsname{38.6}
\expandafter\def\csname v@timit/whisperx/gsm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/whisperx/gsm/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/whisperx/gsm/sbias\endcsname{60}
\expandafter\def\csname v@timit/whisperx/gsm/sbias-signed\endcsname{$+60$}
\expandafter\def\csname v@timit/whisperx/gsm/w10\endcsname{14.9}
\expandafter\def\csname v@timit/whisperx/gsm/w100\endcsname{91.0}
\expandafter\def\csname v@timit/whisperx/gsm/w20\endcsname{29.0}
\expandafter\def\csname v@timit/whisperx/gsm/w50\endcsname{60.2}
\expandafter\def\csname v@timit/whisperx/mp3/dmae\endcsname{0.4}
\expandafter\def\csname v@timit/whisperx/mp3/dw20\endcsname{0.6}
\expandafter\def\csname v@timit/whisperx/mp3/dw50\endcsname{0.3}
\expandafter\def\csname v@timit/whisperx/mp3/ebias\endcsname{2}
\expandafter\def\csname v@timit/whisperx/mp3/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/whisperx/mp3/fail\endcsname{0}
\expandafter\def\csname v@timit/whisperx/mp3/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisperx/mp3/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisperx/mp3/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisperx/mp3/mae\endcsname{47.3}
\expandafter\def\csname v@timit/whisperx/mp3/median\endcsname{38.3}
\expandafter\def\csname v@timit/whisperx/mp3/over500\endcsname{0.0}
\expandafter\def\csname v@timit/whisperx/mp3/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/whisperx/mp3/sbias\endcsname{60}
\expandafter\def\csname v@timit/whisperx/mp3/sbias-signed\endcsname{$+60$}
\expandafter\def\csname v@timit/whisperx/mp3/w10\endcsname{14.8}
\expandafter\def\csname v@timit/whisperx/mp3/w100\endcsname{91.1}
\expandafter\def\csname v@timit/whisperx/mp3/w20\endcsname{29.0}
\expandafter\def\csname v@timit/whisperx/mp3/w50\endcsname{60.4}
\expandafter\def\csname v@timit/whisperx/opus/dmae\endcsname{0.7}
\expandafter\def\csname v@timit/whisperx/opus/dw20\endcsname{0.8}
\expandafter\def\csname v@timit/whisperx/opus/dw50\endcsname{0.5}
\expandafter\def\csname v@timit/whisperx/opus/ebias\endcsname{2}
\expandafter\def\csname v@timit/whisperx/opus/ebias-signed\endcsname{$+2$}
\expandafter\def\csname v@timit/whisperx/opus/fail\endcsname{0}
\expandafter\def\csname v@timit/whisperx/opus/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisperx/opus/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisperx/opus/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisperx/opus/mae\endcsname{47.6}
\expandafter\def\csname v@timit/whisperx/opus/median\endcsname{38.5}
\expandafter\def\csname v@timit/whisperx/opus/over500\endcsname{0.0}
\expandafter\def\csname v@timit/whisperx/opus/rtf\endcsname{0.013}
\expandafter\def\csname v@timit/whisperx/opus/sbias\endcsname{60}
\expandafter\def\csname v@timit/whisperx/opus/sbias-signed\endcsname{$+60$}
\expandafter\def\csname v@timit/whisperx/opus/w10\endcsname{14.7}
\expandafter\def\csname v@timit/whisperx/opus/w100\endcsname{91.0}
\expandafter\def\csname v@timit/whisperx/opus/w20\endcsname{28.7}
\expandafter\def\csname v@timit/whisperx/opus/w50\endcsname{60.1}
\expandafter\def\csname v@timit/whisperx/pcm/dmae\endcsname{0.3}
\expandafter\def\csname v@timit/whisperx/pcm/dw20\endcsname{0.3}
\expandafter\def\csname v@timit/whisperx/pcm/dw50\endcsname{0.2}
\expandafter\def\csname v@timit/whisperx/pcm/ebias\endcsname{1}
\expandafter\def\csname v@timit/whisperx/pcm/ebias-signed\endcsname{$+1$}
\expandafter\def\csname v@timit/whisperx/pcm/fail\endcsname{0}
\expandafter\def\csname v@timit/whisperx/pcm/fail-assert\endcsname{0}
\expandafter\def\csname v@timit/whisperx/pcm/fail-crash\endcsname{0}
\expandafter\def\csname v@timit/whisperx/pcm/fail-other\endcsname{0}
\expandafter\def\csname v@timit/whisperx/pcm/mae\endcsname{47.3}
\expandafter\def\csname v@timit/whisperx/pcm/median\endcsname{38.1}
\expandafter\def\csname v@timit/whisperx/pcm/over500\endcsname{0.0}
\expandafter\def\csname v@timit/whisperx/pcm/rtf\endcsname{0.014}
\expandafter\def\csname v@timit/whisperx/pcm/sbias\endcsname{59}
\expandafter\def\csname v@timit/whisperx/pcm/sbias-signed\endcsname{$+59$}
\expandafter\def\csname v@timit/whisperx/pcm/w10\endcsname{15.1}
\expandafter\def\csname v@timit/whisperx/pcm/w100\endcsname{91.0}
\expandafter\def\csname v@timit/whisperx/pcm/w20\endcsname{29.2}
\expandafter\def\csname v@timit/whisperx/pcm/w50\endcsname{60.5}
\expandafter\def\csname v@tn/seoul/del10/ctcm/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/seoul/del10/ctcm/clean-median\endcsname{8.2}
\expandafter\def\csname v@tn/seoul/del10/ctcm/clean-o500\endcsname{0.16}
\expandafter\def\csname v@tn/seoul/del10/ctcm/clean-w20\endcsname{80.9}
\expandafter\def\csname v@tn/seoul/del10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/ctcm/mae\endcsname{44.0}
\expandafter\def\csname v@tn/seoul/del10/ctcm/median\endcsname{8.8}
\expandafter\def\csname v@tn/seoul/del10/ctcm/o500\endcsname{2.25}
\expandafter\def\csname v@tn/seoul/del10/ctcm/w20\endcsname{77.0}
\expandafter\def\csname v@tn/seoul/del10/ctcw/clean-mae\endcsname{13.7}
\expandafter\def\csname v@tn/seoul/del10/ctcw/clean-median\endcsname{7.2}
\expandafter\def\csname v@tn/seoul/del10/ctcw/clean-o500\endcsname{0.07}
\expandafter\def\csname v@tn/seoul/del10/ctcw/clean-w20\endcsname{85.9}
\expandafter\def\csname v@tn/seoul/del10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/ctcw/mae\endcsname{41.8}
\expandafter\def\csname v@tn/seoul/del10/ctcw/median\endcsname{7.7}
\expandafter\def\csname v@tn/seoul/del10/ctcw/o500\endcsname{2.14}
\expandafter\def\csname v@tn/seoul/del10/ctcw/w20\endcsname{81.9}
\expandafter\def\csname v@tn/seoul/del10/mfa/clean-mae\endcsname{21.9}
\expandafter\def\csname v@tn/seoul/del10/mfa/clean-median\endcsname{10.9}
\expandafter\def\csname v@tn/seoul/del10/mfa/clean-o500\endcsname{0.24}
\expandafter\def\csname v@tn/seoul/del10/mfa/clean-w20\endcsname{70.0}
\expandafter\def\csname v@tn/seoul/del10/mfa/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/mfa/mae\endcsname{65.1}
\expandafter\def\csname v@tn/seoul/del10/mfa/median\endcsname{12.2}
\expandafter\def\csname v@tn/seoul/del10/mfa/o500\endcsname{3.23}
\expandafter\def\csname v@tn/seoul/del10/mfa/w20\endcsname{65.5}
\expandafter\def\csname v@tn/seoul/del10/post/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/del10/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/del10/post/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/del10/post/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/del10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/post/mae\endcsname{29.6}
\expandafter\def\csname v@tn/seoul/del10/post/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/del10/post/o500\endcsname{1.43}
\expandafter\def\csname v@tn/seoul/del10/post/w20\endcsname{86.6}
\expandafter\def\csname v@tn/seoul/del10/posttn/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/seoul/del10/posttn/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/del10/posttn/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/del10/posttn/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/del10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/posttn/mae\endcsname{12.1}
\expandafter\def\csname v@tn/seoul/del10/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/del10/posttn/o500\endcsname{0.13}
\expandafter\def\csname v@tn/seoul/del10/posttn/w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/del10/rel/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/seoul/del10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/del10/rel/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/del10/rel/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/del10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/rel/mae\endcsname{12.3}
\expandafter\def\csname v@tn/seoul/del10/rel/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/del10/rel/o500\endcsname{0.12}
\expandafter\def\csname v@tn/seoul/del10/rel/w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/del10/s6fin/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/del10/s6fin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/del10/s6fin/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/del10/s6fin/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/del10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/s6fin/mae\endcsname{12.5}
\expandafter\def\csname v@tn/seoul/del10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/del10/s6fin/o500\endcsname{0.14}
\expandafter\def\csname v@tn/seoul/del10/s6fin/w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/del10/tn10/clean-mae\endcsname{11.9}
\expandafter\def\csname v@tn/seoul/del10/tn10/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/del10/tn10/clean-o500\endcsname{0.10}
\expandafter\def\csname v@tn/seoul/del10/tn10/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/del10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/tn10/mae\endcsname{38.3}
\expandafter\def\csname v@tn/seoul/del10/tn10/median\endcsname{5.7}
\expandafter\def\csname v@tn/seoul/del10/tn10/o500\endcsname{1.92}
\expandafter\def\csname v@tn/seoul/del10/tn10/w20\endcsname{85.4}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/clean-mae\endcsname{11.7}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/clean-w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/mae\endcsname{38.3}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/median\endcsname{5.7}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/o500\endcsname{1.93}
\expandafter\def\csname v@tn/seoul/del10/tn10s1/w20\endcsname{85.3}
\expandafter\def\csname v@tn/seoul/del10/tn20/clean-mae\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/del10/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/del10/tn20/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/del10/tn20/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/del10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/tn20/mae\endcsname{37.4}
\expandafter\def\csname v@tn/seoul/del10/tn20/median\endcsname{5.8}
\expandafter\def\csname v@tn/seoul/del10/tn20/o500\endcsname{1.88}
\expandafter\def\csname v@tn/seoul/del10/tn20/w20\endcsname{85.4}
\expandafter\def\csname v@tn/seoul/del10/ts/clean-mae\endcsname{11.5}
\expandafter\def\csname v@tn/seoul/del10/ts/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/del10/ts/clean-o500\endcsname{0.09}
\expandafter\def\csname v@tn/seoul/del10/ts/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/del10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/ts/mae\endcsname{44.3}
\expandafter\def\csname v@tn/seoul/del10/ts/median\endcsname{5.7}
\expandafter\def\csname v@tn/seoul/del10/ts/o500\endcsname{2.31}
\expandafter\def\csname v@tn/seoul/del10/ts/w20\endcsname{85.0}
\expandafter\def\csname v@tn/seoul/del10/turbofin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/del10/turbofin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/del10/turbofin/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/del10/turbofin/clean-w20\endcsname{89.4}
\expandafter\def\csname v@tn/seoul/del10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/del10/turbofin/mae\endcsname{13.2}
\expandafter\def\csname v@tn/seoul/del10/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/del10/turbofin/o500\endcsname{0.19}
\expandafter\def\csname v@tn/seoul/del10/turbofin/w20\endcsname{89.1}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/clean-median\endcsname{8.2}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/clean-o500\endcsname{0.15}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/clean-w20\endcsname{81.0}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/mae\endcsname{29.9}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/median\endcsname{9.3}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/o500\endcsname{0.54}
\expandafter\def\csname v@tn/seoul/ins10/ctcm/w20\endcsname{74.3}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/clean-mae\endcsname{13.7}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/clean-median\endcsname{7.3}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/clean-o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/clean-w20\endcsname{85.8}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/mae\endcsname{26.9}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/median\endcsname{8.2}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/o500\endcsname{0.49}
\expandafter\def\csname v@tn/seoul/ins10/ctcw/w20\endcsname{78.7}
\expandafter\def\csname v@tn/seoul/ins10/mfa/clean-mae\endcsname{21.7}
\expandafter\def\csname v@tn/seoul/ins10/mfa/clean-median\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/ins10/mfa/clean-o500\endcsname{0.23}
\expandafter\def\csname v@tn/seoul/ins10/mfa/clean-w20\endcsname{70.0}
\expandafter\def\csname v@tn/seoul/ins10/mfa/failed\endcsname{140}
\expandafter\def\csname v@tn/seoul/ins10/mfa/mae\endcsname{47.9}
\expandafter\def\csname v@tn/seoul/ins10/mfa/median\endcsname{12.8}
\expandafter\def\csname v@tn/seoul/ins10/mfa/o500\endcsname{1.54}
\expandafter\def\csname v@tn/seoul/ins10/mfa/w20\endcsname{63.4}
\expandafter\def\csname v@tn/seoul/ins10/post/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/seoul/ins10/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/post/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/ins10/post/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/ins10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/post/mae\endcsname{13.9}
\expandafter\def\csname v@tn/seoul/ins10/post/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/ins10/post/o500\endcsname{0.16}
\expandafter\def\csname v@tn/seoul/ins10/post/w20\endcsname{88.4}
\expandafter\def\csname v@tn/seoul/ins10/posttn/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/seoul/ins10/posttn/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/posttn/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/ins10/posttn/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/ins10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/posttn/mae\endcsname{10.9}
\expandafter\def\csname v@tn/seoul/ins10/posttn/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/posttn/o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/ins10/posttn/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/ins10/rel/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/ins10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/rel/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/ins10/rel/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/ins10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/rel/mae\endcsname{11.4}
\expandafter\def\csname v@tn/seoul/ins10/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/rel/o500\endcsname{0.07}
\expandafter\def\csname v@tn/seoul/ins10/rel/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/mae\endcsname{11.1}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/ins10/s6fin/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/ins10/tn10/clean-mae\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/ins10/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/tn10/clean-o500\endcsname{0.10}
\expandafter\def\csname v@tn/seoul/ins10/tn10/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/ins10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/tn10/mae\endcsname{22.3}
\expandafter\def\csname v@tn/seoul/ins10/tn10/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/ins10/tn10/o500\endcsname{0.83}
\expandafter\def\csname v@tn/seoul/ins10/tn10/w20\endcsname{87.9}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/clean-mae\endcsname{11.6}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/mae\endcsname{22.2}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/o500\endcsname{0.87}
\expandafter\def\csname v@tn/seoul/ins10/tn10s1/w20\endcsname{87.7}
\expandafter\def\csname v@tn/seoul/ins10/tn20/clean-mae\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/ins10/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/ins10/tn20/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/ins10/tn20/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/ins10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/tn20/mae\endcsname{23.8}
\expandafter\def\csname v@tn/seoul/ins10/tn20/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/ins10/tn20/o500\endcsname{0.97}
\expandafter\def\csname v@tn/seoul/ins10/tn20/w20\endcsname{87.5}
\expandafter\def\csname v@tn/seoul/ins10/ts/clean-mae\endcsname{11.5}
\expandafter\def\csname v@tn/seoul/ins10/ts/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/ts/clean-o500\endcsname{0.09}
\expandafter\def\csname v@tn/seoul/ins10/ts/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/ins10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/ts/mae\endcsname{33.6}
\expandafter\def\csname v@tn/seoul/ins10/ts/median\endcsname{5.7}
\expandafter\def\csname v@tn/seoul/ins10/ts/o500\endcsname{1.63}
\expandafter\def\csname v@tn/seoul/ins10/ts/w20\endcsname{85.7}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/clean-w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/mae\endcsname{11.7}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/o500\endcsname{0.10}
\expandafter\def\csname v@tn/seoul/ins10/turbofin/w20\endcsname{89.3}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/clean-median\endcsname{8.3}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/clean-o500\endcsname{0.15}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/clean-w20\endcsname{81.0}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/mae\endcsname{32.5}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/median\endcsname{8.9}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/o500\endcsname{1.08}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/sub-mae\endcsname{96.1}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/sub-median\endcsname{12.1}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/sub-o500\endcsname{5.21}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/sub-w20\endcsname{61.6}
\expandafter\def\csname v@tn/seoul/mix10/ctcm/w20\endcsname{76.7}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/clean-mae\endcsname{13.7}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/clean-median\endcsname{7.3}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/clean-o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/clean-w20\endcsname{85.8}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/mae\endcsname{28.6}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/median\endcsname{7.8}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/o500\endcsname{0.96}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/sub-mae\endcsname{90.8}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/sub-median\endcsname{11.0}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/sub-o500\endcsname{5.12}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/sub-w20\endcsname{64.1}
\expandafter\def\csname v@tn/seoul/mix10/ctcw/w20\endcsname{81.3}
\expandafter\def\csname v@tn/seoul/mix10/mfa/clean-mae\endcsname{21.7}
\expandafter\def\csname v@tn/seoul/mix10/mfa/clean-median\endcsname{10.9}
\expandafter\def\csname v@tn/seoul/mix10/mfa/clean-o500\endcsname{0.24}
\expandafter\def\csname v@tn/seoul/mix10/mfa/clean-w20\endcsname{69.9}
\expandafter\def\csname v@tn/seoul/mix10/mfa/failed\endcsname{31}
\expandafter\def\csname v@tn/seoul/mix10/mfa/mae\endcsname{38.9}
\expandafter\def\csname v@tn/seoul/mix10/mfa/median\endcsname{12.2}
\expandafter\def\csname v@tn/seoul/mix10/mfa/o500\endcsname{1.28}
\expandafter\def\csname v@tn/seoul/mix10/mfa/sub-mae\endcsname{145.6}
\expandafter\def\csname v@tn/seoul/mix10/mfa/sub-median\endcsname{38.0}
\expandafter\def\csname v@tn/seoul/mix10/mfa/sub-o500\endcsname{6.98}
\expandafter\def\csname v@tn/seoul/mix10/mfa/sub-w20\endcsname{34.1}
\expandafter\def\csname v@tn/seoul/mix10/mfa/w20\endcsname{65.7}
\expandafter\def\csname v@tn/seoul/mix10/post/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/mix10/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/post/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/mix10/post/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/mix10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/post/mae\endcsname{19.2}
\expandafter\def\csname v@tn/seoul/mix10/post/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/mix10/post/o500\endcsname{0.61}
\expandafter\def\csname v@tn/seoul/mix10/post/sub-mae\endcsname{210.6}
\expandafter\def\csname v@tn/seoul/mix10/post/sub-median\endcsname{18.9}
\expandafter\def\csname v@tn/seoul/mix10/post/sub-o500\endcsname{14.80}
\expandafter\def\csname v@tn/seoul/mix10/post/sub-w20\endcsname{51.1}
\expandafter\def\csname v@tn/seoul/mix10/post/w20\endcsname{87.6}
\expandafter\def\csname v@tn/seoul/mix10/posttn/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/mix10/posttn/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/posttn/clean-o500\endcsname{0.04}
\expandafter\def\csname v@tn/seoul/mix10/posttn/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/mix10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/posttn/mae\endcsname{12.2}
\expandafter\def\csname v@tn/seoul/mix10/posttn/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/posttn/o500\endcsname{0.14}
\expandafter\def\csname v@tn/seoul/mix10/posttn/sub-mae\endcsname{149.1}
\expandafter\def\csname v@tn/seoul/mix10/posttn/sub-median\endcsname{10.1}
\expandafter\def\csname v@tn/seoul/mix10/posttn/sub-o500\endcsname{10.52}
\expandafter\def\csname v@tn/seoul/mix10/posttn/sub-w20\endcsname{60.7}
\expandafter\def\csname v@tn/seoul/mix10/posttn/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix10/rel/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/seoul/mix10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/rel/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix10/rel/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/mix10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/rel/mae\endcsname{12.0}
\expandafter\def\csname v@tn/seoul/mix10/rel/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix10/rel/o500\endcsname{0.12}
\expandafter\def\csname v@tn/seoul/mix10/rel/sub-mae\endcsname{145.3}
\expandafter\def\csname v@tn/seoul/mix10/rel/sub-median\endcsname{10.3}
\expandafter\def\csname v@tn/seoul/mix10/rel/sub-o500\endcsname{9.96}
\expandafter\def\csname v@tn/seoul/mix10/rel/sub-w20\endcsname{60.4}
\expandafter\def\csname v@tn/seoul/mix10/rel/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/mae\endcsname{12.1}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/sub-mae\endcsname{140.4}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/sub-median\endcsname{10.0}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/sub-o500\endcsname{9.59}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/sub-w20\endcsname{61.3}
\expandafter\def\csname v@tn/seoul/mix10/s6fin/w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/mix10/tn10/clean-mae\endcsname{11.9}
\expandafter\def\csname v@tn/seoul/mix10/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/tn10/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/mix10/tn10/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/mix10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/tn10/mae\endcsname{29.1}
\expandafter\def\csname v@tn/seoul/mix10/tn10/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/mix10/tn10/o500\endcsname{1.30}
\expandafter\def\csname v@tn/seoul/mix10/tn10/sub-mae\endcsname{148.5}
\expandafter\def\csname v@tn/seoul/mix10/tn10/sub-median\endcsname{10.0}
\expandafter\def\csname v@tn/seoul/mix10/tn10/sub-o500\endcsname{10.43}
\expandafter\def\csname v@tn/seoul/mix10/tn10/sub-w20\endcsname{60.5}
\expandafter\def\csname v@tn/seoul/mix10/tn10/w20\endcsname{86.8}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/clean-mae\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/clean-o500\endcsname{0.12}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/clean-w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/mae\endcsname{28.0}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/o500\endcsname{1.26}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/sub-mae\endcsname{141.0}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/sub-median\endcsname{9.0}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/sub-o500\endcsname{10.06}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/sub-w20\endcsname{62.4}
\expandafter\def\csname v@tn/seoul/mix10/tn10s1/w20\endcsname{86.7}
\expandafter\def\csname v@tn/seoul/mix10/tn20/clean-mae\endcsname{11.9}
\expandafter\def\csname v@tn/seoul/mix10/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix10/tn20/clean-o500\endcsname{0.12}
\expandafter\def\csname v@tn/seoul/mix10/tn20/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/mix10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/tn20/mae\endcsname{29.7}
\expandafter\def\csname v@tn/seoul/mix10/tn20/median\endcsname{5.7}
\expandafter\def\csname v@tn/seoul/mix10/tn20/o500\endcsname{1.36}
\expandafter\def\csname v@tn/seoul/mix10/tn20/sub-mae\endcsname{137.8}
\expandafter\def\csname v@tn/seoul/mix10/tn20/sub-median\endcsname{9.6}
\expandafter\def\csname v@tn/seoul/mix10/tn20/sub-o500\endcsname{8.94}
\expandafter\def\csname v@tn/seoul/mix10/tn20/sub-w20\endcsname{62.4}
\expandafter\def\csname v@tn/seoul/mix10/tn20/w20\endcsname{86.7}
\expandafter\def\csname v@tn/seoul/mix10/ts/clean-mae\endcsname{11.6}
\expandafter\def\csname v@tn/seoul/mix10/ts/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/ts/clean-o500\endcsname{0.10}
\expandafter\def\csname v@tn/seoul/mix10/ts/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/ts/mae\endcsname{37.4}
\expandafter\def\csname v@tn/seoul/mix10/ts/median\endcsname{5.7}
\expandafter\def\csname v@tn/seoul/mix10/ts/o500\endcsname{1.92}
\expandafter\def\csname v@tn/seoul/mix10/ts/sub-mae\endcsname{158.0}
\expandafter\def\csname v@tn/seoul/mix10/ts/sub-median\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/mix10/ts/sub-o500\endcsname{10.06}
\expandafter\def\csname v@tn/seoul/mix10/ts/sub-w20\endcsname{57.4}
\expandafter\def\csname v@tn/seoul/mix10/ts/w20\endcsname{85.5}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/clean-w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/mae\endcsname{12.5}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/o500\endcsname{0.14}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/sub-mae\endcsname{147.8}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/sub-median\endcsname{9.6}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/sub-o500\endcsname{9.78}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/sub-w20\endcsname{61.6}
\expandafter\def\csname v@tn/seoul/mix10/turbofin/w20\endcsname{89.3}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/clean-median\endcsname{8.2}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/clean-o500\endcsname{0.15}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/clean-w20\endcsname{81.0}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/mae\endcsname{50.5}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/median\endcsname{9.6}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/o500\endcsname{2.29}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/sub-mae\endcsname{110.6}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/sub-median\endcsname{15.2}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/sub-o500\endcsname{6.22}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/sub-w20\endcsname{56.4}
\expandafter\def\csname v@tn/seoul/mix20/ctcm/w20\endcsname{72.7}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/clean-mae\endcsname{13.7}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/clean-median\endcsname{7.2}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/clean-o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/clean-w20\endcsname{85.9}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/mae\endcsname{45.2}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/median\endcsname{8.4}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/o500\endcsname{2.09}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/sub-mae\endcsname{110.8}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/sub-median\endcsname{12.4}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/sub-o500\endcsname{6.31}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/sub-w20\endcsname{60.9}
\expandafter\def\csname v@tn/seoul/mix20/ctcw/w20\endcsname{77.2}
\expandafter\def\csname v@tn/seoul/mix20/mfa/clean-mae\endcsname{21.7}
\expandafter\def\csname v@tn/seoul/mix20/mfa/clean-median\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/mix20/mfa/clean-o500\endcsname{0.25}
\expandafter\def\csname v@tn/seoul/mix20/mfa/clean-w20\endcsname{70.2}
\expandafter\def\csname v@tn/seoul/mix20/mfa/failed\endcsname{92}
\expandafter\def\csname v@tn/seoul/mix20/mfa/mae\endcsname{66.9}
\expandafter\def\csname v@tn/seoul/mix20/mfa/median\endcsname{13.5}
\expandafter\def\csname v@tn/seoul/mix20/mfa/o500\endcsname{2.76}
\expandafter\def\csname v@tn/seoul/mix20/mfa/sub-mae\endcsname{170.4}
\expandafter\def\csname v@tn/seoul/mix20/mfa/sub-median\endcsname{59.7}
\expandafter\def\csname v@tn/seoul/mix20/mfa/sub-o500\endcsname{8.77}
\expandafter\def\csname v@tn/seoul/mix20/mfa/sub-w20\endcsname{30.2}
\expandafter\def\csname v@tn/seoul/mix20/mfa/w20\endcsname{61.6}
\expandafter\def\csname v@tn/seoul/mix20/post/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/mix20/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/post/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix20/post/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix20/post/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/post/mae\endcsname{30.5}
\expandafter\def\csname v@tn/seoul/mix20/post/median\endcsname{5.8}
\expandafter\def\csname v@tn/seoul/mix20/post/o500\endcsname{1.38}
\expandafter\def\csname v@tn/seoul/mix20/post/sub-mae\endcsname{230.6}
\expandafter\def\csname v@tn/seoul/mix20/post/sub-median\endcsname{23.1}
\expandafter\def\csname v@tn/seoul/mix20/post/sub-o500\endcsname{16.05}
\expandafter\def\csname v@tn/seoul/mix20/post/sub-w20\endcsname{48.6}
\expandafter\def\csname v@tn/seoul/mix20/post/w20\endcsname{85.7}
\expandafter\def\csname v@tn/seoul/mix20/posttn/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/mix20/posttn/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/posttn/clean-o500\endcsname{0.04}
\expandafter\def\csname v@tn/seoul/mix20/posttn/clean-w20\endcsname{90.1}
\expandafter\def\csname v@tn/seoul/mix20/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/posttn/mae\endcsname{13.1}
\expandafter\def\csname v@tn/seoul/mix20/posttn/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/posttn/o500\endcsname{0.23}
\expandafter\def\csname v@tn/seoul/mix20/posttn/sub-mae\endcsname{168.9}
\expandafter\def\csname v@tn/seoul/mix20/posttn/sub-median\endcsname{12.2}
\expandafter\def\csname v@tn/seoul/mix20/posttn/sub-o500\endcsname{12.01}
\expandafter\def\csname v@tn/seoul/mix20/posttn/sub-w20\endcsname{57.5}
\expandafter\def\csname v@tn/seoul/mix20/posttn/w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/mix20/rel/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/mix20/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/rel/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix20/rel/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/mix20/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/rel/mae\endcsname{12.5}
\expandafter\def\csname v@tn/seoul/mix20/rel/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix20/rel/o500\endcsname{0.15}
\expandafter\def\csname v@tn/seoul/mix20/rel/sub-mae\endcsname{173.4}
\expandafter\def\csname v@tn/seoul/mix20/rel/sub-median\endcsname{12.1}
\expandafter\def\csname v@tn/seoul/mix20/rel/sub-o500\endcsname{12.15}
\expandafter\def\csname v@tn/seoul/mix20/rel/sub-w20\endcsname{57.9}
\expandafter\def\csname v@tn/seoul/mix20/rel/w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/mae\endcsname{12.7}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/o500\endcsname{0.18}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/sub-mae\endcsname{168.6}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/sub-median\endcsname{11.5}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/sub-o500\endcsname{11.87}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/sub-w20\endcsname{59.4}
\expandafter\def\csname v@tn/seoul/mix20/s6fin/w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/mix20/tn10/clean-mae\endcsname{12.0}
\expandafter\def\csname v@tn/seoul/mix20/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/tn10/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/mix20/tn10/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix20/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/tn10/mae\endcsname{45.6}
\expandafter\def\csname v@tn/seoul/mix20/tn10/median\endcsname{5.9}
\expandafter\def\csname v@tn/seoul/mix20/tn10/o500\endcsname{2.46}
\expandafter\def\csname v@tn/seoul/mix20/tn10/sub-mae\endcsname{166.2}
\expandafter\def\csname v@tn/seoul/mix20/tn10/sub-median\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/mix20/tn10/sub-o500\endcsname{11.87}
\expandafter\def\csname v@tn/seoul/mix20/tn10/sub-w20\endcsname{59.3}
\expandafter\def\csname v@tn/seoul/mix20/tn10/w20\endcsname{83.9}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/clean-mae\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/clean-o500\endcsname{0.12}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/mae\endcsname{46.0}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/median\endcsname{5.9}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/o500\endcsname{2.46}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/sub-mae\endcsname{161.0}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/sub-median\endcsname{11.2}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/sub-o500\endcsname{10.85}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/sub-w20\endcsname{59.7}
\expandafter\def\csname v@tn/seoul/mix20/tn10s1/w20\endcsname{83.8}
\expandafter\def\csname v@tn/seoul/mix20/tn20/clean-mae\endcsname{12.0}
\expandafter\def\csname v@tn/seoul/mix20/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix20/tn20/clean-o500\endcsname{0.13}
\expandafter\def\csname v@tn/seoul/mix20/tn20/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/mix20/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/tn20/mae\endcsname{46.1}
\expandafter\def\csname v@tn/seoul/mix20/tn20/median\endcsname{6.0}
\expandafter\def\csname v@tn/seoul/mix20/tn20/o500\endcsname{2.53}
\expandafter\def\csname v@tn/seoul/mix20/tn20/sub-mae\endcsname{166.9}
\expandafter\def\csname v@tn/seoul/mix20/tn20/sub-median\endcsname{12.2}
\expandafter\def\csname v@tn/seoul/mix20/tn20/sub-o500\endcsname{11.55}
\expandafter\def\csname v@tn/seoul/mix20/tn20/sub-w20\endcsname{58.7}
\expandafter\def\csname v@tn/seoul/mix20/tn20/w20\endcsname{83.6}
\expandafter\def\csname v@tn/seoul/mix20/ts/clean-mae\endcsname{11.7}
\expandafter\def\csname v@tn/seoul/mix20/ts/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/ts/clean-o500\endcsname{0.10}
\expandafter\def\csname v@tn/seoul/mix20/ts/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix20/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/ts/mae\endcsname{67.6}
\expandafter\def\csname v@tn/seoul/mix20/ts/median\endcsname{6.2}
\expandafter\def\csname v@tn/seoul/mix20/ts/o500\endcsname{4.02}
\expandafter\def\csname v@tn/seoul/mix20/ts/sub-mae\endcsname{195.0}
\expandafter\def\csname v@tn/seoul/mix20/ts/sub-median\endcsname{16.3}
\expandafter\def\csname v@tn/seoul/mix20/ts/sub-o500\endcsname{13.45}
\expandafter\def\csname v@tn/seoul/mix20/ts/sub-w20\endcsname{52.9}
\expandafter\def\csname v@tn/seoul/mix20/ts/w20\endcsname{80.8}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/clean-o500\endcsname{0.04}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/clean-w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/mae\endcsname{13.9}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/o500\endcsname{0.26}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/sub-mae\endcsname{169.9}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/sub-median\endcsname{11.6}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/sub-o500\endcsname{12.29}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/sub-w20\endcsname{59.4}
\expandafter\def\csname v@tn/seoul/mix20/turbofin/w20\endcsname{89.1}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/clean-median\endcsname{8.2}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/clean-o500\endcsname{0.16}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/clean-w20\endcsname{81.0}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/mae\endcsname{24.6}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/median\endcsname{8.6}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/o500\endcsname{0.67}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/sub-mae\endcsname{67.9}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/sub-median\endcsname{10.5}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/sub-o500\endcsname{3.76}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/sub-w20\endcsname{67.0}
\expandafter\def\csname v@tn/seoul/mix5/ctcm/w20\endcsname{78.6}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/clean-mae\endcsname{13.7}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/clean-median\endcsname{7.3}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/clean-o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/clean-w20\endcsname{85.9}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/mae\endcsname{21.3}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/median\endcsname{7.5}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/o500\endcsname{0.52}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/sub-mae\endcsname{76.5}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/sub-median\endcsname{9.8}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/sub-o500\endcsname{4.12}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/sub-w20\endcsname{65.6}
\expandafter\def\csname v@tn/seoul/mix5/ctcw/w20\endcsname{83.5}
\expandafter\def\csname v@tn/seoul/mix5/mfa/clean-mae\endcsname{21.7}
\expandafter\def\csname v@tn/seoul/mix5/mfa/clean-median\endcsname{10.9}
\expandafter\def\csname v@tn/seoul/mix5/mfa/clean-o500\endcsname{0.22}
\expandafter\def\csname v@tn/seoul/mix5/mfa/clean-w20\endcsname{70.0}
\expandafter\def\csname v@tn/seoul/mix5/mfa/failed\endcsname{20}
\expandafter\def\csname v@tn/seoul/mix5/mfa/mae\endcsname{34.8}
\expandafter\def\csname v@tn/seoul/mix5/mfa/median\endcsname{11.6}
\expandafter\def\csname v@tn/seoul/mix5/mfa/o500\endcsname{0.94}
\expandafter\def\csname v@tn/seoul/mix5/mfa/sub-mae\endcsname{123.4}
\expandafter\def\csname v@tn/seoul/mix5/mfa/sub-median\endcsname{41.5}
\expandafter\def\csname v@tn/seoul/mix5/mfa/sub-o500\endcsname{4.30}
\expandafter\def\csname v@tn/seoul/mix5/mfa/sub-w20\endcsname{34.4}
\expandafter\def\csname v@tn/seoul/mix5/mfa/w20\endcsname{67.6}
\expandafter\def\csname v@tn/seoul/mix5/post/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/seoul/mix5/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/post/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/mix5/post/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix5/post/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/post/mae\endcsname{15.0}
\expandafter\def\csname v@tn/seoul/mix5/post/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix5/post/o500\endcsname{0.37}
\expandafter\def\csname v@tn/seoul/mix5/post/sub-mae\endcsname{171.6}
\expandafter\def\csname v@tn/seoul/mix5/post/sub-median\endcsname{14.8}
\expandafter\def\csname v@tn/seoul/mix5/post/sub-o500\endcsname{10.75}
\expandafter\def\csname v@tn/seoul/mix5/post/sub-w20\endcsname{54.3}
\expandafter\def\csname v@tn/seoul/mix5/post/w20\endcsname{88.6}
\expandafter\def\csname v@tn/seoul/mix5/posttn/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/seoul/mix5/posttn/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/posttn/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix5/posttn/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/mix5/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/posttn/mae\endcsname{11.2}
\expandafter\def\csname v@tn/seoul/mix5/posttn/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/posttn/o500\endcsname{0.08}
\expandafter\def\csname v@tn/seoul/mix5/posttn/sub-mae\endcsname{127.5}
\expandafter\def\csname v@tn/seoul/mix5/posttn/sub-median\endcsname{10.0}
\expandafter\def\csname v@tn/seoul/mix5/posttn/sub-o500\endcsname{7.35}
\expandafter\def\csname v@tn/seoul/mix5/posttn/sub-w20\endcsname{60.9}
\expandafter\def\csname v@tn/seoul/mix5/posttn/w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/mix5/rel/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/seoul/mix5/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/rel/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix5/rel/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/mix5/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/rel/mae\endcsname{11.1}
\expandafter\def\csname v@tn/seoul/mix5/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/rel/o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/mix5/rel/sub-mae\endcsname{128.7}
\expandafter\def\csname v@tn/seoul/mix5/rel/sub-median\endcsname{10.3}
\expandafter\def\csname v@tn/seoul/mix5/rel/sub-o500\endcsname{7.53}
\expandafter\def\csname v@tn/seoul/mix5/rel/sub-w20\endcsname{61.5}
\expandafter\def\csname v@tn/seoul/mix5/rel/w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/mae\endcsname{11.3}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/o500\endcsname{0.07}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/sub-mae\endcsname{128.6}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/sub-median\endcsname{9.9}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/sub-o500\endcsname{8.42}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/sub-w20\endcsname{62.0}
\expandafter\def\csname v@tn/seoul/mix5/s6fin/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix5/tn10/clean-mae\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/mix5/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/tn10/clean-o500\endcsname{0.10}
\expandafter\def\csname v@tn/seoul/mix5/tn10/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/mix5/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/tn10/mae\endcsname{20.5}
\expandafter\def\csname v@tn/seoul/mix5/tn10/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/mix5/tn10/o500\endcsname{0.71}
\expandafter\def\csname v@tn/seoul/mix5/tn10/sub-mae\endcsname{125.5}
\expandafter\def\csname v@tn/seoul/mix5/tn10/sub-median\endcsname{9.9}
\expandafter\def\csname v@tn/seoul/mix5/tn10/sub-o500\endcsname{8.42}
\expandafter\def\csname v@tn/seoul/mix5/tn10/sub-w20\endcsname{62.4}
\expandafter\def\csname v@tn/seoul/mix5/tn10/w20\endcsname{88.2}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/clean-mae\endcsname{11.6}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/mae\endcsname{20.1}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/o500\endcsname{0.74}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/sub-mae\endcsname{112.1}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/sub-median\endcsname{9.0}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/sub-o500\endcsname{7.53}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/sub-w20\endcsname{65.1}
\expandafter\def\csname v@tn/seoul/mix5/tn10s1/w20\endcsname{88.1}
\expandafter\def\csname v@tn/seoul/mix5/tn20/clean-mae\endcsname{11.7}
\expandafter\def\csname v@tn/seoul/mix5/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/mix5/tn20/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/mix5/tn20/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/mix5/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/tn20/mae\endcsname{20.5}
\expandafter\def\csname v@tn/seoul/mix5/tn20/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/mix5/tn20/o500\endcsname{0.75}
\expandafter\def\csname v@tn/seoul/mix5/tn20/sub-mae\endcsname{127.2}
\expandafter\def\csname v@tn/seoul/mix5/tn20/sub-median\endcsname{9.9}
\expandafter\def\csname v@tn/seoul/mix5/tn20/sub-o500\endcsname{8.06}
\expandafter\def\csname v@tn/seoul/mix5/tn20/sub-w20\endcsname{61.1}
\expandafter\def\csname v@tn/seoul/mix5/tn20/w20\endcsname{88.1}
\expandafter\def\csname v@tn/seoul/mix5/ts/clean-mae\endcsname{11.4}
\expandafter\def\csname v@tn/seoul/mix5/ts/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/ts/clean-o500\endcsname{0.09}
\expandafter\def\csname v@tn/seoul/mix5/ts/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/mix5/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/ts/mae\endcsname{24.7}
\expandafter\def\csname v@tn/seoul/mix5/ts/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/mix5/ts/o500\endcsname{1.06}
\expandafter\def\csname v@tn/seoul/mix5/ts/sub-mae\endcsname{144.9}
\expandafter\def\csname v@tn/seoul/mix5/ts/sub-median\endcsname{11.3}
\expandafter\def\csname v@tn/seoul/mix5/ts/sub-o500\endcsname{8.78}
\expandafter\def\csname v@tn/seoul/mix5/ts/sub-w20\endcsname{60.2}
\expandafter\def\csname v@tn/seoul/mix5/ts/w20\endcsname{87.6}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/clean-o500\endcsname{0.03}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/clean-w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/mae\endcsname{11.2}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/sub-mae\endcsname{122.0}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/sub-median\endcsname{9.7}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/sub-o500\endcsname{7.53}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/sub-w20\endcsname{64.2}
\expandafter\def\csname v@tn/seoul/mix5/turbofin/w20\endcsname{89.4}
\expandafter\def\csname v@tn/seoul/of\endcsname{1{,}294}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/clean-median\endcsname{8.2}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/clean-o500\endcsname{0.16}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/clean-w20\endcsname{81.1}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/mae\endcsname{18.9}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/median\endcsname{8.5}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/o500\endcsname{0.24}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/sub-mae\endcsname{79.6}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/sub-median\endcsname{12.8}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/sub-o500\endcsname{3.85}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/sub-w20\endcsname{61.6}
\expandafter\def\csname v@tn/seoul/sub10/ctcm/w20\endcsname{79.4}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/clean-mae\endcsname{13.6}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/clean-median\endcsname{7.3}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/clean-o500\endcsname{0.06}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/clean-w20\endcsname{85.8}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/mae\endcsname{16.2}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/median\endcsname{7.5}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/o500\endcsname{0.17}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/sub-mae\endcsname{82.8}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/sub-median\endcsname{10.9}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/sub-o500\endcsname{4.25}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/sub-w20\endcsname{65.3}
\expandafter\def\csname v@tn/seoul/sub10/ctcw/w20\endcsname{84.1}
\expandafter\def\csname v@tn/seoul/sub10/mfa/clean-mae\endcsname{21.8}
\expandafter\def\csname v@tn/seoul/sub10/mfa/clean-median\endcsname{10.8}
\expandafter\def\csname v@tn/seoul/sub10/mfa/clean-o500\endcsname{0.24}
\expandafter\def\csname v@tn/seoul/sub10/mfa/clean-w20\endcsname{70.1}
\expandafter\def\csname v@tn/seoul/sub10/mfa/failed\endcsname{11}
\expandafter\def\csname v@tn/seoul/sub10/mfa/mae\endcsname{29.7}
\expandafter\def\csname v@tn/seoul/sub10/mfa/median\endcsname{11.6}
\expandafter\def\csname v@tn/seoul/sub10/mfa/o500\endcsname{0.64}
\expandafter\def\csname v@tn/seoul/sub10/mfa/sub-mae\endcsname{129.5}
\expandafter\def\csname v@tn/seoul/sub10/mfa/sub-median\endcsname{37.8}
\expandafter\def\csname v@tn/seoul/sub10/mfa/sub-o500\endcsname{6.19}
\expandafter\def\csname v@tn/seoul/sub10/mfa/sub-w20\endcsname{35.7}
\expandafter\def\csname v@tn/seoul/sub10/mfa/w20\endcsname{67.6}
\expandafter\def\csname v@tn/seoul/sub10/post/clean-mae\endcsname{10.4}
\expandafter\def\csname v@tn/seoul/sub10/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/post/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/seoul/sub10/post/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/sub10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/post/mae\endcsname{15.3}
\expandafter\def\csname v@tn/seoul/sub10/post/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/sub10/post/o500\endcsname{0.31}
\expandafter\def\csname v@tn/seoul/sub10/post/sub-mae\endcsname{198.9}
\expandafter\def\csname v@tn/seoul/sub10/post/sub-median\endcsname{18.0}
\expandafter\def\csname v@tn/seoul/sub10/post/sub-o500\endcsname{13.22}
\expandafter\def\csname v@tn/seoul/sub10/post/sub-w20\endcsname{51.5}
\expandafter\def\csname v@tn/seoul/sub10/post/w20\endcsname{88.4}
\expandafter\def\csname v@tn/seoul/sub10/posttn/clean-mae\endcsname{10.3}
\expandafter\def\csname v@tn/seoul/sub10/posttn/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/posttn/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/seoul/sub10/posttn/clean-w20\endcsname{90.0}
\expandafter\def\csname v@tn/seoul/sub10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/posttn/mae\endcsname{11.8}
\expandafter\def\csname v@tn/seoul/sub10/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/sub10/posttn/o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/sub10/posttn/sub-mae\endcsname{143.3}
\expandafter\def\csname v@tn/seoul/sub10/posttn/sub-median\endcsname{10.4}
\expandafter\def\csname v@tn/seoul/sub10/posttn/sub-o500\endcsname{8.96}
\expandafter\def\csname v@tn/seoul/sub10/posttn/sub-w20\endcsname{60.5}
\expandafter\def\csname v@tn/seoul/sub10/posttn/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/sub10/rel/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/seoul/sub10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/rel/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/seoul/sub10/rel/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/sub10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/rel/mae\endcsname{11.0}
\expandafter\def\csname v@tn/seoul/sub10/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/rel/o500\endcsname{0.04}
\expandafter\def\csname v@tn/seoul/sub10/rel/sub-mae\endcsname{137.8}
\expandafter\def\csname v@tn/seoul/sub10/rel/sub-median\endcsname{9.9}
\expandafter\def\csname v@tn/seoul/sub10/rel/sub-o500\endcsname{8.72}
\expandafter\def\csname v@tn/seoul/sub10/rel/sub-w20\endcsname{62.2}
\expandafter\def\csname v@tn/seoul/sub10/rel/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/clean-mae\endcsname{10.4}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/clean-w20\endcsname{89.9}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/mae\endcsname{11.4}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/o500\endcsname{0.07}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/sub-mae\endcsname{136.5}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/sub-median\endcsname{9.9}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/sub-o500\endcsname{8.87}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/sub-w20\endcsname{62.6}
\expandafter\def\csname v@tn/seoul/sub10/s6fin/w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/sub10/tn10/clean-mae\endcsname{11.7}
\expandafter\def\csname v@tn/seoul/sub10/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/tn10/clean-o500\endcsname{0.10}
\expandafter\def\csname v@tn/seoul/sub10/tn10/clean-w20\endcsname{89.7}
\expandafter\def\csname v@tn/seoul/sub10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/tn10/mae\endcsname{26.6}
\expandafter\def\csname v@tn/seoul/sub10/tn10/median\endcsname{5.5}
\expandafter\def\csname v@tn/seoul/sub10/tn10/o500\endcsname{1.06}
\expandafter\def\csname v@tn/seoul/sub10/tn10/sub-mae\endcsname{131.7}
\expandafter\def\csname v@tn/seoul/sub10/tn10/sub-median\endcsname{9.0}
\expandafter\def\csname v@tn/seoul/sub10/tn10/sub-o500\endcsname{9.03}
\expandafter\def\csname v@tn/seoul/sub10/tn10/sub-w20\endcsname{63.8}
\expandafter\def\csname v@tn/seoul/sub10/tn10/w20\endcsname{87.2}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/clean-mae\endcsname{11.6}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/mae\endcsname{25.6}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/o500\endcsname{1.00}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/sub-mae\endcsname{128.8}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/sub-median\endcsname{9.1}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/sub-o500\endcsname{8.44}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/sub-w20\endcsname{63.7}
\expandafter\def\csname v@tn/seoul/sub10/tn10s1/w20\endcsname{87.2}
\expandafter\def\csname v@tn/seoul/sub10/tn20/clean-mae\endcsname{11.7}
\expandafter\def\csname v@tn/seoul/sub10/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/sub10/tn20/clean-o500\endcsname{0.11}
\expandafter\def\csname v@tn/seoul/sub10/tn20/clean-w20\endcsname{89.6}
\expandafter\def\csname v@tn/seoul/sub10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/tn20/mae\endcsname{25.3}
\expandafter\def\csname v@tn/seoul/sub10/tn20/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/sub10/tn20/o500\endcsname{1.01}
\expandafter\def\csname v@tn/seoul/sub10/tn20/sub-mae\endcsname{129.5}
\expandafter\def\csname v@tn/seoul/sub10/tn20/sub-median\endcsname{9.2}
\expandafter\def\csname v@tn/seoul/sub10/tn20/sub-o500\endcsname{8.32}
\expandafter\def\csname v@tn/seoul/sub10/tn20/sub-w20\endcsname{63.0}
\expandafter\def\csname v@tn/seoul/sub10/tn20/w20\endcsname{87.3}
\expandafter\def\csname v@tn/seoul/sub10/ts/clean-mae\endcsname{11.4}
\expandafter\def\csname v@tn/seoul/sub10/ts/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/ts/clean-o500\endcsname{0.09}
\expandafter\def\csname v@tn/seoul/sub10/ts/clean-w20\endcsname{89.8}
\expandafter\def\csname v@tn/seoul/sub10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/ts/mae\endcsname{34.9}
\expandafter\def\csname v@tn/seoul/sub10/ts/median\endcsname{5.6}
\expandafter\def\csname v@tn/seoul/sub10/ts/o500\endcsname{1.68}
\expandafter\def\csname v@tn/seoul/sub10/ts/sub-mae\endcsname{158.1}
\expandafter\def\csname v@tn/seoul/sub10/ts/sub-median\endcsname{11.5}
\expandafter\def\csname v@tn/seoul/sub10/ts/sub-o500\endcsname{9.92}
\expandafter\def\csname v@tn/seoul/sub10/ts/sub-w20\endcsname{58.3}
\expandafter\def\csname v@tn/seoul/sub10/ts/w20\endcsname{86.2}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/clean-w20\endcsname{89.5}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/mae\endcsname{13.0}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/o500\endcsname{0.17}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/sub-mae\endcsname{156.6}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/sub-median\endcsname{9.8}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/sub-o500\endcsname{10.69}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/sub-w20\endcsname{60.9}
\expandafter\def\csname v@tn/seoul/sub10/turbofin/w20\endcsname{89.3}
\expandafter\def\csname v@tn/seoul/utt\endcsname{1{,}047}
\expandafter\def\csname v@tn/timit/del10/ctcm/clean-mae\endcsname{17.2}
\expandafter\def\csname v@tn/timit/del10/ctcm/clean-median\endcsname{9.7}
\expandafter\def\csname v@tn/timit/del10/ctcm/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/ctcm/clean-w20\endcsname{73.9}
\expandafter\def\csname v@tn/timit/del10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/ctcm/mae\endcsname{31.9}
\expandafter\def\csname v@tn/timit/del10/ctcm/median\endcsname{10.3}
\expandafter\def\csname v@tn/timit/del10/ctcm/o500\endcsname{0.99}
\expandafter\def\csname v@tn/timit/del10/ctcm/w20\endcsname{70.8}
\expandafter\def\csname v@tn/timit/del10/ctcw/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/timit/del10/ctcw/clean-median\endcsname{9.1}
\expandafter\def\csname v@tn/timit/del10/ctcw/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/ctcw/clean-w20\endcsname{76.1}
\expandafter\def\csname v@tn/timit/del10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/ctcw/mae\endcsname{32.3}
\expandafter\def\csname v@tn/timit/del10/ctcw/median\endcsname{9.7}
\expandafter\def\csname v@tn/timit/del10/ctcw/o500\endcsname{1.04}
\expandafter\def\csname v@tn/timit/del10/ctcw/w20\endcsname{72.7}
\expandafter\def\csname v@tn/timit/del10/mfa/clean-mae\endcsname{19.2}
\expandafter\def\csname v@tn/timit/del10/mfa/clean-median\endcsname{12.0}
\expandafter\def\csname v@tn/timit/del10/mfa/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/mfa/clean-w20\endcsname{68.1}
\expandafter\def\csname v@tn/timit/del10/mfa/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/mfa/mae\endcsname{64.7}
\expandafter\def\csname v@tn/timit/del10/mfa/median\endcsname{14.2}
\expandafter\def\csname v@tn/timit/del10/mfa/o500\endcsname{3.36}
\expandafter\def\csname v@tn/timit/del10/mfa/w20\endcsname{59.8}
\expandafter\def\csname v@tn/timit/del10/post/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/del10/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/del10/post/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/post/clean-w20\endcsname{89.1}
\expandafter\def\csname v@tn/timit/del10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/post/mae\endcsname{23.4}
\expandafter\def\csname v@tn/timit/del10/post/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/del10/post/o500\endcsname{1.02}
\expandafter\def\csname v@tn/timit/del10/post/w20\endcsname{86.1}
\expandafter\def\csname v@tn/timit/del10/posttn/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/del10/posttn/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/posttn/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/del10/posttn/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/del10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/posttn/mae\endcsname{11.0}
\expandafter\def\csname v@tn/timit/del10/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/posttn/o500\endcsname{0.05}
\expandafter\def\csname v@tn/timit/del10/posttn/w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/del10/rel/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/del10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/del10/rel/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/rel/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/del10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/rel/mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/del10/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/del10/rel/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/rel/w20\endcsname{88.9}
\expandafter\def\csname v@tn/timit/del10/s6fin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/del10/s6fin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/s6fin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/s6fin/clean-w20\endcsname{88.6}
\expandafter\def\csname v@tn/timit/del10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/s6fin/mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/del10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/s6fin/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/del10/s6fin/w20\endcsname{88.5}
\expandafter\def\csname v@tn/timit/del10/tn10/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/del10/tn10/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/tn10/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/tn10/clean-w20\endcsname{88.9}
\expandafter\def\csname v@tn/timit/del10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/tn10/mae\endcsname{24.8}
\expandafter\def\csname v@tn/timit/del10/tn10/median\endcsname{5.7}
\expandafter\def\csname v@tn/timit/del10/tn10/o500\endcsname{0.86}
\expandafter\def\csname v@tn/timit/del10/tn10/w20\endcsname{85.0}
\expandafter\def\csname v@tn/timit/del10/tn10s1/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/del10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/del10/tn10s1/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/del10/tn10s1/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/del10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/tn10s1/mae\endcsname{24.9}
\expandafter\def\csname v@tn/timit/del10/tn10s1/median\endcsname{5.7}
\expandafter\def\csname v@tn/timit/del10/tn10s1/o500\endcsname{0.87}
\expandafter\def\csname v@tn/timit/del10/tn10s1/w20\endcsname{84.9}
\expandafter\def\csname v@tn/timit/del10/tn20/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/del10/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/tn20/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/del10/tn20/clean-w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/del10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/tn20/mae\endcsname{24.8}
\expandafter\def\csname v@tn/timit/del10/tn20/median\endcsname{5.8}
\expandafter\def\csname v@tn/timit/del10/tn20/o500\endcsname{0.85}
\expandafter\def\csname v@tn/timit/del10/tn20/w20\endcsname{84.9}
\expandafter\def\csname v@tn/timit/del10/ts/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/del10/ts/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/del10/ts/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/del10/ts/clean-w20\endcsname{89.2}
\expandafter\def\csname v@tn/timit/del10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/ts/mae\endcsname{28.2}
\expandafter\def\csname v@tn/timit/del10/ts/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/del10/ts/o500\endcsname{1.21}
\expandafter\def\csname v@tn/timit/del10/ts/w20\endcsname{84.8}
\expandafter\def\csname v@tn/timit/del10/turbofin/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/del10/turbofin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/turbofin/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/del10/turbofin/clean-w20\endcsname{88.4}
\expandafter\def\csname v@tn/timit/del10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/del10/turbofin/mae\endcsname{11.3}
\expandafter\def\csname v@tn/timit/del10/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/del10/turbofin/o500\endcsname{0.06}
\expandafter\def\csname v@tn/timit/del10/turbofin/w20\endcsname{88.3}
\expandafter\def\csname v@tn/timit/ins10/ctcm/clean-mae\endcsname{17.2}
\expandafter\def\csname v@tn/timit/ins10/ctcm/clean-median\endcsname{9.6}
\expandafter\def\csname v@tn/timit/ins10/ctcm/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/ctcm/clean-w20\endcsname{73.9}
\expandafter\def\csname v@tn/timit/ins10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/ctcm/mae\endcsname{25.4}
\expandafter\def\csname v@tn/timit/ins10/ctcm/median\endcsname{11.3}
\expandafter\def\csname v@tn/timit/ins10/ctcm/o500\endcsname{0.08}
\expandafter\def\csname v@tn/timit/ins10/ctcm/w20\endcsname{67.2}
\expandafter\def\csname v@tn/timit/ins10/ctcw/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/timit/ins10/ctcw/clean-median\endcsname{9.1}
\expandafter\def\csname v@tn/timit/ins10/ctcw/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/ins10/ctcw/clean-w20\endcsname{76.0}
\expandafter\def\csname v@tn/timit/ins10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/ctcw/mae\endcsname{25.2}
\expandafter\def\csname v@tn/timit/ins10/ctcw/median\endcsname{10.7}
\expandafter\def\csname v@tn/timit/ins10/ctcw/o500\endcsname{0.07}
\expandafter\def\csname v@tn/timit/ins10/ctcw/w20\endcsname{69.2}
\expandafter\def\csname v@tn/timit/ins10/mfa/clean-mae\endcsname{19.2}
\expandafter\def\csname v@tn/timit/ins10/mfa/clean-median\endcsname{12.1}
\expandafter\def\csname v@tn/timit/ins10/mfa/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/ins10/mfa/clean-w20\endcsname{68.1}
\expandafter\def\csname v@tn/timit/ins10/mfa/failed\endcsname{39}
\expandafter\def\csname v@tn/timit/ins10/mfa/mae\endcsname{35.0}
\expandafter\def\csname v@tn/timit/ins10/mfa/median\endcsname{13.4}
\expandafter\def\csname v@tn/timit/ins10/mfa/o500\endcsname{0.57}
\expandafter\def\csname v@tn/timit/ins10/mfa/w20\endcsname{60.9}
\expandafter\def\csname v@tn/timit/ins10/post/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/ins10/post/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/ins10/post/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/post/clean-w20\endcsname{89.2}
\expandafter\def\csname v@tn/timit/ins10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/post/mae\endcsname{13.0}
\expandafter\def\csname v@tn/timit/ins10/post/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/post/o500\endcsname{0.05}
\expandafter\def\csname v@tn/timit/ins10/post/w20\endcsname{87.7}
\expandafter\def\csname v@tn/timit/ins10/posttn/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/ins10/posttn/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/posttn/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/posttn/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/ins10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/posttn/mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/ins10/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/posttn/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/ins10/posttn/w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/ins10/rel/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/ins10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/ins10/rel/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/rel/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/ins10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/rel/mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/ins10/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/ins10/rel/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/rel/w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/ins10/s6fin/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/ins10/s6fin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/s6fin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/s6fin/clean-w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/ins10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/s6fin/mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/ins10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/s6fin/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/s6fin/w20\endcsname{88.6}
\expandafter\def\csname v@tn/timit/ins10/tn10/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/ins10/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/ins10/tn10/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/tn10/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/ins10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/tn10/mae\endcsname{14.3}
\expandafter\def\csname v@tn/timit/ins10/tn10/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/ins10/tn10/o500\endcsname{0.18}
\expandafter\def\csname v@tn/timit/ins10/tn10/w20\endcsname{87.8}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/mae\endcsname{14.1}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/o500\endcsname{0.18}
\expandafter\def\csname v@tn/timit/ins10/tn10s1/w20\endcsname{87.7}
\expandafter\def\csname v@tn/timit/ins10/tn20/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/ins10/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/tn20/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/ins10/tn20/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/ins10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/tn20/mae\endcsname{15.7}
\expandafter\def\csname v@tn/timit/ins10/tn20/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/ins10/tn20/o500\endcsname{0.29}
\expandafter\def\csname v@tn/timit/ins10/tn20/w20\endcsname{87.2}
\expandafter\def\csname v@tn/timit/ins10/ts/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/ins10/ts/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/ins10/ts/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/ins10/ts/clean-w20\endcsname{89.3}
\expandafter\def\csname v@tn/timit/ins10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/ts/mae\endcsname{18.9}
\expandafter\def\csname v@tn/timit/ins10/ts/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/ins10/ts/o500\endcsname{0.33}
\expandafter\def\csname v@tn/timit/ins10/ts/w20\endcsname{86.1}
\expandafter\def\csname v@tn/timit/ins10/turbofin/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/ins10/turbofin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/turbofin/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/ins10/turbofin/clean-w20\endcsname{88.5}
\expandafter\def\csname v@tn/timit/ins10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/ins10/turbofin/mae\endcsname{11.2}
\expandafter\def\csname v@tn/timit/ins10/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/ins10/turbofin/o500\endcsname{0.03}
\expandafter\def\csname v@tn/timit/ins10/turbofin/w20\endcsname{88.4}
\expandafter\def\csname v@tn/timit/mix10/ctcm/clean-mae\endcsname{17.0}
\expandafter\def\csname v@tn/timit/mix10/ctcm/clean-median\endcsname{9.7}
\expandafter\def\csname v@tn/timit/mix10/ctcm/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/ctcm/clean-w20\endcsname{74.0}
\expandafter\def\csname v@tn/timit/mix10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/ctcm/mae\endcsname{25.2}
\expandafter\def\csname v@tn/timit/mix10/ctcm/median\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix10/ctcm/o500\endcsname{0.28}
\expandafter\def\csname v@tn/timit/mix10/ctcm/sub-mae\endcsname{54.0}
\expandafter\def\csname v@tn/timit/mix10/ctcm/sub-median\endcsname{15.7}
\expandafter\def\csname v@tn/timit/mix10/ctcm/sub-o500\endcsname{1.56}
\expandafter\def\csname v@tn/timit/mix10/ctcm/sub-w20\endcsname{57.1}
\expandafter\def\csname v@tn/timit/mix10/ctcm/w20\endcsname{70.0}
\expandafter\def\csname v@tn/timit/mix10/ctcw/clean-mae\endcsname{16.3}
\expandafter\def\csname v@tn/timit/mix10/ctcw/clean-median\endcsname{9.1}
\expandafter\def\csname v@tn/timit/mix10/ctcw/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/ctcw/clean-w20\endcsname{76.1}
\expandafter\def\csname v@tn/timit/mix10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/ctcw/mae\endcsname{25.1}
\expandafter\def\csname v@tn/timit/mix10/ctcw/median\endcsname{10.0}
\expandafter\def\csname v@tn/timit/mix10/ctcw/o500\endcsname{0.35}
\expandafter\def\csname v@tn/timit/mix10/ctcw/sub-mae\endcsname{62.4}
\expandafter\def\csname v@tn/timit/mix10/ctcw/sub-median\endcsname{17.8}
\expandafter\def\csname v@tn/timit/mix10/ctcw/sub-o500\endcsname{1.70}
\expandafter\def\csname v@tn/timit/mix10/ctcw/sub-w20\endcsname{52.4}
\expandafter\def\csname v@tn/timit/mix10/ctcw/w20\endcsname{72.0}
\expandafter\def\csname v@tn/timit/mix10/mfa/clean-mae\endcsname{19.1}
\expandafter\def\csname v@tn/timit/mix10/mfa/clean-median\endcsname{11.9}
\expandafter\def\csname v@tn/timit/mix10/mfa/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/mfa/clean-w20\endcsname{68.2}
\expandafter\def\csname v@tn/timit/mix10/mfa/failed\endcsname{10}
\expandafter\def\csname v@tn/timit/mix10/mfa/mae\endcsname{42.5}
\expandafter\def\csname v@tn/timit/mix10/mfa/median\endcsname{13.2}
\expandafter\def\csname v@tn/timit/mix10/mfa/o500\endcsname{1.40}
\expandafter\def\csname v@tn/timit/mix10/mfa/sub-mae\endcsname{111.7}
\expandafter\def\csname v@tn/timit/mix10/mfa/sub-median\endcsname{48.8}
\expandafter\def\csname v@tn/timit/mix10/mfa/sub-o500\endcsname{2.84}
\expandafter\def\csname v@tn/timit/mix10/mfa/sub-w20\endcsname{28.6}
\expandafter\def\csname v@tn/timit/mix10/mfa/w20\endcsname{61.2}
\expandafter\def\csname v@tn/timit/mix10/post/clean-mae\endcsname{10.4}
\expandafter\def\csname v@tn/timit/mix10/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix10/post/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/post/clean-w20\endcsname{89.1}
\expandafter\def\csname v@tn/timit/mix10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/post/mae\endcsname{17.2}
\expandafter\def\csname v@tn/timit/mix10/post/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/mix10/post/o500\endcsname{0.48}
\expandafter\def\csname v@tn/timit/mix10/post/sub-mae\endcsname{131.9}
\expandafter\def\csname v@tn/timit/mix10/post/sub-median\endcsname{17.5}
\expandafter\def\csname v@tn/timit/mix10/post/sub-o500\endcsname{8.66}
\expandafter\def\csname v@tn/timit/mix10/post/sub-w20\endcsname{51.0}
\expandafter\def\csname v@tn/timit/mix10/post/w20\endcsname{86.9}
\expandafter\def\csname v@tn/timit/mix10/posttn/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix10/posttn/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix10/posttn/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix10/posttn/clean-w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/mix10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/posttn/mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/mix10/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix10/posttn/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix10/posttn/sub-mae\endcsname{110.9}
\expandafter\def\csname v@tn/timit/mix10/posttn/sub-median\endcsname{11.1}
\expandafter\def\csname v@tn/timit/mix10/posttn/sub-o500\endcsname{5.97}
\expandafter\def\csname v@tn/timit/mix10/posttn/sub-w20\endcsname{60.1}
\expandafter\def\csname v@tn/timit/mix10/posttn/w20\endcsname{88.6}
\expandafter\def\csname v@tn/timit/mix10/rel/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix10/rel/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/rel/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/mix10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/rel/mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/mix10/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix10/rel/o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/rel/sub-mae\endcsname{106.5}
\expandafter\def\csname v@tn/timit/mix10/rel/sub-median\endcsname{9.3}
\expandafter\def\csname v@tn/timit/mix10/rel/sub-o500\endcsname{6.39}
\expandafter\def\csname v@tn/timit/mix10/rel/sub-w20\endcsname{63.2}
\expandafter\def\csname v@tn/timit/mix10/rel/w20\endcsname{88.9}
\expandafter\def\csname v@tn/timit/mix10/s6fin/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix10/s6fin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix10/s6fin/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/s6fin/clean-w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/mix10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/s6fin/mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/mix10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix10/s6fin/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix10/s6fin/sub-mae\endcsname{105.6}
\expandafter\def\csname v@tn/timit/mix10/s6fin/sub-median\endcsname{9.6}
\expandafter\def\csname v@tn/timit/mix10/s6fin/sub-o500\endcsname{6.39}
\expandafter\def\csname v@tn/timit/mix10/s6fin/sub-w20\endcsname{63.5}
\expandafter\def\csname v@tn/timit/mix10/s6fin/w20\endcsname{88.5}
\expandafter\def\csname v@tn/timit/mix10/tn10/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix10/tn10/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix10/tn10/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/tn10/clean-w20\endcsname{88.9}
\expandafter\def\csname v@tn/timit/mix10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/tn10/mae\endcsname{19.2}
\expandafter\def\csname v@tn/timit/mix10/tn10/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/mix10/tn10/o500\endcsname{0.48}
\expandafter\def\csname v@tn/timit/mix10/tn10/sub-mae\endcsname{111.4}
\expandafter\def\csname v@tn/timit/mix10/tn10/sub-median\endcsname{10.2}
\expandafter\def\csname v@tn/timit/mix10/tn10/sub-o500\endcsname{5.68}
\expandafter\def\csname v@tn/timit/mix10/tn10/sub-w20\endcsname{60.2}
\expandafter\def\csname v@tn/timit/mix10/tn10/w20\endcsname{86.3}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/clean-o500\endcsname{0.00}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/mae\endcsname{19.0}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/o500\endcsname{0.47}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/sub-mae\endcsname{108.8}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/sub-median\endcsname{9.7}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/sub-o500\endcsname{6.11}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/sub-w20\endcsname{61.1}
\expandafter\def\csname v@tn/timit/mix10/tn10s1/w20\endcsname{86.4}
\expandafter\def\csname v@tn/timit/mix10/tn20/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/mix10/tn20/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix10/tn20/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix10/tn20/clean-w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/mix10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/tn20/mae\endcsname{19.5}
\expandafter\def\csname v@tn/timit/mix10/tn20/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/mix10/tn20/o500\endcsname{0.51}
\expandafter\def\csname v@tn/timit/mix10/tn20/sub-mae\endcsname{104.0}
\expandafter\def\csname v@tn/timit/mix10/tn20/sub-median\endcsname{8.3}
\expandafter\def\csname v@tn/timit/mix10/tn20/sub-o500\endcsname{5.40}
\expandafter\def\csname v@tn/timit/mix10/tn20/sub-w20\endcsname{63.1}
\expandafter\def\csname v@tn/timit/mix10/tn20/w20\endcsname{86.2}
\expandafter\def\csname v@tn/timit/mix10/ts/clean-mae\endcsname{10.4}
\expandafter\def\csname v@tn/timit/mix10/ts/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/mix10/ts/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix10/ts/clean-w20\endcsname{89.2}
\expandafter\def\csname v@tn/timit/mix10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/ts/mae\endcsname{22.7}
\expandafter\def\csname v@tn/timit/mix10/ts/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/mix10/ts/o500\endcsname{0.73}
\expandafter\def\csname v@tn/timit/mix10/ts/sub-mae\endcsname{111.5}
\expandafter\def\csname v@tn/timit/mix10/ts/sub-median\endcsname{13.4}
\expandafter\def\csname v@tn/timit/mix10/ts/sub-o500\endcsname{6.11}
\expandafter\def\csname v@tn/timit/mix10/ts/sub-w20\endcsname{56.4}
\expandafter\def\csname v@tn/timit/mix10/ts/w20\endcsname{85.4}
\expandafter\def\csname v@tn/timit/mix10/turbofin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/mix10/turbofin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix10/turbofin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix10/turbofin/clean-w20\endcsname{88.4}
\expandafter\def\csname v@tn/timit/mix10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix10/turbofin/mae\endcsname{11.0}
\expandafter\def\csname v@tn/timit/mix10/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix10/turbofin/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix10/turbofin/sub-mae\endcsname{95.8}
\expandafter\def\csname v@tn/timit/mix10/turbofin/sub-median\endcsname{8.8}
\expandafter\def\csname v@tn/timit/mix10/turbofin/sub-o500\endcsname{5.68}
\expandafter\def\csname v@tn/timit/mix10/turbofin/sub-w20\endcsname{64.3}
\expandafter\def\csname v@tn/timit/mix10/turbofin/w20\endcsname{88.4}
\expandafter\def\csname v@tn/timit/mix20/ctcm/clean-mae\endcsname{17.1}
\expandafter\def\csname v@tn/timit/mix20/ctcm/clean-median\endcsname{9.7}
\expandafter\def\csname v@tn/timit/mix20/ctcm/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/ctcm/clean-w20\endcsname{74.0}
\expandafter\def\csname v@tn/timit/mix20/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/ctcm/mae\endcsname{36.4}
\expandafter\def\csname v@tn/timit/mix20/ctcm/median\endcsname{11.7}
\expandafter\def\csname v@tn/timit/mix20/ctcm/o500\endcsname{1.01}
\expandafter\def\csname v@tn/timit/mix20/ctcm/sub-mae\endcsname{72.5}
\expandafter\def\csname v@tn/timit/mix20/ctcm/sub-median\endcsname{18.8}
\expandafter\def\csname v@tn/timit/mix20/ctcm/sub-o500\endcsname{2.68}
\expandafter\def\csname v@tn/timit/mix20/ctcm/sub-w20\endcsname{51.6}
\expandafter\def\csname v@tn/timit/mix20/ctcm/w20\endcsname{66.0}
\expandafter\def\csname v@tn/timit/mix20/ctcw/clean-mae\endcsname{16.3}
\expandafter\def\csname v@tn/timit/mix20/ctcw/clean-median\endcsname{9.1}
\expandafter\def\csname v@tn/timit/mix20/ctcw/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/ctcw/clean-w20\endcsname{76.1}
\expandafter\def\csname v@tn/timit/mix20/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/ctcw/mae\endcsname{36.1}
\expandafter\def\csname v@tn/timit/mix20/ctcw/median\endcsname{11.1}
\expandafter\def\csname v@tn/timit/mix20/ctcw/o500\endcsname{0.86}
\expandafter\def\csname v@tn/timit/mix20/ctcw/sub-mae\endcsname{78.3}
\expandafter\def\csname v@tn/timit/mix20/ctcw/sub-median\endcsname{22.9}
\expandafter\def\csname v@tn/timit/mix20/ctcw/sub-o500\endcsname{2.68}
\expandafter\def\csname v@tn/timit/mix20/ctcw/sub-w20\endcsname{47.2}
\expandafter\def\csname v@tn/timit/mix20/ctcw/w20\endcsname{67.6}
\expandafter\def\csname v@tn/timit/mix20/mfa/clean-mae\endcsname{19.2}
\expandafter\def\csname v@tn/timit/mix20/mfa/clean-median\endcsname{12.2}
\expandafter\def\csname v@tn/timit/mix20/mfa/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/mfa/clean-w20\endcsname{67.9}
\expandafter\def\csname v@tn/timit/mix20/mfa/failed\endcsname{27}
\expandafter\def\csname v@tn/timit/mix20/mfa/mae\endcsname{73.0}
\expandafter\def\csname v@tn/timit/mix20/mfa/median\endcsname{17.5}
\expandafter\def\csname v@tn/timit/mix20/mfa/o500\endcsname{3.83}
\expandafter\def\csname v@tn/timit/mix20/mfa/sub-mae\endcsname{129.9}
\expandafter\def\csname v@tn/timit/mix20/mfa/sub-median\endcsname{47.5}
\expandafter\def\csname v@tn/timit/mix20/mfa/sub-o500\endcsname{6.07}
\expandafter\def\csname v@tn/timit/mix20/mfa/sub-w20\endcsname{27.5}
\expandafter\def\csname v@tn/timit/mix20/mfa/w20\endcsname{54.1}
\expandafter\def\csname v@tn/timit/mix20/post/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/mix20/post/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/mix20/post/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/post/clean-w20\endcsname{89.2}
\expandafter\def\csname v@tn/timit/mix20/post/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/post/mae\endcsname{22.9}
\expandafter\def\csname v@tn/timit/mix20/post/median\endcsname{5.7}
\expandafter\def\csname v@tn/timit/mix20/post/o500\endcsname{0.80}
\expandafter\def\csname v@tn/timit/mix20/post/sub-mae\endcsname{150.3}
\expandafter\def\csname v@tn/timit/mix20/post/sub-median\endcsname{25.3}
\expandafter\def\csname v@tn/timit/mix20/post/sub-o500\endcsname{9.38}
\expandafter\def\csname v@tn/timit/mix20/post/sub-w20\endcsname{47.7}
\expandafter\def\csname v@tn/timit/mix20/post/w20\endcsname{85.2}
\expandafter\def\csname v@tn/timit/mix20/posttn/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix20/posttn/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/posttn/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix20/posttn/clean-w20\endcsname{88.9}
\expandafter\def\csname v@tn/timit/mix20/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/posttn/mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/mix20/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/posttn/o500\endcsname{0.03}
\expandafter\def\csname v@tn/timit/mix20/posttn/sub-mae\endcsname{119.6}
\expandafter\def\csname v@tn/timit/mix20/posttn/sub-median\endcsname{12.0}
\expandafter\def\csname v@tn/timit/mix20/posttn/sub-o500\endcsname{6.94}
\expandafter\def\csname v@tn/timit/mix20/posttn/sub-w20\endcsname{57.4}
\expandafter\def\csname v@tn/timit/mix20/posttn/w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix20/rel/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix20/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix20/rel/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/rel/clean-w20\endcsname{89.1}
\expandafter\def\csname v@tn/timit/mix20/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/rel/mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/mix20/rel/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/rel/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix20/rel/sub-mae\endcsname{123.8}
\expandafter\def\csname v@tn/timit/mix20/rel/sub-median\endcsname{11.8}
\expandafter\def\csname v@tn/timit/mix20/rel/sub-o500\endcsname{7.81}
\expandafter\def\csname v@tn/timit/mix20/rel/sub-w20\endcsname{58.9}
\expandafter\def\csname v@tn/timit/mix20/rel/w20\endcsname{88.9}
\expandafter\def\csname v@tn/timit/mix20/s6fin/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/mix20/s6fin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/s6fin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/s6fin/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix20/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/s6fin/mae\endcsname{11.2}
\expandafter\def\csname v@tn/timit/mix20/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/s6fin/o500\endcsname{0.04}
\expandafter\def\csname v@tn/timit/mix20/s6fin/sub-mae\endcsname{120.5}
\expandafter\def\csname v@tn/timit/mix20/s6fin/sub-median\endcsname{11.2}
\expandafter\def\csname v@tn/timit/mix20/s6fin/sub-o500\endcsname{7.81}
\expandafter\def\csname v@tn/timit/mix20/s6fin/sub-w20\endcsname{59.1}
\expandafter\def\csname v@tn/timit/mix20/s6fin/w20\endcsname{88.5}
\expandafter\def\csname v@tn/timit/mix20/tn10/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix20/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix20/tn10/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/tn10/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/mix20/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/tn10/mae\endcsname{28.5}
\expandafter\def\csname v@tn/timit/mix20/tn10/median\endcsname{5.8}
\expandafter\def\csname v@tn/timit/mix20/tn10/o500\endcsname{1.15}
\expandafter\def\csname v@tn/timit/mix20/tn10/sub-mae\endcsname{127.7}
\expandafter\def\csname v@tn/timit/mix20/tn10/sub-median\endcsname{12.2}
\expandafter\def\csname v@tn/timit/mix20/tn10/sub-o500\endcsname{8.04}
\expandafter\def\csname v@tn/timit/mix20/tn10/sub-w20\endcsname{56.8}
\expandafter\def\csname v@tn/timit/mix20/tn10/w20\endcsname{84.1}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/mae\endcsname{28.7}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/median\endcsname{5.8}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/o500\endcsname{1.13}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/sub-mae\endcsname{124.4}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/sub-median\endcsname{11.2}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/sub-o500\endcsname{7.33}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/sub-w20\endcsname{58.4}
\expandafter\def\csname v@tn/timit/mix20/tn10s1/w20\endcsname{83.9}
\expandafter\def\csname v@tn/timit/mix20/tn20/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/mix20/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/tn20/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix20/tn20/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix20/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/tn20/mae\endcsname{28.5}
\expandafter\def\csname v@tn/timit/mix20/tn20/median\endcsname{5.9}
\expandafter\def\csname v@tn/timit/mix20/tn20/o500\endcsname{1.08}
\expandafter\def\csname v@tn/timit/mix20/tn20/sub-mae\endcsname{119.4}
\expandafter\def\csname v@tn/timit/mix20/tn20/sub-median\endcsname{11.2}
\expandafter\def\csname v@tn/timit/mix20/tn20/sub-o500\endcsname{7.41}
\expandafter\def\csname v@tn/timit/mix20/tn20/sub-w20\endcsname{59.1}
\expandafter\def\csname v@tn/timit/mix20/tn20/w20\endcsname{83.9}
\expandafter\def\csname v@tn/timit/mix20/ts/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/mix20/ts/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/mix20/ts/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix20/ts/clean-w20\endcsname{89.4}
\expandafter\def\csname v@tn/timit/mix20/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/ts/mae\endcsname{34.9}
\expandafter\def\csname v@tn/timit/mix20/ts/median\endcsname{5.9}
\expandafter\def\csname v@tn/timit/mix20/ts/o500\endcsname{1.42}
\expandafter\def\csname v@tn/timit/mix20/ts/sub-mae\endcsname{143.9}
\expandafter\def\csname v@tn/timit/mix20/ts/sub-median\endcsname{19.2}
\expandafter\def\csname v@tn/timit/mix20/ts/sub-o500\endcsname{8.83}
\expandafter\def\csname v@tn/timit/mix20/ts/sub-w20\endcsname{50.3}
\expandafter\def\csname v@tn/timit/mix20/ts/w20\endcsname{82.1}
\expandafter\def\csname v@tn/timit/mix20/turbofin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/mix20/turbofin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/turbofin/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix20/turbofin/clean-w20\endcsname{88.4}
\expandafter\def\csname v@tn/timit/mix20/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix20/turbofin/mae\endcsname{11.1}
\expandafter\def\csname v@tn/timit/mix20/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix20/turbofin/o500\endcsname{0.03}
\expandafter\def\csname v@tn/timit/mix20/turbofin/sub-mae\endcsname{115.2}
\expandafter\def\csname v@tn/timit/mix20/turbofin/sub-median\endcsname{10.2}
\expandafter\def\csname v@tn/timit/mix20/turbofin/sub-o500\endcsname{7.57}
\expandafter\def\csname v@tn/timit/mix20/turbofin/sub-w20\endcsname{62.5}
\expandafter\def\csname v@tn/timit/mix20/turbofin/w20\endcsname{88.3}
\expandafter\def\csname v@tn/timit/mix5/ctcm/clean-mae\endcsname{17.2}
\expandafter\def\csname v@tn/timit/mix5/ctcm/clean-median\endcsname{9.7}
\expandafter\def\csname v@tn/timit/mix5/ctcm/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/ctcm/clean-w20\endcsname{73.9}
\expandafter\def\csname v@tn/timit/mix5/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/ctcm/mae\endcsname{20.8}
\expandafter\def\csname v@tn/timit/mix5/ctcm/median\endcsname{10.0}
\expandafter\def\csname v@tn/timit/mix5/ctcm/o500\endcsname{0.14}
\expandafter\def\csname v@tn/timit/mix5/ctcm/sub-mae\endcsname{43.1}
\expandafter\def\csname v@tn/timit/mix5/ctcm/sub-median\endcsname{12.6}
\expandafter\def\csname v@tn/timit/mix5/ctcm/sub-o500\endcsname{0.91}
\expandafter\def\csname v@tn/timit/mix5/ctcm/sub-w20\endcsname{61.0}
\expandafter\def\csname v@tn/timit/mix5/ctcm/w20\endcsname{72.2}
\expandafter\def\csname v@tn/timit/mix5/ctcw/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/timit/mix5/ctcw/clean-median\endcsname{9.1}
\expandafter\def\csname v@tn/timit/mix5/ctcw/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/ctcw/clean-w20\endcsname{76.0}
\expandafter\def\csname v@tn/timit/mix5/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/ctcw/mae\endcsname{20.2}
\expandafter\def\csname v@tn/timit/mix5/ctcw/median\endcsname{9.5}
\expandafter\def\csname v@tn/timit/mix5/ctcw/o500\endcsname{0.14}
\expandafter\def\csname v@tn/timit/mix5/ctcw/sub-mae\endcsname{48.1}
\expandafter\def\csname v@tn/timit/mix5/ctcw/sub-median\endcsname{14.9}
\expandafter\def\csname v@tn/timit/mix5/ctcw/sub-o500\endcsname{0.91}
\expandafter\def\csname v@tn/timit/mix5/ctcw/sub-w20\endcsname{56.7}
\expandafter\def\csname v@tn/timit/mix5/ctcw/w20\endcsname{74.2}
\expandafter\def\csname v@tn/timit/mix5/mfa/clean-mae\endcsname{19.2}
\expandafter\def\csname v@tn/timit/mix5/mfa/clean-median\endcsname{12.1}
\expandafter\def\csname v@tn/timit/mix5/mfa/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/mfa/clean-w20\endcsname{68.2}
\expandafter\def\csname v@tn/timit/mix5/mfa/failed\endcsname{5}
\expandafter\def\csname v@tn/timit/mix5/mfa/mae\endcsname{31.6}
\expandafter\def\csname v@tn/timit/mix5/mfa/median\endcsname{12.5}
\expandafter\def\csname v@tn/timit/mix5/mfa/o500\endcsname{0.75}
\expandafter\def\csname v@tn/timit/mix5/mfa/sub-mae\endcsname{97.3}
\expandafter\def\csname v@tn/timit/mix5/mfa/sub-median\endcsname{42.5}
\expandafter\def\csname v@tn/timit/mix5/mfa/sub-o500\endcsname{2.44}
\expandafter\def\csname v@tn/timit/mix5/mfa/sub-w20\endcsname{31.1}
\expandafter\def\csname v@tn/timit/mix5/mfa/w20\endcsname{65.0}
\expandafter\def\csname v@tn/timit/mix5/post/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/mix5/post/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/mix5/post/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/post/clean-w20\endcsname{89.2}
\expandafter\def\csname v@tn/timit/mix5/post/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/post/mae\endcsname{13.4}
\expandafter\def\csname v@tn/timit/mix5/post/median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix5/post/o500\endcsname{0.19}
\expandafter\def\csname v@tn/timit/mix5/post/sub-mae\endcsname{140.3}
\expandafter\def\csname v@tn/timit/mix5/post/sub-median\endcsname{22.6}
\expandafter\def\csname v@tn/timit/mix5/post/sub-o500\endcsname{9.45}
\expandafter\def\csname v@tn/timit/mix5/post/sub-w20\endcsname{48.2}
\expandafter\def\csname v@tn/timit/mix5/post/w20\endcsname{88.1}
\expandafter\def\csname v@tn/timit/mix5/posttn/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/mix5/posttn/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/posttn/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix5/posttn/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix5/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/posttn/mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/mix5/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/posttn/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix5/posttn/sub-mae\endcsname{101.2}
\expandafter\def\csname v@tn/timit/mix5/posttn/sub-median\endcsname{9.5}
\expandafter\def\csname v@tn/timit/mix5/posttn/sub-o500\endcsname{6.10}
\expandafter\def\csname v@tn/timit/mix5/posttn/sub-w20\endcsname{63.4}
\expandafter\def\csname v@tn/timit/mix5/posttn/w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix5/rel/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix5/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix5/rel/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/rel/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/mix5/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/rel/mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix5/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix5/rel/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/rel/sub-mae\endcsname{104.6}
\expandafter\def\csname v@tn/timit/mix5/rel/sub-median\endcsname{8.9}
\expandafter\def\csname v@tn/timit/mix5/rel/sub-o500\endcsname{7.01}
\expandafter\def\csname v@tn/timit/mix5/rel/sub-w20\endcsname{64.3}
\expandafter\def\csname v@tn/timit/mix5/rel/w20\endcsname{89.1}
\expandafter\def\csname v@tn/timit/mix5/s6fin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/mix5/s6fin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/s6fin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/s6fin/clean-w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/mix5/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/s6fin/mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/mix5/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/s6fin/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/s6fin/sub-mae\endcsname{99.5}
\expandafter\def\csname v@tn/timit/mix5/s6fin/sub-median\endcsname{8.7}
\expandafter\def\csname v@tn/timit/mix5/s6fin/sub-o500\endcsname{6.10}
\expandafter\def\csname v@tn/timit/mix5/s6fin/sub-w20\endcsname{65.5}
\expandafter\def\csname v@tn/timit/mix5/s6fin/w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/mix5/tn10/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/mix5/tn10/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/tn10/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/tn10/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/mix5/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/tn10/mae\endcsname{14.6}
\expandafter\def\csname v@tn/timit/mix5/tn10/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/mix5/tn10/o500\endcsname{0.29}
\expandafter\def\csname v@tn/timit/mix5/tn10/sub-mae\endcsname{103.2}
\expandafter\def\csname v@tn/timit/mix5/tn10/sub-median\endcsname{8.6}
\expandafter\def\csname v@tn/timit/mix5/tn10/sub-o500\endcsname{7.62}
\expandafter\def\csname v@tn/timit/mix5/tn10/sub-w20\endcsname{64.3}
\expandafter\def\csname v@tn/timit/mix5/tn10/w20\endcsname{87.8}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/clean-mae\endcsname{10.6}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/mae\endcsname{14.6}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/o500\endcsname{0.28}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/sub-mae\endcsname{108.5}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/sub-median\endcsname{9.0}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/sub-o500\endcsname{7.32}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/sub-w20\endcsname{61.6}
\expandafter\def\csname v@tn/timit/mix5/tn10s1/w20\endcsname{87.6}
\expandafter\def\csname v@tn/timit/mix5/tn20/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/mix5/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/tn20/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix5/tn20/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/mix5/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/tn20/mae\endcsname{14.9}
\expandafter\def\csname v@tn/timit/mix5/tn20/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/mix5/tn20/o500\endcsname{0.30}
\expandafter\def\csname v@tn/timit/mix5/tn20/sub-mae\endcsname{116.2}
\expandafter\def\csname v@tn/timit/mix5/tn20/sub-median\endcsname{8.8}
\expandafter\def\csname v@tn/timit/mix5/tn20/sub-o500\endcsname{7.93}
\expandafter\def\csname v@tn/timit/mix5/tn20/sub-w20\endcsname{63.1}
\expandafter\def\csname v@tn/timit/mix5/tn20/w20\endcsname{87.6}
\expandafter\def\csname v@tn/timit/mix5/ts/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/mix5/ts/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/mix5/ts/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix5/ts/clean-w20\endcsname{89.3}
\expandafter\def\csname v@tn/timit/mix5/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/ts/mae\endcsname{16.6}
\expandafter\def\csname v@tn/timit/mix5/ts/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/ts/o500\endcsname{0.38}
\expandafter\def\csname v@tn/timit/mix5/ts/sub-mae\endcsname{105.9}
\expandafter\def\csname v@tn/timit/mix5/ts/sub-median\endcsname{11.7}
\expandafter\def\csname v@tn/timit/mix5/ts/sub-o500\endcsname{6.10}
\expandafter\def\csname v@tn/timit/mix5/ts/sub-w20\endcsname{58.8}
\expandafter\def\csname v@tn/timit/mix5/ts/w20\endcsname{87.5}
\expandafter\def\csname v@tn/timit/mix5/turbofin/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/mix5/turbofin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/turbofin/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix5/turbofin/clean-w20\endcsname{88.5}
\expandafter\def\csname v@tn/timit/mix5/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/mix5/turbofin/mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/mix5/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/mix5/turbofin/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/mix5/turbofin/sub-mae\endcsname{101.1}
\expandafter\def\csname v@tn/timit/mix5/turbofin/sub-median\endcsname{8.7}
\expandafter\def\csname v@tn/timit/mix5/turbofin/sub-o500\endcsname{6.71}
\expandafter\def\csname v@tn/timit/mix5/turbofin/sub-w20\endcsname{64.3}
\expandafter\def\csname v@tn/timit/mix5/turbofin/w20\endcsname{88.4}
\expandafter\def\csname v@tn/timit/of\endcsname{1{,}344}
\expandafter\def\csname v@tn/timit/sub10/ctcm/clean-mae\endcsname{17.2}
\expandafter\def\csname v@tn/timit/sub10/ctcm/clean-median\endcsname{9.7}
\expandafter\def\csname v@tn/timit/sub10/ctcm/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/ctcm/clean-w20\endcsname{73.8}
\expandafter\def\csname v@tn/timit/sub10/ctcm/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/ctcm/mae\endcsname{18.9}
\expandafter\def\csname v@tn/timit/sub10/ctcm/median\endcsname{10.2}
\expandafter\def\csname v@tn/timit/sub10/ctcm/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/ctcm/sub-mae\endcsname{45.7}
\expandafter\def\csname v@tn/timit/sub10/ctcm/sub-median\endcsname{15.3}
\expandafter\def\csname v@tn/timit/sub10/ctcm/sub-o500\endcsname{0.25}
\expandafter\def\csname v@tn/timit/sub10/ctcm/sub-w20\endcsname{56.6}
\expandafter\def\csname v@tn/timit/sub10/ctcm/w20\endcsname{71.9}
\expandafter\def\csname v@tn/timit/sub10/ctcw/clean-mae\endcsname{16.4}
\expandafter\def\csname v@tn/timit/sub10/ctcw/clean-median\endcsname{9.1}
\expandafter\def\csname v@tn/timit/sub10/ctcw/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/ctcw/clean-w20\endcsname{76.0}
\expandafter\def\csname v@tn/timit/sub10/ctcw/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/ctcw/mae\endcsname{18.7}
\expandafter\def\csname v@tn/timit/sub10/ctcw/median\endcsname{9.6}
\expandafter\def\csname v@tn/timit/sub10/ctcw/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/ctcw/sub-mae\endcsname{54.9}
\expandafter\def\csname v@tn/timit/sub10/ctcw/sub-median\endcsname{17.8}
\expandafter\def\csname v@tn/timit/sub10/ctcw/sub-o500\endcsname{0.61}
\expandafter\def\csname v@tn/timit/sub10/ctcw/sub-w20\endcsname{52.3}
\expandafter\def\csname v@tn/timit/sub10/ctcw/w20\endcsname{73.9}
\expandafter\def\csname v@tn/timit/sub10/mfa/clean-mae\endcsname{19.2}
\expandafter\def\csname v@tn/timit/sub10/mfa/clean-median\endcsname{12.1}
\expandafter\def\csname v@tn/timit/sub10/mfa/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/mfa/clean-w20\endcsname{68.1}
\expandafter\def\csname v@tn/timit/sub10/mfa/failed\endcsname{5}
\expandafter\def\csname v@tn/timit/sub10/mfa/mae\endcsname{32.2}
\expandafter\def\csname v@tn/timit/sub10/mfa/median\endcsname{12.5}
\expandafter\def\csname v@tn/timit/sub10/mfa/o500\endcsname{0.72}
\expandafter\def\csname v@tn/timit/sub10/mfa/sub-mae\endcsname{102.3}
\expandafter\def\csname v@tn/timit/sub10/mfa/sub-median\endcsname{47.5}
\expandafter\def\csname v@tn/timit/sub10/mfa/sub-o500\endcsname{3.01}
\expandafter\def\csname v@tn/timit/sub10/mfa/sub-w20\endcsname{29.2}
\expandafter\def\csname v@tn/timit/sub10/mfa/w20\endcsname{63.4}
\expandafter\def\csname v@tn/timit/sub10/post/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/sub10/post/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/sub10/post/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/post/clean-w20\endcsname{89.1}
\expandafter\def\csname v@tn/timit/sub10/post/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/post/mae\endcsname{14.5}
\expandafter\def\csname v@tn/timit/sub10/post/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/sub10/post/o500\endcsname{0.31}
\expandafter\def\csname v@tn/timit/sub10/post/sub-mae\endcsname{133.3}
\expandafter\def\csname v@tn/timit/sub10/post/sub-median\endcsname{19.5}
\expandafter\def\csname v@tn/timit/sub10/post/sub-o500\endcsname{6.78}
\expandafter\def\csname v@tn/timit/sub10/post/sub-w20\endcsname{50.4}
\expandafter\def\csname v@tn/timit/sub10/post/w20\endcsname{87.7}
\expandafter\def\csname v@tn/timit/sub10/posttn/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/sub10/posttn/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/sub10/posttn/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/posttn/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/sub10/posttn/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/posttn/mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/sub10/posttn/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/sub10/posttn/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/posttn/sub-mae\endcsname{109.6}
\expandafter\def\csname v@tn/timit/sub10/posttn/sub-median\endcsname{10.6}
\expandafter\def\csname v@tn/timit/sub10/posttn/sub-o500\endcsname{5.40}
\expandafter\def\csname v@tn/timit/sub10/posttn/sub-w20\endcsname{60.3}
\expandafter\def\csname v@tn/timit/sub10/posttn/w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/sub10/rel/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/sub10/rel/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/sub10/rel/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/rel/clean-w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/sub10/rel/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/rel/mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/sub10/rel/median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/sub10/rel/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/rel/sub-mae\endcsname{108.0}
\expandafter\def\csname v@tn/timit/sub10/rel/sub-median\endcsname{9.5}
\expandafter\def\csname v@tn/timit/sub10/rel/sub-o500\endcsname{5.96}
\expandafter\def\csname v@tn/timit/sub10/rel/sub-w20\endcsname{62.6}
\expandafter\def\csname v@tn/timit/sub10/rel/w20\endcsname{89.0}
\expandafter\def\csname v@tn/timit/sub10/s6fin/clean-mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/sub10/s6fin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/sub10/s6fin/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/s6fin/clean-w20\endcsname{88.7}
\expandafter\def\csname v@tn/timit/sub10/s6fin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/s6fin/mae\endcsname{10.8}
\expandafter\def\csname v@tn/timit/sub10/s6fin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/sub10/s6fin/o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/s6fin/sub-mae\endcsname{103.0}
\expandafter\def\csname v@tn/timit/sub10/s6fin/sub-median\endcsname{9.3}
\expandafter\def\csname v@tn/timit/sub10/s6fin/sub-o500\endcsname{5.45}
\expandafter\def\csname v@tn/timit/sub10/s6fin/sub-w20\endcsname{63.0}
\expandafter\def\csname v@tn/timit/sub10/s6fin/w20\endcsname{88.6}
\expandafter\def\csname v@tn/timit/sub10/tn10/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/sub10/tn10/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/sub10/tn10/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/tn10/clean-w20\endcsname{88.9}
\expandafter\def\csname v@tn/timit/sub10/tn10/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/tn10/mae\endcsname{17.9}
\expandafter\def\csname v@tn/timit/sub10/tn10/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/sub10/tn10/o500\endcsname{0.41}
\expandafter\def\csname v@tn/timit/sub10/tn10/sub-mae\endcsname{110.3}
\expandafter\def\csname v@tn/timit/sub10/tn10/sub-median\endcsname{9.9}
\expandafter\def\csname v@tn/timit/sub10/tn10/sub-o500\endcsname{5.96}
\expandafter\def\csname v@tn/timit/sub10/tn10/sub-w20\endcsname{61.4}
\expandafter\def\csname v@tn/timit/sub10/tn10/w20\endcsname{86.8}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/clean-mae\endcsname{10.7}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/clean-median\endcsname{5.3}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/clean-o500\endcsname{0.01}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/mae\endcsname{17.7}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/o500\endcsname{0.36}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/sub-mae\endcsname{105.8}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/sub-median\endcsname{10.0}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/sub-o500\endcsname{5.15}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/sub-w20\endcsname{61.5}
\expandafter\def\csname v@tn/timit/sub10/tn10s1/w20\endcsname{86.7}
\expandafter\def\csname v@tn/timit/sub10/tn20/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/sub10/tn20/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/sub10/tn20/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/tn20/clean-w20\endcsname{88.8}
\expandafter\def\csname v@tn/timit/sub10/tn20/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/tn20/mae\endcsname{16.9}
\expandafter\def\csname v@tn/timit/sub10/tn20/median\endcsname{5.6}
\expandafter\def\csname v@tn/timit/sub10/tn20/o500\endcsname{0.33}
\expandafter\def\csname v@tn/timit/sub10/tn20/sub-mae\endcsname{101.7}
\expandafter\def\csname v@tn/timit/sub10/tn20/sub-median\endcsname{9.1}
\expandafter\def\csname v@tn/timit/sub10/tn20/sub-o500\endcsname{5.30}
\expandafter\def\csname v@tn/timit/sub10/tn20/sub-w20\endcsname{63.7}
\expandafter\def\csname v@tn/timit/sub10/tn20/w20\endcsname{87.1}
\expandafter\def\csname v@tn/timit/sub10/ts/clean-mae\endcsname{10.5}
\expandafter\def\csname v@tn/timit/sub10/ts/clean-median\endcsname{5.2}
\expandafter\def\csname v@tn/timit/sub10/ts/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/ts/clean-w20\endcsname{89.3}
\expandafter\def\csname v@tn/timit/sub10/ts/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/ts/mae\endcsname{19.8}
\expandafter\def\csname v@tn/timit/sub10/ts/median\endcsname{5.5}
\expandafter\def\csname v@tn/timit/sub10/ts/o500\endcsname{0.60}
\expandafter\def\csname v@tn/timit/sub10/ts/sub-mae\endcsname{115.1}
\expandafter\def\csname v@tn/timit/sub10/ts/sub-median\endcsname{13.2}
\expandafter\def\csname v@tn/timit/sub10/ts/sub-o500\endcsname{5.81}
\expandafter\def\csname v@tn/timit/sub10/ts/sub-w20\endcsname{55.7}
\expandafter\def\csname v@tn/timit/sub10/ts/w20\endcsname{86.4}
\expandafter\def\csname v@tn/timit/sub10/turbofin/clean-mae\endcsname{10.9}
\expandafter\def\csname v@tn/timit/sub10/turbofin/clean-median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/sub10/turbofin/clean-o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/turbofin/clean-w20\endcsname{88.5}
\expandafter\def\csname v@tn/timit/sub10/turbofin/failed\endcsname{0}
\expandafter\def\csname v@tn/timit/sub10/turbofin/mae\endcsname{11.0}
\expandafter\def\csname v@tn/timit/sub10/turbofin/median\endcsname{5.4}
\expandafter\def\csname v@tn/timit/sub10/turbofin/o500\endcsname{0.02}
\expandafter\def\csname v@tn/timit/sub10/turbofin/sub-mae\endcsname{109.1}
\expandafter\def\csname v@tn/timit/sub10/turbofin/sub-median\endcsname{9.9}
\expandafter\def\csname v@tn/timit/sub10/turbofin/sub-o500\endcsname{6.22}
\expandafter\def\csname v@tn/timit/sub10/turbofin/sub-w20\endcsname{62.1}
\expandafter\def\csname v@tn/timit/sub10/turbofin/w20\endcsname{88.4}
\expandafter\def\csname v@tn/timit/utt\endcsname{1{,}259}
\expandafter\def\csname v@tr/buckeye/bar/mae\endcsname{21.5}
\expandafter\def\csname v@tr/buckeye/bar/median\endcsname{10.7}
\expandafter\def\csname v@tr/buckeye/bar/w20\endcsname{70.7}
\expandafter\def\csname v@tr/buckeye/cut\endcsname{0}
\expandafter\def\csname v@tr/buckeye/diff-mae\endcsname{0.0}
\expandafter\def\csname v@tr/buckeye/diff-w20\endcsname{0.6}
\expandafter\def\csname v@tr/buckeye/en/mae\endcsname{12.1}
\expandafter\def\csname v@tr/buckeye/en/median\endcsname{6.2}
\expandafter\def\csname v@tr/buckeye/en/w20\endcsname{85.2}
\expandafter\def\csname v@tr/buckeye/multi/mae\endcsname{12.1}
\expandafter\def\csname v@tr/buckeye/multi/median\endcsname{6.1}
\expandafter\def\csname v@tr/buckeye/multi/w20\endcsname{85.8}
\expandafter\def\csname v@tr/buckeye/untrained/mae\endcsname{36.8}
\expandafter\def\csname v@tr/buckeye/untrained/median\endcsname{25.2}
\expandafter\def\csname v@tr/buckeye/untrained/w20\endcsname{40.1}
\expandafter\def\csname v@tr/closes/ifa/mae\endcsname{96}
\expandafter\def\csname v@tr/closes/ifa/w20\endcsname{87}
\expandafter\def\csname v@tr/closes/seoul/mae\endcsname{83}
\expandafter\def\csname v@tr/closes/seoul/w20\endcsname{79}
\expandafter\def\csname v@tr/closes/vox/mae\endcsname{86}
\expandafter\def\csname v@tr/closes/vox/w20\endcsname{75}
\expandafter\def\csname v@tr/cov/covered/en\endcsname{22.4}
\expandafter\def\csname v@tr/cov/covered/gap\endcsname{8.1}
\expandafter\def\csname v@tr/cov/covered/multi\endcsname{14.3}
\expandafter\def\csname v@tr/cov/covered/n\endcsname{32}
\expandafter\def\csname v@tr/cov/diff\endcsname{8.1}
\expandafter\def\csname v@tr/cov/diff-hi\endcsname{12.9}
\expandafter\def\csname v@tr/cov/diff-lo\endcsname{2.9}
\expandafter\def\csname v@tr/cov/macro\endcsname{10.0}
\expandafter\def\csname v@tr/cov/macro-hi\endcsname{16.5}
\expandafter\def\csname v@tr/cov/macro-lo\endcsname{3.8}
\expandafter\def\csname v@tr/cov/not-covered/en\endcsname{33.4}
\expandafter\def\csname v@tr/cov/not-covered/gap\endcsname{16.1}
\expandafter\def\csname v@tr/cov/not-covered/multi\endcsname{17.3}
\expandafter\def\csname v@tr/cov/not-covered/n\endcsname{58}
\expandafter\def\csname v@tr/cov/w20-behind\endcsname{5.2}
\expandafter\def\csname v@tr/cov/w20-behind-hi\endcsname{$+10.2$}
\expandafter\def\csname v@tr/cov/w20-behind-lo\endcsname{$-0.9$}
\expandafter\def\csname v@tr/cut-max\endcsname{53}
\expandafter\def\csname v@tr/cut-min\endcsname{31}
\expandafter\def\csname v@tr/en-beats\endcsname{15}
\expandafter\def\csname v@tr/en-n-bar\endcsname{16}
\expandafter\def\csname v@tr/english-max-diff\endcsname{0.3}
\expandafter\def\csname v@tr/ifa/bar/mae\endcsname{335.4}
\expandafter\def\csname v@tr/ifa/bar/median\endcsname{28.3}
\expandafter\def\csname v@tr/ifa/bar/w20\endcsname{38.1}
\expandafter\def\csname v@tr/ifa/cut\endcsname{31}
\expandafter\def\csname v@tr/ifa/diff-mae\endcsname{6.9}
\expandafter\def\csname v@tr/ifa/diff-w20\endcsname{6.7}
\expandafter\def\csname v@tr/ifa/en-nolang/mae\endcsname{26.1}
\expandafter\def\csname v@tr/ifa/en-nolang/median\endcsname{10.6}
\expandafter\def\csname v@tr/ifa/en-nolang/w20\endcsname{71.5}
\expandafter\def\csname v@tr/ifa/en/mae\endcsname{22.2}
\expandafter\def\csname v@tr/ifa/en/median\endcsname{10.5}
\expandafter\def\csname v@tr/ifa/en/w20\endcsname{71.7}
\expandafter\def\csname v@tr/ifa/multi-nolang/mae\endcsname{15.5}
\expandafter\def\csname v@tr/ifa/multi-nolang/median\endcsname{8.6}
\expandafter\def\csname v@tr/ifa/multi-nolang/w20\endcsname{78.5}
\expandafter\def\csname v@tr/ifa/multi/mae\endcsname{15.3}
\expandafter\def\csname v@tr/ifa/multi/median\endcsname{8.6}
\expandafter\def\csname v@tr/ifa/multi/w20\endcsname{78.4}
\expandafter\def\csname v@tr/ifa/untrained/mae\endcsname{167.3}
\expandafter\def\csname v@tr/ifa/untrained/median\endcsname{51.0}
\expandafter\def\csname v@tr/ifa/untrained/w20\endcsname{27.7}
\expandafter\def\csname v@tr/long/bar/mae\endcsname{19.5}
\expandafter\def\csname v@tr/long/bar/median\endcsname{11.6}
\expandafter\def\csname v@tr/long/bar/w20\endcsname{68.1}
\expandafter\def\csname v@tr/long/cut\endcsname{1}
\expandafter\def\csname v@tr/long/diff-mae\endcsname{0.1}
\expandafter\def\csname v@tr/long/diff-w20\endcsname{0.3}
\expandafter\def\csname v@tr/long/en/mae\endcsname{10.4}
\expandafter\def\csname v@tr/long/en/median\endcsname{5.3}
\expandafter\def\csname v@tr/long/en/w20\endcsname{89.2}
\expandafter\def\csname v@tr/long/multi/mae\endcsname{10.3}
\expandafter\def\csname v@tr/long/multi/median\endcsname{5.2}
\expandafter\def\csname v@tr/long/multi/w20\endcsname{89.5}
\expandafter\def\csname v@tr/long/untrained/mae\endcsname{50.4}
\expandafter\def\csname v@tr/long/untrained/median\endcsname{26.8}
\expandafter\def\csname v@tr/long/untrained/w20\endcsname{39.2}
\expandafter\def\csname v@tr/matched/ifa/speakers\endcsname{1}
\expandafter\def\csname v@tr/matched/ifa/utterances\endcsname{333}
\expandafter\def\csname v@tr/matched/seoul/speakers\endcsname{4}
\expandafter\def\csname v@tr/matched/seoul/utterances\endcsname{1{,}294}
\expandafter\def\csname v@tr/matched/vox/speakers\endcsname{26}
\expandafter\def\csname v@tr/matched/vox/utterances\endcsname{439}
\expandafter\def\csname v@tr/nolang-max\endcsname{0.6}
\expandafter\def\csname v@tr/seen/diff\endcsname{$-1.7$}
\expandafter\def\csname v@tr/seen/diff-hi\endcsname{$+4.1$}
\expandafter\def\csname v@tr/seen/diff-lo\endcsname{$-8.1$}
\expandafter\def\csname v@tr/seen/macro\endcsname{$-0.6$}
\expandafter\def\csname v@tr/seen/macro-hi\endcsname{$+7.4$}
\expandafter\def\csname v@tr/seen/macro-lo\endcsname{$-10.3$}
\expandafter\def\csname v@tr/seen/seen/en\endcsname{25.7}
\expandafter\def\csname v@tr/seen/seen/gap\endcsname{11.4}
\expandafter\def\csname v@tr/seen/seen/multi\endcsname{14.3}
\expandafter\def\csname v@tr/seen/seen/n\endcsname{80}
\expandafter\def\csname v@tr/seen/unseen/en\endcsname{30.3}
\expandafter\def\csname v@tr/seen/unseen/gap\endcsname{13.1}
\expandafter\def\csname v@tr/seen/unseen/multi\endcsname{17.2}
\expandafter\def\csname v@tr/seen/unseen/n\endcsname{10}
\expandafter\def\csname v@tr/seen/w20-behind\endcsname{0.6}
\expandafter\def\csname v@tr/seen/w20-behind-hi\endcsname{$+6.4$}
\expandafter\def\csname v@tr/seen/w20-behind-lo\endcsname{$-5.7$}
\expandafter\def\csname v@tr/seoul/bar/mae\endcsname{21.3}
\expandafter\def\csname v@tr/seoul/bar/median\endcsname{10.9}
\expandafter\def\csname v@tr/seoul/bar/w20\endcsname{70.2}
\expandafter\def\csname v@tr/seoul/cut\endcsname{53}
\expandafter\def\csname v@tr/seoul/diff-mae\endcsname{12.9}
\expandafter\def\csname v@tr/seoul/diff-w20\endcsname{11.0}
\expandafter\def\csname v@tr/seoul/en-nolang/mae\endcsname{24.8}
\expandafter\def\csname v@tr/seoul/en-nolang/median\endcsname{8.1}
\expandafter\def\csname v@tr/seoul/en-nolang/w20\endcsname{79.2}
\expandafter\def\csname v@tr/seoul/en/mae\endcsname{24.2}
\expandafter\def\csname v@tr/seoul/en/median\endcsname{8.2}
\expandafter\def\csname v@tr/seoul/en/w20\endcsname{79.1}
\expandafter\def\csname v@tr/seoul/multi-nolang/mae\endcsname{11.2}
\expandafter\def\csname v@tr/seoul/multi-nolang/median\endcsname{5.3}
\expandafter\def\csname v@tr/seoul/multi-nolang/w20\endcsname{90.0}
\expandafter\def\csname v@tr/seoul/multi/mae\endcsname{11.3}
\expandafter\def\csname v@tr/seoul/multi/median\endcsname{5.3}
\expandafter\def\csname v@tr/seoul/multi/w20\endcsname{90.0}
\expandafter\def\csname v@tr/seoul/untrained/mae\endcsname{87.2}
\expandafter\def\csname v@tr/seoul/untrained/median\endcsname{28.2}
\expandafter\def\csname v@tr/seoul/untrained/w20\endcsname{37.8}
\expandafter\def\csname v@tr/swb/bar/mae\endcsname{36.5}
\expandafter\def\csname v@tr/swb/bar/median\endcsname{11.6}
\expandafter\def\csname v@tr/swb/bar/w20\endcsname{64.2}
\expandafter\def\csname v@tr/swb/cut\endcsname{15}
\expandafter\def\csname v@tr/swb/diff-mae\endcsname{4.1}
\expandafter\def\csname v@tr/swb/diff-w20\endcsname{2.2}
\expandafter\def\csname v@tr/swb/en/mae\endcsname{27.1}
\expandafter\def\csname v@tr/swb/en/median\endcsname{7.8}
\expandafter\def\csname v@tr/swb/en/w20\endcsname{78.5}
\expandafter\def\csname v@tr/swb/multi/mae\endcsname{23.0}
\expandafter\def\csname v@tr/swb/multi/median\endcsname{7.5}
\expandafter\def\csname v@tr/swb/multi/w20\endcsname{80.7}
\expandafter\def\csname v@tr/swb/untrained/mae\endcsname{54.6}
\expandafter\def\csname v@tr/swb/untrained/median\endcsname{26.1}
\expandafter\def\csname v@tr/swb/untrained/w20\endcsname{39.4}
\expandafter\def\csname v@tr/timit-g711u/bar/mae\endcsname{25.3}
\expandafter\def\csname v@tr/timit-g711u/bar/median\endcsname{12.5}
\expandafter\def\csname v@tr/timit-g711u/bar/w20\endcsname{63.1}
\expandafter\def\csname v@tr/timit-g711u/cut\endcsname{3}
\expandafter\def\csname v@tr/timit-g711u/diff-mae\endcsname{0.3}
\expandafter\def\csname v@tr/timit-g711u/diff-w20\endcsname{0.1}
\expandafter\def\csname v@tr/timit-g711u/en/mae\endcsname{11.1}
\expandafter\def\csname v@tr/timit-g711u/en/median\endcsname{5.5}
\expandafter\def\csname v@tr/timit-g711u/en/w20\endcsname{88.3}
\expandafter\def\csname v@tr/timit-g711u/multi/mae\endcsname{10.8}
\expandafter\def\csname v@tr/timit-g711u/multi/median\endcsname{5.4}
\expandafter\def\csname v@tr/timit-g711u/multi/w20\endcsname{88.4}
\expandafter\def\csname v@tr/timit-g711u/untrained/mae\endcsname{41.6}
\expandafter\def\csname v@tr/timit-g711u/untrained/median\endcsname{25.5}
\expandafter\def\csname v@tr/timit-g711u/untrained/w20\endcsname{40.9}
\expandafter\def\csname v@tr/timit/bar/mae\endcsname{19.1}
\expandafter\def\csname v@tr/timit/bar/median\endcsname{12.0}
\expandafter\def\csname v@tr/timit/bar/w20\endcsname{68.2}
\expandafter\def\csname v@tr/timit/cut\endcsname{3}
\expandafter\def\csname v@tr/timit/diff-mae\endcsname{0.3}
\expandafter\def\csname v@tr/timit/diff-w20\endcsname{0.1}
\expandafter\def\csname v@tr/timit/en/mae\endcsname{10.8}
\expandafter\def\csname v@tr/timit/en/median\endcsname{5.3}
\expandafter\def\csname v@tr/timit/en/w20\endcsname{89.0}
\expandafter\def\csname v@tr/timit/multi/mae\endcsname{10.5}
\expandafter\def\csname v@tr/timit/multi/median\endcsname{5.2}
\expandafter\def\csname v@tr/timit/multi/w20\endcsname{89.1}
\expandafter\def\csname v@tr/timit/untrained/mae\endcsname{41.2}
\expandafter\def\csname v@tr/timit/untrained/median\endcsname{25.3}
\expandafter\def\csname v@tr/timit/untrained/w20\endcsname{41.5}
\expandafter\def\csname v@tr/tok/diff\endcsname{7.1}
\expandafter\def\csname v@tr/tok/diff-hi\endcsname{11.8}
\expandafter\def\csname v@tr/tok/diff-lo\endcsname{1.9}
\expandafter\def\csname v@tr/tok/macro\endcsname{8.8}
\expandafter\def\csname v@tr/tok/macro-hi\endcsname{15.6}
\expandafter\def\csname v@tr/tok/macro-lo\endcsname{2.8}
\expandafter\def\csname v@tr/tok/no-token/en\endcsname{32.8}
\expandafter\def\csname v@tr/tok/no-token/gap\endcsname{15.4}
\expandafter\def\csname v@tr/tok/no-token/multi\endcsname{17.4}
\expandafter\def\csname v@tr/tok/no-token/n\endcsname{64}
\expandafter\def\csname v@tr/tok/token/en\endcsname{22.0}
\expandafter\def\csname v@tr/tok/token/gap\endcsname{8.3}
\expandafter\def\csname v@tr/tok/token/multi\endcsname{13.8}
\expandafter\def\csname v@tr/tok/token/n\endcsname{26}
\expandafter\def\csname v@tr/tok/w20-behind\endcsname{3.9}
\expandafter\def\csname v@tr/tok/w20-behind-hi\endcsname{$+9.5$}
\expandafter\def\csname v@tr/tok/w20-behind-lo\endcsname{$-2.3$}
\expandafter\def\csname v@tr/vox-seen/cut\endcsname{45}
\expandafter\def\csname v@tr/vox-seen/diff-mae\endcsname{11.4}
\expandafter\def\csname v@tr/vox-seen/diff-w20\endcsname{18.9}
\expandafter\def\csname v@tr/vox-seen/en-nolang/mae\endcsname{26.2}
\expandafter\def\csname v@tr/vox-seen/en-nolang/median\endcsname{13.7}
\expandafter\def\csname v@tr/vox-seen/en-nolang/w20\endcsname{62.7}
\expandafter\def\csname v@tr/vox-seen/en/mae\endcsname{25.7}
\expandafter\def\csname v@tr/vox-seen/en/median\endcsname{13.3}
\expandafter\def\csname v@tr/vox-seen/en/w20\endcsname{63.1}
\expandafter\def\csname v@tr/vox-seen/multi-nolang/mae\endcsname{14.4}
\expandafter\def\csname v@tr/vox-seen/multi-nolang/median\endcsname{7.7}
\expandafter\def\csname v@tr/vox-seen/multi-nolang/w20\endcsname{81.3}
\expandafter\def\csname v@tr/vox-seen/multi/mae\endcsname{14.3}
\expandafter\def\csname v@tr/vox-seen/multi/median\endcsname{7.7}
\expandafter\def\csname v@tr/vox-seen/multi/w20\endcsname{82.0}
\expandafter\def\csname v@tr/vox-seen/untrained/mae\endcsname{75.6}
\expandafter\def\csname v@tr/vox-seen/untrained/median\endcsname{66.4}
\expandafter\def\csname v@tr/vox-seen/untrained/w20\endcsname{19.1}
\expandafter\def\csname v@tr/vox-unseen/cut\endcsname{43}
\expandafter\def\csname v@tr/vox-unseen/diff-mae\endcsname{13.1}
\expandafter\def\csname v@tr/vox-unseen/diff-w20\endcsname{18.3}
\expandafter\def\csname v@tr/vox-unseen/en-nolang/mae\endcsname{30.1}
\expandafter\def\csname v@tr/vox-unseen/en-nolang/median\endcsname{13.5}
\expandafter\def\csname v@tr/vox-unseen/en-nolang/w20\endcsname{60.8}
\expandafter\def\csname v@tr/vox-unseen/en/mae\endcsname{30.3}
\expandafter\def\csname v@tr/vox-unseen/en/median\endcsname{13.5}
\expandafter\def\csname v@tr/vox-unseen/en/w20\endcsname{60.6}
\expandafter\def\csname v@tr/vox-unseen/multi-nolang/mae\endcsname{17.0}
\expandafter\def\csname v@tr/vox-unseen/multi-nolang/median\endcsname{7.7}
\expandafter\def\csname v@tr/vox-unseen/multi-nolang/w20\endcsname{78.9}
\expandafter\def\csname v@tr/vox-unseen/multi/mae\endcsname{17.2}
\expandafter\def\csname v@tr/vox-unseen/multi/median\endcsname{7.7}
\expandafter\def\csname v@tr/vox-unseen/multi/w20\endcsname{78.9}
\expandafter\def\csname v@tr/vox-unseen/untrained/mae\endcsname{69.9}
\expandafter\def\csname v@tr/vox-unseen/untrained/median\endcsname{64.1}
\expandafter\def\csname v@tr/vox-unseen/untrained/w20\endcsname{18.4}
\expandafter\def\csname v@tr/vox/better-mae\endcsname{81}
\expandafter\def\csname v@tr/vox/better-w20\endcsname{72}
\expandafter\def\csname v@tr/vox/cut\endcsname{44}
\expandafter\def\csname v@tr/vox/diff-mae\endcsname{12.4}
\expandafter\def\csname v@tr/vox/diff-w20\endcsname{18.6}
\expandafter\def\csname v@tr/vox/en-nolang/mae\endcsname{28.5}
\expandafter\def\csname v@tr/vox/en-nolang/median\endcsname{13.5}
\expandafter\def\csname v@tr/vox/en-nolang/w20\endcsname{61.6}
\expandafter\def\csname v@tr/vox/en/mae\endcsname{28.3}
\expandafter\def\csname v@tr/vox/en/median\endcsname{13.4}
\expandafter\def\csname v@tr/vox/en/w20\endcsname{61.7}
\expandafter\def\csname v@tr/vox/multi-nolang/mae\endcsname{15.9}
\expandafter\def\csname v@tr/vox/multi-nolang/median\endcsname{7.7}
\expandafter\def\csname v@tr/vox/multi-nolang/w20\endcsname{80.0}
\expandafter\def\csname v@tr/vox/multi/mae\endcsname{15.9}
\expandafter\def\csname v@tr/vox/multi/median\endcsname{7.7}
\expandafter\def\csname v@tr/vox/multi/w20\endcsname{80.2}
\expandafter\def\csname v@tr/vox/n-lang\endcsname{90}
\expandafter\def\csname v@tr/vox/untrained/mae\endcsname{72.3}
\expandafter\def\csname v@tr/vox/untrained/median\endcsname{65.0}
\expandafter\def\csname v@tr/vox/untrained/w20\endcsname{18.7}
\expandafter\def\csname v@trl/better-mae\endcsname{81}
\expandafter\def\csname v@trl/better-w20\endcsname{72}
\expandafter\def\csname v@trl/big-median-dw20\endcsname{19}
\expandafter\def\csname v@trl/big-worse\endcsname{0}
\expandafter\def\csname v@trl/kor/all-w20\endcsname{90}
\expandafter\def\csname v@trl/kor/en-w20\endcsname{79}
\expandafter\def\csname v@trl/median-bounds\endcsname{11}
\expandafter\def\csname v@trl/median-dw20\endcsname{17}
\expandafter\def\csname v@trl/n-big\endcsname{10}
\expandafter\def\csname v@trl/n-small\endcsname{17}
\expandafter\def\csname v@trl/n-under10\endcsname{34}
\expandafter\def\csname v@trl/n-vox\endcsname{90}
\expandafter\def\csname v@trl/nld/all-w20\endcsname{78}
\expandafter\def\csname v@trl/nld/en-w20\endcsname{72}
\expandafter\def\csname v@trl/same-w20\endcsname{18}
\expandafter\def\csname v@trl/worse-w20\endcsname{0}
\expandafter\def\csname v@vox/ft-ctcm-full/clean/mae\endcsname{20.7}
\expandafter\def\csname v@vox/ft-ctcm-full/clean/median\endcsname{12.9}
\expandafter\def\csname v@vox/ft-ctcm-full/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ctcm-full/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ctcm-full/clean/w20\endcsname{66.9}
\expandafter\def\csname v@vox/ft-ctcm-full/clean/w50\endcsname{91.4}
\expandafter\def\csname v@vox/ft-ctcm-lora/clean/mae\endcsname{20.3}
\expandafter\def\csname v@vox/ft-ctcm-lora/clean/median\endcsname{12.9}
\expandafter\def\csname v@vox/ft-ctcm-lora/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ctcm-lora/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ctcm-lora/clean/w20\endcsname{67.4}
\expandafter\def\csname v@vox/ft-ctcm-lora/clean/w50\endcsname{92.5}
\expandafter\def\csname v@vox/ft-ctcw-full/clean/mae\endcsname{18.5}
\expandafter\def\csname v@vox/ft-ctcw-full/clean/median\endcsname{11.0}
\expandafter\def\csname v@vox/ft-ctcw-full/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ctcw-full/clean/w100\endcsname{97.5}
\expandafter\def\csname v@vox/ft-ctcw-full/clean/w20\endcsname{73.5}
\expandafter\def\csname v@vox/ft-ctcw-full/clean/w50\endcsname{93.2}
\expandafter\def\csname v@vox/ft-ctcw-lora/clean/mae\endcsname{18.8}
\expandafter\def\csname v@vox/ft-ctcw-lora/clean/median\endcsname{11.3}
\expandafter\def\csname v@vox/ft-ctcw-lora/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ctcw-lora/clean/w100\endcsname{97.3}
\expandafter\def\csname v@vox/ft-ctcw-lora/clean/w20\endcsname{73.1}
\expandafter\def\csname v@vox/ft-ctcw-lora/clean/w50\endcsname{92.8}
\expandafter\def\csname v@vox/ft-ts-1k-s1/clean/mae\endcsname{16.7}
\expandafter\def\csname v@vox/ft-ts-1k-s1/clean/median\endcsname{8.3}
\expandafter\def\csname v@vox/ft-ts-1k-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-1k-s1/clean/w100\endcsname{97.6}
\expandafter\def\csname v@vox/ft-ts-1k-s1/clean/w20\endcsname{78.3}
\expandafter\def\csname v@vox/ft-ts-1k-s1/clean/w50\endcsname{93.0}
\expandafter\def\csname v@vox/ft-ts-1k/clean/mae\endcsname{15.9}
\expandafter\def\csname v@vox/ft-ts-1k/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-1k/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-1k/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-1k/clean/w20\endcsname{80.0}
\expandafter\def\csname v@vox/ft-ts-1k/clean/w50\endcsname{93.6}
\expandafter\def\csname v@vox/ft-ts-4k/clean/mae\endcsname{15.6}
\expandafter\def\csname v@vox/ft-ts-4k/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-4k/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-4k/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-4k/clean/w20\endcsname{79.5}
\expandafter\def\csname v@vox/ft-ts-4k/clean/w50\endcsname{93.7}
\expandafter\def\csname v@vox/ft-ts-6k/clean/mae\endcsname{15.6}
\expandafter\def\csname v@vox/ft-ts-6k/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-6k/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-6k/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-6k/clean/w20\endcsname{79.7}
\expandafter\def\csname v@vox/ft-ts-6k/clean/w50\endcsname{93.2}
\expandafter\def\csname v@vox/ft-ts-a02/clean/mae\endcsname{16.9}
\expandafter\def\csname v@vox/ft-ts-a02/clean/median\endcsname{8.6}
\expandafter\def\csname v@vox/ft-ts-a02/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-a02/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-a02/clean/w20\endcsname{78.3}
\expandafter\def\csname v@vox/ft-ts-a02/clean/w50\endcsname{92.8}
\expandafter\def\csname v@vox/ft-ts-attn/clean/mae\endcsname{16.2}
\expandafter\def\csname v@vox/ft-ts-attn/clean/median\endcsname{8.2}
\expandafter\def\csname v@vox/ft-ts-attn/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-attn/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-attn/clean/w20\endcsname{79.2}
\expandafter\def\csname v@vox/ft-ts-attn/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-aug0-s1/clean/mae\endcsname{15.3}
\expandafter\def\csname v@vox/ft-ts-aug0-s1/clean/median\endcsname{7.2}
\expandafter\def\csname v@vox/ft-ts-aug0-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug0-s1/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-aug0-s1/clean/w20\endcsname{80.6}
\expandafter\def\csname v@vox/ft-ts-aug0-s1/clean/w50\endcsname{94.1}
\expandafter\def\csname v@vox/ft-ts-aug0-s2/clean/mae\endcsname{15.3}
\expandafter\def\csname v@vox/ft-ts-aug0-s2/clean/median\endcsname{7.3}
\expandafter\def\csname v@vox/ft-ts-aug0-s2/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug0-s2/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-aug0-s2/clean/w20\endcsname{80.9}
\expandafter\def\csname v@vox/ft-ts-aug0-s2/clean/w50\endcsname{93.7}
\expandafter\def\csname v@vox/ft-ts-aug0/clean/mae\endcsname{15.0}
\expandafter\def\csname v@vox/ft-ts-aug0/clean/median\endcsname{7.3}
\expandafter\def\csname v@vox/ft-ts-aug0/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug0/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-aug0/clean/w20\endcsname{80.5}
\expandafter\def\csname v@vox/ft-ts-aug0/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-aug100/clean/mae\endcsname{16.7}
\expandafter\def\csname v@vox/ft-ts-aug100/clean/median\endcsname{8.9}
\expandafter\def\csname v@vox/ft-ts-aug100/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug100/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-aug100/clean/w20\endcsname{79.0}
\expandafter\def\csname v@vox/ft-ts-aug100/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-aug25-s1/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-aug25-s1/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-aug25-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug25-s1/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-aug25-s1/clean/w20\endcsname{81.0}
\expandafter\def\csname v@vox/ft-ts-aug25-s1/clean/w50\endcsname{94.0}
\expandafter\def\csname v@vox/ft-ts-aug25-s2/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-aug25-s2/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-aug25-s2/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug25-s2/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-aug25-s2/clean/w20\endcsname{80.6}
\expandafter\def\csname v@vox/ft-ts-aug25-s2/clean/w50\endcsname{93.6}
\expandafter\def\csname v@vox/ft-ts-aug25/clean/mae\endcsname{15.6}
\expandafter\def\csname v@vox/ft-ts-aug25/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-aug25/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug25/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-aug25/clean/w20\endcsname{80.4}
\expandafter\def\csname v@vox/ft-ts-aug25/clean/w50\endcsname{93.5}
\expandafter\def\csname v@vox/ft-ts-aug75/clean/mae\endcsname{16.4}
\expandafter\def\csname v@vox/ft-ts-aug75/clean/median\endcsname{8.1}
\expandafter\def\csname v@vox/ft-ts-aug75/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-aug75/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-aug75/clean/w20\endcsname{78.7}
\expandafter\def\csname v@vox/ft-ts-aug75/clean/w50\endcsname{93.2}
\expandafter\def\csname v@vox/ft-ts-augamr-s1/clean/mae\endcsname{15.6}
\expandafter\def\csname v@vox/ft-ts-augamr-s1/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-augamr-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-augamr-s1/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-augamr-s1/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-augamr-s1/clean/w50\endcsname{93.7}
\expandafter\def\csname v@vox/ft-ts-augamr/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-augamr/clean/median\endcsname{7.3}
\expandafter\def\csname v@vox/ft-ts-augamr/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-augamr/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-augamr/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-augamr/clean/w50\endcsname{93.4}
\expandafter\def\csname v@vox/ft-ts-auxw-s1/clean/mae\endcsname{15.6}
\expandafter\def\csname v@vox/ft-ts-auxw-s1/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-auxw-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-auxw-s1/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-auxw-s1/clean/w20\endcsname{79.7}
\expandafter\def\csname v@vox/ft-ts-auxw-s1/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-auxw/clean/mae\endcsname{15.9}
\expandafter\def\csname v@vox/ft-ts-auxw/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-auxw/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-auxw/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-auxw/clean/w20\endcsname{79.5}
\expandafter\def\csname v@vox/ft-ts-auxw/clean/w50\endcsname{93.0}
\expandafter\def\csname v@vox/ft-ts-auxwp-s1/clean/mae\endcsname{14.8}
\expandafter\def\csname v@vox/ft-ts-auxwp-s1/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-auxwp-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-auxwp-s1/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-auxwp-s1/clean/w20\endcsname{80.9}
\expandafter\def\csname v@vox/ft-ts-auxwp-s1/clean/w50\endcsname{94.0}
\expandafter\def\csname v@vox/ft-ts-auxwp/clean/mae\endcsname{16.2}
\expandafter\def\csname v@vox/ft-ts-auxwp/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-auxwp/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-auxwp/clean/w100\endcsname{97.6}
\expandafter\def\csname v@vox/ft-ts-auxwp/clean/w20\endcsname{79.6}
\expandafter\def\csname v@vox/ft-ts-auxwp/clean/w50\endcsname{92.8}
\expandafter\def\csname v@vox/ft-ts-dec/clean/mae\endcsname{17.6}
\expandafter\def\csname v@vox/ft-ts-dec/clean/median\endcsname{9.6}
\expandafter\def\csname v@vox/ft-ts-dec/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-dec/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-dec/clean/w20\endcsname{75.3}
\expandafter\def\csname v@vox/ft-ts-dec/clean/w50\endcsname{92.8}
\expandafter\def\csname v@vox/ft-ts-full/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-full/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-full/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-full/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-full/clean/w20\endcsname{80.5}
\expandafter\def\csname v@vox/ft-ts-full/clean/w50\endcsname{93.6}
\expandafter\def\csname v@vox/ft-ts-lora-argmax/clean/mae\endcsname{17.5}
\expandafter\def\csname v@vox/ft-ts-lora-argmax/clean/median\endcsname{9.3}
\expandafter\def\csname v@vox/ft-ts-lora-argmax/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora-argmax/clean/w100\endcsname{97.5}
\expandafter\def\csname v@vox/ft-ts-lora-argmax/clean/w20\endcsname{77.4}
\expandafter\def\csname v@vox/ft-ts-lora-argmax/clean/w50\endcsname{92.3}
\expandafter\def\csname v@vox/ft-ts-lora-en-nolang/clean/mae\endcsname{28.5}
\expandafter\def\csname v@vox/ft-ts-lora-en-nolang/clean/median\endcsname{13.5}
\expandafter\def\csname v@vox/ft-ts-lora-en-nolang/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora-en-nolang/clean/w100\endcsname{94.3}
\expandafter\def\csname v@vox/ft-ts-lora-en-nolang/clean/w20\endcsname{61.6}
\expandafter\def\csname v@vox/ft-ts-lora-en-nolang/clean/w50\endcsname{85.9}
\expandafter\def\csname v@vox/ft-ts-lora-en/clean/mae\endcsname{28.3}
\expandafter\def\csname v@vox/ft-ts-lora-en/clean/median\endcsname{13.4}
\expandafter\def\csname v@vox/ft-ts-lora-en/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora-en/clean/w100\endcsname{94.5}
\expandafter\def\csname v@vox/ft-ts-lora-en/clean/w20\endcsname{61.7}
\expandafter\def\csname v@vox/ft-ts-lora-en/clean/w50\endcsname{85.8}
\expandafter\def\csname v@vox/ft-ts-lora-full/clean/mae\endcsname{18.9}
\expandafter\def\csname v@vox/ft-ts-lora-full/clean/median\endcsname{13.3}
\expandafter\def\csname v@vox/ft-ts-lora-full/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora-full/clean/w100\endcsname{98.9}
\expandafter\def\csname v@vox/ft-ts-lora-full/clean/w20\endcsname{67.3}
\expandafter\def\csname v@vox/ft-ts-lora-full/clean/w50\endcsname{93.5}
\expandafter\def\csname v@vox/ft-ts-lora-nolang/clean/mae\endcsname{15.9}
\expandafter\def\csname v@vox/ft-ts-lora-nolang/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-lora-nolang/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora-nolang/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-lora-nolang/clean/w20\endcsname{80.0}
\expandafter\def\csname v@vox/ft-ts-lora-nolang/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-lora-r1/clean/mae\endcsname{16.2}
\expandafter\def\csname v@vox/ft-ts-lora-r1/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-lora-r1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora-r1/clean/w100\endcsname{97.5}
\expandafter\def\csname v@vox/ft-ts-lora-r1/clean/w20\endcsname{79.8}
\expandafter\def\csname v@vox/ft-ts-lora-r1/clean/w50\endcsname{92.8}
\expandafter\def\csname v@vox/ft-ts-lora-r5/clean/mae\endcsname{15.7}
\expandafter\def\csname v@vox/ft-ts-lora-r5/clean/median\endcsname{8.1}
\expandafter\def\csname v@vox/ft-ts-lora-r5/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora-r5/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-lora-r5/clean/w20\endcsname{79.0}
\expandafter\def\csname v@vox/ft-ts-lora-r5/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-lora/clean/mae\endcsname{15.9}
\expandafter\def\csname v@vox/ft-ts-lora/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-lora/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lora/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-lora/clean/w20\endcsname{80.2}
\expandafter\def\csname v@vox/ft-ts-lora/clean/w50\endcsname{93.4}
\expandafter\def\csname v@vox/ft-ts-lr1e4/clean/mae\endcsname{16.0}
\expandafter\def\csname v@vox/ft-ts-lr1e4/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-lr1e4/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lr1e4/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-lr1e4/clean/w20\endcsname{79.8}
\expandafter\def\csname v@vox/ft-ts-lr1e4/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-lr5e4/clean/mae\endcsname{15.7}
\expandafter\def\csname v@vox/ft-ts-lr5e4/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-lr5e4/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-lr5e4/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-lr5e4/clean/w20\endcsname{79.6}
\expandafter\def\csname v@vox/ft-ts-lr5e4/clean/w50\endcsname{93.6}
\expandafter\def\csname v@vox/ft-ts-post-10ms-4k/clean/mae\endcsname{14.8}
\expandafter\def\csname v@vox/ft-ts-post-10ms-4k/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-4k/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-4k/clean/w100\endcsname{98.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-4k/clean/w20\endcsname{80.9}
\expandafter\def\csname v@vox/ft-ts-post-10ms-4k/clean/w50\endcsname{94.0}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr2e4/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr2e4/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr2e4/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr2e4/clean/w100\endcsname{98.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr2e4/clean/w20\endcsname{79.8}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr2e4/clean/w50\endcsname{93.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr5e3/clean/mae\endcsname{15.7}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr5e3/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr5e3/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr5e3/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr5e3/clean/w20\endcsname{79.8}
\expandafter\def\csname v@vox/ft-ts-post-10ms-lr5e3/clean/w50\endcsname{93.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-r64/clean/mae\endcsname{15.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-r64/clean/median\endcsname{7.3}
\expandafter\def\csname v@vox/ft-ts-post-10ms-r64/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-r64/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-post-10ms-r64/clean/w20\endcsname{80.0}
\expandafter\def\csname v@vox/ft-ts-post-10ms-r64/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-post-10ms-rand/clean/mae\endcsname{15.8}
\expandafter\def\csname v@vox/ft-ts-post-10ms-rand/clean/median\endcsname{7.3}
\expandafter\def\csname v@vox/ft-ts-post-10ms-rand/clean/over500\endcsname{0.05}
\expandafter\def\csname v@vox/ft-ts-post-10ms-rand/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-post-10ms-rand/clean/w20\endcsname{79.7}
\expandafter\def\csname v@vox/ft-ts-post-10ms-rand/clean/w50\endcsname{93.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms-round/clean/mae\endcsname{15.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-round/clean/median\endcsname{7.3}
\expandafter\def\csname v@vox/ft-ts-post-10ms-round/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-round/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-round/clean/w20\endcsname{79.7}
\expandafter\def\csname v@vox/ft-ts-post-10ms-round/clean/w50\endcsname{94.0}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s1/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s1/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s1/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s1/clean/w20\endcsname{80.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s1/clean/w50\endcsname{93.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s2/clean/mae\endcsname{15.8}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s2/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s2/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s2/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s2/clean/w20\endcsname{79.3}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s2/clean/w50\endcsname{93.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s3/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s3/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s3/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s3/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s3/clean/w20\endcsname{79.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s3/clean/w50\endcsname{93.7}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s4/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s4/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s4/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s4/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s4/clean/w20\endcsname{79.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-s4/clean/w50\endcsname{94.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-tn10/clean/mae\endcsname{15.7}
\expandafter\def\csname v@vox/ft-ts-post-10ms-tn10/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-post-10ms-tn10/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms-tn10/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-post-10ms-tn10/clean/w20\endcsname{79.2}
\expandafter\def\csname v@vox/ft-ts-post-10ms-tn10/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-post-10ms/clean/mae\endcsname{15.6}
\expandafter\def\csname v@vox/ft-ts-post-10ms/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-post-10ms/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-10ms/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-post-10ms/clean/w20\endcsname{79.9}
\expandafter\def\csname v@vox/ft-ts-post-10ms/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-post-5ms/clean/mae\endcsname{16.2}
\expandafter\def\csname v@vox/ft-ts-post-5ms/clean/median\endcsname{7.2}
\expandafter\def\csname v@vox/ft-ts-post-5ms/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-5ms/clean/w100\endcsname{97.6}
\expandafter\def\csname v@vox/ft-ts-post-5ms/clean/w20\endcsname{79.6}
\expandafter\def\csname v@vox/ft-ts-post-5ms/clean/w50\endcsname{93.0}
\expandafter\def\csname v@vox/ft-ts-post-s1/clean/mae\endcsname{15.4}
\expandafter\def\csname v@vox/ft-ts-post-s1/clean/median\endcsname{8.0}
\expandafter\def\csname v@vox/ft-ts-post-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-s1/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-s1/clean/w20\endcsname{80.1}
\expandafter\def\csname v@vox/ft-ts-post-s1/clean/w50\endcsname{93.7}
\expandafter\def\csname v@vox/ft-ts-post-s2/clean/mae\endcsname{15.4}
\expandafter\def\csname v@vox/ft-ts-post-s2/clean/median\endcsname{8.0}
\expandafter\def\csname v@vox/ft-ts-post-s2/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-s2/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-s2/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-post-s2/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-post-s3/clean/mae\endcsname{15.4}
\expandafter\def\csname v@vox/ft-ts-post-s3/clean/median\endcsname{8.0}
\expandafter\def\csname v@vox/ft-ts-post-s3/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-s3/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-s3/clean/w20\endcsname{79.1}
\expandafter\def\csname v@vox/ft-ts-post-s3/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-post-s4/clean/mae\endcsname{15.4}
\expandafter\def\csname v@vox/ft-ts-post-s4/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-post-s4/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-s4/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-post-s4/clean/w20\endcsname{80.6}
\expandafter\def\csname v@vox/ft-ts-post-s4/clean/w50\endcsname{94.1}
\expandafter\def\csname v@vox/ft-ts-post-sidon-s1/clean/mae\endcsname{15.4}
\expandafter\def\csname v@vox/ft-ts-post-sidon-s1/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-post-sidon-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-sidon-s1/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-sidon-s1/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-post-sidon-s1/clean/w50\endcsname{93.4}
\expandafter\def\csname v@vox/ft-ts-post-sidon/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-post-sidon/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-post-sidon/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-sidon/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-post-sidon/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-post-sidon/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-post-tn10-s1/clean/mae\endcsname{15.0}
\expandafter\def\csname v@vox/ft-ts-post-tn10-s1/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-post-tn10-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-tn10-s1/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-post-tn10-s1/clean/w20\endcsname{80.6}
\expandafter\def\csname v@vox/ft-ts-post-tn10-s1/clean/w50\endcsname{94.0}
\expandafter\def\csname v@vox/ft-ts-post-tn10/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-post-tn10/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-post-tn10/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post-tn10/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-post-tn10/clean/w20\endcsname{80.4}
\expandafter\def\csname v@vox/ft-ts-post-tn10/clean/w50\endcsname{93.6}
\expandafter\def\csname v@vox/ft-ts-post/clean/mae\endcsname{15.3}
\expandafter\def\csname v@vox/ft-ts-post/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-post/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-post/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-post/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-post/clean/w50\endcsname{93.9}
\expandafter\def\csname v@vox/ft-ts-r128/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-r128/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-r128/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-r128/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-r128/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-r128/clean/w50\endcsname{94.0}
\expandafter\def\csname v@vox/ft-ts-r16/clean/mae\endcsname{16.0}
\expandafter\def\csname v@vox/ft-ts-r16/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-r16/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-r16/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-r16/clean/w20\endcsname{80.0}
\expandafter\def\csname v@vox/ft-ts-r16/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-r64/clean/mae\endcsname{15.3}
\expandafter\def\csname v@vox/ft-ts-r64/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-r64/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-r64/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-r64/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-r64/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-r8/clean/mae\endcsname{16.6}
\expandafter\def\csname v@vox/ft-ts-r8/clean/median\endcsname{8.1}
\expandafter\def\csname v@vox/ft-ts-r8/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-r8/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-r8/clean/w20\endcsname{79.2}
\expandafter\def\csname v@vox/ft-ts-r8/clean/w50\endcsname{92.8}
\expandafter\def\csname v@vox/ft-ts-round-s1/clean/mae\endcsname{15.7}
\expandafter\def\csname v@vox/ft-ts-round-s1/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-round-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-round-s1/clean/w100\endcsname{97.8}
\expandafter\def\csname v@vox/ft-ts-round-s1/clean/w20\endcsname{79.7}
\expandafter\def\csname v@vox/ft-ts-round-s1/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-round/clean/mae\endcsname{15.2}
\expandafter\def\csname v@vox/ft-ts-round/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-round/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-round/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-round/clean/w20\endcsname{80.2}
\expandafter\def\csname v@vox/ft-ts-round/clean/w50\endcsname{93.9}
\expandafter\def\csname v@vox/ft-ts-s6-final-s1/clean/mae\endcsname{15.9}
\expandafter\def\csname v@vox/ft-ts-s6-final-s1/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-s6-final-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-s6-final-s1/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-s6-final-s1/clean/w20\endcsname{79.7}
\expandafter\def\csname v@vox/ft-ts-s6-final-s1/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-s6-final/clean/mae\endcsname{16.8}
\expandafter\def\csname v@vox/ft-ts-s6-final/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-s6-final/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-s6-final/clean/w100\endcsname{97.3}
\expandafter\def\csname v@vox/ft-ts-s6-final/clean/w20\endcsname{79.3}
\expandafter\def\csname v@vox/ft-ts-s6-final/clean/w50\endcsname{92.4}
\expandafter\def\csname v@vox/ft-ts-s6-post-s1/clean/mae\endcsname{15.4}
\expandafter\def\csname v@vox/ft-ts-s6-post-s1/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-s6-post-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-s6-post-s1/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-s6-post-s1/clean/w20\endcsname{80.4}
\expandafter\def\csname v@vox/ft-ts-s6-post-s1/clean/w50\endcsname{93.9}
\expandafter\def\csname v@vox/ft-ts-s6-post/clean/mae\endcsname{15.2}
\expandafter\def\csname v@vox/ft-ts-s6-post/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-s6-post/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-s6-post/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-s6-post/clean/w20\endcsname{80.0}
\expandafter\def\csname v@vox/ft-ts-s6-post/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-s6-sidon-s1/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-s6-sidon-s1/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-s6-sidon-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-s6-sidon-s1/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-s6-sidon-s1/clean/w20\endcsname{80.0}
\expandafter\def\csname v@vox/ft-ts-s6-sidon-s1/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-s6-sidon/clean/mae\endcsname{15.8}
\expandafter\def\csname v@vox/ft-ts-s6-sidon/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-s6-sidon/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-s6-sidon/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-s6-sidon/clean/w20\endcsname{79.3}
\expandafter\def\csname v@vox/ft-ts-s6-sidon/clean/w50\endcsname{92.8}
\expandafter\def\csname v@vox/ft-ts-seed1/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-seed1/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-seed1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-seed1/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-seed1/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-seed1/clean/w50\endcsname{93.6}
\expandafter\def\csname v@vox/ft-ts-seed2/clean/mae\endcsname{15.3}
\expandafter\def\csname v@vox/ft-ts-seed2/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-seed2/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-seed2/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-seed2/clean/w20\endcsname{81.1}
\expandafter\def\csname v@vox/ft-ts-seed2/clean/w50\endcsname{93.9}
\expandafter\def\csname v@vox/ft-ts-seed3/clean/mae\endcsname{14.8}
\expandafter\def\csname v@vox/ft-ts-seed3/clean/median\endcsname{7.4}
\expandafter\def\csname v@vox/ft-ts-seed3/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-seed3/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-seed3/clean/w20\endcsname{80.4}
\expandafter\def\csname v@vox/ft-ts-seed3/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-seed4/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-seed4/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-seed4/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-seed4/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-seed4/clean/w20\endcsname{80.2}
\expandafter\def\csname v@vox/ft-ts-seed4/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-tn10-s1/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-tn10-s1/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-tn10-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-tn10-s1/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-tn10-s1/clean/w20\endcsname{80.7}
\expandafter\def\csname v@vox/ft-ts-tn10-s1/clean/w50\endcsname{94.2}
\expandafter\def\csname v@vox/ft-ts-tn10/clean/mae\endcsname{16.4}
\expandafter\def\csname v@vox/ft-ts-tn10/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-tn10/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-tn10/clean/w100\endcsname{97.6}
\expandafter\def\csname v@vox/ft-ts-tn10/clean/w20\endcsname{79.2}
\expandafter\def\csname v@vox/ft-ts-tn10/clean/w50\endcsname{92.6}
\expandafter\def\csname v@vox/ft-ts-tn20/clean/mae\endcsname{16.2}
\expandafter\def\csname v@vox/ft-ts-tn20/clean/median\endcsname{8.0}
\expandafter\def\csname v@vox/ft-ts-tn20/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-tn20/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-tn20/clean/w20\endcsname{79.2}
\expandafter\def\csname v@vox/ft-ts-tn20/clean/w50\endcsname{93.0}
\expandafter\def\csname v@vox/ft-ts-turbo-final-s1/clean/mae\endcsname{16.6}
\expandafter\def\csname v@vox/ft-ts-turbo-final-s1/clean/median\endcsname{8.5}
\expandafter\def\csname v@vox/ft-ts-turbo-final-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-turbo-final-s1/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-turbo-final-s1/clean/w20\endcsname{78.9}
\expandafter\def\csname v@vox/ft-ts-turbo-final-s1/clean/w50\endcsname{92.9}
\expandafter\def\csname v@vox/ft-ts-turbo-final/clean/mae\endcsname{16.3}
\expandafter\def\csname v@vox/ft-ts-turbo-final/clean/median\endcsname{8.0}
\expandafter\def\csname v@vox/ft-ts-turbo-final/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-turbo-final/clean/w100\endcsname{97.5}
\expandafter\def\csname v@vox/ft-ts-turbo-final/clean/w20\endcsname{78.6}
\expandafter\def\csname v@vox/ft-ts-turbo-final/clean/w50\endcsname{92.5}
\expandafter\def\csname v@vox/ft-ts-turbo-post-10ms/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-turbo-post-10ms/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-turbo-post-10ms/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-turbo-post-10ms/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-turbo-post-10ms/clean/w20\endcsname{79.5}
\expandafter\def\csname v@vox/ft-ts-turbo-post-10ms/clean/w50\endcsname{93.5}
\expandafter\def\csname v@vox/ft-ts-turbo-post-s1/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-turbo-post-s1/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-turbo-post-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-turbo-post-s1/clean/w100\endcsname{98.0}
\expandafter\def\csname v@vox/ft-ts-turbo-post-s1/clean/w20\endcsname{80.5}
\expandafter\def\csname v@vox/ft-ts-turbo-post-s1/clean/w50\endcsname{94.2}
\expandafter\def\csname v@vox/ft-ts-turbo-post/clean/mae\endcsname{15.6}
\expandafter\def\csname v@vox/ft-ts-turbo-post/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-turbo-post/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-turbo-post/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-turbo-post/clean/w20\endcsname{78.8}
\expandafter\def\csname v@vox/ft-ts-turbo-post/clean/w50\endcsname{93.1}
\expandafter\def\csname v@vox/ft-ts-turbo-s1/clean/mae\endcsname{15.3}
\expandafter\def\csname v@vox/ft-ts-turbo-s1/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-turbo-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-turbo-s1/clean/w100\endcsname{98.1}
\expandafter\def\csname v@vox/ft-ts-turbo-s1/clean/w20\endcsname{80.6}
\expandafter\def\csname v@vox/ft-ts-turbo-s1/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-turbo-s2/clean/mae\endcsname{16.0}
\expandafter\def\csname v@vox/ft-ts-turbo-s2/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-turbo-s2/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-turbo-s2/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-turbo-s2/clean/w20\endcsname{80.0}
\expandafter\def\csname v@vox/ft-ts-turbo-s2/clean/w50\endcsname{93.0}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10-s1/clean/mae\endcsname{15.8}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10-s1/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10-s1/clean/over500\endcsname{0.05}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10-s1/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10-s1/clean/w20\endcsname{80.2}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10-s1/clean/w50\endcsname{93.4}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10/clean/mae\endcsname{16.9}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10/clean/over500\endcsname{0.09}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10/clean/w100\endcsname{97.5}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10/clean/w20\endcsname{79.2}
\expandafter\def\csname v@vox/ft-ts-turbo-tn10/clean/w50\endcsname{92.6}
\expandafter\def\csname v@vox/ft-ts-turbo/clean/mae\endcsname{15.9}
\expandafter\def\csname v@vox/ft-ts-turbo/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-turbo/clean/over500\endcsname{0.05}
\expandafter\def\csname v@vox/ft-ts-turbo/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-turbo/clean/w20\endcsname{80.7}
\expandafter\def\csname v@vox/ft-ts-turbo/clean/w50\endcsname{93.3}
\expandafter\def\csname v@vox/ft-ts-v3-final-s1/clean/mae\endcsname{16.0}
\expandafter\def\csname v@vox/ft-ts-v3-final-s1/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-v3-final-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3-final-s1/clean/w100\endcsname{97.7}
\expandafter\def\csname v@vox/ft-ts-v3-final-s1/clean/w20\endcsname{79.9}
\expandafter\def\csname v@vox/ft-ts-v3-final-s1/clean/w50\endcsname{93.1}
\expandafter\def\csname v@vox/ft-ts-v3-final/clean/mae\endcsname{16.2}
\expandafter\def\csname v@vox/ft-ts-v3-final/clean/median\endcsname{7.8}
\expandafter\def\csname v@vox/ft-ts-v3-final/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3-final/clean/w100\endcsname{97.5}
\expandafter\def\csname v@vox/ft-ts-v3-final/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-v3-final/clean/w50\endcsname{93.0}
\expandafter\def\csname v@vox/ft-ts-v3-post-10ms/clean/mae\endcsname{14.8}
\expandafter\def\csname v@vox/ft-ts-v3-post-10ms/clean/median\endcsname{7.3}
\expandafter\def\csname v@vox/ft-ts-v3-post-10ms/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3-post-10ms/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-v3-post-10ms/clean/w20\endcsname{81.2}
\expandafter\def\csname v@vox/ft-ts-v3-post-10ms/clean/w50\endcsname{94.2}
\expandafter\def\csname v@vox/ft-ts-v3-post-s1/clean/mae\endcsname{14.8}
\expandafter\def\csname v@vox/ft-ts-v3-post-s1/clean/median\endcsname{7.6}
\expandafter\def\csname v@vox/ft-ts-v3-post-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3-post-s1/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-v3-post-s1/clean/w20\endcsname{80.3}
\expandafter\def\csname v@vox/ft-ts-v3-post-s1/clean/w50\endcsname{94.0}
\expandafter\def\csname v@vox/ft-ts-v3-post/clean/mae\endcsname{15.2}
\expandafter\def\csname v@vox/ft-ts-v3-post/clean/median\endcsname{7.9}
\expandafter\def\csname v@vox/ft-ts-v3-post/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3-post/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-v3-post/clean/w20\endcsname{80.9}
\expandafter\def\csname v@vox/ft-ts-v3-post/clean/w50\endcsname{93.8}
\expandafter\def\csname v@vox/ft-ts-v3-s1/clean/mae\endcsname{15.0}
\expandafter\def\csname v@vox/ft-ts-v3-s1/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-v3-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3-s1/clean/w100\endcsname{98.2}
\expandafter\def\csname v@vox/ft-ts-v3-s1/clean/w20\endcsname{81.0}
\expandafter\def\csname v@vox/ft-ts-v3-s1/clean/w50\endcsname{94.2}
\expandafter\def\csname v@vox/ft-ts-v3-s2/clean/mae\endcsname{15.9}
\expandafter\def\csname v@vox/ft-ts-v3-s2/clean/median\endcsname{8.0}
\expandafter\def\csname v@vox/ft-ts-v3-s2/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3-s2/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-v3-s2/clean/w20\endcsname{79.4}
\expandafter\def\csname v@vox/ft-ts-v3-s2/clean/w50\endcsname{93.0}
\expandafter\def\csname v@vox/ft-ts-v3/clean/mae\endcsname{15.5}
\expandafter\def\csname v@vox/ft-ts-v3/clean/median\endcsname{7.5}
\expandafter\def\csname v@vox/ft-ts-v3/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-v3/clean/w100\endcsname{97.9}
\expandafter\def\csname v@vox/ft-ts-v3/clean/w20\endcsname{80.7}
\expandafter\def\csname v@vox/ft-ts-v3/clean/w50\endcsname{93.7}
\expandafter\def\csname v@vox/ft-ts-wt-s1/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-wt-s1/clean/median\endcsname{8.0}
\expandafter\def\csname v@vox/ft-ts-wt-s1/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-wt-s1/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-wt-s1/clean/w20\endcsname{79.4}
\expandafter\def\csname v@vox/ft-ts-wt-s1/clean/w50\endcsname{94.2}
\expandafter\def\csname v@vox/ft-ts-wt/clean/mae\endcsname{15.1}
\expandafter\def\csname v@vox/ft-ts-wt/clean/median\endcsname{7.7}
\expandafter\def\csname v@vox/ft-ts-wt/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/ft-ts-wt/clean/w100\endcsname{98.3}
\expandafter\def\csname v@vox/ft-ts-wt/clean/w20\endcsname{79.8}
\expandafter\def\csname v@vox/ft-ts-wt/clean/w50\endcsname{93.6}
\expandafter\def\csname v@vox/whisper-tm-cal/clean/mae\endcsname{72.3}
\expandafter\def\csname v@vox/whisper-tm-cal/clean/median\endcsname{65.0}
\expandafter\def\csname v@vox/whisper-tm-cal/clean/over500\endcsname{0.00}
\expandafter\def\csname v@vox/whisper-tm-cal/clean/w100\endcsname{75.7}
\expandafter\def\csname v@vox/whisper-tm-cal/clean/w20\endcsname{18.7}
\expandafter\def\csname v@vox/whisper-tm-cal/clean/w50\endcsname{40.7}
\makeatother

